A case study on parametric verification of failure detectors

Partial synchrony is a model of computation in many distributed algorithms and modern blockchains. These algorithms are typically parameterized in the number of participants, and their correctness requires the existence of bounds on message delays and on the relative speed of processes after reaching Global Stabilization Time. These characteristics make partially synchronous algorithms parameterized in the number of processes, and parametric in time bounds, which render automated verification of partially synchronous algorithms challenging. In this paper, we present a case study on formal verification of both safety and liveness of the Chandra and Toueg failure detector that is based on partial synchrony. To this end, we first introduce and formalize the class of symmetric point-to-point algorithms that contains the failure detector. Second, we show that these symmetric point-to-point algorithms have a cutoff, and the cutoff results hold in three models of computation: synchrony, asynchrony, and partial synchrony. As a result, one can verify them by model checking small instances, but the verification problem stays parametric in time. Next, we specify the failure detector and the partial synchrony assumptions in three frameworks: TLA+, IVy, and counter automata. Importantly, we tune our modeling to use the strength of each method: (1) We are using counters to encode message buffers with counter automata, (2) we are using first-order relations to encode message buffers in IVy, and (3) we are using both approaches in TLA+. By running the tools for TLA+ and counter automata, we demonstrate safety for fixed time bounds. By running IVy, we prove safety for arbitrary time bounds. Moreover, we show how to verify liveness of the failure detector by reducing the verification problem to safety verification. Thus, both properties are verified by developing inductive invariants with IVy.

==> forte21/cutoff-intro.tex <==
%In~\cite{tran2020netys}, Thanh-Hai et al. introduced a class of
%symmetric point-to-point distributed algorithms, and the failure detector~\cite{CT96} is one example of this class.
%Thanh-Hai et al. also proved the cutoffs on a number of processes for this class under either synchrony or asynchrony.
In this section, we extend the cutoffs of symmetric point-to-point distributed algorithms in~\cite{tran2020netys} for partial synchrony.
%This class contains the Chandra and Toueg failure detector.
%Since there are many models of partial synchrony, our work here focuses on the case of unknown bounds $\Delta$ and $\Phi$.
%their formalization of the global transition system, and their cutoffs on a number of processes for partial synchrony in case of unknown $\Delta$ and $\Phi$.
%It is straightforward to adapt our approach to other models of partial synchrony in~\cite{DLS88,CT96}.



Notice that time parameters in partial synchrony only reduce the execution space compared to asynchrony.
Hence, we can formalize the system behaviors under partial synchrony by extending the formalization of the system behaviors under asynchrony in~\cite{tran2020netys} with the notion of time, message ages, time constraints under partial synchrony.
(Our formalization is left for the full report~\cite{fdSpec}.)

%\begin{figure}[htb]


%\emph{Time.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that the configuration $\gconf{0}$ is at time 0, and that four configurations $\gconf{4k + 1}, \ldots, \gconf{4k + 4}$ are at time $k + 1$ for every $k \geq 0$. 
%
%\emph{Admissible sequences of configurations under partial synchrony.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that $\pi$ is partially synchronous if Constraints~\ref{delta} and~\ref{phi} hold in $\pi$.
%
%partialy .  the formalization of the global transition system under asynchrony in~\cite{tran2020netys} can be reused, but we need to formal
%
%
%From now on, we denote $\mathcal{A}(\Delta, \Phi)$ a symmtric point-to-point algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$.
%
%
%To do that, we first formalize time constraints with bounds $\Delta$ and $\Phi$, and the
%transition system for the global system under partial synchrony. Then we present
%the cutoffs for the symmetric point-to-point class under partial synchrony, and
%support observances and lemmas to prove the cutoffs. Our proofs here are very
%similar to ones for cutoffs in[38], but we need to add more arguments to reason
%about time constraints under partial synchrony.
%
%
%
%
%Our work here is based on the formalization and definitions in~\cite{tran2020netys}. 
%Our cutoffs are presented in Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}.
%Moreover, we denote $\mathcal{G}_N$ a global transition of an instance of $\mathcal{A}$ with $N$ processes\footnote{The definition of a global transition $\gsys{N}$ is provided in~\cite{tran2020netys}.}.

%In this section, we extend 
%their formalization of system behaviors, and the cutoffs for partial synchrony in case of unknown $\Delta$ and $\Phi$.
%It is straightforward to adopt our results for other models of partial synchrony in~\cite{DLS88,CT96}.
%
%
%Our work here is based on the formalization and definitions in~\cite{tran2020netys}. 
%From now on, we denote $\mathcal{A}(\Delta, \Phi, 1)$ a symmetric point-to-point algorithm with unknown bounds $\Delta$ and $\Phi$, and the GST $T_0 = 1$.
%Moreover, we denote $\mathcal{G}_N$ a global transition of an instance of $\mathcal{A}$ with $N$ processes\footnote{The definition of a global transition $\gsys{N}$ is provided in~\cite{tran2020netys}.}.
%First, we introduce the notion of time in admissible sequences of configurations.
%The definition of admissible sequences of configurations is provided on Pages 8--9~\cite{tran2020netys}.
%Then, we define admissible sequences of configurations under partial synchrony.
%
%\emph{Time.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that the configuration $\gconf{0}$ is at time 0, and that four configurations $\gconf{4k + 1}, \ldots, \gconf{4k + 4}$ are at time $k + 1$ for every $k \geq 0$. 
%
%\emph{Admissible sequences of configurations under partial synchrony.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that $\pi$ is partially synchronous if Constraints~\ref{delta} and~\ref{phi} hold in $\pi$.
%
%

%\paragraph{Cutoffs.} 
%Let $i$ be a process index, and $\omega_{\{i\}}$ be an \ltlx{} (the stuttering-insensitive linear temporal logic) formula in which every predicate takes one of the forms: $P_1(i)$ or $P_2(i, i)$.
%Let $k$ and $\ell$ be different process indexes, and $\psi_{\{k, \ell\}}$  be an \ltlx{} formula in which every predicate takes one of the forms: $Q_1(k)$, or $Q_2(\ell)$, or $Q_3(k, \ell)$, or $Q_4(\ell, k)$. 
%In a nutshell, our results allow us to verify properties in the form of
%$\bigwedge_{k, \ell \in \nid}^{k \neq \ell} \psi_{\{k, \ell\}}$
%on a symmetric point-to-point algorithm under partial synchrony by checking small instances with two processes.
In a nutshell, our cutoff results for the symmetric point-to-point class allow us to verify the mentioned properties on the failure detector under partial synchrony by checking small instances with one and/or two processes.
%The formal statements and proofs of our cutoffs are technical, and left for Appendix~\ref{sec:cutoff}. 
%(Appendix~\ref{sec:cutoff} contains two cutoffs.)
%
%The cutoffs for symmetric point-to-point algorithms with unknown bounds $\Delta$ and $\Phi$ are presented in Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}.
%In our formalization, an execution under partial synchrony is formalized as an \emph{admissible sequence of configurations} under partial synchrony.
%
%Since the proofs of these theorems are similar, we here
%focus on only Theorem~\ref{thm:NCutoffTwoIndexes}. 
%The proof of Theorem~\ref{thm:NCutoffTwoIndexes} follows the approach in~\cite{emerson1995reasoning,tran2020netys}, and is based on the following observations:
Intuitively, the proofs of our cutoffs 
%follows the approach in~\cite{emerson1995reasoning,tran2020netys}, and is 
are based on the following observations:

\begin{itemize}[nosep]
\item The global transition system and the desired property are symmetric~\cite{tran2020netys}.

\item Let $\gsys{2}$ and $\gsys{N}$ be two instances of a symmetric point-to-point algorithm with 2 and $N$ processes, respectively.
By~\cite{tran2020netys}, two instances $\gsys{2}$ and $\gsys{N}$  are trace equivalent under a set of predicates in the desired property.
	
\item We will now discuss that the constraints maintain partial synchrony. Let $\pi_N$ be an execution in $\mathcal{G}_N$. 
We construct an execution $\pi_2$ in $\mathcal{G}_2$ by applying the index projection to $\pi_N$ (formally defined in~\cite{tran2020netys}).
%The index projection is defined in~\cite{tran2020netys}.
Intuitively, the index projection discards processes $3..N$ as well as their corresponding messages and buffers.
Moreover, for every $k,\ell \in \{1, 2\}$, the index projection preserves (i) at which point in time process $k$ takes a step, and (ii) what action process $k$ takes at a time $t \geq 0$, and (iii) messages from process $k$ to process $\ell$.
%Moreover, the process-index projection preserves in-transit messages between process 1 and proc
Figure~\ref{fig:3to2} demonstrates an execution in $\mathcal{G}_2$ that is constructed based on a given execution in $\mathcal{G}_3$ with the index projection.
%Notice that the process-index projection does not change when a process takes a step, and what action a process takes at time $t \geq 0$.
Observe that Constraints~\ref{delta} and~\ref{phi} are maintained in this projection.
%If partial synchrony constraints hold on $\pi_N$, it is straightforward that these constraints also hold on~$\pi_2$. 
	%\vspace{-2mm}
	%\begin{figure}[htb]
	%	\centering
	
	
	





\item Let $\pi_2$ be an execution in $\mathcal{G}_2$. 
We construct an execution $\pi_N$ in $\mathcal{G}_N$ based on $\pi_2$ such that all processes $3..N$ crash from the beginning, and $\pi_2$ is an index projection of $\pi_N$~\cite{tran2020netys}. 
For example, Figure~\ref{fig:2to3} demonstrates an execution in $\mathcal{G}_3$ that is constructed based on an given execution in $\mathcal{G}_2$.
If Constraints~\ref{delta} and~\ref{phi} hold on $\pi_2$, these constraints also hold on $\pi_N$. 
%Then, time constraints under partial synchrony satisfy on $\pi_N$.



%It is straightforward that if time constraints under partial synchrony hold on $\pi_2$.
%By applying the process-index projection to $\pi_N$, we obtain an execution $\pi_2$ in $\mathcal{G}_2$ such that time constraints under partial synchrony hold on $\pi_2$.
%Notice that the process-index projection does not change when a process takes a step, and what action a process does at time $t \geq 0$.
%For example, Figur~\ref{fig:3to2} demonstrates an execution in $\mathcal{G}_2$ that is constructed based on one in $\mathcal{G}_3$.


%The reserve direction also holds.
%These results are proved in Appendix~\ref{sec:cutoff}.
\end{itemize}



%\begin{center}	
\begin{figure}[tb]
	\centering
	\resizebox{.85\textwidth}{!}{
		\begin{tikzpicture}[x=1cm,y=0.4cm]
		\draw[-stealth] (-3,0)--(5,0) node[right] {};
		
		\draw[-stealth] (-3,1.2)--(5,1.2) node[right] {};
		
		\draw[-stealth] (-3,2.4)--(5,2.4) node[right] {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a1) at (-2, 2.4) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a2) at (-1, 1.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a3) at (-2.5,1.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a4) at (-1.5, 0) {};
		
		
		\draw[thick,->] (a3) to (a1);
		
		\draw[thick,->] (a3) to (a2);
		
		\draw[thick,->] (a3) to (a4);
		
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b1) at (-0.5, 2.4) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b2) at (0.5, 2.4) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b3) at (1.5, 1.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b4) at (1, 0) {};
		
		
		\draw[thick,->] (b1) to (b2);
		
		\draw[thick,->] (b1) to (b3);
		
		\draw[thick,->] (b1) to (b4);
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c1) at (3.25, 2.4) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c2) at (4, 1.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c3) at (3.5, 0) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c4) at (2.5, 0) {};
		
		
		\draw[thick,->] (c4) to (c1);
		
		\draw[thick,->] (c4) to (c2);
		
		\draw[thick,->] (c4) to (c3);
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,0) {$p_1$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,1.2) {$p_2$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,2.4) {$p_3$};
		
		\node[draw, circle] at (-5,1.2) {$\mathcal{G}_3$};
		
		\draw[dashed, fill=blue!30] (-6,-1)--(5.5,-1) node[right] {};
		
		
		
		\draw[-stealth] (-3,-3.2)--(5,-3.2) node[right] {};
		
		\draw[-stealth] (-3,-2)--(5,-2) node[right] {};
		
		
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d2) at (-1, -2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d3) at (-2.5,-2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d4) at (-1.5, -3.2) {};
		
		
		\draw[thick,->] (d3) to (d2);
		
		\draw[thick,->] (d3) to (d4);
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e2) at (4, -2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e3) at (3.5, -3.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e4) at (2.5, -3.2) {};
		
		
		\draw[thick,->] (e4) to (e2);
		
		\draw[thick,->] (e4) to (e3);
		
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,-3.2) {$p_1$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,-2) {$p_2$};
		
		
		\node[circle,draw] at (-5,-2.6) {$\mathcal{G}_2$};
		
		
		\end{tikzpicture}
	}
	\caption{Given execution in $\mathcal{G}_3$, construct an execution in $\mathcal{G}_2$ by index projection.}  \label{fig:3to2}
	%	\end{figure}
	%\vspace{-2mm}
%\end{center}
\end{figure}

\begin{figure}[tb]
%\begin{center}
	\centering
	\resizebox{.85\textwidth}{!}{
		\begin{tikzpicture}[x=1cm,y=0.4cm]
		
		
		
		\draw[dashed, fill=blue!30] (-6,5)--(5.5,5) node[right] {};
		
		
		
		\draw[-stealth] (-3,6)--(5,6) node[right] {};
		
		\draw[-stealth] (-3,7.2)--(5,7.2) node[right] {};
		
		
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d2) at (-1, 7.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d3) at (-2.5, 7.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d4) at (-1.5, 6) {};
		
		
		\draw[thick,->] (d3) to (d2);
		
		\draw[thick,->] (d3) to (d4);
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e2) at (4, 7.2) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e3) at (3.5, 6) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e4) at (2.5, 6) {};
		
		
		\draw[thick,->] (e4) to (e2);
		
		\draw[thick,->] (e4) to (e3);
		
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8, 6) {$p_1$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,7.2) {$p_2$};
		
		
		\node[circle,draw] at (-5,6.6) {$\mathcal{G}_2$}; 
		
		
		
		\draw[-stealth] (-3,1.4)--(5,1.4) node[right] {};
		
		\draw[-stealth] (-3,2.6)--(5,2.6) node[right] {};
		
		\draw[-stealth] (-3,3.8)--(5,3.8) node[right] {};
		
		\node[inner sep=0pt,minimum size=3pt] (a1) at (-1.8, 3.8) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a2) at (-1, 2.6) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a3) at (-2.5,2.6) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a4) at (-1.5, 1.4) {};
		
		
		\draw[dashed,->] (a3) to (a1);
		
		\draw[thick,->] (a3) to (a2);
		
		\draw[thick,->] (a3) to (a4);
		
		
		
		
		\node[inner sep=0pt,minimum size=3pt] (c1) at (3.1, 3.8) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c2) at (4, 2.6) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c3) at (3.5, 1.4) {};
		
		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c4) at (2.5, 1.4) {};
		
		
		\draw[dashed,->] (c4) to (c1);
		
		\draw[thick,->] (c4) to (c2);
		
		\draw[thick,->] (c4) to (c3);
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,1.4) {$p_1$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,2.6) {$p_2$};
		
		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,3.8) {$p_3$};
		
		\node[circle,draw] at (-5,2.6) {$\mathcal{G}_3$};
		
		\node[anchor=south west,inner sep=0] at (-3.2,3.6) {\includegraphics[width=0.2cm]{./forte21/img/fire.jpeg}};
		
		
		\node[anchor=south west,inner sep=0] at (-1.8,3.6) {\includegraphics[width=0.2cm]{./forte21/img/fire.jpeg}};
		
		\node[anchor=south west,inner sep=0] at (3.1,3.6) {\includegraphics[width=0.2cm]{./forte21/img/fire.jpeg}};
		
		
		\end{tikzpicture}
	}
	\caption{Construct an execution in $\mathcal{G}_3$ based on a given execution in $\mathcal{G}_2$.}
	\label{fig:2to3}
\end{figure}
%\end{center}


%From now on, we denote $\mathcal{A}(\Delta, \Phi)$ a symmetric point-to-point algorithm with unknown bounds $\Delta$ and $\Phi$.
%Recall that in this case we have the GST $T_0 = 1$.
%Moreover, we denote $\mathcal{G}_N(\Delta, \Phi)$ a global transition of an instance of $\mathcal{A}(\Delta, \Phi)$ with $N$ processes.
%Our proofs here are very similar to ones for cutoffs in~\cite{tran2020netys}, but we need to add more arguments to reason about time constraints under partial synchrony.
%The detailed proofs of Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes} are left in Appendix~\ref{sec:cutoff}.
%To do that, we first formalize time constraints with bounds $\Delta$ and $\Phi$, and the transition system for the global system under partial synchrony.
%Then we present the cutoffs for the symmetric point-to-point class under partial synchrony, and support observances and lemmas to prove the cutoffs.
%Our proofs here are very similar to ones for cutoffs in\cite{tran2020netys}, but we need to add more arguments to reason about time constraints under partial synchrony.
%
%
%Since there are different partially synchronous models, we here focus on the case where the bounds $\Delta$ and $\Phi$ are unknown and eventually hold after some GST $T_0$. 
%In detail, two following constraints hold in every execution trace
%\begin{itemize}[nosep]
%\newcounter{foo}	
%\item Constraint 1: If message $m$ is placed in the message buffer from process $q$ to process $p$ by some $Send(m, p)$ at a time $s_1$, and if process $p$ executes a $Receive(p)$ at a time $s_2$ with $s_2 \geq s_1 + \Delta \geq T_0$, then message $m$ must be delivered to $p$ at time $s_2$ or earlier. 
%\refstepcounter{foo}\thefoo\label{const:delta}
%\item Constraint 2:  In every time interval $\left[ t, t + \Phi \right]$ with $t \geq T_0$, every correct process must take at least one step. 
%\refstepcounter{foo}\thefoo\label{const:phi}
%\end{itemize}
%Our results are easy to extend for other partially synchronous models.
%
%Our work here is based on definitions and constructions in~\cite{tran2020netys}. From now on, we denote $\mathcal{A}(\Delta, \Phi, T_0)$ a symmetric point-to-point algorithm with the bounds $\Delta$ and $\Phi$, and the GST $T_0$ under partial synchrony. 
%Moreover, we denote $\mathcal{G}_N$ a global transition of an instance of $\mathcal{A}$ with $N$ processes~\footnote{The definition of a global transition $\gsys{N}$ is provided in~\cite{tran2020netys}.}.
%First, we introduce the notion of time in admissible sequences of configurations.
%The definition of admissible sequences of configurations is provided on Pages 8--9~\cite{tran2020netys}.
%Then, we define admissible sequences of configurations under partial synchrony.
%
%\emph{Time.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that the configuration $\gconf{0}$ is at time 0, and that four configurations $\gconf{4k + 1}, \ldots, \gconf{4k + 4}$ are at time $k + 1$ for every $k \geq 0$. 
%
%\emph{Admissible sequences of configurations under partial synchrony.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
%We say that $\pi$ is partially synchronous if Constraints~\ref{const:delta} and~\ref{const:phi} hold in $\pi$.
%
%
%We now prove the cutoff results of symmetric point-to-point algorithms under partial synchrony in Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}.




==> forte21/cutoff.tex <==
In~\cite{tran2020netys}, Thanh-Hai et al. introduced a class of
symmetric point-to-point distributed algorithms, and the failure detector~\cite{CT96} is one example of this class.
Thanh-Hai et al. also proved two following cutoffs for this class under either synchrony or asynchrony: 
\begin{enumerate}[nosep]
	\item Let $i$ be an index, and $\omega_{\{i\}}$ be an \ltlx{} (the stuttering-insensitive linear temporal logic) formula in which every predicate takes one of the forms: $P_1(i)$ or $P_2(i, i)$.
	Properties of the form $\bigwedge_{i \in \nid} \omega_{\{i\}}$ have a cutoff of 1. 
	
	\item Let $i$ and $j$ be different indexes, and $\psi_{\{i, j\}}$  be an \ltlx{} formula in which every predicate takes one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i, j)$, or $Q_4(j, i)$. Properties of the form  $\bigwedge_{i, j \in \nid}^{i \neq j} \psi_{\{i, j\}}$ have a cutoff of 2.
\end{enumerate}
In this section, we extend their formalization of the global transition system, and their cutoffs on a number of processes for partial synchrony in case of unknown bounds $\Delta$ and $\Phi$.
It is straightforward to adapt our approach to other models of partial synchrony in~\cite{DLS88,CT96}.


Time parameters in partial synchrony only reduce the execution space compared to asynchrony.
Hence, we can formalize the system behaviors under partialy synchrony by extending the formalization of the system behaviors under asynchrony in~\cite{tran2020netys} with the notion of time, message ages, time constraints, and admissible sequences of configurations under partial synchrony.


%Our cutoff results are presented in Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}.

%To do that, we first formalize time constraints with bounds $\Delta$ and $\Phi$, and the transition system for the global system under partial synchrony.
%Then we present the cutoffs for the symmetric point-to-point class under partial synchrony, and support observances and lemmas to prove the cutoffs.
%Our proofs here are very similar to ones for cutoffs in\cite{tran2020netys}, but we need to add more arguments to reason about time constraints under partial synchrony.
%
%
%Since there are different partially synchronous models, we here focus on the case where the bounds $\Delta$ and $\Phi$ are unknown and eventually hold after some GST $T_0$. 
%In detail, two following constraints hold in every execution trace
%\begin{itemize}[nosep]
%\item Constraint 1: If message $m$ is placed in the message buffer from process $q$ to process $p$ by some $Send(m, p)$ at a time $s_1$, and if process $p$ executes a $Receive(p)$ at a time $s_2$ with $s_2 \geq s_1 + \Delta \geq T_0$, then message $m$ must be delivered to $p$ at time $s_2$ or earlier. 
%\refstepcounter{foo}\thefoo\label{const:delta}
%\item Constraint 2:  In every time interval $\left[ t, t + \Phi \right]$ with $t \geq T_0$, every correct process must take at least one step. 
%\refstepcounter{foo}\thefoo\label{const:phi}
%\end{itemize}
%Our results are easy to extend for other partially synchronous models.
%
%Our work here is based on definitions and constructions in~\cite{tran2020netys}. 
The notion of time, message ages, time constraints, and admissible sequences of configurations under partial synchrony are defined as follows.
From now on, we denote $\mathcal{A}$ a symmetric point-to-point algorithm with unknown bounds $\Delta$ and $\Phi$.
Moreover, we denote $\mathcal{G}_N$ a global transition system of an instance of $\mathcal{A}$ with $N$ processes that is formalized in~\cite{tran2020netys}.
We denote $\nid$ a set of process indexes.

%The definition of admissible sequences of configurations is provided on Pages 8--9~\cite{tran2020netys}.
%Then, we formalize Constraints~\ref{delta} and~\ref{phi}, and define admissible sequences of configurations under partial synchrony.

\textbf{Time.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$~\footnote{The definition of an admissible sequence of configurations is provided in~\cite{tran2020netys}.	}. 
We say that the configuration $\gconf{0}$ is at time 0, and that four configurations $\gconf{4k - 3}, \ldots, \gconf{4k}$ are at time $k$ for every $k > 0$. 

Recall that in~\cite{tran2020netys}, a global transition contains a sequence of four sub-rounds: \textit{Schedule, Send, Receive,} and \textit{Computation}.
In an admissible sequence $\pi = \gconf{0} \gconf{1} \ldots $ of global configurations in $\mathcal{G}_N$, for every $k > 0$, every sub-sequence of four configurations $\gconf{4k-3}\ldots\gconf{4k}$ presents one global transition.
Configuration $\gconf{4k-3}$ is in sub-round Schedule, and configuration $\gconf{4k}$ is in sub-round Computation for every $k > 0$.


\textbf{Message ages.} Now we discuss the formalization of message ages. 
For every sent message $m$, the global system packages it with a tag containing its current age, i.e., $(m, \mathit{age}_m)$. When message $m$ has been added to the message buffer in sub-round Send, its age is 0.
In our formalization, message ages are increased by 1 in sub-round Schedule.
Formally, for every time $k \geq 0$, for every process $s, r \in \nid$, the following constraints hold:
\begin{enumerate}[nosep]
\item For every message $(m, \textit{age}_m)$ in $\getBuf{\gconf{4k}}{s}{r}$, there exists  $(m^{\prime}, \textit{age}_{m^{\prime}})$ in $\getBuf{\gconf{4k+1}}{s}{r}$
such that $m = m^{\prime}$ and $\textit{age}_m = \textit{age}_{m^{\prime}} + 1$.

\item For every message $(m^{\prime}, \textit{age}_{m^{\prime}})$ in $\getBuf{\gconf{4k+1}}{s}{r}$, there exists $(m, \textit{age}_m)$ in $\getBuf{\gconf{4k}}{s}{r}$ 
such that $m = m^{\prime}$ and $\textit{age}_m = \textit{age}_{m^{\prime}} + 1$.
\end{enumerate}
%Recall that for every $k > 0$, $\getBuf{\gconf{4k+1}}{s}{r}$ is a configuration in sub-round \textit{Schedule}, and $\getBuf{\gconf{4k+4}}{s}{r}$ is a configuration in sub-round \textit{Computation}.
The first constraint ensures that every in-transit message age will be added one time-unit.
The second constraint ensures that no new messages will be added in $\getBuf{\gconf{4k+1}}{s}{r}$.

Moreover, the age of an in-transit message is unchanged in other sub-rounds.
Formally, for every time $k > 0$, for every $0 \leq \ell \leq 3$, for every pair of processes $s, r \in \nid$, for every message $(m, \textit{age}_m)$ in $\getBuf{\gconf{4k-\ell}}{s}{r}$, there exists  $(m^{\prime}, \textit{age}_{m^{\prime}})$ in $\getBuf{\gconf{4k-3}}{s}{r}$
such that $m = m^{\prime}$ and $\textit{age}_m = \textit{age}_{m^{\prime}}$.

\textbf{Partial synchrony constraints.} With the above definitions, Constraints~\ref{delta} and \ref{phi} 
can be formalized as follows, respectively: 
\begin{enumerate}[nosep,label=(\alph*)]
\item For every process $r \in \nid$, for every time $k > 0$, if  $\Enable(\kappa_{4k-1},r,\locrcv) = \True$, then for every process $s \in \nid$, there exists no message $(m, \textit{age}_m)$ in $\getBuf{\gconf{4k-1}}{s}{r}$ such that $\textit{age}_m \geq \Delta$.
%Predicate $\Enable(\kappa_{4k+3},r,\locrcv)$ refers to whether process $p$ takes a step in sub-round Receive at time $k$.

\item For every process $i \in \nid$, for every time interval $[k, k + \Phi ]$, if we have that $\getPC{\getProc{\gconf{\ell}}{i}} \neq \loccrash$ for every configuration index $4k-3 \leq \ell \leq 4(k + \Phi)$,
then there exists a configuration index $4k-3 \leq \ell_0 \leq 4(k + \Phi)$ such that  $\Enable(\kappa_{\ell_0},i,\mathit{loc}) = \True$ where $\mathit{loc}$ is one of locations $\locsnd, \locrcv,$ or $\loccomp$.
\end{enumerate}
Predicate $\Enable(\kappa_{k},r,\mathit{loc})$ refers to whether process $p$ takes a step in configuration $\kappa_{k}$ for every $k \geq 0$.


\textbf{Admissible sequences of configurations under partial synchrony.} Let $\pi = \gconf{0} \gconf{1} \ldots $ be an admissible sequence of global configurations in $\mathcal{G}_N$. 
We say that $\pi$ is under partial synchrony if Constraints~\ref{delta} and~\ref{phi} hold in $\pi$.

\textbf{Cutoffs.} Now we discuss the cutoffs for symmetric point-to-point algorithms with unknown bounds $\Delta$ and $\Phi$ that are presented in Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}.

\newcommand{\thmNCutoffOneIndex}{
	Let $\mathcal{A}$ be a~\classname{} algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$. 
	Let $\gsys{1}$ and $\gsys{N}$ be instances of $\mathcal{A}$ with 1 and $N$ processes respectively for some $N \geq 1$.
	Let $\mathit{Path}_1$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{1}$ and in $\gsys{N}$ under partial synchrony, respectively.
	Let $\omega_{\{i\}}$ be a \ltlx{} formula  in which every predicate takes one of the forms: $P_1(i)$ or $P_2(i, i)$ where $i$ is an index in $\nid$. 
	It follows that \\
	$\Big(\forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models \bigwedge_{i \in \nid}  \omega_{\{i\}} \Big) \; \Leftrightarrow \; \Big(\forall \pi_1 \in \mathit{Path}_1 \colon \gsys{1}, \pi_1 \models  \omega_{\{1\}}\Big)$
	%  $
	%  \gsys{N}, \ginitconf{N} \models \bigwedge_{i \in \nid} \omega_{\{i\}} $ if and only if 
	%  $
	%  \gsys{1}, \ginitconf{1} \models  \pone
	%  $.
}

\begin{theorem} \label{thm:NCutoffOneIndex}
	\thmNCutoffOneIndex
\end{theorem}

\newcommand{\thmNCutoffTwoIndexes}{
	Let $\mathcal{A}$ be a~\classname{} algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$. 
	Let $\gsys{2}$ and $\gsys{N}$ be instances of $\mathcal{A}$ with 2 and $N$ processes respectively for some $N \geq 2$.
	Let $\mathit{Path}_2$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{2}$ and in $\gsys{N}$ under partial synchrony, respectively.
	Let $\psi_{\{i, j\}}$ be an \ltlx{} formula in which every predicate takes one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i, j)$, or $Q_4(j, i)$ where $i$ and $j$ are different indexes in $\nid$.
	It follows that:\\
	$\big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}} \big)  \Leftrightarrow  \big(  \forall \pi_2 \in \mathit{Path}_2 \colon \gsys{2}, \pi_2 \models    \psi_{\{1, 2 \}} \big) $
	
	
	%  $\gsys{N}, \ginitconf{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} \ptwo 
	%  $
	%  if and only if
	%  $
	%  \gsys{2}, \ginitconf{2} \models  \psi_{\{1, 2 \}}$
}


\begin{theorem} \label{thm:NCutoffTwoIndexes}
	\thmNCutoffTwoIndexes  
\end{theorem}


Since the proofs of these theorems are similar, we here
focus on only Theorem~\ref{thm:NCutoffTwoIndexes}. 
The proof of Theorem~\ref{thm:NCutoffTwoIndexes} follows the approach in~\cite{emerson1995reasoning,tran2020netys}, and is based on the following observations:
\begin{itemize}[nosep]
	\item The global transition system and the desired property are symmetric~\cite{tran2020netys}.
	
	\item Let $\gsys{2}$ and $\gsys{N}$ be two instances of a symmetric point-to-point algorithm with 2 and $N$ processes, respectively.
	By~\cite{tran2020netys}, two instances $\gsys{2}$ and $\gsys{N}$  are trace equivalent under a set of predicates in the desired property.
	
	\item We will now discuss that the constraints maintain partial synchrony. 
	Let $\pi_N$ be an execution in $\mathcal{G}_N$. By applying the index projection to $\pi_N$, we obtain an execution $\pi_2$ in $\mathcal{G}_2$~\cite{tran2020netys}.
	Intuitively, the index projection throws away processes $3..N$ as well as their corresponding messages and buffers.
	Moreover, for every $i,j \in \{1, 2\}$, the index projection preserves (i) when process $i$ takes a step, and (ii) what action process $i$ takes at time $t \geq 0$, and (iii) messages between process $i$ and process $j$.
	%Moreover, the process-index projection preserves in-transit messages between process 1 and proc
	For example, Figure~\ref{fig:3to2} demonstrates an execution in $\mathcal{G}_2$ that is constructed based on a given execution in $\mathcal{G}_3$ with the index projection.
	The index projection is defined in~\cite{tran2020netys}.
	%Notice that the process-index projection does not change when a process takes a step, and what action a process takes at time $t \geq 0$.
	If partial synchrony constraints hold on $\pi_N$, these constraints also hold on~$\pi_2$. 
	This result is proved in Lemma~\ref{lem:ps1}.
	%\vspace{-2mm}
	%\begin{figure}[htb]
	%	\centering
%	\begin{center}
%		\resizebox{.85\textwidth}{!}{
%			\begin{tikzpicture}[x=1cm,y=0.4cm]
%			\draw[-stealth] (-3,0)--(5,0) node[right] {};
%			
%			\draw[-stealth] (-3,1.2)--(5,1.2) node[right] {};
%			
%			\draw[-stWe will now discuss that the constraints maintain partial synchrony. ealth] (-3,2.4)--(5,2.4) node[right] {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a1) at (-2, 2.4) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a2) at (-1, 1.2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a3) at (-2.5,1.2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a4) at (-1.5, 0) {};
%			
%			
%			\draw[thick,->] (a3) to (a1);
%			
%			\draw[thick,->] (a3) to (a2);
%			
%			\draw[thick,->] (a3) to (a4);
%			
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b1) at (-0.5, 2.4) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b2) at (0.5, 2.4) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b3) at (1.5, 1.2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b4) at (1, 0) {};
%			
%			
%			\draw[thick,->] (b1) to (b2);
%			
%			\draw[thick,->] (b1) to (b3);
%			
%			\draw[thick,->] (b1) to (b4);
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c1) at (3.25, 2.4) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c2) at (4, 1.2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c3) at (3.5, 0) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c4) at (2.5, 0) {};
%			
%			
%			\draw[thick,->] (c4) to (c1);
%			
%			\draw[thick,->] (c4) to (c2);
%			
%			\draw[thick,->] (c4) to (c3);
%			
%			\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,0) {$p_1$};
%			
%			\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,1.2) {$p_2$};
%			
%			\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,2.4) {$p_3$};
%			
%			\node[draw, circle] at (-5,1.2) {$\mathcal{G}_3$};
%			
%			\draw[dashed, fill=blue!30] (-6,-1)--(5.5,-1) node[right] {};
%			
%			
%			
%			\draw[-stealth] (-3,-3.2)--(5,-3.2) node[right] {};
%			
%			\draw[-stealth] (-3,-2)--(5,-2) node[right] {};
%			
%			
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d2) at (-1, -2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d3) at (-2.5,-2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d4) at (-1.5, -3.2) {};
%			
%			
%			\draw[thick,->] (d3) to (d2);
%			
%			\draw[thick,->] (d3) to (d4);
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e2) at (4, -2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e3) at (3.5, -3.2) {};
%			
%			\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e4) at (2.5, -3.2) {};
%			
%			
%			\draw[thick,->] (e4) to (e2);
%			
%			\draw[thick,->] (e4) to (e3);
%			
%			
%			\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,-3.2) {$p_1$};
%			
%			\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,-2) {$p_2$};
%			
%			
%			\node[circle,draw] at (-5,-2.6) {$\mathcal{G}_2$};
%			
%			
%			\end{tikzpicture}
%		}
%		\captionof{figure}{Construct an execution in $\mathcal{G}_2$ based on one in $\mathcal{G}_3$ by applying the index projection.}  \label{fig:3to2_t}
%		%\end{figure}
%		%\vspace{-2mm}
%	\end{center}
	
	
	
	
	
	
	
	\item Let $\pi_2$ be an execution in $\mathcal{G}_2$. 
	We construct an execution $\pi_N$ in $\mathcal{G}_N$ based on $\pi_2$ such that all processes $3..N$ crash from the beginning, and $\pi_2$ is an index projection of $\pi_N$~\cite{tran2020netys}. 
	For instance, Figure~\ref{fig:2to3} demonstrates an execution in $\mathcal{G}_3$ that is constructed based on one in $\mathcal{G}_2$.
	If partial synchrony constraints hold on $\pi_2$, these constraints also hold on $\pi_N$. 
	This result is proved in Lemma~\ref{lem:ps2}.
	%Then, time constraints under partial synchrony satisfy on $\pi_N$.
	
	
	
	%It is straightforward that if time constraints under partial synchrony hold on $\pi_2$.
	%By applying the process-index projection to $\pi_N$, we obtain an execution $\pi_2$ in $\mathcal{G}_2$ such that time constraints under partial synchrony hold on $\pi_2$.
	%Notice that the process-index projection does not change when a process takes a step, and what action a process does at time $t \geq 0$.
	%For example, Figur~\ref{fig:3to2} demonstrates an execution in $\mathcal{G}_2$ that is constructed based on one in $\mathcal{G}_3$.
	
	
	%The reserve direction also holds.
	%These results are proved in Appendix~\ref{sec:cutoff}.
\end{itemize}






%\begin{figure}
%\begin{center}
%	
%	
%	%	\centering
%	\resizebox{.85\textwidth}{!}{
%		\begin{tikzpicture}[x=1cm,y=0.4cm]
%		
%		
%		
%		\draw[dashed, fill=blue!30] (-6,5)--(5.5,5) node[right] {};
%		
%		
%		
%		\draw[-stealth] (-3,6)--(5,6) node[right] {};
%		
%		\draw[-stealth] (-3,7.2)--(5,7.2) node[right] {};
%		
%		
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d2) at (-1, 7.2) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d3) at (-2.5, 7.2) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d4) at (-1.5, 6) {};
%		
%		
%		\draw[thick,->] (d3) to (d2);
%		
%		\draw[thick,->] (d3) to (d4);
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e2) at (4, 7.2) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e3) at (3.5, 6) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e4) at (2.5, 6) {};
%		
%		
%		\draw[thick,->] (e4) to (e2);
%		
%		\draw[thick,->] (e4) to (e3);
%		
%		
%		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8, 6) {$p_1$};
%		
%		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,7.2) {$p_2$};
%		
%		
%		\node[circle,draw] at (-5,6.6) {$\mathcal{G}_2$}; 
%		
%		
%		
%		\draw[-stealth] (-3,1.4)--(5,1.4) node[right] {};
%		
%		\draw[-stealth] (-3,2.6)--(5,2.6) node[right] {};
%		
%		\draw[-stealth] (-3,3.8)--(5,3.8) node[right] {};
%		
%		\node[inner sep=0pt,minimum size=3pt] (a1) at (-1.8, 3.8) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a2) at (-1, 2.6) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a3) at (-2.5,2.6) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a4) at (-1.5, 1.4) {};
%		
%		
%		\draw[dashed,->] (a3) to (a1);
%		
%		\draw[thick,->] (a3) to (a2);
%		
%		\draw[thick,->] (a3) to (a4);
%		
%		
%		
%		
%		\node[inner sep=0pt,minimum size=3pt] (c1) at (3.1, 3.8) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c2) at (4, 2.6) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c3) at (3.5, 1.4) {};
%		
%		\node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c4) at (2.5, 1.4) {};
%		
%		
%		\draw[dashed,->] (c4) to (c1);
%		
%		\draw[thick,->] (c4) to (c2);
%		
%		\draw[thick,->] (c4) to (c3);
%		
%		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,1.4) {$p_1$};
%		
%		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,2.6) {$p_2$};
%		
%		\node[rectangle,inner sep=0pt, draw=gray!75,fill=gray!20,minimum size=4mm] at (-3.8,3.8) {$p_3$};
%		
%		\node[circle,draw] at (-5,2.6) {$\mathcal{G}_3$};
%		
%		\node[anchor=south west,inner sep=0] at (-3.2,3.6) {\includegraphics[width=0.2cm]{img/fire.jpeg}};
%		
%		
%		\node[anchor=south west,inner sep=0] at (-1.8,3.6) {\includegraphics[width=0.2cm]{img/fire.jpeg}};
%		
%		\node[anchor=south west,inner sep=0] at (3.1,3.6) {\includegraphics[width=0.2cm]{img/fire.jpeg}};
%		
%		
%		\end{tikzpicture}
%	}
%	\captionof{figure}{Construct an execution in $\mathcal{G}_3$ based on a given execution in $\mathcal{G}_2$.}
%	\label{fig:2to3_t}
%	%\end{figure}
%\end{center}
\begin{lemma} \label{lem:ps1}
Let $\mathcal{A}$ be a~\classname{} algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$. 
Let $\gsys{2}$ and $\gsys{N}$ be instances of $\mathcal{A}$ with 2 and $N$ processes, respectively, for some $N \geq 2$.
Let $\mathit{Path}_2$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{2}$ and in $\gsys{N}$ under partial synchrony, respectively.
Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ be an admissible sequences of configurations in $\gsys{N}$.
Let $\pi^2 = \gconf{0}^2 \gconf{1}^2 \ldots$ be a sequence of configurations in $\gsys{2}$ such that $\gconf{k}^2$ be an index projection of $\gconf{k}^N$ on indexes $\{ 1, 2\}$ for every $k \geq 0$.
It follows that
\begin{enumerate}[nosep,label=(\alph*)]
\item Constraint~\ref{delta} holds on $\pi^2$.
\item Constraint~\ref{phi} holds on $\pi^2$.
\end{enumerate}

\end{lemma}

\begin{proof}
Recall that the index projection is defined on Page~13~\cite{tran2020netys}.
In the following, we denote $p^2$ and $p^N$ two processes such that they have the same index, and $p^2$ is a process in $\gsys{2}$, and $p^N$ is a process in $\gsys{N}$.
We prove Lemma~\ref{lem:ps1} by contradiction.

(a)
Assume that Constraint~\ref{delta} does not hold on $\pi^2$.
Hence, there exist a time $\ell > 0$, and two processes $s^2, r^2 \in \tid$ in $\gsys{2}$ such that after $r^2$ executes Receive at a time $\ell$, there exists an old message in a message buffer from process $s^2$ to process $r^2$.
By the definition of the index projection, for every $k \geq 0$, we have that:
\begin{itemize}[nosep]
	\item Let $p^N, q^N \in \{1, 2\}$ be two processes in $\gsys{N}$, and $p^2, q^2$ be corresponding processes in $\gsys{2}$.
	For every $k \geq 0$, two message buffers from process $p^2$ to process $q^2$ in $\gconf{k}^2$, and from process $p^N$ to process $q^N$ in $\gconf{k}^N$ are the same.
	
	\item Let $p^N \in \{1, 2\}$ be a process in $\gsys{N}$, and $p^2$ be a corresponding process in $\gsys{2}$. 
	For every $k \geq 0$, process $p^2$ takes an action \textit{act} in configuration $\gconf{k}^2$ if and only if process $p^N$ takes the same action in configuration $\gconf{k}^N$.
\end{itemize}
It implies that process $r^N$ in $\gsys{N}$ also executes Receive at a time $\ell$, and there exists an old message in a buffer from process $s^N$ to process $r^N$.
Contradiction. 

(b) By applying similar arguments in case (a). $\qed$
\end{proof}

\begin{lemma} \label{lem:ps2}
	Let $\mathcal{A}$ be a~\classname{} algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$. 
	Let $\gsys{2}$ and $\gsys{N}$ be instances of $\mathcal{A}$ with 2 and $N$ processes, respectively, for some $N \geq 2$.
	Let $\mathit{Path}_2$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{2}$ and in $\gsys{N}$ under partial synchrony, respectively.
	Let $\pi^2 = \gconf{0}^2 \gconf{1}^2 \ldots$ be an admissible sequences of configurations in $\gsys{2}$.
	Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ be a sequence of configurations in $\gsys{N}$ such that (i) every process $p \in 3..N$ crashes from the beginning, and (ii) $\gconf{k}^2$ be an index projection of $\gconf{k}^N$ on indexes $\{ 1, 2\}$ for every $k \geq 0$.
	It follows that
	\begin{enumerate}[nosep,label=(\alph*)]
		\item Constraint~\ref{delta} holds on $\pi^N$.
		\item Constraint~\ref{phi} holds on $\pi^N$.
	\end{enumerate}
\end{lemma}

\begin{proof}
By applying similar arguments in the proof of Lemma~\ref{lem:ps1}, and the facts that every process $p \in 3..N$ crashes from the beginning, and that $\gconf{k}^2$ be an index projection of $\gconf{k}^N$ on indexes $\{ 1, 2\}$ for every $k \geq 0$. $\qed$
\end{proof}

%\newcommand{\thmNCutoffOneIndex}{
%	Let $\mathcal{A}(\Delta, \Phi, T_0)$ be a~\classname{} algorithm under partial synchrony with the bounds $\Delta$ and $\Phi$ and the GST $T_0$. 
%	Let $\gsys{1}$ and $\gsys{N}$ be instances of $\mathcal{A}(\Delta, \Phi, T_0)$ with 1 and $N$ processes respectively for some $N \geq 1$.
%	Let $\mathit{Path}_1$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{1}$ and in $\gsys{N}$ under partial synchrony, respectively.
%	Let $\omega_{\{i\}}$ be a \ltlx{} formula  in which every predicate takes one of the forms: $P_1(i)$ or $P_2(i, i)$ where $i$ is an index in $\nid$. 
%	It follows that \\
%	$\Big(\forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models \bigwedge_{i \in \nid}  \omega_{\{i\}} \Big) \; \Leftrightarrow \; \Big(\forall \pi_1 \in \mathit{Path}_1 \colon \gsys{1}, \pi_1 \models  \omega_{\{1\}}\Big)$
%	%  $
%	%  \gsys{N}, \ginitconf{N} \models \bigwedge_{i \in \nid} \omega_{\{i\}} $ if and only if 
%	%  $
%	%  \gsys{1}, \ginitconf{1} \models  \pone
%	%  $.
%}

%\begin{theorem} 
%%	\label{thm:NCutoffOneIndex}
%	\thmNCutoffOneIndex
%\end{theorem}

%\newcommand{\thmNCutoffTwoIndexes}{
%	Let $\mathcal{A}(\Delta, \Phi, T_0)$ be a~\classname{} algorithm under partial synchrony with the bounds $\Delta$ and $\Phi$ and the GST $T_0$. 
%	Let $\gsys{2}$ and $\gsys{N}$ be instances of $\mathcal{A}(\Delta, \Phi, T_0)$ with 2 and $N$ processes respectively for some $N \geq 1$.
%	Let $\mathit{Path}_2$ and $\mathit{Path}_N$ be sets of all admissible sequences of configurations in $\gsys{2}$ and in $\gsys{N}$ under partial synchrony, respectively.
%	Let $\psi_{\{i, j\}}$ be an \ltlx{} formula in which every predicate takes one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i, j)$, or $Q_4(j, i)$ where $i$ and $j$ are different indexes in $\nid$.
%	It follows that:\\
%	$\big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}} \big)  \Leftrightarrow  \big(  \forall \pi_2 \in \mathit{Path}_2 \colon \gsys{2}, \pi_2 \models    \psi_{\{1, 2 \}} \big) $
%	
%	
%	%  $\gsys{N}, \ginitconf{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} \ptwo 
%	%  $
%	%  if and only if
%	%  $
%	%  \gsys{2}, \ginitconf{2} \models  \psi_{\{1, 2 \}}$
%}



%\begin{theorem} 
%%	\label{thm:NCutoffTwoIndexes}
%	\thmNCutoffTwoIndexes  
%\end{theorem}

%The proofs of Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes} follow the standard approach in~\cite{emerson1995reasoning}, and uses the results in~\cite{tran2020netys}.
%Since the proofs of these theorems are similar, we here focus on only Theorem~\ref{thm:NCutoffTwoIndexes}.
%The proof of Theorem~\ref{thm:NCutoffTwoIndexes} is based on the following observances and results:
%\begin{enumerate}[nosep]
%	\item Every transposition on a set of process indexes $\nid$ preserves the structure of the desired property for every $N \geq 1$. This result follows immediately by the form of the desired property.
%	
%	\item Every transposition on a set of process indexes $\nid$ preserves the structure of the global transition system $\gsys{N}$ for every $N \geq 1$. This result is proved in Lemma 2 in~\cite{tran2020netys}.
%	
%	\item $\gsys{2}$ and $\gsys{N}$ are trace equivalent under a set $AP_{\{1,2\}}$ of predicates that take one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i,j)$, or $Q_4(j,i)$. 
%	We prove this result in Lemma~\ref{lem:traceEquiv}. 
%	This result is an extended version of Lemma 5 in~\cite{tran2020netys} with Constraints~\ref{delta} and~\ref{phi} on the bounds $\Delta$ and $\Phi$ and the GST $T_0$.
%	
%	\item Let $\mathit{Path}_N$ be sets of all admissible sequences of configurations under partial synchrony in $\mathcal{G}_N$. It follows that 
%	\begin{align*}
%	& \big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}} \big) \\ \Leftrightarrow   &  \bigwedge^{i \neq j}_{i, j \in \nid} \big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models   \psi_{\{i, j\}} \big)
%	\end{align*}
%	We prove this result in Lemma~\ref{lem:move-bigvee-out}.
%%	\item By similar arguments in the proof of Theorem 2 in~\cite{tran2020netys}. 
%%	By Lemma~\ref{lem:traceEquiv}, these arguments hold under partial synchrony. 
%\end{enumerate}
%
%
%
%\newcommand{\lemTraceEquiv}{
%	Let $\mathcal{A}(\Delta, \Phi)$ denote a symmetric point-to-point algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$. 
%	Let $\gsys{2}$ and $\gsys{N}$ be two transition systems such that all processes in $\gsys{2}$ and $\gsys{N}$ follow $\mathcal{A}(\Delta, \Phi)$, and $N \geq 2$.
%	Let $AP_{\{1, 2\}}$ be a set of predicates that take one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i, j)$, or $Q_4(j, i)$.
%	It follows that $\gsys{N}$ and $\gsys{2}$ are trace equivalent under $AP_{\{1,2\}}$.
%}
%
%
%\begin{lemma} \label{lem:traceEquiv}
%	\lemTraceEquiv
%\end{lemma}
%
%\begin{proof}
%The proof of Lemma~\ref{lem:traceEquiv} is based on Lemmas 3 and 4 in~\cite{tran2020netys}.
%Moreover, we need to prove that admissible sequences of configurations constructed in Lemmas 3 and 4 in\cite{tran2020netys} also satisfy Constraints~\ref{delta} and~\ref{phi} on the bounds $\Delta$ and $\Phi$, and the GST $T_0$ hold.
%In other words, those constructed sequences are admissible under
%partial synchrony.
%
%
%($\Rightarrow$) 	
%Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ be a sequence of configurations of $\gsys{N}$ such that $\pi^N$ is admissible under partial synchrony.
%By Lemma 3 in~\cite{tran2020netys}, there exists a sequence $\pi^2 = \gconf{0}^N \gconf{1}^N \ldots $ of configurations of $\gsys{2}$ such that
%$\pi^2$ is admissible in $\gsys{2}$ and $\gconf{k}^2$ is the index projection of $\gconf{k}^N$ on indexes $\{1, 2\}$ for every $k \geq 0$~\footnote{The definition of the index projection is provided on Page 13~\cite{tran2020netys}}.
%By the definition of the index projection, we have that:
%\begin{itemize}
%	\item For every $p, q \in \{1, 2\}$, for every $k \geq 0$, the set of in-transit messages from process $p$ to process $q$ in two configurations $\gconf{k}^2$ and $\gconf{k}^N$ are the same.
%	
%	\item For every $k \geq 0$, the set of active processes and their enable actions in two configurations $\gconf{k}^2$ and $\gconf{k}^N$ are the same.
%\end{itemize}
%Hence, Constraints~\ref{delta} and~\ref{phi} on the bounds $\Delta$ and $\Phi$, and the GST $T_0$ hold in a sequence $\pi^2$.
%In other words, $\pi^2$ is an admissible sequence of configurations of $\gsys{2}$ under partial synchrony.
%
%($\Leftarrow$) By applying similar arguments and the fact that other processes $3 \ldots N$ are initially crashed. $\qed$
%\end{proof}
%
%\newcommand{\lemMoveBigVeeOut}{
%	Let $\mathcal{A}(\Delta, \Phi)$ be a~\classname{} algorithm under partial synchrony with unknown bounds $\Delta$ and $\Phi$.
%	Let $\gsys{N}$ be an instance of $\mathcal{A}(\Delta, \Phi)$ with $N$ processes for some $N \geq 1$, and $\mathit{Path}_N$ be sets of all admissible sequences of configurations under partial synchrony in $\mathcal{G}_N$. 
%	Let $\psi_{\{i, j\}}$ be an \ltlx{} formula in which every predicate takes one of the forms: $Q_1(i)$, or $Q_2(j)$, or $Q_3(i, j)$, or $Q_4(j, i)$ where $i$ and $j$ are different indexes in $\nid$.
%	It follows that 
%	\begin{align}
%	& \big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}} \big) \label{fm1} \\ \Leftrightarrow   
%	&  \bigwedge^{i \neq j}_{i, j \in \nid} \big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models   \psi_{\{i, j\}} \big)
%	\label{fm2}
%	\end{align}
%}
%
%\begin{lemma} \label{lem:move-bigvee-out}
%\lemMoveBigVeeOut
%\end{lemma}
%
%\begin{proof}
%$(\Rightarrow)$ Let $\pi^N$ be an arbitrary admissible sequence of configurations under partial synchrony in $\mathit{Path}_N$. 
%We have $\gsys{N}, \pi^N \vDash \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}}$. 
%Let $i_0$ and $j_0$ be arbitrary indexes in $\nid$ such that $i_0 \neq j_0$.
%We have $\gsys{N}, \pi^N \vDash \psi_{\{i_0, j_0 \}}$. 
%Hence, for every $\pi^N \in \mathit{Path}_N$, for every pair of indexes $i_0$ and $j_0$ in $\nid$ such that $i_0 \neq j_0$, it follows that $\gsys{N}, \pi^N \vDash \psi_{\{i_0, j_0 \}}$. 
%Therefore, for every pair of indexes $i_0$ and $j_0$ in $\nid$ such that $i_0 \neq j_0$, for every $\pi^N \in \mathit{Path}_N$, it follows that $\gsys{N}, \pi^N \vDash \psi_{\{i_0, j_0 \}}$. 
%In other words, Formula~(\ref{fm1}) implies Formula~(\ref{fm2}).
%
%$(\Leftarrow)$ By applying similar arguments.
%$\qed$
%\end{proof}
%
%In the following, we present the proof sketch of Theorem~\ref{thm:NCutoffTwoIndexes}.
%\paragraph{Proof sketch of Theorem~\ref{thm:NCutoffTwoIndexes}.}
%(The following arguments are similar to ones in the proof of Theorem 2 in~\cite{tran2020netys}.)
%We have $\big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j} \limits_{i, j \in \nid} \psi_{\{i, j\}} \big) \\
%\Leftrightarrow \;\; 
%\big(  \bigwedge^{i \neq j}_{i, j \in \nid} ( \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models   \psi_{\{i, j\}} ) \big) $ by Lemma~\ref{lem:move-bigvee-out}.
%% \begin{align*}
%%  & \Big(  \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \bigwedge^{i \neq j}_{i, j \in \nid} \psi_{\{i, j\}} \Big) \\  
%%  \Leftrightarrow \;\; &
%% \Big(  \bigwedge^{i \neq j}_{i, j \in \nid} \big( \forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models   \psi_{\{i, j\}} \big) \Big) 
%% \end{align*}
%%  by Proposition~\ref{prop:MoveQuantifiersTwo} (on page~\pageref{prop:MoveQuantifiersTwo},  Appendix~\ref{app:proof}). 
%Let $i$ and $j$ be two process indexes in a set 
%$\nid$ such that $i \neq j$.
%Both $\transposition^1 = \swapij{i}{1}$ and $\transposition^2 = \swapij{j}{2}$ are transpositions on $\nid$ (*). 
%%  Let $\pi_N = \gconf{N}^0 \gconf{N}^1 \ldots$ be an admissible sequence of configurations in $\gsys{N}$.
%By Lemma 2 in~\cite{tran2020netys}, the application of both transpositions $\swapij{i}{1}$ and $\swapij{j}{2}$ preserves the structure of $\gsys{N}$.
%Hence, we have that  $\transposition^2 ( (\transposition^1 ( \gsys{N}) ) )  = \transposition^2 ( \gsys{N} )  = \gsys{N}$, and 
%$\transposition^2 ( (\transposition^1 ( \ginitconf{N}) ) )  = \transposition^2 ( \ginitconf{N} ) = \ginitconf{N}$.
%Moreover, we have (i) $\psi_{\{\switchIndex{\transposition^1}{i}, \switchIndex{\transposition^2}{j}\}}  = \psi_{\{1, 2\}}$, 
%
%Since $\psi_{\{i, j\}}$ is an \ltlx{} formula, $\All \psi_{\{i, j\}}$ is a CTL*\textbackslash{}X formula where $\All$ is a path operator in CTL*\textbackslash{}X (see~\cite{clarke2018model}). 
%By the semantics of the operator $\All$, it follows  $\forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models  \psi_{\{i, j\}}$ if and only if $\gsys{N}, \ginitconf{N} \models \All \psi_{\{i, j\}}$.
%By point (*), it follows $\gsys{N}, \ginitconf{N} \models \All \psi_{\{i, j\}}$ if and only if $\gsys{N}, \ginitconf{N} \models \All \psi_{\{1, 2\}}$.
%
%We have 
%$ 
%\gsys{N}, \ginitconf{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} \All \psi(i, j)$ if and only if $\gsys{N}, \ginitconf{N} \models \All \psi(1, 2)
%$, because both $i$ and $j$ are arbitrary and different.  
%By the semantics of the operator $\All$, we have $\gsys{N}, \ginitconf{N} \models \All \psi(1, 2)$ if and only if $\forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models \psi(1, 2)$.  
%By Lemma \ref{lem:traceEquiv}, it follows $\forall \pi_N \in \mathit{Path}_N \colon \gsys{N}, \pi_N \models \psi(1, 2)$ if and only if $\forall \pi_2 \in \mathit{Path}_2 \colon \gsys{2}, \pi_2 \models \psi(1, 2)$ 
%.
%Then, Theorem \ref{thm:NCutoffTwoIndexes} holds.
%$\qed$
%%\end{proof}
%
%%\newcommand{\lemSnderRcver}{
%%
%%}
%%
%%\begin{lemma}  \label{lem:snder-rcver}
%%	content...
%%\end{lemma}
%%
%%\subsection{The simplified failure detector with one sender and one receiver}
%%
%%By Theorems~\ref{thm:NCutoffOneIndex} and~\ref{thm:NCutoffTwoIndexes}, we can verify the properties Strong accuracy, Eventually strong accuracy and Strong completeness on  Chandra and Toueg\textquotesingle{}s by checking small instances with only two isomorphic processes.
%%In this section, we present a simplified version of the failure detector of Chandra and Toueg. 
%%The simplified failure detector requires only one sender and one receiver, instead of two isomorphic processes.
%%This simplification help us reduce the complexity of the encoding of the failure detector and the verification work.
%%
%%The sender follows Task 1 in Algorithm~\ref{algo:detector1}; however, the sender does nothing in Task 2 and Task 3.
%%Moreover, the sender does not think of the receiver.
%%Hence, the sender does not have local variables \textit{suspected} and \textit{timeout} as in Algorithm~\ref{algo:detector1}.
%%The receiver follows the intialization step, and Task 2, and Task 3 in Algorithm~\ref{algo:detector1}, but it does not send any message in Task 1.
%%In the simplified model, there is only one message buffer from the sender to the receiver.
%%Moreover, the interesting properties Strong accuracy (SA), Eventually strong accuracy (ESA), and Strong completeness (SC) can be transformed as the following:
%%\begin{center}
%%$
%%\begin{aligned}
%%\mathit{SA}^{\prime} & \triangleq \G ((\mathit{Correct}(s) \land \mathit{Correct}(r)) \Rightarrow \lnot \mathit{Suspected}) \\
%%\mathit{ESA}^{\prime} & \triangleq \F \G ((\mathit{Correct}(s) \land \mathit{Correct}(r)) \Rightarrow \lnot \mathit{Suspected}) \\
%%\mathit{SC}^{\prime} & \triangleq \F \G ((\mathit{Correct}(s) \land \lnot\mathit{Correct}(r)) \Rightarrow \mathit{Suspected})
%%\end{aligned}
%%$
%%\end{center}
%%where $s$ refers to the sender, and $r$ refers to the receiver, and $\mathit{Suspected}$ refers to whether the receiver suspects the sender.
%%
%%While the simplified failure detector is not a symmetric point-to-point algorithm, it is easy to construct a transition system for the simplified failure detector by following the approach introduced in~\cite{tran2020netys}.
%%Intuitively, a global configuration $\gconf{}$ of the simplified failure detector is a tuple 
%%\[
%%((\mathit{pc}_s), (\mathit{pc}_r, \mathit{wT}, \mathit{timeout}, \mathit{suspected}), \mathit{act}_s, \mathit{act}_r, \mathit{buf})
%%\]
%%where
%%\begin{itemize}
%%	\item $s$ refers to the sender, 
%%	\item $r$ refers to the receiver, 
%%	\item $(\mathit{pc}_s)$ refers to the local state of the sender,
%%	\item $(\mathit{pc}_r, \mathit{wT}, \mathit{timeout}, \mathit{suspected})$ refers to the local state of the receiver,
%%	\item $\mathit{wT}$ refers to how long the receiver has waited for the sender, 
%%	\item $\mathit{act}_p$ refers to whether process $p$ is active in $\gconf{}$, and
%%	\item $\mathit{buf}$ refers to the message buffer from the sender to the receiver.
%%\end{itemize} 
%%
%%%The transition system for the simplified failure detector is formalized and presented in Appendix~\ref{sec:formalize}.
%%
%%
%%Theorem~\ref{thm:sa} says that we can verify the property Strong accuracy (SA) on an instance with 2 processes of Chandra and Toueg\textquotesingle{}s failure detector by checking the corresponding instance of the simplified failure detector.
%%
%%
%%\newcommand{\thmSA}{
%%	Let $\gsys{2}(\delta_0, \phi_0, T_0)$ be an instance of the failure detector of Chandra and Toueg with 2 processes, $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$. 
%%	Let $\mathit{Path}_{\mathcal{G}}$ be a set of admissible sequences of configurations of $\gsys{2}(\delta_0, \phi_0, T_0)$ under partial synchrony.
%%	Let $\mathcal{S}(\delta_0, \phi_0, T_0)$ be an instance of the simplified failure detector with $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$.
%%	Let $\mathit{Path}_{\mathcal{S}}$ be a set of admissible sequences of configurations of $\mathcal{S}(\delta_0, \phi_0, T_0)$ under partial synchrony.
%%	It follows that
%%	\[ \forall \pi \in \mathit{Path}_{\mathcal{G}} \colon \pi \vDash SA \Leftrightarrow \forall \pi \in \mathit{Path}_{\mathcal{S}} \colon \pi \vDash SA^{\prime} \]
%%}
%%
%%\begin{theorem} \label{thm:sa}
%%\thmSA
%%\end{theorem}
%%
%%To prove Theorem~\ref{thm:sa}, we introduce the following notations, Definitions~\ref{def:i-snder-proj} and~\ref{def:j-rcver-proj}, and prove Lemma~\ref{lem:snder-rcver-agree}. 
%%
%%
%%\emph{Notations.}
%%The below notations follow the approach in~\cite{tran2020netys}. Let $\gconf{}^{\mathcal{G}}$ be a configuration in $\gsys{2}(\delta_0, \phi_0, T_0)$. For every $i \in \{1, 2\}$, for every $k \geq 0$, we let
%%\begin{itemize}[nosep]
%%%\item $\mathit{Correct}(\gconf{}^{\mathcal{G}}, i)$ denotes whether process $i$ is correct in configuration $\gconf{}^{\mathcal{G}}$, and
%%
%%\item $\mathit{lstate}(\gconf{}^{\mathcal{G}}, i)$ denotes the state of process $i$ in $\gconf{}^{\mathcal{G}}$, and
%%
%%\item $\mathit{v}(\mathit{lstate}(\gconf{}^{\mathcal{G}}, i))$ denotes the value of local variable $v$ of process $i$ in $\gconf{}^{\mathcal{G}}$, and
%%
%%\item $\mathit{active}(\gconf{}^{\mathcal{G}}, i)$ denotes whether process $i$ is active in $\gconf{}^{\mathcal{G}}$, and
%%
%%\item $\mathit{buf}(\gconf{}^{\mathcal{G}}, i, j)$ denotes the message buffer from process $i$ to process $j$ in $\gconf{}^{\mathcal{G}}$.
%%\end{itemize}
%%We override notations by writing %$\mathit{Correct}(\gconf{}^{\mathcal{S}}, p)$, 
%%$\mathit{lstate}(\gconf{}^{\mathcal{S}}, p)$, 
%%$\mathit{v}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, p))$,
%%$\mathit{active}(\gconf{}^{\mathcal{S}}, p)$,
%%and $\mathit{buf}(\gconf{}^{\mathcal{S}})$ where $\gconf{}^{\mathcal{S}}$ is a configurations of $\mathcal{S}(\delta_0, \phi_0, T_0)$, and $p$ refers to either the sender or the receiver, and 
%%$\mathit{buf}(\gconf{}^{\mathcal{S}})$ is the message buffer in $\gconf{}^{\mathcal{S}}$.
%%Recall that the sender has a local variable $\mathit{pc}$, and 
%%$\mathit{pc}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, s))$ refers to whether the sender is correct in $\gconf{}^{\mathcal{S}}$.
%%
%%\newcommand{\defISnderProj}{
%%	Let $\gsys{2}(\delta_0, \phi_0, T_0)$ be an instance of the failure detector of Chandra and Toueg with 2 processes, $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$. 
%%	Let $\mathcal{S}(\delta_0, \phi_0, T_0)$ be an instance of the simplified failure detector with $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$.
%%	Let $\gconf{}^{\mathcal{G}}$ be a configuration in $\gsys{2}(\delta_0, \phi_0, T_0)$, and $\gconf{}^{\mathcal{S}}$ be a configuration in $\mathcal{S}(\delta_0, \phi_0, T_0)$.
%%	Let $i$ and $j$ be numbers such that $i, j \in \{ 1, 2\}$ and $i \neq j$.
%%	Configuration $\gconf{}^{\mathcal{S}}$ is called the \emph{$i$-snder projection} of configuration $\gconf{}^{\mathcal{G}}$ if the following properties hold:
%%	\begin{enumerate}[nosep]
%%	\item $\mathit{pc}(\mathit{lstate}(\gconf{}^{\mathcal{G}}, i)) = \mathit{pc}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, s))$,
%%	
%%	\item $\mathit{active}(\gconf{}^{\mathcal{G}}, i) = \mathit{active}(\gconf{}^{\mathcal{S}}, s)$, and
%%	
%%	\item $\mathit{buf}(\gconf{}^{\mathcal{G}}, i, j) = \mathit{buf}(\gconf{}^{\mathcal{S}})$
%%	\end{enumerate}
%%	where $s$ refers to the sender.
%%}
%%
%%\begin{definition}
%%\emph{\textbf{(i-snder projection)}} 
%%\defISnderProj{} \label{def:i-snder-proj}
%%\end{definition}
%%
%%
%%\newcommand{\defJRcverProj}{
%%	Let $\gsys{2}(\delta_0, \phi_0, T_0)$ be an instance of Chandra and Toueg\textquotesingle{}s failure detector with 2 processes, $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$. 
%%	Let $\mathcal{S}(\delta_0, \phi_0, T_0)$ be an instance of the simplified failure detector with $\Delta = \delta_0$, $\Phi = \phi_0$ and GST $= T_0$.
%%	Let $\gconf{}^{\mathcal{G}}$ be a configuration in $\gsys{2}(\delta_0, \phi_0, T_0)$, and $\gconf{}^{\mathcal{S}}$ be a configuration in $\mathcal{S}(\delta_0, \phi_0, T_0)$.
%%	Let $i$ and $j$ be numbers such that $i, j \in \{ 1, 2\}$ and $i \neq j$.
%%	Configuration $\gconf{}^{\mathcal{S}}$ is called the \emph{$j$-rcver projection} of configuration $\gconf{}^{\mathcal{G}}$ if the following properties hold:
%%	\begin{enumerate}[nosep]
%%		\item $\mathit{pc}(\mathit{lstate}(\gconf{}^{\mathcal{G}}, j)) = \mathit{pc}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, r))$,
%%		
%%		\item $\mathit{timeout}(\mathit{lstate}(\gconf{}^{\mathcal{G}}, j)) = \mathit{timeout}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, r))$,
%%		
%%		\item $\mathit{suspected}(\mathit{lstate}(\gconf{}^{\mathcal{G}}, j)) = \mathit{suspected}(\mathit{lstate}(\gconf{}^{\mathcal{S}}, r))$,
%%		
%%		\item $\mathit{active}(\gconf{}^{\mathcal{G}}, j) = \mathit{active}(\gconf{}^{\mathcal{S}}, r)$, and
%%		
%%		\item $\mathit{buf}(\gconf{}^{\mathcal{G}}, i, j) = \mathit{buf}(\gconf{}^{\mathcal{S}})$
%%	\end{enumerate}
%%	where $r$ refers to the receiver.
%%}
%%
%%\begin{definition}
%%\emph{\textbf{(j-rcver projection)}} 
%%\defJRcverProj
%%\label{def:j-rcver-proj}
%%\end{definition}
%%
%
%



==> forte21/experiments.tex <==
In this section, we describe our experiments with~\tlap{}, \fast{} and Ivy.
We ran the following experiments on a virtual machine with Core i7-6600U CPU and 8GB DDR4. 
Our specifications can be found at~\cite{fdSpec}.

%In the following experiments, we verify Strong accuracy, Eventually strong accuracy, and Strong completeness on the failure detector in different cases, e.g., fixed parameters or arbitrary parameters.
%Our experiments show that partial synchrony indeed is a challenge to existing verification frameworks, and requires more research.

\subsection{Model checkers for~\tlap{}: TLC and~\apalache{}}

In our work, we use~\tlap{}~\cite{lamport2002specifying} to specify the failure detector with both encoding techniques for the message buffer, and the abstraction in Section~\ref{sec:encoding}.
Then, we use the model checkers TLC~\cite{yu1999model} and~\apalache{}~\cite{konnov2019tla} to verify instances with
fixed bounds $\Delta$ and $\Phi$, and the GST $T_0 = 1$.
This approach helps us to search constraints in inductive invariants in case of fixed parameters.
The main reason is that counterexamples and inductive invariants in case of fixed parameters, e.g., $\Delta \leq 1$ and $\Phi \leq 1$, are simpler than in case of arbitrary parameters.
Hence, if a counterexample is found, we can quickly analyze it, and change constraints in an inductive invariant candidate.	
After obtaining inductive invariants in small cases, we can generalize them for cases of arbitrary bounds, and check with theorem provers, e.g., Ivy.

%In the following, we present how to encode the send action in~\tlap{},
%and describe the experiments related to the model checkers TLC and~\apalache{}.

%\tlap{} is an untyped specification language based on Temporal Logic of Actions (TLA)~\cite{lamport1994temporal}, and the Zermelo-Fr{\"a}nkel set theory with the axiom of choice. 
\tlap{} offers a rich syntax for sets, functions, tuples, records, sequences, and control structures~\cite{lamport2002specifying}.
Hence, it is straightforward to apply the encoding techniques and the abstraction presented in Section~\ref{sec:encoding} in~\tlap{}.
For example, Figure~\ref{fig:send-tla} represents a \tlap{} action \emph{SSnd} for sending a new message in case of $\Delta > 0$.
Variables $\mathit{ePC}$ and $\mathit{sPC}$ are program counters for the environment and the sender, respectively.
Line 1 is a precondition, and refers to that the environment is in subround Send.
Lines 2--3 say that if the sender is active in subround Send, the counter $\mathit{buf}^{\prime}$ is increased by 1.
Otherwise, two counters $\mathit{buf}$ and $\mathit{buf}^{\prime}$ are the same (Line 4).
Line 5 implies that the environment is still in the subround Send, but it is now the receiver\textquotesingle{}s turn.
Line 6 guarantees that other variables are unchanged in this action.
The details are left for Appendix~\ref{sec:tla-spec}.
\begin{figure}[ht]
	\input{send-tla}
	\caption{Sending a new message in~\tlap{} in case of $\Delta > 0$}
	\label{fig:send-tla}
\end{figure}
%In Appendix~\ref{sec:tla-spec}, we present the~\tlap{} specification of the failure detector with our inductive invariant for the safety propery Strong accuracy.
%In this specification, the message buffer is encoded with a function.

Now we present the experiments with TLC and~\apalache{}. 
From now on, we call the case of GST $T = 1$ the \emph{initial stabilization}.
%~\footnote{in case of unknown $\Delta$ and $\Phi$, GST $T_0$ is also 1, and both bounds $\Delta$ and $\Phi$ are arbitrary.}
We used these tools to verify (i) the safety property Strong accuracy, and (ii) an inductive invariant for Strong accuracy, and (iii) an inductive invariant for a safety property reduced from the liveness property Strong completeness in case of fixed bounds and the initial stabilization.
The inductive invariants verified here are very close to the inductive invariants in case of arbitrary bounds $\Delta$ and $\Phi$.
Strong completeness is a bounded liveness property; therefore, it becomes a safety property.
Reduction from the liveness properties of the failure detector to safety ones is left in Appendix~\ref{sec:reduction}.





%From now on, we call the case of $T_0 = 1$ the \emph{initial stabilization} one.
Table~\ref{tab:exp-sa-inv} summarizes the results in verification of Strong accuracy in case of the initial stabilization, and fixed bounds $\Delta$ and $\Phi$.
To make the comparison of verification tools readable, Table~\ref{tab:exp-sa-inv} shows the experiments with three tools TLC, \apalache{}, and \fast{}.
The column ``\#states'' shows the number of distinct states explored by TLC.
The column ``\#depth'' shows the maximum execution length reached by TLC and~\apalache{}.
The column ``buf'' shows how to encode the message buffer.
The column ``LOC'' shows the number of lines in the specification of the system behaviors (without comments).
The symbol ``-'' (minus) refers to that the experiments are intentionally missing since~\fast{} does not support the encoding of the message buffer with a predicate.
In this case, we initially set $\timeout{} = 6 \times \Phi + \Delta$, and Strong accuracy is satisfied.
The experiments show that TLC finished its tasks faster than others, and  \apalache{} prefers the encoding of the message buffer with a predicate.
The abbreviation ``TO'' means a timeout of 6 hours.


\begin{table}
	\centering
	\caption{The experiments on checking Strong accuracy with TLC, \apalache{}, and \fast{} in case of fixed parameters. 
		In this case, Strong accuracy is satisfied.} \label{tab:exp-sa-inv}
	\begin{tabular}{>{\centering\arraybackslash}p{0.4cm} |  >{\centering\arraybackslash}p{0.4cm} | 
			>{\centering\arraybackslash}p{0.4cm} |
			>{\raggedleft\arraybackslash}p{0.7cm}
			>{\raggedleft\arraybackslash}p{1.2cm}
			>{\raggedleft\arraybackslash}p{0.9cm}
			>{\raggedleft\arraybackslash}p{0.8cm}	
			>{\raggedleft\arraybackslash}p{1.1cm} |
			>{\raggedleft\arraybackslash}p{0.7cm}
			>{\raggedleft\arraybackslash}p{0.9cm}
			>{\raggedleft\arraybackslash}p{0.8cm} |
			>{\raggedleft\arraybackslash}p{0.7cm} 
			>{\raggedleft\arraybackslash}p{0.8cm}
			>{\raggedleft\arraybackslash}p{1.1cm}} 
		\multirow{2}{*}{\#} & \multirow{2}{*}{$\Delta$} & \multirow{2}{*}{$\Phi$} & \multicolumn{5}{c|}{TLC} & \multicolumn{3}{c|}{\apalache{}} & \multicolumn{3}{c}{\fast} \\   
		\cline{4-14}
		& & & time & \#states & depth & buf & LOC & time & depth & buf & time & buf & LOC \\
		\hline
		1  & \multirow{2}{*}{2} &  \multirow{2}{*}{4} & 3s & 10.2K & 176 & fnc & 190 & 8m & 176 & fnc & - & - & - \\
		2  &  &  & 3s & 10.2K & 176 & cntr & 266 & 9m & 176 & cntr & 16m & cntr & 387 \\
		\hline
		3  & \multirow{2}{*}{4} &  \multirow{2}{*}{4} & 3s & 16.6K & 183 & fnc & 190 & 12m & 183 & fnc & - & - & - \\
		4  &  &  & 3s & 16.6K & 183 & cntr & 487 & 35m & 183 & cntr & TO & cntr & 2103 \\
		\hline
		5  & \multirow{2}{*}{4} &  \multirow{2}{*}{5} & 3s & 44.7K & 267 & fnc & 190 & TO & 222 & fnc & - & - & - \\
		6  &  &  & 3s & 44.7K &  267 & cntr & 487 & TO & 223 & cntr & TO & cntr & 2103 \\
	\end{tabular}
\end{table}

%\begin{table}[!htbp]
%	\centering
%	\caption{The experiments on checking Strong accuracy with TLC, \apalache{}, and \fast{} in case of fixed parameters. 
%		In this case, Strong accuracy is satisfied.} \label{tab:exp-sa-inv}
%	\begin{tabular}{>{\centering\arraybackslash}p{0.4cm} |  >{\centering\arraybackslash}p{0.4cm} | 
%			>{\centering\arraybackslash}p{0.4cm} |
%			>{\centering\arraybackslash}p{2cm}
%			>{\centering\arraybackslash}p{2.2cm}			
%			>{\raggedleft\arraybackslash}p{1cm}
%			>{\raggedleft\arraybackslash}p{1.2cm}} 
%		\multirow{2}{*}{\#} & \multirow{2}{*}{$\Delta$} & \multirow{2}{*}{$\Phi$} & \multirow{2}{*}{Tool} & Encoding of & \multirow{2}{*}{Time}  & \multirow{2}{*}{\#Line$_S$}  \\  
%		&  &  &  & message buffer &  &    \\  
%		\hline
%		1  & \multirow{5}{*}{2}   &  \multirow{5}{*}{4} & TLC & fnc & 3s & 190   \\                
%		2  &    &   & TLC & cntr & 3s & 266  \\                
%		3  &    &   & \apalache{} & fnc & 11m & 190   \\                
%		4  &    &   & \apalache{} & cntr & 14m & 266   \\                
%		5  &    &   & \fast{} & cntr & 2m & 387   \\                
%		\hline
%		1  & \multirow{5}{*}{4}   &  \multirow{5}{*}{4} & TLC & fnc & 3s & 190   \\                
%		2  &    &   & TLC & cntr & 3s & 487  \\                
%		3  &    &   & \apalache{} & fnc & 19m & 190   \\                
%		4  &    &   & \apalache{} & cntr & 47m & 266   \\                
%		5  &    &   & \fast{} & cntr & 17m & 2103 \\                                        
%	\end{tabular}
%\end{table}



\begin{table}[!htbp]
	\centering
	\caption{The experiments on checking Strong accuracy with TLC, \apalache{}, and \fast{} in case of fixed parameters. 
		In this case, Strong accuracy is violated.} \label{tab:exp-sa-inv-bug}
	\begin{tabular}{>{\centering\arraybackslash}p{0.4cm} |  >{\centering\arraybackslash}p{0.4cm} | 
			>{\centering\arraybackslash}p{0.4cm} |
			>{\raggedleft\arraybackslash}p{0.7cm}
			>{\raggedleft\arraybackslash}p{1.4cm}
			>{\raggedleft\arraybackslash}p{1.1cm}
			>{\raggedleft\arraybackslash}p{0.9cm} |
			>{\raggedleft\arraybackslash}p{1cm}
			>{\raggedleft\arraybackslash}p{1.1cm}
			>{\raggedleft\arraybackslash}p{0.9cm} |
			>{\raggedleft\arraybackslash}p{0.7cm} 
			>{\raggedleft\arraybackslash}p{0.9cm}} 
		\multirow{2}{*}{\#} & \multirow{2}{*}{$\Delta$} & \multirow{2}{*}{$\Phi$} & \multicolumn{4}{c|}{TLC} & \multicolumn{3}{c|}{\apalache{}} & \multicolumn{2}{c}{\fast} \\   
		\cline{4-12}
		& & & time & \#states & depth & buf & time & depth & buf & time & buf  \\
		\hline
		1  & \multirow{2}{*}{2} &  \multirow{2}{*}{4} & 1s & 840 & 43 & fnc  & 11s & 42 & fnc & - & - \\
		2  &  &  & 1s & 945 & 43 & cntr & 12s & 42 & cntr & 10m & cntr  \\
		\hline
		3  & \multirow{2}{*}{4} &  \multirow{2}{*}{4} & 2s & 1.3K & 48 & fnc & 15s & 42 & fnc & - & - \\
		4  &  &  & 2s & 2.4K & 56 & cntr & 16s & 42 & cntr & TO & cntr                     \\
		\hline
		5  & 20 & 20 & TO & 22.1K & 77 & fnc & 1h15m & 168 & fnc & - & - \\
	\end{tabular}
\end{table}

Table~\ref{tab:exp-sa-inv-bug} summarizes the results in verification of Strong accuracy with the tools TLC, \apalache{}, and \fast{} in case of the initial stabilization, and small bounds $\Delta$ and $\Phi$, and initially $\timeout{} = \Delta + 1$.
The meaning of other columns is the same as in Table~\ref{tab:exp-sa-inv}.
The abbreviation ``TO'' means a timeout of 6 hours.
In this case, Strong accuracy is violated, and~\apalache{} is the winner.




Table~\ref{tab:exp-sa-iinv} summarizes the results in verification of inductive invariants for Strong accuracy and Strong completeness with TLC and \apalache{} in case of the initial stabilization, and small bounds $\Delta$ and $\Phi$.
The message buffer was encoded with a predicate in these experiments.
In these experiments, inductive invariants hold, and \apalache{} is faster than TLC in verifying them.

As one sees from the above tables,~\apalache{} is fast at proving inductive invariants, and at finding a counterexample when a desired safety property is violated.
TLC is a better option in cases where a safety property is satisfied.

In order to prove correctness of the failure detector in cases where parameters $\Delta$ and $\Phi$ are arbitrary, the user can use the interactive theorem prover \tlap{} Proof System (\tlaps{})~\cite{chaudhuri2010tla+}.
However, proving the failure detector with \tlaps{} requires more human effort than with Ivy.
Another shortcoming of \tlaps{} is that it does not provide a counterexample when an inductive invariant candidate is violated.
Hence, we did not prove the failure detector with \tlaps{}.

\begin{table}
	\centering
	\caption{The experiments on checking inductive invariants  with the tools TLC and~\apalache{}. 
		In this case, inductive invariants are satisfied.} \label{tab:exp-sa-iinv}
	\begin{tabular}{>{\centering\arraybackslash}p{0.4cm} |  >{\centering\arraybackslash}p{0.4cm} | 
			>{\centering\arraybackslash}p{0.4cm} |
			>{\centering\arraybackslash}p{3.3cm} |
			>{\raggedleft\arraybackslash}p{0.7cm}
			>{\raggedleft\arraybackslash}p{1.4cm} |
			>{\centering\arraybackslash}p{2.4cm}} 
		\multirow{2}{*}{\#} & \multirow{2}{*}{$\Delta$} & \multirow{2}{*}{$\Phi$} & \multirow{2}{*}{Property} & \multicolumn{2}{c|}{TLC} & \apalache{}   \\  
		\cline{5-7}
		&  &  &  & time & \#states & \multicolumn{1}{c}{time}   \\  
		\hline
		1  & 4   &  40 & Strong accuracy & 33m & 347.3M & 12s \\    
		\hline
		2  &  4   &  10 & Strong completeness & 44m & 13.4M & 17s
	\end{tabular}
\end{table}



\subsection{\fast{}}

A shortcoming of the model checkers TLC and~\apalache{} is that parameters $\Delta$ and $\Phi$ must be fixed before running these tools.
\fast{} is a tool designed to reason about safety properties of counter systems, i.e. automata extended with unbounded integer variables~\cite{bardin2006fast}.
If $\Delta$ is fixed, and the message buffer is encoded with a counter, the failure detector becomes a counter system.
In our experiments, we specified the failure detector in~\fast{}, and checked them with different configurations of parameters: (i) the initial stabilization, and fixed bounds $\Delta$ and $\Phi$, and (ii) the initial stabilization, fixed $\Delta$, but arbitrary $\Phi$.



Figure~\ref{fig:send-fast} represents a \fast{} transition for sending a new message in case of $\Delta > 0$.
Line~2 describes the (symbolic) source state of the transition, and region \texttt{incMsgAge} is a set of configurations in the failure detector that is reachable from a transition for increasing message ages.
Line 3 mentions the (symbolic) destination state of the transition, and region \texttt{sSnd} is a set of configurations in the failure detector that is reachable from a transition named ``SSnd\_Active'' for sending a new message.
Line 4 represents the guard of this transition, and operator \&\& is the logical AND operator.
%This characteristic makes ~\fast{} specifications less readable.
Line 5 is an action.
Every unprimed variable that is not written in Line 5 is unchanged.


\begin{figure}[thp]
	\centering
	\begin{minipage}{.7\linewidth}
	\begin{algorithmic}[1] 
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		 
		\State \textbf{transition} SSnd\_Active  $\coloneq \{$
		\State $\qquad $\textbf{from} $\coloneq$ incMsgAge;
		\State $\qquad $\textbf{to} $\coloneq$ ssnd;
		\State $\qquad $\textbf{guard} $\coloneq$ sTimer = 0;
		\State $\qquad $\textbf{action} := buf$^{\prime}$ = buf + 1; $\}$;
	\end{algorithmic}\caption{Sending a new message in~\fast{} in case of $\Delta > 0$} 
	\label{fig:send-fast}
	\end{minipage}
\end{figure}


The input language of~\fast{} is based on Presburger arithmetics
for both system and properties specification.
Hence, we cannot apply the encoding of the message buffer with a predicate in~\fast{}.

Tables~\ref{tab:exp-sa-inv} and~\ref{tab:exp-sa-inv-bug} described in the previous subsection summarize the experiments with~\fast{}, and other tools where all parameters are fixed.
Moreover, we ran~\fast{} to verify Strong accuracy in case of the initial stabilization, $\Delta \leq 4$, and arbitrary bound $\Phi$.
\fast{} is a semi-decision procedure; therefore, it does not terminate on some inputs.
Unfortunately,~\fast{} could not prove Strong accuracy in case of arbitrary bound $\Phi$, and crashed after 30 minutes.



\subsection{Ivy}

While TLC, \apalache{}, and~\fast{} can automatically verify some instances of the failure detector with fixed parameters, these tools cannot handle cases with arbitrary bounds $\Delta$ and $\Phi$.
To overcome this problem, we specify and prove correctness of the failure detector with the interactive theorem prover Ivy~\cite{ivy}.
In the following, we first discuss the encoding of the failure detector in Ivy, and then presents the experiments with Ivy.


Since bound $\Phi$ is arbitrary, we need to encode the message buffer with a predicate.
In Ivy, we declare
$\texttt{relation } \existsMsgOfAge(X \colon \tnumber)$. 
Type \texttt{num} is interpreted as integers.
Since Ivy does not support primed variables, we need an additional relation $\tmpExistsMsgOfAge(X : \tnumber)$.  
Intuitively, we first compute and store the value of~\existsMsgOfAge{} in the next state in~\tmpExistsMsgOfAge{}, then copy the value of~\tmpExistsMsgOfAge{} back to~\existsMsgOfAge{}.
We do not consider the requirement of \tmpExistsMsgOfAge{} as a shortcoming of Ivy since it is still straightforward to transform the ideas in Section~\ref{sec:encoding} to Ivy.

Figure~\ref{fig:send-ivy} represents how to add a fresh message in the message buffer in Ivy.
Line~1 means that $\tmpExistsMsgOfAge$ is assigned an arbitrary value. 
Line~2 guarantees the appearance of a fresh message.
Line~3 ensures that every in-transit message in $\existsMsgOfAge$ is preserved in $\tmpExistsMsgOfAge$.
Line~4 copies the value of $\tmpExistsMsgOfAge$ back to $\existsMsgOfAge$.

\vspace{-2mm}
\begin{figure}[thp]
\begin{algorithmic}[1] 
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		 
		\State $\tmpExistsMsgOfAge(X) \coloneq *;$
		\State \textbf{assume} $\tmpExistsMsgOfAge(0);$
		\State \textbf{assume forall} $X \colon \tnumber \qdot 0 < X \rightarrow \existsMsgOfAge(X) = \tmpExistsMsgOfAge(X);$
		\State $\existsMsgOfAge(X) \coloneq \tmpExistsMsgOfAge(X);$
\end{algorithmic}
\caption{Adding a fresh message in Ivy} 
\label{fig:send-ivy}
\end{figure}
\vspace{-4mm}

Importantly, our specifications are not in decidable theories supported by Ivy.
In Formula~\ref{eq:inc2}, the interpreted function $``+"$ (addition) is applied to a universally quantified variable $x$.

The standard way to check whether a safety property \textit{Prop} holds in an Ivy specification is to find an inductive invariant \textit{IndInv} with \textit{Prop}, and to (interactively) prove that \textit{Indinv} holds in the specification. 
To verify the liveness properties Eventually strong accuracy and Strong completeness, we reduced them into safety properties by applying the reduction technique in Appendix~\ref{sec:reduction}, and found inductive invariants containing the resulted safety properties.
These inductive invariants are the generalization of the inductive invariants in case of fixed parameters that were found in the previous experiments.

\begin{table}
	\centering
	\caption{The experiments on verification of inductive invariants of the failure detector with Ivy in case of arbitrary $\Delta$ and $\Phi$.} \label{tab:exp-iinv-ivy}
	\begin{tabular}{>{\centering\arraybackslash}p{0.5cm} |  			>{\centering\arraybackslash}p{3cm} |
			>{\raggedright\arraybackslash}p{1.8cm} 
			>{\raggedleft\arraybackslash}p{1cm}
			>{\raggedleft\arraybackslash}p{1.1cm}
			>{\raggedleft\arraybackslash}p{1.3cm}
			>{\raggedleft\arraybackslash}p{2.5cm}} 
		\multirow{2}{*}{\#} & \multirow{2}{*}{Property} & \multirow{2}{*}{$\;\;\timeout{}_{\text{init}}$} & \multirow{2}{*}{time} & \multirow{2}{*}{LOC} & \multirow{2}{*}{$\#\text{line}_I$} & \#strengthening  \\ 
		& &  & & & & steps \\                 
		\hline
		1  & Strong accuracy & $= 6 \times \Phi + \Delta$ & 4s & 183 & 30 & 0 \\    
		\hline
		\multirow{2}{*}{2}  & \multirow{2}{*}{\shortstack[c]{Eventually \\ strong accuracy}} & \multirow{2}{*}{$= \star$} & \multirow{2}{*}{4s} & \multirow{2}{*}{186} & \multirow{2}{*}{35} & \multirow{2}{*}{0} \\                
		& &  &  & & &\\                      		
		\hline
		3  & \multirow{3}{*}{Strong completeness} & $= 6 \times \Phi + \Delta $ & 8s & 203 & 111 & 0 \\                
		4  & & $\geq 6 \times \Phi + \Delta$ &  22s & 207 & 124 & 15 \\                
		5  & & $= \star$ & 44s & 207 & 129 & 0\\                
	\end{tabular}
\end{table}

Table~\ref{tab:exp-iinv-ivy} shows the experiments on verification of the failure detector with Ivy in case of unknown bounds $\Delta$ and $\Phi$.
The symbol $\star$ refers to that the initial value of \timeout{} is arbitrary.
The column ``$\#\text{line}_I$'' shows the number of lines of an inductive invariant, and the column ``$\#\text{strengthening steps}$'' shows the number of lines of strengthening steps that we provided for Ivy.
The meaning of other columns is the same as in Table~\ref{tab:exp-sa-inv}.
While our specifications are not in decidable theories supported in Ivy, our experiments show that Ivy needs no user-given strengthening steps to prove most of our inductive invariants.
Hence, it took us about 4 weeks to learn Ivy from scratch, and to prove these inductive invariants.% in Table~\ref{tab:exp-iinv-ivy}.

The most important thing to prove a property satisfied in an Ivy specification is to find an inductive invariant.
A detailed explanation of the inductive invariants in Table~\ref{tab:exp-iinv-ivy} is provided in Appendixes~\ref{sec:sa}--\ref{sec:sc_fixed}.
%While our specification describes executions of the Chandra and Toueg failure detector, many time constraints on network behaviors, correct processes, and failures in our inductive invariants can be reused to
%prove other algorithms under many partially synchronous models.
Some unexpected behaviors of Ivy (and Z3) that we faced in our work are discussed in Appendix~\ref{sec:unexpected}.

%Despite the above challenge, Ivy is a potential framework to verify algorithms with arbitrary parameters.

%We found that the Ivy language is convenient to specify the failure detector.
%It took us 1 week to learn Ivy\jw{Not sure that belongs here. We might
%but this into the conclusions???} from scratch and to complete the first Ivy specification for the simplified failure detectors, and to prove some simple inductive invariant, e.g., type invariants.
%
%
%\jw{the following needs to be written differently. Not sure how}
%Then, we tried to prove\jw{?} an inductive invariant candidate for Strong accuracy with Ivy before but Ivy could not prove it and not return a counterexample in 30 minutes.
%Notice that our specification is not in Ivy\textquotesingle{}s decidable theories.
%One shortcoming in Ivy is the lack of examples with its advanced features on its official website~\cite{ivy}, especially for proving inductive invariants.
%It took us one more week to learn Ivy\textquotesingle{}s advanced features from~\cite{ivyTendermint}, and to fix an inductive invariant, and to add proof hints for Ivy. 
%The proof hints are about 50 lines.
%Ivy could prove this version of our specification; however, we found the unexpected behavior of Ivy which described in details in Section~\ref{sec:unexpected}.
%In detail, we ran Ivy to check some formula that is not an inductive invariant in the simplified failure detectors, but Ivy considered this formula as an inductive invariant in our specification.
%It took us~1 week to find the reasons and a solution for our encoding.
%Importantly, the new version contains no proof hints.
%Now Ivy can prove an inductive invariant in a minute, and find a counterexample in a wrong inductive invariant in a minute.
%Totally, it took us 3 weeks to verify the property Strong accuracy on the simplified failure detectors with Ivy.
%
%After that, we spent two weeks to find inductive invariants for Eventually strong accuracy and Strong completeness, and to prove them with Ivy.
%Ivy can prove these inductive invariants quickly.







==> forte21/fast-intro.tex <==
 is a tool designed to reason about safety properties of counter systems,
i.e. automata extended with unbounded integer variables~\cite{bardin2006fast}.
The input language of FAST is based heavily on Presburger arithmetics
for both system and properties specification.
Moreover, this language supports the control structure of the automaton (nodes and transitions), Boolean operators, control statements (\texttt{IF THEN ELSE} and assignments), and regions that represent (symbolic) sets of states. 
Hence, the input language of FAST is expressive enough to specify many algorithms such as the fault-tolerant TTP protocol~\cite{kopetztime}.
However,~\fast{} does not offer some common data structures, e.g., sets, functions, and records. 

To efficiently compute the reachability set, FAST applies mordern techniques: acceleration, flattening, and reduction.
FAST has been used to verify many algorithms, e.g., the TTP protocol, and the MESI protocol.

Finally, \fast{} is a semi-decision procedures. So, it does not terminate on some inputs.




==> forte21/fd.tex <==
%In this section, we discuss one benchmark of failure detectors~\cite{CT96}, and the cutoff results in~\cite{tran2020netys} that we can extend to the failure detector under partial synchrony.

This section describes the Chandra and Toueg failure detector~\cite{CT96}, and the cutoff results~\cite{tran2020netys} that we can extend to this failure detector under partial synchrony.

\begin{algorithm}[htb] 
	\caption{The eventually perfect failure detector algorithm in \cite{CT96}} \label{algo:detector1}
	\begin{algorithmic}[1] 
		\State \emph{Every process $p \in \nid$ executes the following}:
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\For{$\textbf{all } q \in \nid $}    \Comment{Initalization step}
		\State $\fdtimeout{p}{q} \coloneq \text{default-value}$ %; $\suspected{p}{q} = \False$ \}  \label{algo:initStep1} %\label{algo:initStep2}
		\State $\fdsuspected{p}{q} \coloneq \False$ \             \label{algo:initStep2}
		\EndFor
		%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\State Send ``alive'' to all $q \in  \nid$ \label{algo:task1}
		\Comment{Task 1: repeat periodically}
		%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
		\For{\textbf{all} $q  \in \nid$}  \label{algo:task2}    \Comment{Task 2: repeat periodically}
		\If{$\fdsuspected{p}{q} = \False \textbf{ and not hear } q \text{ during last } \fdtimeout{p}{q} \text{ ticks}$} 
		\State $\fdsuspected{p}{q} \coloneq \True$    
		\EndIf    
		\EndFor
		%    
		\If{$\fdsuspected{p}{q}$} \label{algo:task3} 
		\Comment{Task 3: when receive ``alive'' from $q$}
		\State $\fdtimeout{p}{q} \coloneq \fdtimeout{p}{q} + 1$ %; $\fdsuspected{p}{q} = \False$ \}
		\State $\fdsuspected{p}{q} \coloneq \False$ 
		\EndIf            
	\end{algorithmic}
\end{algorithm} 

A failure detector can be seen as an oracle to get information about crash failures in the distributed system. 
A failure detector usually guarantees some of the following properties~\cite{CT96} (numbers $\nid$ denote the process identifiers):
\begin{itemize}[nosep] \label{properties}
	\item Strong Accuracy: No process is suspected before it crashes.	
	
	$
	\begin{aligned}
	\qquad \G (\A p, q \in \nid \colon (\mathit{Correct}(p) \land \mathit{Correct}(q)) \Rightarrow \lnot \mathit{Suspected}(p, q))
	\end{aligned}
	$
	
	\item Eventual Strong Accuracy: There is a time after which correct processes are not suspected by any correct process.
	
	$
	\begin{aligned}
	\qquad \F \G (\A p, q \in \nid \colon (\mathit{Correct}(p) \land \mathit{Correct}(q)) \Rightarrow \lnot \mathit{Suspected}(p, q))
	\end{aligned}
	$
	
	\item Strong Completeness: Eventually every crashed process is  permanently suspected by every correct process.
	
	$
	\begin{aligned}
	\qquad \F \G (\A p, q \in \nid \colon (\mathit{Correct}(p) \land \lnot\mathit{Correct}(q)) \Rightarrow \mathit{Suspected}(p, q))
	\end{aligned}
	$
\end{itemize}
where $\F$ and $\G$ are operators in LTL (linear temporal logic), predicate $\mathit{Suspect}(p, q)$ refers to whether process $p$ suspects process $q$ in crashing, and predicate $\mathit{Correct}(p)$ refers to whether process $p$ is correct.
However, process $p$ might crash later (and not recover).
A crashed process $p$ satisfies $\lnot \mathit{Correct}(p)$.


Algorithm~\ref{algo:detector1} presents the pseudo-code of the failure detector of~\cite{CT96}.
A system instance has $N$ processes that  communicate with each other by sending-to-all and receiving messages through unbounded $N^2$ point-to-point communication channels.  
A process performs local computation based on received messages (we assume that a
process also receives the messages that it sends to itself).
In one system step, all processes may take up to one step.
Some processes may crash, i.e., stop operating.
Correct processes follow Algorithm~\ref{algo:detector1} to detect crashes in the system.
Initially, every correct process sets a default value for a timeout of each other, i.e. how long it should wait for others 
%(Line~\ref{algo:initStep1}), 
and assumes that no processes have crashed (Line~\ref{algo:initStep2}). 
Every correct process $p$ has three tasks: (i) repeatedly sends an ``alive'' message to all (Line~\ref{algo:task1}), 
and (ii) repeatedly produces predictions about crashes of other processes based on timeouts (Line~\ref{algo:task2}),
and (iii) increases a timeout for process $q$ if $p$ has learned that its suspicion on $q$ is wrong (Line~\ref{algo:task3}).
Notice that process $p$ raises suspicion on the operation of process $q$ (Line~\ref{algo:task2}) by considering only information related to $q$: $\fdtimeout{p}{q}, \fdsuspected{p}{q}$, and messages that $p$ has received from $q$ recently.
%In other words, its suspicions about other processes grow independently.


Algorithm~\ref{algo:detector1} does not satisfy  Eventually Strong Accuracy under asynchrony since there exists no bound on message delay, and messages sent by correct processes might always arrive after the timeout expired. 
Liveness of the failure detector is based on the existence of bounds $\Delta$  on the message delay, and $\Phi$ on the relative speed of processes after reaching the global stabilization at some time point $T_0$~\cite{CT96}.
There are many models of partial synchrony~\cite{DLS88,CT96}.
In this paper, we focus only on the case of unknown bounds $\Delta$ and $\Phi$ because other models might call for abstractions.
In this case, $T_0 = 1$, and both parameters $\Delta$ and $\Phi$ are arbitrary.
Moreover, the following constraints hold in every execution:
\begin{itemize}[noitemsep,topsep=0pt]
	\newcounter{foo}	
	\item Constraint \refstepcounter{foo}\thefoo\label{delta}: If message $m$ is placed in the message buffer from process $q$ to process $p$ by some $Send(m, p)$ at a time $s_1 \geq 1$, and if process $p$ executes a $Receive(p)$ at a time $s_2$ with $s_2 \geq s_1 + \Delta$, then message $m$ must be delivered to $p$ at time $s_2$ or earlier.
	
	\item Constraint \refstepcounter{foo}\thefoo\label{phi}:  In every contiguous time interval $\left[ t, t + \Phi \right]$ with $t \geq 1$, every correct process must take at least one step. 
\end{itemize}
These constraints make the failure detector parametric in $\Delta$ and $\Phi$.

Moreover, Algorithm~\ref{algo:detector1} is parameterized by the initial value of the timeout. 
If a default value of the timeout is too small, there exists a case in which sent messages are delivered after the timeout expired.
%If the timeout default is a too-small initial value, messages might always arrive after the initial timeout expires. 
It violates Strong Accuracy.



==> forte21/ivy-intro.tex <==
is a multi-modal verification tool to make design and implementation of distributed protocols and algorithms correct~\cite{mcmillan2020ivy}.
The main characteristic of Ivy is that its language is designed with decidable theories and reasoning in mind.
For example, the effectively propositional fragment (EPR) and stratified function symbols that are decidable fragments in first-order logic are currently supported in Ivy (version 1.7)~\cite{ivy}. 

The standard way to prove that a property $\mathit{Prop}$ holds in an algorithm expressed in Ivy is to provide an inductive invariant $\mathit{IndInv}$ such that three following constraints hold: 
\begin{align}
\mathit{Init} & \Rightarrow \mathit{IndInv} \\
\mathit{IndInv} \land \mathit{Init} & \Rightarrow \mathit{IndInv}^{\prime} \\
\mathit{IndInv} & \Rightarrow \mathit{Prop} 
\end{align}
where $\mathit{Init}$ refers to initial states, and $\mathit{Next}$ refers to system transitions, and $\mathit{IndInv}^{\prime}$ refers to $\mathit{IndInv}$ in a next state.
To prove formulas (1)--(3), Ivy transforms the specification into the SMT-Lib format, and tries to call Z3 to solve generated constraints.
If the specification is decidable and has a bug, Ivy is usually able to provide a counterexample.

Alternative approachs of Ivy to verify specifications are based on eager abstraction and model checking.
Moreover, Ivy supports some liveness-to-safety transformation, and testing methods, and the translation to C++.




==> forte21/ivy.tex <==
Ivy is a multi-modal verification tool for correct design and implementation of distributed protocols and algorithms~\cite{mcmillan2020ivy}.
The main characteristic of Ivy is that its language is designed with decidable theories and reasoning in mind.
For example, the effectively propositional fragment (EPR) and stratified function symbols that are decidable fragments in first-order logic are currently supported in Ivy (version 1.7)~\cite{ivy}. 
This feature makes Ivy stable and predictable in reasoning about specifications with decidable problems.
When a decidable specification has a bug, Ivy is usually able to provide a counterexample.
If a specification is big and complicated, the user can decompose it into smaller component modules and provide proof hints to Ivy.
An alternative approach of Ivy to verify specifications is based on eager abstraction and model checking.
Other advantages of Ivy are that it supports some liveness-to-safety transformation, and testing methods, and the translation to C++.


Figure~\ref{fig:ivyspec} presents a specification with a simple timer in Ivy.
The built-in datatypes in Ivy include just the Boolean type, uninterpreted types, records (structs) over datatypes, and pure first-order functions. 
We declare an uninterpreted type \textsf{number} on Line 1, and interpret type \textsf{number} as type \textsf{int} on Line 2.
Line 4 declares a variable \textsf{timer} with type \textsf{number}.
Next, we describe constraints on initial states (Lines 6-10). 
Variable \textsf{timer}  is non-deterministically initialized (Line 7), but the constraints on Lines 8 and 9 must hold, i.e., $0 \leq \textsf{timer} \leq 5$. 
Procedures in Ivy are called actions and may have side effects on variables.
Importantly, Ivy is a synchronous, reactive programming language~\cite{berry1992esterel}.
Hence, actions are only executed in response to input from the environment, and these actions appear to execute atomically~\cite{mcmillan2020ivy}.
Line 13-19 presents an action \textsf{setNewValue}.
Action \textsf{setNewValue} non-deterministically resets variable \textsf{timer} to 0 (Line 14) or increases \textsf{timer} by 1 if $\textsf{timer} < 5$ (Lines 16 and~17).
Line 20 exports action \textsf{setNewValue} to the environment.
Line 20 and 21 present two invariants in our specification.
Ivy considers the conjunction of these invariants as an inductive invariant that the user wants to prove.
Notice that the specification in Figure~\ref{fig:ivyspec} is decidable, and Ivy can automatically prove the inductive invariant.

The user can run Ivy to check specifications that are not in its decidable theories with the option \textsf{\textquotedblleft complete=fo\textquotedblright}.
For example, our Ivy specification in this work.
However, in this case, Ivy is less stable and depends on fragile heuristics of its backend solver Z3~\cite{DeMouraB08}.

Ivy has been used in verification of Paxos and its variants~\cite{PadonLSS17}, and the Stellar consensus protocol~\cite{losa2020formal}, 
and the Tendermint protocol~\cite{ivyTendermint}.
For more information about Ivy, the user can visit its webpage~\cite{ivy}.

\begin{figure}[thp]
%\begin{CenteredBox}
\begin{multicols}{2}		
\begin{lstlisting}
type number
interpret number -> int

individual timer : number

after init {
  timer := *;    
  assume 0 <= timer;
  assume timer <= 5; 
}


action setNewValue  = {
  if (*) { timer := 0; }
  else {
    assume timer < 5;
    timer := timer + 1;  
  }; 
}

export setNewValue

invariant 0 <= timer
invariant timer <= 5
\end{lstlisting}
\end{multicols}
%\end{CenteredBox}
\caption{A simple timer in Ivy} \label{fig:ivyspec}
\end{figure}

==> forte21/send-tla-old.tex <==
\tlatex
\setboolean{shading}{true}
\@x{\@s{80} 1 \colon
	\@s{4.1} SSnd \defeq \land \, {ePC} = \@w{SSnd}
}
\@x{\@s{80} 2 \colon \@s{47.59} \land  {\IF} ( sTimer = 0 \land sPC = \@w{SSnd}	)\@s{4.1}}%
\@xx{}
\@x{\@s{80} 3 \colon  \@s{55.11} {\THEN} buf {'} \, {=} \, buf \, {+} \, 1\@s{28.7}}
\@xx{}%
\@x{\@s{80} 4 \colon  \@s{55.11} {\ELSE} {\UNCHANGED} buf}%
\@x{\@s{80} 5 \colon  \@s{50.59} {\land} \, ePC {'} \, {=} \, \@w{RNoSnd}}%
\@x{\@s{80} 6 \colon  \@s{50.99} {\land} \, {\UNCHANGED} {\langle} sTimer ,\, rTimer ... {\rangle}}%
\setboolean{shading}{false}



==> forte21/ssched-tla.tex <==
\tlatex
\setboolean{shading}{true}
\@x{\@s{80} 1 \tladot{\colon} \@s{4.1} SSched \tladot{\defeq} \tladot{\land} ePC \tladot{=}\@w{SSched}}%
\@x{\@s{80} 2 \tladot{\colon} \@s{55.99} \@s{3.1} \tladot{\land} ePC \tladot{'} \tladot{=}\@w{RSched}
}%
\@x{\@s{80} 2 \tladot{\colon} \@s{55.99} \@s{3.1} \tladot{\land} \tladot{\lor} \tladot{\land} sTimer \tladot{\geq} 2
}%
\@x{\@s{80} 2 \tladot{\colon} \@s{79.99} \@s{3.1}  \tladot{\land} sTimer \tladot{'} = 0
}%
\@x{\@s{80} 2 \tladot{\colon} \@s{55.99} \@s{3.1} \tladot{\land} \tladot{\lor} \tladot{\land} sTimer \tladot{<} 3 * Phi - 1
}%
\@x{\@s{80} 2 \tladot{\colon} \@s{79.99} \@s{3.1}  \tladot{\land} sTimer \tladot{'} = sTimer + 1
}%
\@x{\@s{80} 2 \tladot{\colon} \@s{55.99} \@s{3.1} \tladot{\land} {\UNCHANGED} {\langle} buf ,\, rTimer ... {\rangle}}%
\setboolean{shading}{false}

%SSched ==  
%/\ ePC = "SSched"
%/\ ePC' = "RSched"  
%/\ \/ /\ sTimer >= 2           /* ensures that the sender went through sub-rounds Receive and Local Computation
%/\ sTimer' = 0          
%/\ UNCHANGED sPC                                                                         
%\/ /\ sTimer < 3 * Phi - 1
%/\ sTimer' =  sTimer + 1
%/\ UNCHANGED sPC                                       
%/\ UNCHANGED << buf, rTimer, rPC, suspected, waitingTime, timeout >>  

==> forte21/tla-intro.tex <==
is an untyped specification language to design, specify, and reason about systems~\cite{lamport2002specifying}.
It is based on Temporal Logic of Actions (TLA)~\cite{lamport1994temporal}, a variant of linear-time temporal logic, for expressing the dynamic system behavior. 
Data structures are represented with Zermelo-Fr{\"a}nkel set theory with the axiom of choice. 
This language offers a rich syntax for sets, functions, tuples, records, sequences, and control structures.


The user can verify a finite-state system specified in~\tlap{} with two model checkers TLC~\cite{yu1999model} and \apalache{}~\cite{konnov2019tla}.
While TLC is an explicit-state model checker, \apalache{} is a symbolic one based on the SMT solver Z3~\cite{DeMouraB08}. 
The users in industrial projects~\cite{newcombe2015amazon,kafka}  reported on finding real bugs by checking \tlap{} specifications with TLC.
\apalache{} was first introduced in 2019, and has been used to check safety of Tendermint consensus for fixed parmaters~\cite{braithwaite2020tendermint}.

To reason about \tlap{} specifications with an infinite set of possible states, the user can write and verify interactive proofs with the \tlap{} Proof System (TLAPS)~\cite{chaudhuri2010tla+}. 
While progress towards proof automation in TLAPS has been made in the last years~\cite{merz2012automatic},
writing interactive proofs is still a challenging task.

==> forte21/tools.tex <==
\subsubsection{\tlap{}}

\input{tla-intro} 

\subsubsection{\fast{}}

\input{fast-intro}

\subsubsection{Ivy}

\input{ivy-intro}

==> netys20/comp-model.tex <==
In this section, we discuss interesting properties of the computational model: partial synchrony where its parameters are fixed and hold eventually \cite{dwork1988consensus}. 
First, we recall some common notations and constraints
in this model. 
Second, we describe two additional assumptions which are safely obtained. 
Finally,
we prove interesting properties in this model.

\subsection{DSL \textquotesingle s computational model}

==> netys20/cutoff.tex <==

In this section, we prove two cutoff results for the number of processes in checking properties $M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i}$  and $M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j}$ 
where $M_N$ is a global transition system defined in Section \ref{sec:GlobalTransSys}, $F_{i}, G_{i, j}$ are arbitrary LTL (linear temporal logic) formulas such that 
predicates in $F_{i}$  inspect only variables with an indexes $i$, and 
predicates in $G_{i, j}$  inspect only variables with two different indexes $i, j$.
These results are obtained with Theorems \ref{thm:NCutoffOneIndex}--\ref{thm:NCutoffTwoIndexes}.


The proof strategies are based on the symmetry properties and automorphisms of the process template and the global transition system. 
The reader can find the definitions of automorphism for states and transition systems in~\cite{emerson1993symmetry,emerson1995reasoning}.
More detailed, the proofs of Theorems \ref{thm:NCutoffOneIndex}--\ref{thm:NCutoffTwoIndexes} are based on following results: 
\begin{itemize}
\item Lemma \ref{lem:SymInitConf} says that every permutation on a set $\nid$ is an automorphism of the initial configuration $\ginitstate{N}$ for every $N \geq 1$;

\item Lemma \ref{lem:SymTransSys} says that every index permutation on a set $\nid$ is an automorphism of the transition system $M_N$ for every $N \geq 1$;

\item Lemma \ref{lem:TraceEquiv} says that $M_N, M_2$ are trace equivalent under a set of predicates which inspect only variables whose indexes is $\{1\}$, $\{2\}$, or both $\{1, 2\}$
for every $N \geq 2$.
\end{itemize}




\subsection{Symmetry and ~\classname{} systems}

Before presenting theorems and lemmas in details, we would like to remind that the application of a permutation  $\perm$ to an indexed object $b$ is obtained from $b$ by simultaneously replacing every occurrence of index $i \in \nid$ by $\perm(i)$.
We overload the permutation by writing $\perm b$ to refer a new object constructed from a object $b$ by applying a permutation $\perm$ to $b$.

If $b$ is an unindexed object, then we have $\perm(b) = b$ for every permutation $\perm$. 
Recall that every message is unindexed.
Moreover, by definition of the process template, every cell in a global two--dimensional variable $x_k$ contains only unindexed values for every $3 \leq k \leq m$.



Lemma \ref{lem:PermArr} shows how a new array $\perm y$ is constructed from an array $y$ with type $\nid \rightarrow \mathcal{T}$ and a permutation $\perm$ where $\mathcal{T}$ is a set of unindexed values.
For example, assume $\conf(\pc) = [L_S, L_C, L_F]$ and $\perm = \{ 1 \mapsto 2, 2 \mapsto 1, 3 \mapsto 3\}$.
For a better reading, we rewrite $\conf(\pc)$ as $[1 \mapsto L_S, 2 \mapsto L_C, 3 \mapsto L_F]$.
Hence, we have 
\begin{align*}
\perm(\conf(\pc)) = \perm\conf(\pc) & = [\perm(1) \mapsto L_S, \perm(2) \mapsto L_C, \perm(3) \mapsto L_F] \\
& = [2 \mapsto L_S, 1 \mapsto L_C, 3 \mapsto L_F] \\
& = [L_C, L_S, L_F]
\end{align*}

\begin{lemma} \label{lem:PermArr}
Let $y$ be an array of type $\tau \colon \nid \rightarrow \mathcal{T}$ where values of type $\mathcal{T}$ are unindexed.
%Assume that $y[i] = c_i$ where $i \in \nid, c_i \in \mathcal{T}$.
Let $\perm, \perm^{-1}$ be permutations such that $\perm^{-1}$ is a inverse function of $\perm$.
It follows $\perm y = [y[\perm^{-1}(1)],  \ldots, y[\perm^{-1}(N)] ]$.
\end{lemma}

\begin{proof}
For a better reading, we rewrite $y$ as $[1 \mapsto y[1], \ldots, N \mapsto y[N]]$.
It follows $\perm y = [\perm(1) \mapsto y[1], \ldots, \perm(N) \mapsto y[N]]$.
By relocating cells in $\perm y $, we have that
$\perm y = [1  \mapsto y[\perm^{-1}(1)],  \ldots, N \mapsto y[\perm^{-1}(N)] ]$.
\end{proof}

We now discuss the symmetry of a process template $U = (\pstates{U}, \rightarrow, {\pinitstate{U}})$ of an instance $\sys{N}$ of an~\idsep{} algorithm. 
Lemma \ref{lem:SymTempInitConf} says that $\pinitstate{U}$ is symmetry.
Lemma \ref{lem:SymTemp} says that $\perm U = U$ for every permutation on $\nid$.
The proof of Lemma \ref{lem:SymTemp} requires three Lemmas \ref{lem:PermLocalNext}, \ref{lem:PermLocalCrash}, and \ref{lem:PermProcStuttering} which says that a permutation on $\nid$ preserves process transitions between process configuration in $U$.

\newcommand{\lemSymTemp}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of $U$.
}

\begin{corollary} \label{lem:SymTemp}
  \lemSymTemp
\end{corollary}

\begin{proof}
  It immediately follows from Lemmas \ref{lem:SymTempInitConf}--\ref{lem:PermProcStutter}.
  Lemma \ref{lem:PermProcType} says that the application of a permutation on process indexes to a process configuration generates a process configuration.
  Lemma \ref{lem:SymTempInitConf} is for the initial process configuration.
  Other lemmas are for process transitions.
\end{proof}

\newcommand{\lemPermProcType}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$,
  and $\rho \in \pstates{U}$ be a process configuration.
  It follows that $\perm \rho \in \pstates{U}$.
}

\begin{lemma} \label{lem:PermProcType}  
  \lemPermProcType
\end{lemma}

\begin{proof}
It immediately follows by Lemma \ref{lem:PermArr} and that fact that every index permutation preserves type information.
\end{proof}

\newcommand{\lemSymTempInitConf}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of the initial configuration $\ginitstate{N}$.
}

\begin{lemma} \label{lem:SymTempInitConf}
  \lemSymTempInitConf
\end{lemma}

\begin{proof}
It immediately follows by definition of $\pinitstate{U}$. \qed
\end{proof}

\newcommand{\lemPermProcSend}{
Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
Let $m \in \msg$ be a message, and $\rho_0, \rho_1$ be process configurations in $\pstates{U}$ such that $\rho_0 \procsnd{m} \rho_1$.
Let $\perm$ be a permutation on $\nid$.
It follows that $\perm \rho_0 \procsnd{m} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcSend}
\lemPermProcSend
\end{lemma}

\begin{proof}
We prove Lemma \ref{lem:PermProcSend} by utilizing the  properties of~\classname{} functions.
First, we have 
\begin{alignat*}{3}
\perm\rho_1(\pc^U) & = \rho_1(\pc) && \quad \text{(by } \rho_1(\pc^U) \text{ is an unindexed value)} \\
& = g_1(\rho_0(\pc^U)) && \quad \text{(by definition of function $g_1$)}              \\
& = g_1(\perm\rho_0(\pc^U)) && \quad \text{(by } \rho(\pc^U) \text{ is an unindexed value)}              
\end{alignat*}

We now check the $\mailbox$. 
Let $i$ be an arbitrary index in $\nid$.
It follows
\begin{alignat*}{3}
\perm\rho_1(\mailbox^U[i]) & = \rho_1(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = \rho_0(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by definition of $\procsnd{m}$)}              \\
& = \perm\rho_0(\mailbox^U[i])  && \quad \text{(by Lemma \ref{lem:PermArr})}  
\end{alignat*}
Hence, we have $\forall i \in \nid \colon \perm\rho_1(\mailbox^U[i]) = \perm\rho(\mailbox^U[i])$.

We now focus on a two--dimensional variable $x^U_3$.
Again, let $i$ be an arbitrary index in $\nid$. It follows
\begin{alignat*}{3}
\perm\rho_1(x^U_3[i]) & = \rho_1(x^U_3[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = f_3 \big( \rho_0(x^U_1),  \rho_1(x^U_2[\perm^{-1}(i)]), && \quad \text{(by definition of   $f_3$)}              \\
&  \qquad \rho_0(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_\ell[\perm^{-1}(i)]) \big) &&              \\
& = f_3 \big( \rho_0(\pc^U),  \rho_1(\mailbox^U[\perm^{-1}(i)]), && \quad \text{(by renaming)}              \\
& \qquad \rho_0(x^U_3[\perm^{-1}(i)]), \ldots, \rho_0(x^U_\ell[\perm^{-1}(i)]) \big) &&      \\
& = f_3 \big( \perm\rho_0(\pc^U),  \perm \rho_1(\mailbox^U[i]), && \quad \text{(by Lemma \ref{lem:PermArr})}              \\
& \qquad \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big) &&           
\end{alignat*}
Hence, we have 
\begin{align*}
\forall i \in \nid \colon \perm\rho_1(x^U_3[i]) =  f_3 \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
& \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
\end{align*}
By similar arguments for other variables, we have  
\begin{align*}
\forall k \in 3..\ell \, \forall i \in \nid \colon \perm\rho_1(x^U_k[i]) =  f_k \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
& \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
\end{align*}
%  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
It follows $\perm \rho_0 \procsnd{m} \perm\rho_1$ by the semantics of the transtion $\procsnd{m}$. \qed
\end{proof}


\newcommand{\lemPermProcReceive}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let $S_1, \ldots, S_N \subseteq \msg$ be $N$ sets of messages, and $\rho_0, \rho_1$ be process configurations such that $\rho_0 \procrcv{S_1}{S_N} \rho_1$. 
  Let $\perm$ be a permutation on $\nid$, and $\perm^{-1}$ be its inverse function.
  It follows that $\perm \rho_0 \procrcv{S_{\perm^{-1}(1)}}{S_{\perm^{-1}(N)}} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcReceive}
  \lemPermProcReceive
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:PermProcReceive} by utilizing the  properties of~\classname{} functions.
  First, we have 
  \begin{alignat*}{3}
  \perm\rho_1(\pc^U) & = \rho_1(\pc) && \quad \text{(by } \rho_1(\pc^U) \text{ is an unindexed value)} \\
  & = g_1(\rho_0(\pc^U)) && \quad \text{(by definition of function $g_1$)}              \\
  & = g_1(\perm\rho_0(\pc^U)) && \quad \text{(by } \rho(\pc^U) \text{ is an unindexed value)}              
  \end{alignat*}
  
  We now check the $\mailbox$. 
  Let $i$ be an arbitrary index in $\nid$.
  It follows
  \begin{alignat*}{3}
  \perm\rho_1(\mailbox^U[i]) & = \rho_1(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
  & = \rho_0(\mailbox^U[\perm^{-1}(i)]) \cup S_{\perm^{-1}(i)} && \quad \text{(by definition of $\procrcv{S_1}{S_N}$)}              \\
  & = \perm\rho_0(\mailbox^U[i]) \cup S_{\perm^{-1}(i)}  && \quad \text{(by Lemma \ref{lem:PermArr})}  
  \end{alignat*}
  Hence, we have $\forall i \in \nid \colon \perm\rho_1(\mailbox^U[i]) = \perm\rho(\mailbox^U[i]) \cup S_{\perm^{-1}(i)}$.
  
  By similar arguments in the proof of Lemma \ref{lem:PermProcReceive}, we have  
  \begin{align*}
  \forall k \in 3..\ell \, \forall i \in \nid \colon \perm\rho_1(x^U_k[i]) =  f_k \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
  & \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
  \end{align*}
  %  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
  It follows $\perm \rho_0 \procrcv{S_{\perm^{-1}(1)}}{S_{\perm^{-1}(N)}} \perm\rho_1$. \qed
\end{proof}

The proofs of Lemmas \ref{lem:PermProcComp}--\ref{lem:PermProcStutter} are similar (and simpler) the above proofs of Lemmas \ref{lem:PermProcSend} and \ref{lem:PermProcReceive}.

\newcommand{\lemPermProcComp}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let and $\rho_0, \rho_1$ be process configurations such that $\rho_0 \proccomp \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \proccomp \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcComp}
  \lemPermProcComp
\end{lemma}

\newcommand{\lemPermProcCrash}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let and $\rho_0, \rho_1$ be process configurations such that $\rho_0 \proccrash \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \proccrash \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcCrash}
  \lemPermProcCrash
\end{lemma}

\newcommand{\lemPermProcStutter}{
  Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let and $\rho_0, \rho_1$ be process configurations such that $\rho_0 \procstutter \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \procstutter \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcStutter}
  \lemPermProcStutter
\end{lemma}

\newcommand{\lemPermLocalNext}{
Let $U = (\pstates{U}, \trans^{U}, \sigma^U, \pinitstate{U})$ be a process template defined as in Section \ref{sec:ProcTemp}.
Let $\rho_0, \rho_1$ be process configurations in $\pstates{U}$.
Assume that there exist $N$ sets $S_1, \ldots, S_N \subseteq \msg$, and a message $m \in \msg$ such that $(\rho_1, m) = \localnext(\rho_0, S_1, \ldots, S_N)$.
Let $\perm$ and $\perm^{-1}$ be two permutations on $\nid$ such that $\perm^{-1}$ is an inverse function of $\perm$.
It follows that  $(\perm\rho_1, m) = \localnext(\perm\rho, S_{\perm^{-1}(1)}, \ldots, S_{\perm^{-1}(N)})$.}

\begin{lemma} \label{lem:PermLocalNext}
\lemPermLocalNext
\end{lemma}

\begin{proof}
%  By definition, we have $\perm(\rho_1, m)  = (\perm(\rho), \perm(m)) = (\perm(\rho), m)$. We prove $(\perm(\rho), m) = \perm(\localnext(\rho, S_1, \ldots, S_N))$ 
We prove Lemma \ref{lem:PermLocalNext} by utilizing the~\idsep{} property.
First, we have 
\begin{alignat*}{3}
 \perm\rho_1(\pc) & = \rho_1(\pc) && \quad \text{(by } \rho_1(\pc) \text{ is an unindexed value)} \\
 & = g_1(\rho_0(\pc)) && \quad \text{(by the~\idsep{} property)}              \\
 & = g_1(\perm\rho_0(\pc)) && \quad \text{(by } \rho(\pc) \text{ is an unindexed value}              
\end{alignat*}

We now check the $\mailbox$. 
Let $i$ be an arbitrary index in $\nid$.
It follows
\begin{alignat*}{3}
\perm\rho_1(\mailbox[i]) & = \rho_1(\mailbox[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = \rho_0(\mailbox[\perm^{-1}(i)]) \cup S_{\perm^{-1}(i)} && \quad \text{(by the~\idsep{} property)}              \\
& = \perm\rho_0(\mailbox[i]) \cup S_{\perm^{-1}(i)} && \quad \text{(by Lemma \ref{lem:PermArr})}  
\end{alignat*}
Hence, we have $\forall i \in \nid \colon \perm\rho_1(\mailbox[i]) = \perm\rho(\mailbox[i]) \cup S_{\perm^{-1}(i)}$.

We now focus on a two--dimensional variable $x^U_3$.
Again, let $i$ be an arbitrary index in $\nid$. It follows
\begin{alignat*}{3}
\perm\rho_1(x^U_3[i]) & = \rho_1(x^U_3[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = f_3 \big( \rho_0(x^U_1),  \rho_1(x^U_2[\perm^{-1}(i)]), && \quad \text{(by~\idsep{} property)}              \\
&  \qquad \rho_0(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_m[\perm^{-1}(i)]) \big) &&              \\
& = f_3 \big( \rho(\pc),  \rho^{\prime}(\mailbox[\perm^{-1}(i)]), && \quad \text{(by renaming)}              \\
& \qquad \rho(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_m[\perm^{-1}(i)]) \big) &&      \\
& = f_3 \big( \perm\rho(\pc),  \rho^{\prime}(\mailbox[\perm^{-1}(i)]), && \quad \text{(by renaming)}              \\
& \qquad \rho(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_m[\perm^{-1}(i)]) \big) &&           
\end{alignat*}
Hence, we have 
\begin{align*}
\forall i \in \nid \colon \perm\rho_1(x^U_3[i]) =  f_3 \big( \rho(\pc),  & \rho^{\prime}(\mailbox[\perm^{-1}(i)]), \\
& \rho(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_m[\perm^{-1}(i)]) \big)
\end{align*}
By similar arguments for other variables, we have  
\begin{align*}
\forall k \in 3..N \, \forall i \in \nid \colon \perm\rho_1(x^U_k[i]) =  f_k \big( & \rho(\pc),   \rho^{\prime}(\mailbox[\perm^{-1}(i)]), \\
& \rho(x^U_k[\perm^{-1}(i)]), \ldots, \rho(x^U_k[\perm^{-1}(i)]) \big)
\end{align*}
%  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
It follows $(\perm\rho_1, m) = \localnext(\perm\rho, S_{\perm^{-1}(1)}, \ldots, S_{\perm^{-1}(N)})$ by the~\idsep{} property. \qed
\end{proof}

\newcommand{\lemPermLocalCrash}{
  Let $U = (\pstates{U}, \xrightarrow{U}, \{\pinitstate{U}\})$ be a process template of $N$ processes.
  Let $\rho_0, \rho_1$ be configurations in $\pstates{U}$, and $\perm$ be a permutation on $\nid$.
  If $\rho_1 = \localfault(\rho_0)$ then $\perm\rho_1 = \localfault(\perm\rho_0)$.
}

\begin{lemma} \label{lem:PermLocalCrash}
  \lemPermLocalCrash
\end{lemma}

\begin{proof}
We have $\perm\rho_1(\pc) = \rho_1(\pc)$, and $\perm\rho_0(\pc) = \rho_0(\pc)$. 
Since $\rho_1(x^U_k) = \rho_0(x^U_k)$ for every $2 \leq k \leq m$, it follows that $\perm\rho_1(x^U_k) = \perm\rho_0(x^U_k)$ for every $2 \leq k \leq m$.
Therefore, we have $\perm\rho_1 = \localfault(\perm\rho_0)$. \qed
\end{proof}

\newcommand{\lemPermProcStuttering}{
  Let $U = (\pstates{U}, \xrightarrow{U}, \{\pinitstate{U}\})$ be a process template of $N$ processes.
  Let $\rho_0, \rho_1$ be configurations in $\pstates{U}$, and $\perm$ be a permutation on $\nid$.
  If $\rho_1  \localstuttering{U} \rho_0$ then $\perm\rho_1  \localstuttering{U} (\perm\rho_0)$.
}



\begin{lemma} \label{lem:PermProcStuttering}
  \lemPermProcStuttering
\end{lemma}

\begin{proof}
  Since $\rho_1(x^U_k) = \rho_0(x^U_k)$ for every $1 \leq k \leq m$, it follows that $\perm\rho_1(x^U_k) = \perm\rho_0(x^U_k)$ for every $1 \leq k \leq m$.
  Therefore, we have $\perm\rho_1  \localstuttering{U} (\perm\rho_0)$. \qed
\end{proof}

We now turn to the symmetry property of the global system of an instance $\sys{N}$ of an~\idsep{} algorithm.
Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
Lemma \ref{lem:SymSys} says that $M_N$ is fully symmetry, and the proof of Lemma \ref{lem:SymSys} requires two Lemmas \ref{lem:SymInitConf} and \ref{lem:SymTransSys}.
Lemma \ref{lem:SymInitConf} is symmetry.
Lemma \ref{lem:SymTransSys} says that every permutation $\perm$ on a set $\nid$ preserves the system transition relation.

\newcommand{{\lemSymSys}}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
  Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
  Let $\perm$ be a permutation on a set $\nid$.
  It follows that $\perm M_N = M_N$.
}

\begin{corollary} \label{lem:SymSys}
  \lemSymSys
\end{corollary}


\begin{proof}
It immediately follows by Lemmas \ref{lem:SymInitConf} and \ref{lem:SymTransSys}, and the fact that a permutations preserves type information and labelled on $M_N$. \qed
\end{proof}


\newcommand{\lemSymInitConf}{
  Let $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$ be a transition system of an instance $\sys{N}$ of an arbitrary~\idsep{} algorithm $\mathcal{A}$.
  Assume that $M_N$ has variables $\gc, \buf, \act, x_1, \ldots, x_m$.
  Let $\perm$ be a permutation on a set $1..N$.
  It follows $\perm(\ginitstate{N}) = \ginitstate{N}$.
}

\begin{lemma} \label{lem:SymInitConf}
  \lemSymInitConf
\end{lemma}



\begin{proof}
  By definition, we have
  \begin{align*}
  \perm(\ginitstate{N}) & = (\perm(\ginitstate{N}(\gc)), \perm(\ginitstate{N}(\buf)),  \ldots , \perm(\ginitstate{N}(x_m)))
  \end{align*}
  First, by definition we have $\perm(\ginitstate{N}(\gc)) = \ginitstate{N}(\gc)$ since $\gc$ is not indexed.
  Second, since $\ginitstate{N}(\buf[i, j]) = \emptyset$ for every $i, j \in \nid$, we have
  \begin{align*}
  \perm(\ginitstate{N}(\buf)) & = \ginitstate{N}(\buf)
  \end{align*}
  %  Consider a subarray $\mathit{arr} \triangleq [\ginitstate{N}(\buf[\perm(1), \perm(1)]), \ldots, \ginitstate{N}(\buf[\perm(1), \perm(N)])]$. 
  %  By definition of $\ginitstate{N}$, we have $\mathit{arr} = [\emptyset, \ldots, \emptyset]$.
  %  Therefore, $\ginitstate{\buf} = \perm(\ginitstate{\buf})$.
  By similar arguments, we have $\perm(\ginitstate{N}(x_k)) = \ginitstate{N}(x_k)$ for every $1 \leq k \leq m$.
  Hence, it follows $\perm(\ginitstate{N}) = \ginitstate{N}$.
  \qed
\end{proof}

\newcommand{\lemSymSysTrans}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
Let $\conf_0, \conf_1$ be two configurations in $\gstates{N}$ such that $\conf_0 \leadsto \conf_1$
Let $\perm$ be a permutation on a set $\nid$.
It follows $\perm \conf_0 \leadsto \perm \conf_1$.
}

\begin{lemma} \label{lem:SymTransSys}
\lemSymSysTrans
\end{lemma}

\begin{proof}
It immediately follows by Lemmas \ref{lem:SymSysTransSched}--\ref{lem:SymSysTransComp} since each lemma is for one subround.
\end{proof}

\newcommand{\lemSymSysTransSched}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
  Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
  Let $\conf_0, \conf_1$ be two configurations in $\gstates{N}$ such that $\conf_0 \transsched \conf_1$
  Let $\perm$ be a permutation on a set $\nid$.
  It follows $\perm \conf_0 \transsched \perm \conf_1$.
}

\begin{lemma} \label{lem:SymSysTransSched}
  \lemSymSysTransSched
\end{lemma}

\begin{proof}
In order to prove that $\perm \conf_0 \transsched \perm \conf_1$, we need to show that all \sched{} constraints hold in $(\perm \conf_0, \perm \conf_1)$.
The most complicated constraint is when a correct process $\pcreate(\conf_0, i)$ becomes crashed in $\conf_1$.
We prove that a process $\pcreate(\perm \conf_0, \perm(i))$ is correct in $\perm \conf_0$, and it is also crashed in $\perm \conf_1$.
By Lemma \ref{lem:PermArr}, we have $\perm\conf_1(\pc[\perm(i)]) = \conf_1(\pc[i]) = L_F$ and $\perm\conf_0(\pc[\perm(i)]) = \conf_0(\pc[i]) \neq L_S$.
By applying similar arguments in Lemma \ref{lem:PermLocalCrash}, it follows that other variables of a process $\pcreate(\perm\conf_1, \perm(i)])$ and $\pcreate(\perm\conf_0, \perm(i)])$ are the same.
Therefore, a process $\pcreate(\perm \conf_1, \perm(i))$ is a fresh faulty one.
\qed 
\end{proof}

\newcommand{\lemSymSysTransSnd}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
  Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
  Let $\conf_0, \conf_1$ be two configurations in $\gstates{N}$ such that $\conf_0 \transsnd \conf_1$
  Let $\perm$ be a permutation on a set $\nid$.
  It follows $\perm \conf_0 \transsnd \perm \conf_1$.
}

\begin{lemma} \label{lem:SymSysTransSnd}
  \lemSymSysTransSnd
\end{lemma}

\begin{proof}
In order to prove that $\perm \conf_0 \transsched \perm \conf_1$, we need to show that all  constraints in the subround Schedule hold in $(\perm \conf_0, \perm \conf_1)$.
The most complicated constraint is for when a correct process $\pcreate(\conf_1, i)$  sends a message $m$ to all in this subround.
We prove that a process $\pcreate(\perm \conf_1, \perm(i))$ also sends a message $m$ to all.

By Lemma \ref{lem:PermArr}, we have
\begin{align*}
 & \perm\conf_1(\pc[\perm(i)])  = \conf_1(\pc[i]) \\
 \, \land \, &  \perm\conf_0(\pc[\perm(i)])  = \conf_0(\pc[i]) = L_S \\
 \, \land \, & \perm\conf_1(\act[\perm(i)]) = \conf_1(\act[i])   \\
 \, \land \, &  \perm\conf_0(\act[\perm(i)]) = \conf_0(\act[i]) 
\end{align*}
Therefore, a process $\pcreate(\perm\conf_0, \perm(i))$ is enable to send a message to all.
By Lemma \ref{lem:PermLocalNext}, since $(\pcreate(\conf_1, i), \{m\}) = \localnext(\pcreate(\conf_0, i), \emptyset, \ldots, \emptyset)$ we have that 
\[
(\pcreate(\perm \conf_1, \perm(i)), \{m\}) = \localnext(\pcreate(\perm \conf_0, \perm(i)), \emptyset, \ldots, \emptyset)
\]
Now we show that a message $m$ is fresh in every message buffer from $\pcreate(\perm \conf_1, \perm(i))$ in $\perm \conf_1$. By Lemma \ref{lem:PermArr}, it follows that
\begin{align*}
\forall i, j \in \nid \colon & \conf_0(\buf[i, j]) = \perm \conf_0(\buf[\perm(i), \perm(j)]) \\
\forall i, j \in \nid \colon & \conf_1(\buf[i, j]) = \perm \conf_1(\buf[\perm(i), \perm(j)])
\end{align*}
It implies
\begin{align*}
\forall i, j \in \nid \colon & m \notin \conf_0(\buf[i, j]) \Leftrightarrow m \notin  \perm  \conf_0(\buf[\perm(i), \perm(j)]) \\
\forall i, j \in \nid \colon & m \in  \conf_1(\buf[i, j]) \Leftrightarrow m \in \perm  \conf_1(\buf[\perm(i), \perm(j)])
\end{align*}
Therefore, a process  $(\pcreate(\conf_1, i)$ also sends a message $m$ to all in this subround. 
Moreover, by Lemma \ref{lem:PermProcStuttering}, processes which are inactive or whose $\pc$ is different from $L_S$ are still inactive in this subround.
It follows that $\perm \conf_0 \transsnd \perm \conf_1$. \qed 
\end{proof}

\newcommand{\lemSymSysTransRcv}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
  Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
  Let $\conf_0, \conf_1$ be two configurations in $\gstates{N}$ such that $\conf_0 \transrcv \conf_1$
  Let $\perm$ be a permutation on a set $\nid$.
  It follows $\perm \conf_0 \transrcv \perm \conf_1$.
}

\begin{lemma} \label{lem:SymSysTransRcv}
  \lemSymSysTransRcv
\end{lemma}

\begin{proof}
  In order to prove that $\perm \conf_0 \transsched \perm \conf_1$, we need to show that all constraints in the subround Receive hold in $(\perm \conf_0, \perm \conf_1)$.
  The most complicated constraint is for when a correct process $\pcreate(\conf_1, i)$  has received sets of messages $S_1, \ldots, S_N$ from processes $\pcreate(\conf_1, 1), \ldots, \pcreate(\conf_1, N)$.
  By similar arguments in \ref{lem:SymSysTransSnd} and \ref{lem:PermLocalNext}, it follows that that $\pcreate(\perm \conf_1, \perm(i))$ has received sets of messages $S_{\perm(1)}, \ldots, S_{\perm(N)}$ from processes $\pcreate(\perm \conf_{1}, \perm(1)), \ldots, \pcreate(\perm \conf_1, \perm(N))$.
  Moreover, by similar arguments in \ref{lem:SymSysTransSnd}, it follows that $\pcreate(\perm \conf_1, \perm(i))$ is enable to receives messages in this round and will be inactive in the next round.
  Hence, all  constraints in the subround Receive which are related to $\pcreate(\perm \conf_1, \perm(i))$ hold in $\perm \conf_1$.
  Moreover, by Lemma \ref{lem:PermProcStuttering}, processes which are inactive or whose $\pc$ is different from $L_R$ are still inactive in this subround.
  It follows that $\perm \conf_0 \transrcv \perm \conf_1$.
  
\qed
\end{proof}

\newcommand{\lemSymSysTransComp}{
  Let $\sys{N}$  be an instance of an~\idsep{} algorithm with $N$ processes.
  Assume that  $\sys{N}$  is modeled as a transition system $M_N = (\gstates{N}, \leadsto, \ginitstate{N})$.
  Let $\conf_0, \conf_1$ be two configurations in $\gstates{N}$ such that $\conf_0 \transsnd \conf_1$
  Let $\perm$ be a permutation on a set $\nid$.
  It follows $\perm \conf_0 \transcomp \perm \conf_1$.
}

\begin{lemma} \label{lem:SymSysTransComp}
  \lemSymSysTransComp
\end{lemma}

\begin{proof}
  By applying similar arguments in Lemmas \ref{lem:SymSysTransSnd} and \ref{lem:SymSysTransRcv}.
\end{proof}


%\begin{itemize}
%\item $M_N, M_2$ are transition systems of two instances $\sys{N}, \sys{2}$ of an~\idsep{} algorithm $\mathcal{A}$, and 
%\item $I_N, I_2$ are initial configurations of $M_N, M_2$.
%\item $F_{i, j}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with two indexes $i, j$.
%\end{itemize} 
%This property is formalized in Theorem \ref{thm:NCutoff}, 
%and its proof has two major steps:
%\begin{enumerate}
%\item Lemma \ref{lem:ProjCheckingProp} says that  $M_N, I_N$ is a model of $F_{i,j} $ for every $i, j \in \nid$ and $i \neq j$ if and only if $M_N, I_N$ is a model of $F_{1,2}$.
%
%\item Lemma \ref{lem:TraceEquiv} says that transition systems $M_N$ and $M_2$ of two instances $\sys{N}$ and $\sys{2}$ of an~\idsep{} algorithm $\mathcal{A}$ are trace equivalent under a set of predicates which inspect only variables with (at most) two indexes $1, 2$.
%\end{enumerate}

\subsection{Cutoff results in the~\idsep{} class}

\begin{theorem} \label{thm:NCutoffOneIndex}
  Let $\mathcal{A}$ be an~\idsep{} algorithm, 
  and $\sys{N}, \sys{1}$ be instances of $\mathcal{A}$ for some $N \geq 2$.
  Let $M_N = (\gstates{N}, \leadsto, \ginitstates{N}), M_2 = (\gstates{2}, \leadsto, \ginitstates{2})$ be transition systems of $\sys{N}, \sys{2}$ where $\ginitstates{N} = \{\ginitstate{N}\} , \ginitstates{2} = \{\ginitstate{2} \}$.
  Let $F_{i}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with  one index $i$.
  It follows 
  \[
  M_N, \ginitstate{N} \models \bigwedge{i \in \nid} F_{i} \Leftrightarrow M_1, \ginitstate{1} \models  F_{1}
  \]
\end{theorem}

\begin{proof}
  Let $i$ be an index in $\nid$.
  There exists a permutation $\perm$ on a set $\nid$ such that $\perm(i) = 1$ .
  By Lemma \ref{lem:ProjCheckingProp}, it follows
  \[
  M_N, \ginitstate{N} \models  F_{i} \Leftrightarrow \perm(M_N), \perm(\ginitstate{N}) \models  F_{\perm(i)}
  \]
  By the assumption, we have $F_{\perm(i)} = F_{1}$.
  By Lemma \ref{lem:SymSys}, it follows $\perm(M_N) = M_N$.
  By Lemma \ref{lem:SymInitConf}, we have $\perm(\ginitstate{N}) = \ginitstate{N}$.
  Therefore, it follows
  \[
  M_N, \ginitstate{N} \models  F_{i} \Leftrightarrow M_N, \ginitstate{N} \models  F_{1}
  \]
  Since $i$ are arbitray, we have
  $
  M_N, \ginitstate{N} \models  F_{1} 
  \Leftrightarrow M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i}
  $.
  By Lemma \ref{lem:TraceEquiv}, we have
  $
  M_N, \ginitstate{N} \models  F_{1} \Leftrightarrow M_2, \ginitstate{2} \models  F_{1}
  $.
  It follows that
  \[
  M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i} \Leftrightarrow M_2, \ginitstate{2} \models  F_{1}
  \]
  Therefore, Theorem \ref{thm:NCutoffTwoIndexes} is correct. \qed
\end{proof}



\begin{theorem} \label{thm:NCutoffTwoIndexes}
  Let $\mathcal{A}$ be an~\idsep{} algorithm, 
  and $\sys{N}, \sys{2}$ be instances of $\mathcal{A}$ for some $N \geq 2$.
  Let $M_N = (\gstates{N}, \leadsto, \ginitstates{N}), M_2 = (\gstates{2}, \leadsto, \ginitstates{2})$ be transition systems of $\sys{N}, \sys{2}$ where $\ginitstates{N} = \{\ginitstate{N}\} , \ginitstates{2} = \{\ginitstate{2} \}$.
  Let $G_{i, j}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with two different indexes $i, j \in \nid$.
  It follows 
  \[
  M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  \]
\end{theorem}

\begin{proof}
  Let $i, j$ be different indexes in $\nid$.
  There exists a permutation $\perm$ on a set $\nid$ such that $\perm(i) = 1$ and $\perm(j) = 2$.
  By Lemma \ref{lem:ProjCheckingProp}, it follows
  \[
  M_N, \ginitstate{N} \models  G_{i, j} \Leftrightarrow \perm(M_N), \perm(\ginitstate{N}) \models  G_{\perm(i), \perm(j)}
  \]
  By the assumption, we have $G_{\perm(i), ,\perm(j)} = G_{1,2}$.
  By Lemma \ref{lem:SymSys}, it follows $\perm(M_N) = M_N$.
  By Lemma \ref{lem:SymInitConf}, we have $\perm(\ginitstate{N}) = \ginitstate{N}$.
  Therefore, it follows
  \[
  M_N, \ginitstate{N} \models  G_{i, j} \Leftrightarrow M_N, \ginitstate{N} \models  G_{1, 2}
  \]
  Since $i,j$ are arbitray, we have
  $
  M_N, \ginitstate{N} \models  G_{1, 2} 
  \Leftrightarrow M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j}
  $.
  By Lemma \ref{lem:TraceEquiv}, we have
  $
  M_N, \ginitstate{N} \models  G_{1, 2} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  $.
  It follows that
  \[
  M_N, \ginitstate{N} \models \bigwedge^{i \in \nid}_{j \in \nid \setminus \{i\}} G_{i, j} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  \]
  Therefore, Theorem \ref{thm:NCutoffTwoIndexes} is correct. \qed
\end{proof}




\subsection{Trace equivanlence}

TODO: WILl rewRWITE.


\begin{lemma} \label{lem:ProjCheckingProp}
Let $\mathcal{A}$ be an~\idsep{} algorithm, 
and $\sys{N}, \sys{2}$ be instances of $\mathcal{A}$ for some $N \geq 2$.
Let $M_N = (\gstates{N}, \leadsto, \ginitstates{N}), M_2 = (\gstates{2}, \leadsto, \ginitstates{2})$ be transition systems of $\sys{N}, \sys{2}$ where $\ginitstates{N} = \{\ginitstate{N}\} , \ginitstates{2} = \{\ginitstate{2} \}$.
Let $F_{i, j}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with (at most) two indexes $i, j$.
It follows 
\[
M_N, \ginitstate{N} \models F_{i, j} \Leftrightarrow \perm(M_N), \perm(\ginitstate{N}) \models  F_{\perm(i), \perm(2)}
\]
\end{lemma}

\subsection{Trace equivalence with path projection}


\begin{lemma} \label{lem:TraceEquiv}
Let $\mathcal{A}$ be an~\idsep{} algorithm, 
and $\sys{N}, \sys{2}$ be instances of $\mathcal{A}$ for some $N \geq 2$.
Let $M_N = (\gstates{N}, \leadsto, \ginitstates{N}), M_2 = (\gstates{2}, \leadsto, \ginitstates{2})$ be transition systems of $\sys{N}, \sys{2}$ where $\ginitstates{N} = \{\ginitstate{N}\} , \ginitstates{2} = \{\ginitstate{2} \}$.
Let $AP$ be a set of predicates which inspect only variables with (at most) two indexes $1, 2$.
It follows that $M_N, M_2$ are trace equivalent under $AP$.
\end{lemma}

In this section, we first show that two instances $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1, 2}(\mathcal{A},  \Delta, \Phi)$ of an arbitrary ``ID--separated'' algorithm $\mathcal{A}$ are trace equivalent under the set $\mathit{AP}$ of atomic predicates whose is in the form of either $p_i.\lpc = \mathit{val}$ or $p_i.X_\ell[p_j] = \mathit{val}$ where $p_i, p_j$ are processes in $\left\{p_1, p_2 \right\}$, and $X_\ell$ is a local variable, and $p_i.X_\ell[p_j]$ is to assess a one--dimensional local variable $X_\ell$ of a process $p_i$ with an index $p_j$, and $p_i.\lpc$ refers to the next instruction block performed by a process $p_i$. This result is presented with Corollary \ref{cor:EquivAtomicFixedLocalRead}.


TODO: move it somewhere else
The first is called \emph{one--dimensional local read} predicates on an index $p_i$, and the later is called \emph{two--dimensional local read} predicates on indexes $p_i, p_j$.
Whenever the context is clear, we simply write local read predicates.

We extend the previous result for quantified formulas 
$ \forall p_i, p_j \colon  F(p_i, p_j)$ where $F(p_i, p_j)$ is a formula based on one--dimensional or two--dimensional local read predicates.
This extended result is presented with Theorem \ref{thm:EquivLocalRead}
The result demonstrates a cutoff result for the number of processes in checking a class of LTL formulas in the form of $\lozenge \square \forall p_i, p_j \colon  F(p_i, p_j)$ or $\square \forall p_i, p_j \colon  F(p_i, p_j)$.
This class of LTL formulas can present many properties such as strong completeness and strong accuracy of the eventually perfect failure detectors in~\cite{CT96}.


\subsection{Local read predicates with fixed indexes }

To prove the trace equivalence of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1, 2}(\mathcal{A}, \Delta, \Phi)$, we first provide the definition of an \emph{admissible} sequence in $\sys{N}$. Intuitively, a sequence of configurations in $\sys{N}$ is admisible if it is a refinement of an admissible execution path in $\sys{N}$.
Moreover, we present a technique for configuration constructions called ID--projection 
Lemma \ref{lem:IDProjConf} shows that a configuration constructed with the~\idsep{} technique from another configuration in $\sys{N}$ is a legal configuration in~$\sys{2}$.
We will apply this construction technique in the proof of trace equivalence for $\sys{2}$ and $\sys{N}$ under a set $\mathit{AP}$.
%Then, Lemmas \ref{lem:IDsProj} and \ref{lem:IDsRefill} shows that a infinite sequence of configurations constructed with these techniques are legal in corresponding system instances, and trace equivalent with the original ones.


\begin{definition} \label{def:AdmisibleSeq}
An infinite sequence of configurations $\pi = \psi_0 \psi_1 \ldots $ is \emph{admissible} in $\sys{N}$ if the following properties hold:
\begin{enumerate}
\item $\psi_0$ is consistent with an initial global state in $\sys{N}$.

\item For every $k > 0$, a finite sequence of configurations $\psi^N_{4k-4} \rightarrow \psi^N_{4k-3} \rightarrow \psi^N_{4k-2} \rightarrow \psi^N_{4k-1} \rightarrow \psi^N_{4k}$ is a refinement of a global transition at a time $k$.

\item Both constraints $\Delta$ and $\Phi$ hold in $\pi$ from the global stabilization time $t_0$.
\end{enumerate}
\end{definition}



\begin{construction} \label{def:IDSep}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with local variables $X_1, \ldots, X_M, \lpc$.
  Let $S_{1..N}(\mathcal{A}, \Delta, \Phi)$  and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$ be two instances of $\mathcal{A}$ for some $N \geq 2$.
  Let $\psi^N$ be an arbitrary configuration of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$.
  A configuration $\psi^2$  is called an ID--projection of $\psi^N$ if following properties hold:
  
  \begin{enumerate}
%    \item A domain of every one-dimensional variable in $\psi^2$ is $\left\{p_1, p_2\right\}$.
%    
%    \item A domain of a one-dimensional variable in $\psi^2$ is $\left\{p_1, p_2\right\}$.
    
    
    \item For every process $p \in \{p_1, p_2\}$, it follows $\psi^N(\gpc[p]) = \psi^2(\gpc[p])$ and  $\psi^N(p).\lpc = \psi^2(p).\lpc$.
    
    \item For every $q, p \in \{p_1, p_2\}$, it follows $\psi^N(\buf{p}{q}) = \psi^2(\buf{p}{q})$, and $\psi^N(p_1).X[p_2] = \psi^2(p_1).X[p_2]$ for every one-dimensional local variable $X$.
    \item For every in--transit message $m$ in $\psi^N$, a message $m$ is also in transit in $\psi^2$ and we have  $\psi^N(\age{m}) = \psi^2(\age{m})$.
    
    %  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if process $p_i^N$ receives a set of messages $\mathit{Msgs}$ in state $s^N_k$, then process $p_i^2$ receives a set of messages $\{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ in state $s^2_k$. \footnote{TODO: Override notations here since $m$ is used for different messages in different system instances.}
    %  
    %  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ and $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ are the same.
    %  
    %  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
    %  
    %  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^N$ crashes at time point $k$, then process $p_i^2$ also crashes at time point $k$.
  \end{enumerate}  
\end{construction}

\newcommand{\lemIDProjConf}{
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $(M + 2)$ local variables $X_1, \ldots, X_M, \lpc{}, \mailbox{}$.
  Let $S_{1..N}(\mathcal{A}, \Delta, \Phi)$  and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$ be two instances of $\mathcal{A}$.
  Let $\psi^N$ be a configuration of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$.
  Let $\psi^2$ be a configuration constructed from $\psi^N$ with the ID--projection technique.
  Then, $\psi^2$ is a configuration of $\sys{2}$
}

\begin{lemma} \label{lem:IDProjConf}
\lemIDProjConf
\end{lemma}

\begin{proof}
    By the ID--projection construction, the following constraints hold: 
  \begin{enumerate}[label=(\roman*)]
    \item $\forall p, q \in \{p_1, p_2\} \, \forall 1 \leq \ell \leq M \colon   \conf{2}{0}(p).X_\ell[q] \in \mathit{Val}_\ell$
    
    \item $\forall p, q \in \{p_1, p_2\} \colon    \conf{2}{0}(p).\mailbox[q] \subseteq \texttt{Msg}^{p}_{q}$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \colon   \conf{2}{0}(\buf{p}{q}) \subseteq \texttt{Msg}^{p}_{q} $
    
    \item $\forall p \in \{p_1, p_2\} \colon   \conf{2}{0}(\gpc[p]) \in \Boolean \land  \conf{2}{0}(p).\lpc \in \isc$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \, \forall m \colon   m \in \psi^2(\buf{p}{q}) \Rightarrow \psi^2(\age{m}) \in \mathbb{N}$ 
  \end{enumerate}
Therefore, a configuration $\psi^2$ is a configuration in $\sys{2}$ \qed
\end{proof}

\newcommand{\lemIDProjPath}{
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $(M + 2)$ local variables $X_1, \ldots, X_M, \lpc{}, \mailbox{}$.
Let $S_{1..N}(\mathcal{A}, \Delta, \Phi)$  and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$ be two instances of $\mathcal{A}$.
Let $\pi^N = \psi^N_0  \psi_1^N\ldots$ be an arbitrary admissible sequence of configurations of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ such that
the global stabilization time in $\pi^N$ is a time $t_0$.
Let $\pi^2 = \psi^2_0 \psi_1^2\ldots$ be an infinite sequence of configurations such that 
(i) a configuration $\conf{2}{k}$ is constructed from a configuration $\conf{N}{k}$ by the ID--projection technique for every $k \geq 0$, and 
(ii) the global stabilization time in $\pi^2$ is also the time $t_0$.
It follows that a sequence $\pi^2$ is admissible in $\sys{2}$.
}


\begin{lemma} \label{lem:IDProjPath}
\lemIDProjPath
\end{lemma}

\begin{proof}
  First, we prove that $\conf{2}{0}$ is consistent with an initial state $\sys{2}$ by the construction. By Lemma \ref{lem:IDProjConf}, it follows that $\conf{2}{0}$ is a configuration in  $\sys{2}$. Since $\conf{N}{0}$ is consistent with an initial state in $\sys{N}$, so is $\conf{2}{0}$ in $\sys{2}$.

  
%  Therefore, $\conf{2}{0}$ is consistent with a global state  in $\sys{2}$.
%  Moreover, since $\conf{N}{0}$ is consistent with an initial state in $\sys{N}$ and the construction of $\conf{2}{0}$, it immediately follows that  $\conf{2}{0}$ is consistent with an initial state $\sys{2}$.

  
  Second, we prove that every sequence $\conf{2}{4k - 4} \rightarrow \ldots \rightarrow \conf{2}{4k}$ is a refinement of a global transition at a time $k$ by induction on $k$.
  \begin{enumerate}
    \item \emph{Base case.} By the lemma hypothesis, we have that
    \[
    \conf{N}{1} \xrightarrow{\sched{}} \conf{N}{1} \xrightarrow{\tsnd{}} \conf{N}{2} \xrightarrow{\trcv{}}  \conf{N}{3} \xrightarrow{\cop{}} \conf{N}{4} 
    \]
    We need to prove that a sequence of configurations $\conf{2}{0} \rightarrow \conf{2}{1} \rightarrow \conf{2}{2} \rightarrow \conf{2}{3} \rightarrow \conf{2}{4}$ 
%    $ \tconfsched{1}  \rightarrow \tconfsnd{1}  \rightarrow \tconfrcv{1}  \rightarrow \sigma^2_1$
%    such that 
%    \[
%    \conf{2}{1} = \tconfsched{1} \land \conf{2}{2} = \tconfsnd{1} \land \conf{2}{3} = \tconfrcv{1} \land \conf{2}{4} = \sigma^2_1
%    \]
    presents respectively subrounds Schedule, Send, Receive, and Computation.
    By Lemma \ref{lem:IDProjConf}, $\conf{2}{k}$ is a configuration in $\sys{2}$ for every $1 \leq k \leq 4$.
    Therefore, we need to prove that every constraint in a subround \texttt{Rnd} hold in the corresponding transition.
    The proof is by cases. \\
    \emph{$\bullet$ Transition $\conf{2}{0} \rightarrow \conf{2}{1}$}. We will show that this transition satisfies every constraint in the subround \sched{}.
    By the construction of $\conf{2}{1}$, we have 
    \begin{itemize}
     \item $\forall p, q \in \{p_1, p_2\} \, \forall 1 \leq \ell \leq M \colon   \conf{2}{1}(p).X_\ell[q] = \conf{N}{1}(p).X_\ell[q]$
    
    \item $\forall p, q \in \{p_1, p_2\} \colon    \conf{2}{1}(p).\mailbox[q] = \conf{N}{1}(p).\mailbox[q]$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \colon   \conf{2}{1}(\buf{p}{q}) = \conf{N}{1}(\buf{p}{q}) $
    
    \item $\forall p \in \{p_1, p_2\} \colon   \conf{2}{1}(\gpc[p]) = \conf{N}{1}(\gpc[p]) \land  \conf{2}{1}(p).\lpc = \conf{N}{1}(p).\lpc$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \, \forall m \in \psi^2(\buf{p}{q}) \colon   \psi^2(\age{m}) = \psi^N(\age{m})$ 
  \end{itemize}
  Since $\conf{N}{0} \rightarrow \conf{N}{1}$ is a send transition, we have that
 \begin{itemize}
    \item $\forall p, q \in \{p_1, p_2\} \, \forall 1 \leq \ell \leq M \colon   \conf{N}{1}(p).X_\ell[q] = \conf{N}{0}(p).X_\ell[q]$
    
    \item $\forall p, q \in \{p_1, p_2\} \colon    \conf{N}{1}(p).\mailbox[q] = \conf{N}{0}(p).\mailbox[q]$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \colon   \conf{N}{1}(\buf{p}{q}) = \conf{N}{0}(\buf{p}{q}) $
    
    \item $\forall p \in \{p_1, p_2\} \colon   \conf{2}{1}(\gpc[p]) \in \Boolean \land  \conf{N}{1}(p).\lpc = \conf{N}{0}(p).\lpc$ 
    
    \item $\forall p, q \in \{p_1, p_2\} \, \forall m \in \psi^N(\buf{p}{q}) \colon  \psi^N_1(\age{m}) = \psi^N_0(\age{m}) + 1$ 
  \end{itemize}
  It follows that every in--transit message age is increased by 1 in $\conf{2}{1}$, and only variable $\gpc$ can be updated in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$.
  Therefore, every constraint in the subround Send holds in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$.

  \emph{$\bullet$ Transition $\conf{2}{1} \rightarrow \conf{2}{2}$}. We will show that this transition satisfies every constraint in the subround Send.
   By the ID--projection construction, a process $p^N_i$ takes a step in this subround Send if and only a process $p^2_i$ takes a step in this subround  for every $i \in \left\{ 1, 2 \right\}$.
  Assume that a process $p^N_i$ performs an instruction $\tsnd(p^N_i, m)$ in a transition $\conf{N}{1} \rightarrow \conf{N}{2}$. We prove that a process $p^2_i$ performs an instruction $\tsnd(p^2_i, m)$ in a transition $\conf{2}{1} \rightarrow \conf{2}{2}$.
  Since $m$ has been sent by a process $p^N_i$, we have
  \begin{align*}
  \, & \forall p^N_j \colon     m \notin \conf{N}{1} \left( \buf{p^N_i}{p^N_j}\right)   \\
  \land \, &   \forall p_j \colon   \conf{N}{2} \left( \buf{p^N_i}{p^N_j}\right) = \left\{ m \right\} \cup \conf{N}{1} \left( \buf{p^N_i}{p^N_j}\right) 
  \end{align*}

  We have $\conf{2}{\ell}(\buf{p^2_i}{q^2_j})  = \conf{N}{\ell}(\buf{p^N_i}{q^N_j})$ for every $1 \leq i, j \leq 2$ and $1 \leq \ell \leq 2$ by the construction of $\conf{2}{2}$ and $\conf{2}{2}$.
  It follows that 
  \begin{align*}
  \, & \forall p^2_j \colon     m \notin \conf{2}{1} \left( \buf{p^2_i}{p^2_j}\right)   \\
  \land \, &   \forall p_j \colon   \conf{2}{2} \left( \buf{p^2_i}{p^2_j}\right) = \left\{ m \right\} \cup \conf{2}{1} \left( \buf{p^2_i}{p^2_j}\right) 
  \end{align*}
  
  Moreover, we have $\conf{2}{2}(\age{m}) = 0$.
  Hence, it follows $\conf{2}{2}.\tsnd(p^2_i, m) = \top$.
  Now we consider which messages  a process $p^2_i$ has received from a process $p_j$ in this round where $i, j \in \left\{ 1, 2 \right\}$. 
  By the construction of $\conf{2}{2}$, we have 
  \begin{align*}
  \conf{2}{2}(p^2_i).\mailbox[p^2_j] & = \conf{N}{2}(p^N_i).\mailbox[p^N_j]
  = \conf{N}{1}(p^N_i).\mailbox[p^N_j] \\
  & = \conf{2}{1}(p^2_i).\mailbox[p^2_j]
  \end{align*}
  
  
%  Since we are considering the subround $\tsnd^N$, it follows  $\conf{N}{1}(\buf{p^2_j}{p^2_i}) \subseteq \conf{N}{2}(\buf{p^2_j}{p^2_i})$.
  Therefore, we need to prove that $\conf{2}{2}.\rop{p^2_i}[p^2_j]  = \emptyset$.
  By the construction of $\conf{2}{2}$, it follows $\conf{2}{1}(\buf{p^2_j}{p^2_i}) \subseteq \conf{2}{2}(\buf{p^2_j}{p^2_i})$.
  It immediately follows that $\conf{2}{2}.\rop{p^2_i}[p^2_j]  = \emptyset$.
  In other worlds, a process $p^2_i$ has not received any message in this round, and it is consistent with the evaluation of $\conf{2}{2}(p^2_i).\mailbox[p^2_j]$ for every $i, j \in \left\{ 1, 2 \right\}$.
  Now we prove that every variable's value  $\conf{2}{2}(p^2_i).X_\ell[p^2_j]$ satisfies the corresponding \idsep{} constraint for every $i, j \in \left\{ 1, 2 \right\}$, and $1 \leq \ell \leq M$.
  Since $\sys{N}$ is ``ID--separation'' and we are considering the subround $\tsnd$, it follows
  \begin{alignat*}{3}
  \conf{N}{2}( p^N_i ).X_\ell [p^N_j] & = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
  & && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M 
  \big)   
  \end{alignat*}
  Since $\conf{N}{2}( p^N_i ).X_\ell [p^N_j] = \conf{2}{2}( p^2_i ).X_\ell [p^2_j]$, we have 
  \begin{alignat*}{3}
  \conf{2}{2}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
  & && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M 
  \big)   
  \end{alignat*}
  It immediately follows that
  \begin{alignat*}{3}
  \conf{2}{2}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
  & && \conf{2}{2}.\trcv(p^2_i)[p^2_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}( p^2_i).X_M 
  \big)   
  \end{alignat*}
  since the later function application is with the same arguments of the first.
  Finally, by the construction of $\conf{2}{2}$, it is easy to check that every ``not--running'' process does not change its local state and not receive any message in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$. Therefore, this transition simulates a subround Send.


  \emph{$\bullet$ Transition $\conf{2}{2} \rightarrow \conf{2}{3}$}. We will show that this transition satisfies every constraint in the subround Receive. 
  By the ID--projection construction, a process $p^N_i$ takes a step in this subround Receive if and only a process $p^2_i$ takes a step in this subround  for every $i \in \left\{ 1, 2 \right\}$.
  Hence, we first consider only ``running'' processes. 
  Assume that a process $p^N_i$ has received a set $S$ of messages from a process $p^N_j$ in a transition $\conf{N}{2} \rightarrow \conf{N}{3}$. 
  We prove that a process $p^2_i$ has received the same set $S$ of messages from a process $p^2_j$ in a transition $\conf{2}{2} \rightarrow \conf{2}{3}$.
  By the construction of $\pi^2$, we have 
  \begin{align*}
    \conf{N}{2}(\buf{p^N_j}{p^N_i}) & = \conf{2}{2}(\buf{p^N_j}{p^N_i}) \\ \conf{N}{3}(\buf{p^N_j}{p^N_i}) & = \conf{2}{3}(\buf{p^N_j}{p^N_i}) \\
    \conf{N}{3}.\trcv(p^N_i)[p^N_j] & = S = \conf{N}{2}(\buf{p^N_j}{p^N_i}) \setminus \conf{N}{3}(\buf{p^N_j}{p^N_i}) 
  \end{align*}
  It follows that $S = \conf{2}{2}(\buf{p^2_i}{p^2_j}) \setminus \conf{2}{3}(\buf{p^2_i}{p^2_j})$.
  Moreover, due to 
  \begin{align*}
  \conf{N}{3}(p^N_i).\lpc[p^N_j] & = \conf{N}{2}(p^N_i).\lpc[p^N_j] \cup S \\
  \conf{N}{3}(p^N_i).\mailbox[p^N_j] & = \conf{2}{3}(p^2_i).\mailbox[p^2_j] \\
  \conf{N}{2}(p^N_i).\mailbox[p^N_j] & = \conf{2}{2}(p^2_i).\mailbox[p^2_j]
  \end{align*}
  we have that 
  $
  \conf{2}{3}(p^2_i).\mailbox[p^2_j] = \conf{2}{2}(p^2_i).\mailbox[p^N_j] \cup S
  $.
  It implies that a process $p^2_i$ has received a set $S$ of messages from a process $p^2_j$.
  By similar arguments in the above proof for the subround Send, it follows that every variable's value $\conf{2}{3}(p^N_i).X_\ell[p^2_j]$  satisfies the corresponding \idsep{} constraint, i.e.
  \begin{alignat*}{3}
  \conf{2}{3}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{2}{2}(p^2_i).\lpc,   \conf{2}{3}(\gpc \left[ p^2_i \right]),  \\
  & && \conf{2}{3}.\trcv(p^2_i)[p^2_j], \conf{2}{2}( p^2_i ).X_1, \ldots, \conf{2}{2}( p^2_i).X_M 
  \big)   
  \end{alignat*}
  Finally, for every ``not--running'' process $p^2 \in \left\{ p^2_1, p^2_2 \right\}$, i.e. $\conf{2}{2}(p^2).\lpc \neq \trcv{}$ or $\conf{2}{3}(\gpc[p^2]) = \bot$, it is easy to check that (i) a process $p^2$ does not update its local state and (ii) message buffers related to  $p^i$ are unchanged. 
  Therefore, every constraint in the subround $\trcv{}$ is satisfied in the transition $\conf{2}{2} \rightarrow \conf{2}{3}$.
  
  \emph{$\bullet$ Transition $\conf{2}{3} \rightarrow \conf{2}{4}$}. We will show that this transition satisfies every constraint in the subround \cop{}.  
  By the construction of $\conf{2}{4}$ and $\conf{N}{4}$, we have
  \begin{alignat*}{3}
    \conf{2}{4}(\buf{p^2_i}{p^2_j}) & = \conf{N}{4}(\buf{p^N_i}{p^N_j}) && = \conf{N}{3}(\buf{p^N_i}{p^N_j}) \\
    & && = \conf{2}{3}(\buf{p^N_i}{p^N_j}) \\    
    \conf{2}{4}(p^2_i).\mailbox[p^2_j] & = \conf{N}{4}(p^2_i).\mailbox[p^2_j] && = \conf{N}{3}(p^2_i).\mailbox[p^2_j] \\
    & && = \conf{2}{3}(p^2_i).\mailbox[p^2_j]    
  \end{alignat*}
  It follows no process has sent or received any message in the transition $\conf{2}{3} \rightarrow \conf{2}{4}$.
  Now we prove that every variable's value  $\conf{2}{2}(p^2_i).X_\ell[p^2_j]$ satisfies the corresponding \idsep{} constraint for every $i, j \in \left\{ 1, 2 \right\}$, and $1 \leq \ell \leq M$.
  It follows  
  \begin{alignat*}{3}
  \conf{2}{4}(p^2_i).X_\ell[p^2_j] & = \conf{N}{3} && (p^N_i).X_\ell[p^N_j]  \\
  & = f_\ell \big( && \cop{}, \conf{N}{3}(p^N_i).\lpc,   \conf{N}{4}(\gpc \left[ p^N_i \right]),  \\
  & && \conf{N}{4}.\trcv(p^N_i)[p^N_j], \conf{N}{3}( p^N_i ).X_1, \ldots, \conf{N}{3}(p^N_i).X_M  \big)  \\
  & = f_\ell \big( && \cop, \conf{2}{3}(p^2_i).\lpc,   \conf{2}{4}(\gpc \left[ p^2_i \right]),  \\
  & && \conf{2}{4}.\trcv(p^2_i)[p^2_j], \conf{2}{3}( p^2_i ).X_1, \ldots, \conf{2}{3}(p^2_i).X_M  \big)    
  \end{alignat*}
  Therefore, every constraint in the subround \cop{} is hold in the transition $\conf{2}{3} \rightarrow \conf{2}{4}$.
  \item \emph{Induction step for a sequence $\conf{2}{4k - 4} \rightarrow \conf{2}{4k - 3} \rightarrow \conf{2}{4k - 2} \rightarrow \conf{2}{4k - 1} \rightarrow \conf{2}{4k}$.} The proof is similar for the base case.
  \item Therefore, every sequence $\conf{2}{4k - 4} \rightarrow \conf{2}{4k - 3} \rightarrow \conf{2}{4k - 2} \rightarrow \conf{2}{4k - 1} \rightarrow \conf{2}{4k}$ is a refinement of a global transition at a time $k$.
  \end{enumerate}
  Thirdly, we prove that both constraints $\Delta$ and $\Phi$ are hold in the path $\pi^2$ by contradiction. 
  \begin{itemize}
  \item \emph{Constraint $\Delta$}: Assume that there exist a transition $\conf{2}{t-1} \xrightarrow{\trcv{}} \conf{2}{t}$ in $\pi^2$ for some $t \geq t_0$, two processes $p^2_i, p^2_j \in \left\{p^2_1, p^2_2 \right\}$, and a message $m$ such that 
  \begin{alignat*}{4}
  \noindent
  \, & m \in \conf{2}{t - 1}(\buf{p^2_j}{p^2_i}) &&  \land  \conf{2}{t - 1}(\gpc[p^2_i])  &&& \,  \land \,  \conf{2}{t - 1}([p^2_i]).\lpc = \trcv{}  \\
  \land \, &   m \in \conf{2}{t}(\buf{p^2_j}{p^2_i})  && \land \conf{2}{t}(\age{m}) \geq \Delta &&& 
%  \land \, &  m \in \conf{2}{t}(\buf{p^2_j}{p^2_i}) && \\
  \end{alignat*}  
  By the construction of configurations $\conf{2}{t}$ and $\conf{2}{t - 1}$, we have 
  \begin{align*}
  \conf{2}{t - 1}(\buf{p^2_j}{p^2_i}) & =  \conf{N}{t - 1}(\buf{p^N_j}{p^N_i}) \\
  \conf{2}{t}(\buf{p^2_j}{p^2_i}) & =  \conf{N}{t}(\buf{p^N_j}{p^N_i}) \\
  \forall m \colon   m \in \conf{2}{t - 1}([p^2_i]).\lpc = \trcv{} & \Rightarrow \conf{2}{t}(\age{m}) = \conf{N}{t}(\age{m})
  \end{align*}
  Therefore, a message $m$ is not delivered to a process $p^N_i$ in the transition $\conf{N}{t-1} \xrightarrow{\trcv{}} \conf{N}{t}$, and it is at least $\Delta$ time--units old in a configuration $\conf{N}{t}$.
  It implies the constraint $\Delta$ is violated in $\pi^N$.
  Contradiction. 
  
  \item \emph{Constraint $\Phi$}: By the proof related to the subround \sched{}, it follows that the transition $\conf{2}{4k} \rightarrow \conf{2}{4k + 1}$ is for the subround \sched{} for every $k \geq 0$. 
  Assume that there exist a number $t \geq t_0$, a correct process $p^2 \in \left\{ p^2_1, p^2_2  \right\}$ such that 
  $
  \conf{2}{4t - 3}(\gpc[p^2])  =  \ldots = \conf{2}{4(t + \Delta) - 3}(\gpc[p^2]) = \bot
  $.
  In other words, a process $p^2$ does not take any step in the time interval $\left[ t, t + \Phi \right]$. 
  By the construction of $\pi^2$, we have that $\conf{2}{k}(\gpc[p^2]) = \conf{N}{k}(\gpc[p^2])$ for every $k \geq 0$.
  Therefore, we have
  \[
  \conf{N}{4t - 3}(\gpc[p^N])  =  \ldots = \conf{N}{4(t + \Delta) - 3}(\gpc[p^N]) = \bot
  \]
  It implies that a process $p^N$ does not take any step in the time interval $\left[ t, t + \Phi \right]$ after the global stabilization time $t_0$. 
  Contradiction.
  

\end{itemize}
  Therefore, a sequence of configurations $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ is an admissible path in $\sys{2}$. \qed                                                                                                                                                                              
\end{proof}

%\begin{construction}
%  Let $t > 0$ be an arbitrary natural number. Let $\lambda^2_k = \conf{2}{4t-4} \leadsto \conf{2}{4t}$ and $\lambda^N_k = \conf{N}{4t-4} \leadsto \conf{N}{4t}$ be finite sequences of configurations in $\sys{2}$ and $\sys{N}$, respectively, such that such sequences are a refinement of some global transition at a time $t$.
%  The sequence $\lambda^N_t$ is called an \idrefill{} of $\lambda^2_t$ if the following properties hold:
%  \begin{enumerate}
%  \item A configuration $\conf{2}{k}$ is an ID--projection of $\conf{N}{k}$ for every $4t - 4 \leq k \leq 4k$.
%  
%  \item Every process $p \in \left\{ p_1, \ldots, p_N \right\}$ takes a step at a time $t$. Formally, we have $\forall p \colon   \conf{N}{4t-3}(\gpc[p])$.
%  
%  \item If a process $p \in \left\{ p_3, \ldots, p_N \right\}$ performs the instruction $\trcv{}$ in this transition, then all in--transit messages which were sent to $p_i$ are delivered in this transition. Formally, we have
%  \begin{align*} \forall p \colon   & \left( \conf{N}{4t-4}(p).\lpc = \trcv{} \land \, \conf{N}{4t-3}.\gpc[p] \right) \\
%  & \qquad \Rightarrow \forall q \colon   \conf{N}{4t-1}(\buf{q}{p} = \emptyset) 
%  \end{align*}
%  \end{enumerate}
%\end{construction}

\begin{lemma} \label{lem:IDRefillConf}
Let $\conf{2}{0} \leadsto \conf{2}{4}$ be a refinement of a global transition in $\sys{2}$.
%Let $k$ be a number and $\conf{2}{k - 1}$ be configuration in $\sys{2}$ such that $k > 0$ and a configuration $\conf{2}{k - 1}$ is consistent with some global state. 
Let $\conf{N}{0}$ be a configuration in $\sys{N}$ such that

\begin{enumerate}  
\item A configuration $\conf{2}{0}$ is an ID--projection of $\conf{N}{0}$.
\item All processes $p^N_3, \ldots, p^N_N$ are already crashed in $\conf{N}{0}$, and their related message buffers are empty.
\item A configuration $\conf{N}{0}$ is consistent with a global state in $\sys{N}$.
\end{enumerate} 

There exist configurations $\conf{N}{1}, \ldots, \conf{N}{4}$ such that a sequence $\conf{N}{0} \leadsto \conf{N}{4}$ is a refinement of a global transition in $\sys{N}$ and $\conf{N}{4}$ is consistent with a global state in $\sys{N}$.
\end{lemma}

\begin{proof}
The proof is by on the construction of configurations $\conf{N}{1}, \ldots, \conf{N}{4}$.
Since processes $p^N_3, \ldots, p^N_N$ are already crashed in $\conf{N}{0}$ and their related buffers are empty, we need to consider only two processes $p^N_1, p^N_2$ and the messages buffers between two processes. 
A configuration $\conf{N}{k}$ for every $1 \leq k \leq 4$ is constructed as following:

  \begin{enumerate}
  \item $\forall i \in 3..N \colon   \conf{N}{k}(p^N_i).\lpc = \texttt{``Crash''}$
  
  \item $\forall i \in 3..N, j \in 1..N \colon   \conf{N}{k}(\buf{p^N_i}{p^N_j}) = \conf{N}{k}(\buf{p^N_j}{p^N_i}) = \emptyset $
  
  \item $\forall i \in 1..2 \colon   \conf{N}{k}(\gpc[p^N_i]) = \conf{2}{k}(\gpc[p^2_i]) \land \conf{N}{k}(p^N_i).\lpc = \conf{2}{k}(p^2_i).\lpc$
  
  \item $\forall i, j \in 1..2 \forall k \in 1..M \colon   \conf{N}{k}(p^N_i).X_k[p^N_j] = \conf{2}{k}(p^2_i).X_k[p^2_j]$
  
  \item $\forall i \in 1..2, j \in 3..N \, \forall \ell \in 1..M \colon   \conf{N}{k}(p^N_i).X_\ell[p^N_j] = \\
  \text{} \quad f_\ell \big(  \texttt{Rnd}, \conf{N}{k-1}(p^N_i).\lpc,  \conf{N}{k-1}(\gpc \left[ p^N_i \right]), \conf{N}{k-1}.\trcv(p^N_i)[p^N_j],  \\    
  \text{        } \qquad \conf{N}{k-1}( p^N_i ).X_1, \ldots,  \conf{N}{k-1}(p^N_i).X_M 
  \big)   $
  
  \item $\forall i, j \in \left\{1, 2 \right\}  \colon   \conf{N}{k}(p^N_i).\mailbox[p^N_j] = \conf{2}{k}(p^2_i).\mailbox[p^2_j]$
  
  \item $\forall i \in 1..2, j \in 3..N  \colon   \conf{N}{k}(p^N_i).\mailbox[p^N_j] = \emptyset$
\end{enumerate}  
It immediately follows from the construction that every configuration $\conf{N}{k}$ is one in $\sys{N}$. Now we consider each transition. 

\emph{$\bullet$ Transition $\conf{N}{0} \rightarrow \conf{N}{1}$}. Since neither process states nor message buffers are changed in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$, it immediately follows that neither process states nor message buffers are changed in the transition $\conf{N}{0} \rightarrow \conf{N}{1}$. Therefore, every constraint for the subround \sched{} holds in the transition $\conf{N}{0} \rightarrow \conf{N}{1}$. 

\emph{$\bullet$ Transition $\conf{N}{1} \rightarrow \conf{N}{2}$}. 
Let $p^N_i \in \left\{ p^N_1, p^N_2 \right\}$ be a ``running'' process in this transition.
By similar arguments in the proof of Lemma \ref{lem:IDsProjInf} for the subround Send, it follows that (i) a message $m$ has been sent by a process $p^N_i$ in this transition if and only if a message $m$ has been sent by a process $p^2_i$ in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$, and (ii) no in--transit message is removed in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$.
Moreover, for every $1 \leq \ell \leq M$, for every $p^N_j \in \left\{ p^N_1, p^N_2 \right\}$, we have 
\begin{alignat*}{3}
\conf{N}{2}(p^N_i).X_\ell[p^N_j] & = \conf{2}{2} && (p^2_i).X_\ell[p^2_j]  \\
& = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
& && \conf{2}{2}.\trcv(p^N_i)[p^N_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}(p^2_i).X_M  \big)  \\
& = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
& && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M  \big)    
\end{alignat*}
Hence, every constraint for the subround Send holds in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$. 

\emph{$\bullet$ Transition $\conf{N}{1} \rightarrow \conf{N}{2}$}. 
Let $p^N_i \in \left\{ p^N_1, p^N_2 \right\}$ be a ``running'' process in this transition.
By similar arguments in the proof of Lemma \ref{lem:IDsProjInf} for the subround Send, it follows that (i) a message $m$ has been sent by a process $p^N_i$ in this transition if and only if a message $m$ has been sent by a process $p^2_i$ in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$, and (ii) no in--transit message is removed in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$.
Moreover, for every $1 \leq \ell \leq M$, for every $p^N_j \in \left\{ p^N_1, p^N_2 \right\}$, we have 
\begin{alignat*}{3}
\conf{N}{2}(p^N_i).X_\ell[p^N_j] & = \conf{2}{2} && (p^2_i).X_\ell[p^2_j]  \\
& = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
& && \conf{2}{2}.\trcv(p^N_i)[p^N_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}(p^2_i).X_M  \big)  \\
& = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
& && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M  \big)    
\end{alignat*}
The variable value at indexes $p^N_3, \ldots, p^N_N$ is satisfied the ``ID--separated'' constraint by the construction.
Hence, every constraint for the subround Send holds in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$. 

\emph{$\bullet$ Transitions $\conf{N}{2} \rightarrow \conf{N}{3} \rightarrow \conf{N}{4}$}. By applying similar arguments in the proof of Lemma \ref{lem:IDProjPath} and in the above proof for the case Send.

As a result, Lemma \ref{lem:IDRefillConf} is correct.
\qed
\end{proof}

\begin{lemma} \label{lem:IDRefillment}
Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$.
There exists an admissible sequences of configurations $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ in $\sys{N}$ such that a configuration $\conf{2}{k}$ is an ID--projection of $\conf{N}{k}$ for every $k \geq 0$.
\end{lemma}




\begin{proof}
  We prove Lemma \ref{lem:IDRefillment} by a constructive proof.
  First, we describe the initial state of $\pi^N$, and iteratively construct a subsequence $\conf{N}{4t-4} \leadsto \conf{N}{4t}$ for every $t > 0$.
  Let $\conf{N}{0}$ be a state of $\sys{N}$ such that 
  \begin{enumerate}
  \item $\forall i \in 3..N \colon   \conf{N}{0}(p^N_i).\lpc = \texttt{``Crash''}$

  \item $\forall i \in 3..N, j \in 1..N \colon   \conf{N}{0}(\buf{p^N_i}{p^N_j}) = \conf{N}{0}(\buf{p^N_j}{p^N_i}) = \emptyset $
  
  \item $\forall i \in 1..2 \colon   \conf{N}{0}(\gpc[p^N_i]) = \conf{2}{0}(\gpc[p^2_i]) \land \conf{N}{0}(p^N_i).\lpc = \conf{2}{0}(p^2_i).\lpc$
  
  \item $\forall i, j \in 1..2 \forall k \in 1..M \colon   \conf{N}{0}(p^N_i).X_k[p^N_j] = \conf{2}{0}(p^2_i).X_k[p^2_j]$

  \item $\forall i \in 1..2, j \in 3..N \, \forall k \in 1..M \colon   \conf{N}{0}(p^N_i).X_k[p^N_j] = \conf{2}{0}(p^2_i).X_k[p^2_1]$
    
  \item $\forall i, j \in \left\{1, 2 \right\}  \colon   \conf{N}{0}(p^N_i).\mailbox[p^N_j] = \conf{2}{0}(p^2_i).\mailbox[p^2_j]$
  
  \item $\forall i \in 1..2, j \in 3..N  \colon   \conf{N}{0}(p^N_i).\mailbox[p^N_j] = \emptyset$
  \end{enumerate}
  It is easy to check that (i) $\conf{N}{0}$ is an initial state in $\sys{N}$ and (ii) a configuration $\conf{2}{0}$ is an ID--projection of $\conf{N}{0}$.

  For the construction of the postfix, we iteratively apply the construction and arguments in Lemma \ref{lem:IDRefillConf} for every $k$.
  \qed
\end{proof}


\newcommand{\corEquivAtomicFixedLocalRead}{
Let $\mathit{AP}$ be a set of atomic predicates whose is in the form of either $p_i.\lpc = \mathit{val}$ or $p_i.X_\ell[p_j] = \mathit{val}$ where $p_i, p_j$ are processes in $\left\{p_1, p_2 \right\}$, and $X_\ell$ is a local variable.
Then, two systems $\sys{2}$  and $\sys{N}$ are trace equivalent under $\mathit{AP}$.
}

\begin{corollary} \label{cor:EquivAtomicFixedLocalRead}
\corEquivAtomicFixedLocalRead
\end{corollary}

\begin{proof}
It immediately follows by Lemmas \ref{lem:IDProjPath} and \ref{lem:IDRefillConf}.
\end{proof}



\newcommand{\lemEquivFixedLocalRead}{
  Let $\idsepalgo{}$ be an \idsep{} algorithm with fixed values for $\Delta$ and $\Phi$.
  Let $\sys{2}$ and $\sys{N}$ be two instances of $\idsepalgo$
  Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ and $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ be admissable infinite sequences of configurations respectively in $\sys{2}$ and $\sys{N}$ such that a configuration $\conf{2}{k}$ is an ID--projection of a configuration $\conf{N}{k}$ for every $k \geq 0$.
  Let $F(p_1, p_2)$ be an arbitrary formula based on local read prediates with indexes $p_1, p_2$.
  It follows that $\conf{2}{k} \models F(p_1, p_2)$ if and only if $\conf{N}{k} \models F(p_1, p_2)$ for every $k \geq 0$.
}

\begin{lemma} \label{lem:EquivFixedLocalRead}
\lemEquivFixedLocalRead
\end{lemma}

\begin{proof}
  Let $k$ be a number such that $k \geq 0$. We prove the direction $(\Rightarrow)$ by induction on the structure of $F(p_1, p_2)$. 
  The base case immediately follows by Corollary \ref{cor:EquivAtomicFixedLocalRead}. 
  The proof of the induction step is by cases for the negation $\lnot$ and the conjunction $\land$ since the rest of connectives can be replaced with such connectives. 
  Notice that every quantified variable in $F(p_1, p_2)$ is bounded in a finite domain $\left\{p_1, p_2\right\}$, we could eliminate the quantifer $\forall$ with the conjuction $\land$.
  
  \begin{itemize}   
  \item  \emph{Case $ F(p_1, p_2) = \lnot F_1(p_1, p_2)$.} 
  By the induction hypothesis, it follows that $\conf{2}{k} \models F_1(p_1, p_2) \Rightarrow \conf{N}{k} \models F_1(p_1, p_2)$. 
  Hence, we have that if $\conf{2}{k} \models \lnot F_1(p_1, p_2)$, then $\conf{N}{k} \models \lnot F_1(p_1, p_2)$. 
  
  \item \emph{Case $ F(p_1, p_2) =  F_1(p_1, p_2) \land F_2(p_1, p_2)$.}
  By the induction hypothesis, it follows that $\conf{2}{k} \models F_i(p_1, p_2) \Rightarrow \conf{N}{k} \models F_i(p_1, p_2)$ for every $1 \leq i \leq 2$.
  Hence, we have that if $\conf{2}{k} \models \lnot F(p_1, p_2)$, then $\conf{N}{k} \models \lnot F(p_1, p_2)$. 
  
  
  \end{itemize}
  
  
  
  Hence, the direction $(\Rightarrow)$ holds. The proof for another direction is similar.
\qed
\end{proof}

\subsection{Quantified formulas with local read predicates}

%The following results are with 
To extend the previous result, we first prove Lemmas \ref{lem:RenameOne}--\ref{lem:RenameTwo} which says that two instances $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ of an \idsep algorithm are equivalent under a renaming function where $u, v$ are distinguished processes' id. 
Then, Theorem \ref{thm:EquivLocalRead} says that two instances  $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ of an~\idsep algorithm $\mathcal{A}$ are equivalent under a renaming function and a local read formula $F(p_u, p_v)$ where $u, v$ are distinguished processes' id. 
Finally, we provide a discussion about the application in checking a class of LTL formulas in the form of $\lozenge \square \forall p_i, p_j \colon   F(p_i, p_j)$.


\newcommand{\lemRenameOne}{
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm.
  Let $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ be instances of $\mathcal{A}$  where $p_u, p_v$ are distinguished processes. 
  Let $h \colon \left\{p_1, p_2\right\} \rightarrow \left\{ p_u, p_v \right\}$ be a bijective function such that $h(p_1) = p_v$ and $h(p_2) = p_v$.
%  \begin{enumerate}
%  \item 
  Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$. Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%  \begin{subequations}
  \begin{align*}
  \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h(p_i)}{h(p_j)}) \\
  \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h(p_i)]) \\
  \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h(p_i)).X[h(p_j)] \\
  \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h(p_i)).\lpc 
  \end{align*} 
  
%\end{subequations}
%  for every $p_i, p_j \in \left\{p_1, p_2\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$.
%  Then, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
%  
%   \item Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be an admissible sequence of configuration in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$. Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%  \begin{subequations}
%  \begin{align}
%  \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h^{-1}(p_i)}{h^{-1}(p_j)}) \\
%  \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h^{-1}(p_i)]) \\
%  \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h^{-1}(p_i)).X[h^{-1}(p_j)] \\
%  \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h^{-1}(p_i)).\lpc 
%  \end{align} 
%  \end{subequations}
%  for every $p_i, p_j \in \left\{p_u, p_v\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$ and $h^{-1}$ is a inverse function of a renaming function $h$.
%  Then, a sequence $\pi^{\prime}$ is admissible in $\sys{2}$.
%  \end{enumerate}
  }

\begin{lemma} \label{lem:RenameOne}
\lemRenameOne
\end{lemma}

\begin{proof}
The existence of $\pi^{\prime}$ is demonstrated by a constructive proof.
  By similar arguments in the proof of Lemma \ref{lem:IDProjConf}, it follows that $\conf{\prime}{0}$ is an initial state in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
  By similar arguments in the proof of Lemma \ref{lem:IDProjPath}, it follow that $\conf{\prime}{4t - 4} \leadsto \conf{\prime}{4t}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ for every $t \geq t_0$, and both constraints $\Delta$ and $\Phi$ hold in $\pi^{\prime}$.
  Hence, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
  
%  \item By similar arguments in the above proof, it follows that the sequence $\pi$ is admissible in $\sys{2}$. \qed
%\end{enumerate}
\end{proof}

\newcommand{\lemRenameTwo}{
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm.
  Let $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ be instances of $\mathcal{A}$  where $p_u, p_v$ are distinguished processes. 
  Let $h \colon \left\{p_1, p_2\right\} \rightarrow \left\{ p_u, p_v \right\}$ be a bijective function such that $h(p_1) = p_v$ and $h(p_2) = p_v$.
%  \begin{enumerate}
%    \item Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$. Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%    %  \begin{subequations}
%    \begin{align}
%    \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h(p_i)}{h(p_j)}) \\
%    \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h(p_i)]) \\
%    \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h(p_i)).X[h(p_j)] \\
%    \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h(p_i)).\lpc 
%    \end{align} 
%    
    %\end{subequations}
    %  for every $p_i, p_j \in \left\{p_1, p_2\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$.
    %  Then, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
    %  
    %   \item 
    Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be an admissible sequence of configuration in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$. Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
    %  \begin{subequations}
      \begin{align*}
      \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h^{-1}(p_i)}{h^{-1}(p_j)}) \\
      \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h^{-1}(p_i)]) \\
      \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h^{-1}(p_i)).X[h^{-1}(p_j)] \\
      \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h^{-1}(p_i)).\lpc 
      \end{align*} 
    %  \end{subequations}
      for every $p_i, p_j \in \left\{p_u, p_v\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$ and $h^{-1}$ is a inverse function of a renaming function $h$.
      Then, a sequence $\pi^{\prime}$ is admissible in $\sys{2}$.
%  \end{enumerate}
}

\begin{lemma} \label{lem:RenameTwo}
  \lemRenameTwo
\end{lemma}

\begin{proof}
  By similar arguments in the proof of \ref{lem:RenameOne}, it follows that the sequence $\pi$ is admissible in $\sys{2}$. \qed  
\end{proof}

\newcommand{\thmEquivLocalRead}{
  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
  Let $F(p_u, p_v)$ be a local read formula where $p_u, p_v \in \left\{ p_1, \ldots, p_N \right\}$.
  Let $h$ be a bijective renaming function such that $h(p_1) = p_u$ and $h(p_v) = p_2$.
  \begin{enumerate}
  \item Let $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ be an admissible infinite sequence of configurations in $\sys{N}$. There exists an admissible infinite sequence of configurations $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$   in $\sys{2}$ such that if $\conf{N}{k} \models F(p_u, p_v)$ then $\conf{2}{k} \models F(h^{-1}(p_u), ^{-1}(p_v))$ for every $k \geq 0$  where $h^{-1}$ is a inverse function.
        
  \item Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ be an admissible infinite sequence of configurations in $\sys{2}$. There exists an admissible infinite sequence of configurations $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$   in $\sys{N}$ such that if $\conf{2}{k} \models F(h^{-1}(p_u), h^{-1}(p_v))$ then $\conf{N}{k} \models F(p_u, p_v)$ for every $k \geq 0$
  where $h^{-1}$ is a inverse function.
  \end{enumerate}
}


\begin{theorem} \label{thm:EquivLocalRead}
  \thmEquivLocalRead
\end{theorem}

\begin{proof}
  We first present a proof for part 1. 
  By Lemma \ref{lem:IDProjPath}, there exist an admissible sequence  of configurations $\pi = \conf{}{0} \conf{}{1} \ldots$ in $S_{u, v}(\mathcal{A})$ such that a configuration $\conf{}{k}$ is an~\idsep{} of $\conf{N}{k}$ for every $k \geq 0$.
  By Lemma \ref{lem:EquivFixedLocalRead}, it follows that if $\conf{N}{k} \models F(p_u, p_v)$
  then $\conf{}{k} \models F(p_u, p_v)$ for every $k \geq 0$.
  By Lemma \ref{lem:EquivFixedLocalRead}, it follows that if $\conf{N}{k} \models F(p_u, p_v)$
  then $\conf{2}{k} \models F(h^{-1}(p_u), h^{-1}(p_v))$ for every $k \geq 0$.
    
  The proof for part 2 is similar.  \qed
\end{proof}

\newcommand{\lemStrongLivenessWithFiniteDomains}{
  Let $S$ be a labelled transition system, and $\varphi_1, \ldots \varphi_n$ be first-order predicates.
  Assume that $S \models \square \lozenge \left( \varphi_1 \lor \ldots \lor \varphi_n \right) $.
  There exists a number $i$ such that $1 \leq i \leq n$ and $S \models \square \lozenge  \varphi_i $.
}


\begin{lemma} \label{lem:StrongLivenessWithFiniteDomains}
\lemStrongLivenessWithFiniteDomains
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:StrongLivenessWithFiniteDomains} by contradiction.
  Assume that $S \not\models \square \lozenge \varphi_i$ for every $i$. 
  It follows that $S \models \lozenge \square \lnot \varphi_i$ for every $i$.
  Let $\pi = \sigma_0 \sigma_1 \ldots$ be an arbitrary path of $S$.
  It follow that $\exists t_i \colon t_i \geq 0 \land \big( \forall t \colon t \geq t_i \Rightarrow \sigma_t \models \lnot \varphi_i \big)$ for every $1 \leq i \leq n$.
  Let $T = \mathop{\mathit{MAX}} \left\{t_1, \ldots , t_n \right\}$.
  It follows that $\forall t \colon t \geq T \Rightarrow \sigma_t \models \lnot \varphi_i $ for every $1 \leq i \leq n$.
  It implies that $\exists T \colon T \geq 0 \land \big( \forall t \colon t \geq T \Rightarrow \sigma_t \models \bigwedge_{1 \leq i \leq n} \lnot \varphi_i \big)$. 
  In other words, we have $S \not\models \square \lozenge \left( \varphi_1 \lor \ldots \lor \varphi_n \right)$.
  Contradiction. \qed
\end{proof}

\newcommand{\corNCutoffInStrongLiveness}{
  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
  Let $F(p, q)$ be a local read formula with free variables $p, q$. 
  It follows $\sys{N} \models \lozenge \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q) $ if and only if $\sys{2} \models \lozenge \square \forall p, q \in \{p^2_1, p^2_2 \} \colon  F(p, q) $.
}

\begin{corollary} \label{cor:NCutoffInStrongLiveness}
\corNCutoffInStrongLiveness
\end{corollary}

\begin{proof} We prove both directions by contradiction. 
  To keep the presentation simple, we use two notations  $G_N \triangleq \sys{N} \models \lozenge \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q)$ and $G_2 \triangleq \sys{2} \models \lozenge \square \forall p, q \in \{p^2_1,  p^2_2 \} \colon  F(p, q)$ in the following proofs.
  \begin{enumerate}
  \item Assume that $\sys{N} \models G_N $ but $\sys{2} \not\models G_2 $.
  We have
  \begin{align*}
    \sys{2} \not\models G_2
  \, \Leftrightarrow \,  & \sys{2} \not\models \lozenge \square \bigwedge_{p, q \in \{p^2_1, p^2_2 \}}   F(p, q)  \\
  \, \Leftrightarrow \,    & \sys{2} \models  \square \lozenge \bigvee_{p, q \in \{p_1, p_2 \}} \lnot F(p, q)
  \end{align*}
  
 
  Hence, there exists $p^2_0, q^2_0 \in \left\{p^2_1, p^2_2\right\}$ such that $
  \sys{2} \models \square \lozenge \lnot F(p^2_0, q^2_0)$ by Lemma \ref{lem:StrongLivenessWithFiniteDomains}.
  By Theorem \ref{thm:EquivLocalRead}, it follows $\sys{N} \models \square \lozenge \lnot F(p^N_0, q^N_0)$.
  Contradiction.
  
  \item  Assume that  $\sys{2} \models G_2 $ but $\sys{N} \lnot\models G_N$. 
  We have
  \begin{align*}
  \sys{N} \not\models G_N
  \, \Leftrightarrow \,  & \sys{N} \not\models \lozenge \square \bigwedge_{p, q \in \{p^N_1, \ldots, p^N_N \}}   F(p, q)  \\
  \, \Leftrightarrow \,    & \sys{N} \models  \square \lozenge \bigvee_{p, q \in \{p^N_1, \ldots, p^N_N \}} \lnot F(p, q)
  \end{align*}
  By Lemma \ref{lem:StrongLivenessWithFiniteDomains}, there exists $p^N_0, q^N_0 \in \left\{p^N_1, \ldots, p^N_N\right\}$ such that $
  \sys{N} \models \square \lozenge \lnot F(p^N_0, q^N_0)$ .
  By Theorem \ref{thm:EquivLocalRead}, there exists $p^2_0, q^2_0 \in \left\{p^2_1,  p^2_2\right\}$  such that $
  \sys{2} \models \square \lozenge \lnot F(p^2_0, q^2_0)$. 
  Contradiction.
  \end{enumerate}
  Therefore, Corollary \ref{cor:NCutoffInStrongLiveness} is correct. \qed
\end{proof}

\newcommand{\corNCutoffInSafety}{
  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
  Let $F(p, q)$ be a local read formula with free variables $p, q$. 
  It follows $\sys{N} \models  \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q) $ if and only if $\sys{2} \models  \square \forall p, q \in \{p^2_1, p^2_2 \} \colon  F(p, q) $.
}

\begin{corollary} \label{cor:NCutoffInSafety}
  \corNCutoffInSafety
\end{corollary}

\begin{proof}
It immediately follows by Corollary \ref{cor:NCutoffInStrongLiveness}. \qed
\end{proof}

\begin{remark}
By Corollaries \ref{cor:NCutoffInStrongLiveness} and \ref{cor:NCutoffInSafety}, the problem of checking many useful properties in the form of $\lozenge \square \forall p, q \colon F(p, q)$ or $ \square \forall p, q \colon F(p, q)$ for~\idsep{} algorithms of all sizes  can be reduced to checking them on instances with two processes where $F(p,q)$ is a formula based on local read atomic predicate.
In other words, such properties of~\idsep{} algorithms have a cutoff of 2.
\end{remark}

%To prove the trace equivalence of $S_{1..N}(\Delta, \Phi)$ and $S_{1, 2}(\Delta, \Phi)$, we first define two techniques for path constructions called ID--projection and ``ID--refillment''.
%Lemmas \ref{lem:IDsProj} and \ref{lem:IDsRefill} shows that finite execution paths constructed with these techniques are legal ones in corresponding system instances.
%Such results are extended for infinite paths in Lemmas  \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}
%
%\subsection{Path constructions}
%
%\begin{definition}
%Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ and $\pi^2 = \gconf{0}^2 \gconf{1}^2 \ldots$ be arbitrary infinite execution paths of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$, respectively.
%Path $\pi^2$  is called a \emph{\proj{k}} of path $\pi^N$ if the following property hold:
%
%\begin{enumerate}
%  \item The global stabilization time of two paths are the same.
%    
%  \item For every $i \in \{p_1, p_2\}$, it follows $\gconf{k}^N(\gpc[p_i]) = \gconf{k}^2(\gpc[p_i])$.
%  
%  \item For every $i, j \in \{1, 2\}$, it follows $\gconf{k}^N(\buf{p_i}{p_j}) = \gconf{k}^2(\buf{p_i}{p_j})$.
%  
%%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if process $p_i^N$ receives a set of messages $\mathit{Msgs}$ in state $s^N_k$, then process $p_i^2$ receives a set of messages $\{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ in state $s^2_k$. \footnote{TODO: Override notations here since $m$ is used for different messages in different system instances.}
%%  
%%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ and $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ are the same.
%%  
%%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
%%  
%%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^N$ crashes at time point $k$, then process $p_i^2$ also crashes at time point $k$.
%\end{enumerate}
%
%\end{definition}
%
%
%\newcommand{\lemIDsProj}{
%Let $\pi^N = s_0^N \ldots  s_\ell^N$ be an arbitrary finite execution path of $S_{1..N}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%There exists a finite path $\pi^2 = s^2_0 \ldots s^2_\ell$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an $\ell$--finite ID--projection path of $\pi^N$.
%}
%
%\begin{lemma} \label{lem:IDsProj}
%\lemIDsProj
%\end{lemma}
%
%\begin{proof}
%  It is easy to see that the first constraint about the stabilization time is satisfied by the definition of those system instances. 
%  In the following, we present how to construct an $\ell$--finite ID--projection path of $\pi^N$, and explain how other constraints are satisfied.
%  The construction is based on the induction on the length $\ell$ of an execution path. 
%  
%  \begin{itemize}
%  \item \emph{Base case $\ell = 0$}. In the base case, path $\pi^N$ has only the initial state. 
%  Lemma \ref{lem:IDsProj} is correct because it is safe to set the initial state of processes and message buffers in $S_{1..2}(\Delta, \Phi)$ such that for every $i, j \in \{1, 2\}$, for every local variable $X$, we have $s_0^N(p_i, X[p_j]) = s_0^2(p_i, X[p_j])$ and $s_0^N(\mathit{msgBuf}^N[i, j]) = s_0^2(\mathit{msgBuf}^N[i, j])$.
%  
%  \item Assume that Lemma \ref{lem:IDsProj} is correct for the case $\ell_0 \geq 0$. We prove the case $\ell_0 + 1$. By the induction hypothesis, there exists a finite path $\rho$ in $S_{1..2}(\Delta, \Phi)$ such that $\rho$ is an $\ell_0$--finite ID--projection path for the prefix $s_0^N \ldots s_{\ell_0}^N$ of $\pi^N$. We will show that we can obtain $\pi^2$ by extending $\rho$ with a reachable state $s^2_{\ell}$. Here (and now) we present only the most complicated case where both $p_1$ and $p_2$ are still correct at time point $\ell$. For other cases where crashes happen, the proof is much simpler. \footnote{TODO: Provide some arguments for cases with crashes.} The construction of $s^2_\ell$ where processes $p^2_1$ and $p^2_2$ are still correct is given below.
%  
%  \begin{enumerate}
%      \item Both processes $\pi^N_i$  and $\pi^2_i$ executes the same action on time point $\ell$ for every $i \in \{1, 2\}$. Notice that the action of $\pi^2_i$ is enable because of the induction hypothesis. As a result, the constraint $\Phi$ still holds in $\pi^2$ until $\ell$. (If not, the constraint $\Phi$ does not hold in the interval $[\ell - \Delta, \ell]$ in the execution path $\pi^N$. Contradiction) Therefore, the extension of $\rho$ in this way constructs a legal finite path which satisfies the second constraint.
%      
%      \item In the Send round in global tick $\ell$, it is easy that if message $m$ has been added to message bufer $\mathit{msgBuf}^N[i, j]$ for every $1 \leq i, j \leq 2$, then a corresponding message $m$ has been also added to message bufer $\mathit{msgBuf}^2[i, j]$. 
%      By the induction hypothesis, it follows that until now message buffers $\mathit{msgBuf}^2[i, j]$ and $\mathit{msgBuf}^N[i, j]$ are the same for every $1 \leq i, j \leq 2$.
%      Because our computational model does not allow ``send'' processes to receive any messages and not to join later rounds, we have that 
%T      \begin{align*}
%       s^N_\ell(p_i, X[p_j]) & = f(\{\}, s^N_{\ell_0}X_1[p_j], \ldots, , s^N_{\ell_0}X_m[p_j]) \text{, and } \\ 
%       s^2_\ell(p_i, X[p_j]) & = f(\{\}, s^2_{\ell_0}X_1[p_j], \ldots, , s^2_{\ell_0}X_m[p_j])
%      \end{align*}
%      for every local variable $X$. Due to the induction hypothesis, we have that $s^N_{\ell_0}X_k[p_j] = s^2_{\ell_0}X_k[p_j]$ for every $k$. It follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$.
%      
%      \item In the Receive round, if message $m$ from process $p^N_j$ has been delivered to process $p^N_i$ for every $1 \leq i, j \leq 2$, then either message $m$ was already in $\mathit{msgBuf}^N[j, i]$ in $\ell_0$ or message $m$ has been added to $\mathit{msgBuf}^N[j, i]$ in the last Send round.
%      In the first case, by induction hypothesis, it follows that $m$ was already in $\mathit{msgBuf}^2[j, i]$  in $\ell_0$. In the later case, by arguments in the second point, it follows that $m$ has been added in $\mathit{msgBuf}^2[j, i]$  in the last Send round.
%      Therefore, it is possible for process $p^2_i$ to receive message $m$ in this Receive round.
%      In other words, if process $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_\ell$, then it is safe to deliver a set of messages $\mathit{Msgs}^2 = \{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ to process $p_i^2$ in state $s^2_\ell$. 
%      Therefore, we can construct $\pi^2$ such that the third constraint holds in $\pi^2$.
%      Because processes $p^N_i$ and $p^2_i$ have received the same set of messages in this round, and message buffers $\mathit{msgBuf}^N[i, j]$ and $\mathit{msgBuf}^2[i, j]$ are the same for every $1 \leq i, j \leq 2$ before entering this round, such message buffers are still the same after this round.
%      Moreover, by similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is a ``Receive'' process, and $X$ is a local variable.
%      
%      \item In the Internal Computation round, since (i) no messages are added to any message buffer and (ii) no messages are delivered, the second and third constraints obviously hold.
%      By similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is an ``Internal Computation'' process, $1 \leq i, j \leq 2$, and $X$ is a local variable.
%     
%      \item By the merge of three round, it follows that constraints 2--6 holds by the construction of $\pi^2$.
%  \end{enumerate}
%  Therefore, Lemma \ref{lem:IDsProj} is correct in case of $\ell$. \footnote{The organization of the definition and proof of Lemma \ref{lem:IDsProj} seems a bit difficult to follow. Perhaps we should split it into smaller trunks.} \qed
%  \end{itemize}
%\end{proof}
%
%\begin{definition}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%  Let $\pi^2 = s_0^2 \ldots s_\ell^2$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%  A finite execution path $\pi^N = s_0^N \ldots s_\ell^N$ is called a \emph{$\ell$--finite ``ID--refillment'' path} of $\pi^2$ if the followings hold:
%  
%  \begin{itemize}
%    \item The stabilization  time of two paths are the same.
%    
%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ executes an operator $\mathit{Op}$ in state $s^2_k$, then process $p_i^N$ executes the same operator $\mathit{Op}$ in state $s^N_k$.
%    
%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if processes $p_i^2$ receives messages $\mathit{Msgs}^2$ in state $s^2_k$, then processes $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_k$ such that
%    \[
%    \mathit{Msgs}^N = \mathit{Msgs}^2 \cup \{ m \mid m \in \mathit{msgBuf}[j][i] \land j \in 3..N \}
%    \]
%    
%    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ and $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ are the same.
%    
%    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
%    
%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ crashes at time point $k$, then process $p_i^N$ also crashes at time point $k$.
%    
%    \item For every $j \in 3..N$, process $p_j^N$ never crashes.
%    
%    \item For every $j \in 3..N$, process $p_j^N$ executes the operator $\mathit{Send}$ in state $s^N_0$.
%    
%    \item For every $j \in 3..N$,  process $p_j^N$ takes a transition in every global tick.
%    
%    
%    \item For every $0 \leq k \leq \ell$, for every $j \in 3..N$, if process $p_j^N$ executes the operator $\mathit{Receive(j)}$ in state $s^N_k$, then every message which was sent to process $j^N$ and but not received will be delivered to process $p_j^N$ in state $s^N_k$.
%    
%  \end{itemize}
%  
%\end{definition}
%
%
%\newcommand{\lemIDsRefill}{
%Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%There exists a finite path $\pi^N = s^N_0 \ldots s^N_\ell$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an $\ell$--finite ``ID--refillment'' path of $\pi^2$.
%}
%
%\begin{lemma} \label{lem:IDsRefill}
%\lemIDsRefill
%\end{lemma}
%
%\begin{proof}
%  The proof of Lemma \ref{lem:IDsRefill} is by the induction on the length $\ell$ of the execution path, and by similar arguments in the proof of Lemma \ref{lem:IDsProj} \qed
%\end{proof}
%
%\begin{definition}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary infinite execution path of $S_{1..N}(\Delta, \Phi)$.
%  An infinite execution path $\pi^2 = s_0^2 s_1^2 \ldots$ is called an \emph{infinite ID--projection path} of $\pi^N$ if for every number $\ell \geq 0$, its prefix $\pi^2 = s_0^2 \ldots s_\ell^2$ is an $\ell$--finite ID--projection path of $\pi^N$.
%\end{definition}
%
%
%\newcommand{\lemIDsProjInf}{
%  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary legal execution path of $S_{1..N}(\Delta, \Phi)$.
%  There exists an infinite path $\pi^2 = s^2_0 s^2_1 \ldots$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an infinite ID--projection path of $\pi^N$.
%}
%
%\begin{lemma} \label{lem:IDsProjInf}
%  \lemIDsProjInf
%\end{lemma}
%
%\begin{proof}
%  We prove Lemma \ref{lem:IDsProjInf} by contradiction.
%  Assume that no infinite path in $S_{1..2}(\Delta, \Phi)$ is an infinite ID--projection path of $\pi^N$.
%  Hence, there exists a number $\ell \geq 0$ such that the prefix $s_0^N \ldots s_\ell^N$ has no $\ell$--finite ID--projection path. in $S_{1..2}(\Delta, \Phi)$. 
%  Contradiction. \qed
%\end{proof}
%
%
%\begin{definition}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..2}(\Delta, \Phi)$  and $S_{1..N}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary infinite execution path of $S_{1..2}(\Delta, \Phi)$.
%  An infinite execution path $\pi^N = s_0^N s_1^N \ldots$ is called an \emph{infinite ``ID--refillment'' path} of $\pi^2$ if for every number $\ell \geq 0$, its prefix $\pi^N = s_0^N \ldots s_\ell^N$ is an $\ell$--finite ``ID--refillment'' path of $\pi^2$.
%\end{definition}
%
%
%\newcommand{\lemIDsRefillInf}{
%  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary legal execution path of $S_{1..2}(\Delta, \Phi)$.
%  There exists an infinite path $\pi^N = s^N_0 s^N_1 \ldots$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an infinite ``ID--refillment'' path of $\pi^2$.
%}
%
%\begin{lemma} \label{lem:IDsRefillInf}
%  \lemIDsRefillInf
%\end{lemma}
%
%\begin{proof}
%  By applying similar arguments in the proof of Lemma \ref{lem:IDsProjInf}.
%  \qed
%\end{proof}
%
%\subsection{A cutoff of the number of processes}
%
%From now on, the notation $\mathit{comp}(p_i, X, p_j, \mathit{val})$ denotes an atomic predicate  which means the local variable $X[p_j]$ of process $p_i$ has the value $\mathit{val}$. 
%
%Moreover the notation $\mathit{comp}(\mathit{msgBuf}[i, j], \mathit{val})$ denotes an atomic predicate  which means the message buff $\mathit{msgBuf}[i, j]$  has the value $\mathit{val}$. 
%Such predicates are called ``var--comp'' and ``buffer--comp'', respectively.
%
%\begin{lemma}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``var--comp'' predicate whose indexes are 1 and 2.
%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
%\end{lemma}
%
%\begin{proof}
%  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
%\end{proof}
%
%\begin{lemma}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``buffer--comp'' predicate whose indexes are 1 and 2.
%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
%\end{lemma}
%
%\begin{proof}
%  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
%\end{proof}
%
%
%\begin{theorem} \label{thm:cutoff}
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathcal{P}$ be a predicate built on ``var--comp'' and ``buffer--comp'' predicates whose indexes are 1 and 2.
%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathcal{P}$.
%\end{theorem}
%
%\begin{proof}
%  We prove Theorem \ref{thm:cutoff} by induction on the structure of predicate $\mathcal{P}$. \qed
%\end{proof}
%
%%If $\textit{var}$ is one dimensional array, we override the notation by writing $\assgn{\textit{var}}{\{id_1\}}{\textit{val}}$.
%%Such predicates are called ``assignment'' ones.



==> netys20/dls.tex <==
\subsubsection{Paramters, variables, and assumptions}
A fault-tolerant algorithm $\mathcal{A}$ in the DSL model~\cite{DLS88} is \emph{parameterized} in the parameters $N, T, F, \Delta, \Phi$ and $t_0$ where 
\begin{itemize}[noitemsep]
\item Parameters $N$ and $T$ are the number of processes, and the maximum number of faulty processes. 
Parameter $F$ refers to the actual number of faulty processes during an execution path of an instance of the algorithm $\mathcal{A}$.

\item Parameter $\Delta$ is used to describe a constraint on message delay.
Parameter $\Phi$ is used to describe a constraint on relative process speed. 
From now on, such constraints are called $\Delta$ and $\Phi$, respectively.
Parameter $t_0$ refers to when constraints $\Delta$ and $\Phi$ hold in an execution path of an instance of the algorithm  $\mathcal{A}$.
These constraints will be formalized with logical formulas later.
\end{itemize}

Moreover, an algorithm $\mathcal{A}$ has following variables and assumptions:
\[
V=\left\{
\begin{array}{lll}
%N, T, F  & \colon \textbf{natural where } 0 \leq T, F \leq N  \\
%\Delta, \Phi, t_0  & \colon \textbf{natural} \\
\gc & \colon \textbf{natural where } 0 \leq \gc  \\
\act   & \colon \textbf{array } [\nid{}] \textbf{ of Boolean}  \\
\buf & \colon \textbf{array } [\nid] [\nid] \textbf{ of } \texttt{Set}(\msg_{ts}) \textbf{ (sets of messages)} \\
x_1 (\textbf{called } \pc)  & \colon \textbf{array } [\nid{}] \textbf{ of } \mathit{BL} = \{ L_S, L_C, L_C, L_F \} \\
x_2 (\textbf{called } \mailbox) & \colon \textbf{array } [\nid] [\nid] \textbf{ of } \texttt{Set}(\msg_{ts}) \\
x_3, \ldots, x_m & \colon \textbf{array } [\nid{}] \textbf{ of arbitrary types } \mathcal{T}_3, \ldots, \mathcal{T}_m 
\end{array}
\right.
\]

\begin{itemize}[noitemsep]

\item There exists a digital global $\gc$ to measure time in natural-number steps.

\item The global variable $\buf[\nid][\nid]$ is a two--dimensional array where $\buf[i, j]$ store all timestamped messages  which were sent from a process $p_i$, but have not been delivered to a process $p_j$ for every $i, j \in \nid$.
We let $\buf[i]$ denote an array $\buf[i][\nid]$ which refers to all message buffers from process $p_i$.


\item The global $\gc$ is used to stamp every message $m$ to record when it was sent.
We let a tuple $m_{ts} \triangleq (m, ts)$ refers to a timestamp version of a message $m$ which is stamped at a time $t$.
By looking at a timestamp and the current value of $\gc$, 
we know how long a message $m$ has been in transit, i.e. $(\gc - m_{ts}[2])$.

\item We let $\msg$ denote a set of messages without timestamps, and $\msg_{ts}$ denote a set of timestamped messages.
The content of a message is unindexed value, and the sender $\mathit{snder}$ and receiver $\mathit{rcver}$ of a message $m$ implicitly refers to indexes of the message buffer where $m$ is stored.




\item\label{const:Hole} Many processes can take a step in one global tick, 
but it is not necessary that a process takes a step in a global tick.
Hence, we assume that there exists a one--dimensional global array $\act[\nid]$ which decides what processes take a step in a current global tick.   

\item Processes are indexed, and correct ones follow a deterministic algorithm. We let $\Proc{\mathit{ID}}$ denote a set of processes whose indexes is the set $\mathit{ID}$, e.g. $\Proc{{\nid}}$.

\item A process $p_i \in \Proc{\nid}$ has $m$ local variables $x_1[i], \ldots, x_m[i]$for some number $m \geq 2$.
The first two variables $x_1[i], x_2[i]$ are special ones, and called $\pc[i]$ and $\mailbox[i]$, respectively. In our paper, these names are changeable.


\item The variable $\pc[i]$ refers to an instruction block which a process $p_i$ will perform when it takes a step.
We assume that there are three normal instruction blocks $L_S, L_R, L_C$ and an exceptional block $L_F$. We let $\mathit{BL} = \{ L_S, L_R, L_C, L_F \}$
If $\pc[i] = L_F$, then a process $p_i$ is fault.


\item The variable $\mailbox[i]$ is a one--dimensional array where $\mailbox[i, j]$ store all messages which a process $p_i$ has received from a process $p_j$ for every $j \in \nid$.

\item Processes communicate to each other by sending and receiving messages by performing instructions $\snd(p_i, m)$ and $\rcv(p_i)$.
However, a process cannot both send and receive messages in one global tick.



\item Intuitively, by executing an instruction $\snd(p_i, m)$, a process $p_i$ will put a message $m$ to every message buffer $\buf[i, j]$ where $j \in \nid$.
Notice that the DLS model supports send--to--one instructions
which allows a process to send a message to another process, 
but we here adopt send instructions to send--to--all.

\item If a process $p_i$ performs an instructions $\rcv(p_i)$, some sets of messages will be removed from message buffers to $p_i$, and added them to $p_i$'s boxes. 
We let $\rcv(p_i)[p_j]$ denote a set of messages which a process $p_i$ has received from a process $p_j$ in the current transition.




%
%\item WE STOP HERE.
%
%\item Every correct process follows the same deterministic algorihthm.
%  
%  \item Parameters $\Delta, \Phi$, and $t_0$ are used to describe  partially synchronous constraints. 
%  These constraints will be introduced with logical formulas later.
%  
%  \item For every pair of processes $p_i, p_j \in \proc$, there exists a message buffer $\buf{p_i}{p_j}$ between them to store messages which were sent by process $p_i$ but have not been delivered to process $p_j$. 
%  The notation $\texttt{Msg}^{p_i}_{p_j}$ refers to a set of possible messages which a process $p_i$ can send to a process $p_j$.
%  There are totally $N^2$ message buffers. 
%  Notice that the message buffers in \cite{DLS88} are in the form of  $\msgbuf{p_i}$ which stores all messages sent to process $p_i$ others but have not delivered for every $p_i \in \proc$.
%  
%
%  
%  %  \item Every process has its own local clock which also measures time in contiguous discrete integer-number steps. 
%  
%  \item Processes communicate to each other by sending and receiving messages with instructions $\sop{p_i}{m}{p_j}$ and $\rop{p_i}$ where $\sop{p_i}{m}{p_j}$ is that a process $p_i$ sends a message $m$ to a process $p_j$, and $\rop{p_i}$ is that some sets of messages are removed from $p_i$'s message buffers and delivered the messages to $p_i$. 
%  
%  \item Every message sent by some process is distinguish in the system viewpoint. 
%  
%  \item A correct process $p$ can perform at most one of instructions $\sop{p_i}{m}{p_j}$ and $\rop{p_i}$ in every local step.
%  
%  \item Every correct process follows a deterministic algorithm with local variables $X_1, \ldots, X_M$ for some number $M \geq 0$, and a variable $\mailbox$ which is indexed by processes' id and used to store all received messages, and a variable \lpc{} which refers to next instruction blocks.
%  Here we assume that the set of instruction blocks is $\isc{} = \left\{ \tsnd{}, \trcv{}, \tcomp{}, \tcrash{} \right\}$, and two blocks $\tsnd{} \text{and } \trcv{}$ can contain instructions for local computation.
%  
%  
%  \item\label{const:Hole} There might be ticks of the global clock when no processes take a step on such ticks.
%  
%  %  \item Faulty process cannot recover.
%
%\item A variable $\gc$ is for a global digital clock which measures time in natural-number steps.
%
%\item A one--dimensional global array $\act$ refers to whether a process takes a step in a current global tick. 
%
%\item A two--dimensional global array $\buf$ refers to message buffers 
%where $\buf[i, j]$ stores in--transit messages from a process $p_i$ to a process $p_j$ for $i, j \in \nid$. 
%Notice that message buffers in \cite{DLS88} are in the form of  $\buf[i]$ 
%which stores all messages sent to process $p_i$ but have not been delivered for $i \in \nid$.
%
%
%\item A one--dimensional local array $\pc$ refers to blocks of instructions 
%which are performs when a process takes a step.
%We assume that there are three instruction blocks $L_S, L_R, L_C$ and an additional special block $L_F$. 
%If $\pc[i] = L_F$ then a process $p_i$ is fault.
%
%
%\item A two--dimensional local array $\mailbox$ refers to mailboxes 
%where $\mailbox[i, j]$ stores all which  a process $p_i$ has received from a process $p_j$ for every $i, j \in \nid$. 
%
%\item Variables $x_1, \ldots, x_m$ are other \emph{local variables} of processes. 
%
%where $N$ is the  number of processes, and $T$ is the maximum number of faulty processes.
%We assume that processes are indexed, and 
%let $\proc$ denote the set of processes where $ID$ is a set of indexes, and $\card{ID} = N$.
\end{itemize}



%These parameters and variables play following roles:
%
%\begin{itemize}[noitemsep]
%  
%  
%\item Parameters $N \text{ and } T$ are in fault-tolerant distributed algorithms 
%where $N$ is the  number of processes, and $T$ is the maximum number of faulty processes.
%We assume that processes are indexed, and 
%let $\proc$ denote the set of processes where $ID$ is a set of indexes, and $\card{ID} = N$.
%
%
%%\item Every process has a unique ID. The set of processes is denoted by $\proc{}$,
%%and it follows that $\card{\proc} = N$.
%
%\item Parameters $\Delta, \Phi$, and $t_0$ are used to describe partially synchronous constraints 
%which will be introduced with logical formulas later.
%
%\item A variable $\gc$ is for a global digital clock which measures time in natural-number steps.
%
%\item A one--dimensional global array $\act$ refers to whether a process takes a step in a current global tick. 
%
%\item A two--dimensional global array $\buf$ refers to message buffers 
%where $\buf[i, j]$ stores in--transit messages from a process $p_i$ to a process $p_j$ for $i, j \in \nid$. 
%Notice that message buffers in \cite{DLS88} are in the form of  $\buf[i]$ 
%which stores all messages sent to process $p_i$ but have not been delivered for $i \in \nid$.
%
%
%\item A one--dimensional local array $\pc$ refers to blocks of instructions 
%which are performs when a process takes a step.
%We assume that there are three instruction blocks $L_S, L_R, L_C$ and an additional special block $L_F$. 
%If $\pc[i] = L_F$ then a process $p_i$ is fault.
%
%
%\item A two--dimensional local array $\mailbox$ refers to mailboxes 
%where $\mailbox[i, j]$ stores all which  a process $p_i$ has received from a process $p_j$ for every $i, j \in \nid$. 
%
%\item Variables $x_1, \ldots, x_m$ are other \emph{local variables} of processes. 
%\end{itemize}
%
%Moreover, the DLS model has following assumptions:
%
%\begin{itemize}[noitemsep]
%
%\item\label{const:Hole} Many processes can take a step in one global tick, 
%but it is not necessary that a process takes a step in a global tick.
%\item A one--dimensional global array $\act$ refers to whether a process takes a step in a current global tick.   
%  
%\item Processes communicate to each other by sending and receiving messages. 
%While the DLS model supports send--to--one instructions
%which allows a process to send a message to another process, 
%we here use send--to--all instructions $\snd(p_i, m)$.
%To receive messages, we apply the same instructions $\rcv(p_i)$ which removes some sets of messages from $p_i$'s message buffers, and added them to $p_i$'s mailboxes. 
%We let $\rcv(p_i)[p_j]$ denote a set of messages from a process $p_j$ which have been delivered to a process $p_i$.
%
%\item A correct process $p_i$ cannot perform both instructions $\snd(p_i, m)$ and $\rcv(p_i)$ one global tick.
%
%\item The global $\gc$ is used to stamp every message $m$ to record when it is sent.
%We let $m.\stamp$ denote the timestamp of a message $m$.
%Therefore, by looking at its natural--numbered timestamp and the current value of $\gc$, 
%we know how long a message $m$ has been in transit, i.e. $(\gc - m.\stamp)$.
%Morever, we let $\msg^i_j$ denote a set of messages with timestamps which a process $p_i$ can send to a process $p_j$.
%
%\item Every correct process follows the same deterministic algorihthm.
%
%
%%\item Every correct process follows a deterministic algorithm with local variables $X_1, \ldots, X_M$ for some number $M \geq 0$, and a variable $\mailbox$ which is indexed by processes' id and used to store all received messages, and a variable \lpc{} which refers to next instruction blocks.
%%Here we assume that the set of instruction blocks is $\isc{} = \left\{ \tsnd{}, \trcv{}, \tcomp{}, \tcrash{} \right\}$, and two blocks $\tsnd{} \text{and } \trcv{}$ can contain instructions for local computation.
%
%\end{itemize}


\subsubsection{Partially synchronous algorithms as transition systems}
Let $\sys{N}$ be an instance of $\mathcal{A}$ whose indexes are $\nid$.
A \emph{global configuration} $\conf$ of the system provides an interpretation of all variables, assigning to each variable $v \in V$ a value $\conf(v)$ in its domain. 
A \emph{local configuration} of a process $p_i$ provides an interpretation of a tuple $\left( pc[i], box[i], x_3[i], \ldots, x_m[i] \right)$ for every $i \in \nid$.
We let $\local(\conf, i)$ denote a local configuration of a process $p_i$ constructed from a global configuration $\conf$.
In the following, we present how to model processes and an instance $\sys{N}$ as a transition system. 

\emph{Process template.} Since every correct process follows a deterministic algorithm, we assume that they are instances of a template $U \triangleq \left(\pstates{U}, \xrightarrow{U}, \pinitstates{U} \right)$ 
where $\pstates{U} % \triangleq \mathit{BL} \times \texttt{Set}(\msg_{ts})^N \times \mathcal{T}_3 \times \ldots \times \mathcal{T}_m
$ is a set of process configurations, and $\xrightarrow{U}$ is a transition relation, and $I_p \subseteq \Sigma_p$ is a set of initial  configurations. 
Assume that the process template has $m$ variables with types called $x^U_1 \colon \mathit{BL}, x^U_2 \colon \texttt{Set}(\msg_{ts})^N, x^U_3 \colon \mathcal{T}_3, \ldots, x^U_m \colon \mathcal{T}_m$, where $\mathcal{T}_3$ is a type whose values are unindexed.
A process configuration is an interpretation of a tuple $\left( x^U_1, \ldots, x^U_m \right)$, assigning to each variable  a value  in its type. 
The relation $\xrightarrow{U}$ is defined based on a relation $\xrightarrow{U, \tau}$ for stuttering steps, and two functions $\localnext, \localfault$  such that
\begin{itemize}[noitemsep]
  \item Function $\localnext \colon  \pstates{U}  \times \texttt{Set}(\msg_{ts})^N \rightarrow \pstates{U} \times \msg$ takes as input a process configuration, $N$ sets $S_1, \ldots, S_N$ of timestamped messages which refers to new delivered messages, and produces as output a next process configuration, and a set $T$ of one message without timestamps which refers to a new sent message.
  Because a process can send at most one message to all in a transition, we have $\card{T} \leq 1$.
  Moreover, since a process cannot send and receive messages in a step, we require that $ S = \emptyset \lor T = \emptyset$. 
  We say $\rho_p \translocalnext{U} \rho_p^{\prime}$  where $\rho_p, \rho_p^{\prime} \in \pstates{U}$ if and only if there exists a set of messages $S \subseteq \msg_{ts}$, a number $t \geq 0$, a message $m \in \msg$ such that $(\rho_p^{\prime}, m) = \localnext(\rho_p, S, t)$.
  Notice that a produced message $m$ is not timestamped since a process cannot access the global $\gc$.
  
  \item Function $\localfault \colon \pstates{U} \rightarrow \pstates{U}$ takes as input a process configuration, and produces as output a faulty process configuration. 
  Formally, for every pair of configurations $\rho, \rho^{\prime} \in \pstates{U}$, we have that 
  $ \rho^{\prime} = \localfault (\rho)$ if and only if $\rho^{\prime}(\pc) = L_F$, and other variables are the same, $ \rho^{\prime}(x^U_k) = \rho(x^U_k)$ for every $2 \leq k \leq m$.
  We say $\rho \translocalfault{U} \rho^{\prime}$ if and only if $\rho^{\prime} = \localfault(\rho)$.
\end{itemize}

For every pair of local configurations $\rho_p, \rho^{\prime} \in \pstates{U}$, we have $\rho \xrightarrow{U} \rho^{\prime}$ if and only if one of following constraints holds: $\rho \localstuttering{U} \rho^{\prime}$, or $\rho \translocalfault{U} \rho^{\prime}$, or $\rho \translocalnext{U} \rho^{\prime}$.
From now on, we let $U_i = \left( \pstates{i}, \xrightarrow{i}, I_i \right)$ denote an instance for a process $p_i$.
Instanced variables are simply written as $x_1[i]$ , $x_2$ , $x_3[i] , \ldots, x_m[i]$,
and two first variables $x_1[i], x_2[2]$ are also called $\pc[i], \buf[i]$, respectively.
%in a global configuration $\conf$ is defined as a ($m+2$)--ary tuple $\left[ \conf(\pc[i]), \conf(\mailbox[i], \conf(x_1[i]), \ldots, \conf(x_m[i]))\right]$.
%We let $\pcreate(i, \conf)$ denote a local configuration constructed from a global configuration $\conf$ and a process index $i$.
Moreover, it follows from the definition that $N$ processes instanced from the template $U$ are isomorphic.

\emph{Global transition system.}
An instance $\sys{N}$ can be model as a transition system $M_N = \left( \gstates{N}, \leadsto, \ginitstates{N} \right)$
where $\gstates{N}$ denote a set of global configurations, and $\leadsto$ is a transition relation in a global tick, and $\ginitstates{N} \subseteq \gstates{N}$ be a set of initial configurations, and $N$ processes are instances of the process template $U$.
%
%Before defining a transition relation between configurations in $\sys{N}$, we would like to discuss a local transition system of processes.
%Since every correct process follows the same deterministic algorithm, we assume that
%they are constructed from a template process \emph{Temp} which is a labeled transition system $\left( \Sigma^i, \rightarrow, \mathit{Id}, \Sigma^i_0 \right)$ where
%\begin{itemize}
%\item $\Sigma^i$ is a set of configurations of a process $p_i$ such that
%\[
%\Sigma^i_0 = \{ \left( \conf(\pc[i]), \conf(\mailbox[i]), \conf(x_1[i]), \ldots, \conf(x_m[i]) \right) \colon \conf \in \Sigma \}
%\]
%\end{itemize}
%
%We let $\conf_1 \leadsto \conf_2$ denote a transition from a state $\conf_1$ to $\conf_2$ at some global tick.
To provide the semantics of the relation $\leadsto$, we first assume that 
every global tick contains four ordered subrounds $\sched{}, \snd{}, \rcv{}$ and $\comp{}$,
and definite a transition relation in every subround.
We let $\xrightarrow{\texttt{Name}}$ denote a transition in a subround $\texttt{Name}$.
Moreover, the transtion relation $\leadsto$ is called a \emph{observance} relation, and other relations $\xrightarrow{\texttt{Name}}$ is called \emph{internal} ones.
The semantics of the relation $\leadsto$ is defined based on the semantics of relations $\xrightarrow{\texttt{Name}}$ which are given in the following.
%Let Σ denote the set of all states
%over V . An assertion over V is a first order formula over V . A state s satisfies an
%assertion φ, denoted s |= φ, if φ evaluates to T by assigning s[v] to every variable
%v appearing in φ. We say that s is a φ-state if s |= φ.

%The computational model in \cite{DLS88} has following assumptions:
%\begin{itemize}
%  \item $N, T$, and $F$ are parameters in fault-tolerant distributed algorithms.
%  
%  \item Every process has a unique ID. The set of processes is denoted by $\proc{}$,
%  and it follows that $\card{\proc} = N$.
%  
%  \item Parameters $\Delta, \Phi$, and $t_0$ are used to describe  partially synchronous constraints. 
%  These constraints will be introduced with logical formulas later.
%  
%  \item For every pair of processes $p_i, p_j \in \proc$, there exists a message buffer $\buf{p_i}{p_j}$ between them to store messages which were sent by process $p_i$ but have not been delivered to process $p_j$. 
%  The notation $\texttt{Msg}^{p_i}_{p_j}$ refers to a set of possible messages which a process $p_i$ can send to a process $p_j$.
%  There are totally $N^2$ message buffers. 
%  Notice that the message buffers in \cite{DLS88} are in the form of  $\msgbuf{p_i}$ which stores all messages sent to process $p_i$ others but have not delivered for every $p_i \in \proc$.
%  
%  \item There exists a global clock  which measures time in contiguous discrete integer-number steps.
%  
%  %  \item Every process has its own local clock which also measures time in contiguous discrete integer-number steps. 
%  
%  \item Processes communicate to each other by sending and receiving messages with instructions $\sop{p_i}{m}{p_j}$ and $\rop{p_i}$ where $\sop{p_i}{m}{p_j}$ is that a process $p_i$ sends a message $m$ to a process $p_j$, and $\rop{p_i}$ is that some sets of messages are removed from $p_i$'s message buffers and delivered the messages to $p_i$. 
%  
%  \item Every message sent by some process is distinguish in the system viewpoint. 
%  
%  \item A correct process $p$ can perform at most one of instructions $\sop{p_i}{m}{p_j}$ and $\rop{p_i}$ in every local step.
%  
%  \item Every correct process follows a deterministic algorithm with local variables $X_1, \ldots, X_M$ for some number $M \geq 0$, and a variable $\mailbox$ which is indexed by processes' id and used to store all received messages, and a variable \lpc{} which refers to next instruction blocks.
%  Here we assume that the set of instruction blocks is $\isc{} = \left\{ \tsnd{}, \trcv{}, \tcomp{}, \tcrash{} \right\}$, and two blocks $\tsnd{} \text{and } \trcv{}$ can contain instructions for local computation.
%  
%  
%  \item\label{const:Hole} There might be ticks of the global clock when no processes take a step on such ticks.
%  
%  %  \item Faulty process cannot recover.
%\end{itemize}
%\emph{Process update}. Since every correct process follows the same deterministic algorithms, we assume that they are constructed from a template $\mathit{Temp} = \left( S, \ltrans, S_0 \right)$ where $S$ is a set of local configurations, $\ltrans$ is a transition relation, and $S_0$ is initial configurations. A global configuration in $\Sigma$ can be considered as a parallel composition of $N$ instances of $\mathit{Temp}$.

\emph{Subround \sched{}}. For  $ \conf_1, \conf_2 \in \gstates{N}$, we have $\conf \transsched \conf^{\prime}$ if and only if
\begin{align*}
& \: \forall i \in \nid \colon \lnot \conf_1(\pc[i]) \\
\land &     \conf_2(\gc) = \conf_1(\gc) + 1   \\
\land &  \: \forall i \in \nid \colon \pcreate(\conf_1, i) \localstuttering{i}  \pcreate(\conf_2, i)   \lor \pcreate(\conf_1, i) \translocalfault{i} \pcreate(\conf_2, i) \\
\land &  \: \card{ i \in \nid \colon \conf_2(\pi[i])} \leq T \\
\land &  \: \forall i, j \in \nid \colon \conf_1(\buf[i,j]) = \conf_2(\buf[i,j])
\end{align*}
Intuitively, the subround \sched{} requires that every process is inactive in the configuration $\conf_1$.
In the subround \sched{}, the system increases the global $\gc$ by 1,  
and nondeterministically introduces new fault processes such that the number of faults is not greater than $T$, 
and keep the message buffers unchanged,
and nondeterministically decides what processes take a step in a current global tick.
The last action is implicitly done by the constraint on $\act$'s type.

\emph{Subround \snd{}}. For  $ \conf_1, \conf_2 \in \gstates{N}$, we have $\conf_1 \tsnd \conf_2$ if and only if
\begin{align*}
&   \conf_2(\gc) = \conf_1(\gc)    \\
\land &  \: \forall i \in \nid \colon \lnot \CanRun(\conf_1, i, L_S) \Leftrightarrow \SFrozen(\conf_1, \conf_2, i)\\
\land &  \: \forall i \in \nid \colon  \CanRun(\conf_1, i, L_S) \Leftrightarrow \exists m \in \msg \colon \predsnd(\conf_1, \conf_2, i, m) \\
\land &  \: \forall i \in \nid \colon \CanRun(\conf_1, i, L_S) \Rightarrow \lnot \conf_2(\act[i])
\end{align*}
where predicates $\CanRun, \SFrozen, \predsnd$ are defined as followings:
\begin{alignat*}{3}
\CanRun(\conf, i, L)  & \triangleq \; && \conf(\act[i]) \land \left( \conf(\pc[i]) = L  \lor  \FCanRun(\conf, i, L) \right)\\
\SFrozen(\conf_1, \conf_2, i)  & \triangleq \; && \land  \pcreate(\conf_1, i) \localstuttering{i} \pcreate(\conf_2, i)  \\
& && \land  \conf_1(\act[i]) = \conf_2(\act[i])   \\
& && \land \forall j \in \nid \colon \conf_1(\buf[i, j]) = \conf_2(\buf[i, j])   \\
\predsnd(\conf_1, \conf_2, i, m)  & \triangleq \; && \land \forall j \in \nid \colon (m, \conf_2(\gc)) \notin \conf_1(\buf[i, j])    \\
& && \land \forall j \in \nid \colon \conf_2(\buf[i, j]) = \{ (m, \conf_2(\gc) \} \cup \conf_1(\buf[i, j]) \,  \\
& && \land (\pcreate(\conf_2, i), \{m\}) = \localnext(\pcreate(\conf_1, i), \emptyset, \conf_2(\gc))  
\end{alignat*}
and predicate $\FCanRun(\conf, i, L)$ decides whethere an active faulty process $p_i$ can take a step here. 
For example, if faults are only clean crashes, then we always set $\FCanRun(\conf, i, L) = \False$.
Intuitively, the subround \snd{} allows only active processes with the blocks $L_S$ or $L_F$ to take one step. 
When the subround \snd{} finishes, such processes become inactive.



\emph{Subround \rcv{}}. For  $ \conf_1, \conf_2 \in \gstates{N}$, we have $\conf_1 \trcv \conf_2$ if and only if
\begin{align*}
&   \conf_2(\gc) = \conf_1(\gc)    \\
\land &  \: \forall i \in \nid \colon \lnot \CanRun(\conf_1, i, L_R) \Leftrightarrow \RFrozen(\conf_1, \conf_2, i)\\
\land &  \: \forall i \in \nid \colon  \CanRun(\conf_1, i, L_R) \Leftrightarrow \exists S \subseteq \msg \colon \predrcv(\conf_1, \conf_2, i, S) \\
\land &  \: \forall i \in \nid \colon \CanRun(\conf_1, i, L_R) \Rightarrow \lnot \conf_2(\act[i]) 
\end{align*}
where predicates $\RFrozen, \predrcv$ are defined as followings:
\begin{alignat*}{3}
\RFrozen(\conf_1, \conf_2, i)  & \triangleq \; && \land  \pcreate(\conf_1, i) \localstuttering{i} \pcreate(\conf_2, i)  \\
& && \land  \conf_2(\act[i]) \subseteq \conf_1(\act[i])   \\
& && \land \forall j \in \nid \colon \conf_1(\buf[i, j]) = \conf_2(\buf[i, j])  
\end{alignat*}

\begin{align*}
& \predrcv(\conf_1, \conf_2, i, S)   \triangleq \exists  S_1, \ldots, S_N \subseteq \msg \colon \\
& \qquad  \land  S = S_1 \cup \ldots \cup S_N \\
& \qquad \land \forall j \in \nid \colon S_j \subseteq \conf_1(\buf[j, i])  \\
& \qquad \land \forall j \in \nid \colon \conf_2(\buf[j, i]) \cup S_j = \conf_1(\buf[j, i]) \\
& \qquad \land (\pcreate(\conf_2, i), \{m\}) = \localnext(\pcreate(\conf_1, i), S, \conf_2(\gc)) 
%& \qquad \land \forall j \in \nid , m^{\prime} \in \msg \colon m \in \conf_2(\buf[j, i]) \land t_0 \leq \conf_2(\gc) \\
%& \qquad \qquad  \Rightarrow \conf_2(\gc) - m.\stamp < \Delta  
\end{align*}

Intuitively, only active processes with the blocks $L_R$ or $L_F$ can take one step in the subround \rcv{}.
When the subround \rcv{} finishes, such processes become inactive.

\emph{Subround \comp{}}. For  $ \conf_1, \conf_2 \in \gstates{N}$, we have $\conf_1 \tcomp \conf_2$ if and only if
\begin{align*}
&   \conf_2(\gc) = \conf_1(\gc)    \\
\land &  \: \forall i \in \nid \colon  \CanRun(\conf_1, i, L_R) \Leftrightarrow \predcomp(\conf_1, \conf_2, i) \\
\land &  \: \forall i, j \in \nid \colon \lnot  \CanRun(\conf_1, i, L_C) \Leftrightarrow \pcreate(\conf_1, i) \localstuttering{i} \pcreate(\conf_2, i) \\
\land &  \: \forall i, j \in \nid \colon \conf_1(\buf[i, j] = \conf_2(\buf[i, j]) \\
\land &  \: \forall i \in \nid \colon \lnot  \conf_2(\act[i]) \\
\end{align*}
where predicate $\predcomp \triangleq (conf_2(\buf[i, j]), \emptyset) = \localnext(\conf_1(\buf[i, j], \emptyset, \conf_2(\gc))  $.
Intuitively, only active processes with the blocks $L_C$ or $L_F$ can take one step in the subround \rcv{}.
Unlike other subrounds, when the subround \rcv{} finishes, it forces that every process becomes inactive. 
Notice that local computations neither receive messages nor send new messages.

\emph{Observance transition $\leadsto$}.  For $ \conf_1, \conf_2 \in \gstates{N}$, we say $\conf_1 \leadsto \conf_2$ if and only if there exist three configurations $\conf_{\sched}, \conf_{\snd}, \conf_{\rcv} \in \gstates{N}$ such that
\[
\conf_1 \transsched \conf_{\sched} \transsnd \conf_{\snd} \transrcv \conf_{\rcv} \transcomp \conf_2
\]

%To keep the representation simple, we discuss constraints for other subrounds together since they share many constraints. 
%\begin{itemize}
%\item  The global $\gc$ is unchanged in these subrounds \snd{}, \rcv{}, and \comp{}. For every $\texttt{act} \in \{ \snd, \rcv, \tcomp \}$, for every $\conf_1, \conf_2 \in \states$,  we have that
%$ \conf_1 \xrightarrow{\texttt{act}} \conf_2 \Rightarrow \conf_1(\gc) =  \conf_2(\gc) $.
%
%\item No messages are sent in the subrounds \rcv{} and \comp{}. For every $\texttt{act} \in \{ \rcv, \tcomp \}$, for every $\conf_1, \conf_2 \in \states$,  we have that
%\[ \conf_1 \xrightarrow{\texttt{act}} \conf_2 \Rightarrow \forall i, j \in  \nid \, \conf_2(\buf[i, j]) \subseteq \conf_1(\buf[i, j]) \]
%
%\item No messages are delivered in the subrounds \snd{} and \comp{}. For every $\texttt{act} \in \{ \rcv, \tcomp \}$, for every $\conf_1, \conf_2 \in \states$,  we have that
%\[ \conf_1 \xrightarrow{\texttt{act}} \conf_2 \Rightarrow \forall i, j \in \nid \, \conf_1(\buf[i, j]) \subseteq \conf_2(\buf[i, j])   \]
%
%$\sop{p}{m}{q}$: The execution of this instruction in a~\snd{} configuration $\confsnd{t}$ can be interpreted with a following formula
%\begin{align*}
%& \,   m \notin \confsched{t} \left( \buf{p_i}{p_j}\right)   \\
%\land &  \,  \confsnd{t} \left( \buf{p_i}{p_j}\right) = \left\{ m \right\} \cup \confsched{t} \left( \buf{p_i}{p_j}\right) 
%%  \land & \,  \forall p^{\prime} \ldotp p^{\prime} \neq p_j \Rightarrow \confsnd{t} \left( \buf{p_i}{p^{\prime}}\right) = \confsched{t} \left( \buf{p_i}{p^{\prime}}\right) )
%\end{align*}
%In other subrounds, no process sends any message.
%\[
%\confsched{t}.\sop{p}{m}{q} = \confrcv{t}.\sop{p}{m}{q} = \sigma_{t}.\sop{p}{m}{q} =  \False 
%\]
%
%\item Every correct process can take at most one step in a global tick. For every $\texttt{act} \in \{ \snd, \rcv, \tcomp \}$, for every $\conf_1, \conf_2 \in \states$,  we have that
%
%\begin{align*}
%\forall t \, \forall p_i \ldotp 
%& \left(\confsched{t} \left( \gpc \left[ p_i \right] \right) \land \confsched{t}(  p_i  ).\lpc = \tsnd{} \right) \\
%& \quad  \Rightarrow  \left(\confsnd{t} \left( p_i \right) = \confrcv{t} \left( p_i \right) = \gconf{t} \left( p_i \right) \land \lnot \confsnd{t} ( \gpc[p_i] ) \right) \\
%\forall t \, \forall p_i \ldotp 
%& \left(\confsnd{t} ( \gpc \left[ p_i \right] ) \land \confsnd{t} (  p_i  ).\lpc = \trcv{} \right) \\
%& \quad \Rightarrow \left( \confsched{t} (p_i ) = \confsnd{t} ( p_i )  \land \confrcv{t} ( p_i ) = \gconf{t} ( p_i ) \land \lnot \confrcv{t} ( \gpc [p_i] ) \right) \\
%\forall t \, \forall p_i \ldotp 
%& \left( \confrcv{t} ( \gpc [ p_i ] ) \land \confrcv{t}(  p_i  ).\lpc = \tcomp{} 
%\right) \\
%& \quad \Rightarrow \left( \confsched{t} (p_i) = \confsnd{t} ( p_i ) =  \confrcv{t} ( p_i ) \land \lnot \gconf{t}(\gpc[p_i]) \right) \\
%\forall t \, \forall p_i \ldotp 
%& \lnot \confsched{t} ( \gpc [ p_i ] ) \\
%& \quad   \Rightarrow  \left(\gconf{t-1} ( p_i )  = \confsched{t} (p_i) = \confsnd{t} ( p_i ) =  \confrcv{t} ( p_i ) = \gconf{t} ( p_i ) \right)
%\end{align*}
%
%\end{itemize}
%
%\begin{align*}
%&   \conf_2(\gc) = \conf_1(\gc)    \\
%\land &  \: \forall i \in \nid \: \forall v \in \{\pc, \mailbox, x_1, \ldots, x_m \} \colon  \\
%& \qquad \left(\conf_1(\act[i]) = \False \lor \conf_1(\pc[i]) \neq L_S \right)  \Rightarrow \conf_2(v[i]) = \conf_1(v[i])  \\
%\land &  \: \forall i \in \nid \colon  (\conf_1(\pc[i]) = L_S \land \conf_1(\act[i]) = \True) \Rightarrow \\
% & \qquad (\conf_2(\pc[i]) = L_R \land \conf_1(\act[i]) = \False) \\
%\land &  \: \forall i \in \nid \colon  (\conf_1(\pc[i]) = L_S \land \conf_1(\act[i]) = \True) \Rightarrow \\ 
%  & \qquad \exists m \in \msg \forall j \in \nid \colon \conf_2(\buf[i, j]) = \{ m \} \cup \conf_1(\buf[i, j]) \\
%\land &  \: \forall i, j \in \nid \colon  (\conf_1(\pc[i]) = L_S \land \conf_1(\act[i]) = \True) \Rightarrow \\ 
%& \qquad \exists m \in \msg \forall j \in \nid \colon \conf_2(\buf[i, j]) = \{ m \} \cup \conf_1(\buf[i, j])  
%\end{align*}


%\emph{Subrounds and intermediate global states.} Since processes can execute different kinds of actions in one global step, we assume that
%\begin{enumerate}[label=(\roman*)]
%  \item Each global step consists of four ordered subrounds: \sched{}, \snd{}, \rcv{}, and~\comp{} where $\cop{}$ contains only local computations based on messages which were received in previous steps. 
%  \item Process configurations are unchanged in the subround \sched{}.
%  \item Message buffers are unchanged in two subrounds \sched{} and \comp{}.
%  \item Each process can take a step in one of three subrounds \snd{}, \rcv{}, and \comp{} in one global tick.
%  %\item A crashed process cannot recover.
%\end{enumerate} 
%The first assumption would refine a global transition at a time $t$ into a sequence of system configurations 
%\[
%\gconf{t-1} \xrightarrow{\sched{}} \confsched{t} \xrightarrow{\tsnd{}} \confsnd{t} \xrightarrow{\trcv{}} \confrcv{t} \xrightarrow{\tcomp{}} \gconf{t}
%\]
%where a system configuration $\rho_{t}^{\texttt{Action}}$ is generated in a subround $\texttt{Action}$, and a system configuration $\gconf{t}$ is consistent with a global state at a time $t$.
%From now on, we would use the notations in Table~\ref{tab:Notations} to keep the representation of later constraints simple. 
%The interpretation for instructions~\snd{} and~\rcv{} will be provided later.
%
%In order to formalize later assumptions, we introduce an additional system variable~\gpc{} whose type is  $\gpc{} : \proc \rightarrow \Boolean$ to describe what processes can take a step in a global transition.
%We first require that the action~\sched{} can set an arbitrary \Boolean value to $\gpc[p_i]$ for every correct process $p_i$, and always set $\False$ to $\gpc[p^{c}_i]$  for every crashed process $p^{c}_i$.
%%, we always have $\gpc[p^c_i] =  and other actions do not change a value of $\pc{}$, i.e. $\confsnd{t}\left(\pc{}\right) = \confrcv{t}\left(\pc{}\right) = \gconf{t}\left(\pc{}\right)$ for every time $t$.
%Now we can formalize other assumptions as followings
%
%\begin{enumerate}[label=(\roman*)]
%  \setcounter{enumi}{1}
%  \item Process configurations are unchanged in the subround \sched{}. 
%  \[\forall t \, \forall p_i \ldotp \gconf{t-1} \left( p_i \right) = \confsched{t} \left( p_i \right)\]
%  
%  \item Message buffers are unchanged in two subrounds \sched{} and \comp{}.
%  \[
%  \forall t \, \forall p_i, p_j \ldotp \gconf{t-1} \left( \buf{p_i}{p_j} \right) = \confsched{t} \left( \buf{p_i}{p_j} \right)
%  \]
%  \[
%  \forall t \, \forall p_i, p_j \ldotp \confrcv{t} \left( \buf{p_i}{p_j} \right) = \gconf{t} \left( \buf{p_i}{p_j} \right)
%  \]
%  
%  \item Each process can take a step in one of three subrounds \snd{}, \rcv{}, and \comp{} in one global tick.
%  
%  \begin{align*}
%  \forall t \, \forall p_i \ldotp 
%  & \left(\confsched{t} \left( \gpc \left[ p_i \right] \right) \land \confsched{t}(  p_i  ).\lpc = \tsnd{} \right) \\
%  & \quad  \Rightarrow  \left(\confsnd{t} \left( p_i \right) = \confrcv{t} \left( p_i \right) = \gconf{t} \left( p_i \right) \land \lnot \confsnd{t} ( \gpc[p_i] ) \right) \\
%  \forall t \, \forall p_i \ldotp 
%  & \left(\confsnd{t} ( \gpc \left[ p_i \right] ) \land \confsnd{t} (  p_i  ).\lpc = \trcv{} \right) \\
%  & \quad \Rightarrow \left( \confsched{t} (p_i ) = \confsnd{t} ( p_i )  \land \confrcv{t} ( p_i ) = \gconf{t} ( p_i ) \land \lnot \confrcv{t} ( \gpc [p_i] ) \right) \\
%  \forall t \, \forall p_i \ldotp 
%  & \left( \confrcv{t} ( \gpc [ p_i ] ) \land \confrcv{t}(  p_i  ).\lpc = \tcomp{} 
%  \right) \\
%  & \quad \Rightarrow \left( \confsched{t} (p_i) = \confsnd{t} ( p_i ) =  \confrcv{t} ( p_i ) \land \lnot \gconf{t}(\gpc[p_i]) \right) \\
%  \forall t \, \forall p_i \ldotp 
%  & \lnot \confsched{t} ( \gpc [ p_i ] ) \\
%  & \quad   \Rightarrow  \left(\gconf{t-1} ( p_i )  = \confsched{t} (p_i) = \confsnd{t} ( p_i ) =  \confrcv{t} ( p_i ) = \gconf{t} ( p_i ) \right)
%  \end{align*}
%  %  \item A crashed process cannot recover.
%  %  \begin{align*}
%  %  \forall t \ldotp 
%  %  & \gconf{t}(p_i).\lpc = \texttt{Crash} \\
%  %  & \quad \Rightarrow \left( \forall t_1 \ldotp t_1 > t \Rightarrow \gconf{t_1}(p_i).\lpc = \texttt{Crash} \land \lnot \confsched{t_1}(\gpc[p_i]). \right)
%  %  \end{align*}
%\end{enumerate} 
%%For example, if $\gconf{t}\left(\pc\left(p_i\right)\right) =  \inactive$, then a process $p_i$ does not take any action at a time $t$.  
%Notice that the definition of~\gpc{} is consistent with the constraint where a process $p$ cannot execute both instructions $\sop{p_i}{m}{p_j}$ and $\rop{p_i}$ in a global tick where $m$ is a message, and $p_i, p_j$ are processes.

%
%\begin{table}
%  \centering
%  \caption{Notations for accessing variables and process configurations from a system configuration $\psi \in \left\{ \gconf{i}, \rho_i^{\texttt{Action}} \right\}$  where \texttt{Action} is one of~\sched{},~\snd{}, and~\rcv{}.}
%  \label{tab:Notations}
%  \begin{tabular}{p{3cm} | p{0.1cm} p{8.5cm}}
%    Notation & &Refers to \\
%    \hline     
%    $\psi(p_i)$ & & a local configuration of a process $p_i \in \proc$  \\
%    $\psi(p_i).X$ & & a value of a local variable $X$ of a process $p_i$  \\
%    $\psi(p_i).X[\mathit{id}]$ & & a value of $X$ at an index $\mathit{id}$ if $X$ is an one-dimensional array \\
%    $\psi(p_i).\sop{p_i}{m}{p_i}$ & & a predicate for whether a message $m$ is sent to a process $p_j$ by a process $p_i$  \\
%    $\psi.\rop{p_i}$ & & a set of messages which have been received by a process $p_i$  \\
%    $\psi.\rop{p_i}[p_j]$ & & a set of messages which were sent by process $p_j$ and have been received by a process $p_i$  \\
%    $\psi \left( X \right)$ & & a value of a global variable $X$  \\
%    $\psi \left(\age{m}\right)$ & & a time-unit old of an in-transit message $m$  
%  \end{tabular}
%\end{table}
%
%Before formalize partially synchronous constraints, we would introduce a function $\texttt{age} : \msg \rightarrow \mathbb{N}$ to describe a time-unit old of a message where $\mathbb{N}$ is a set of natural number (with 0) and \msg{} is a set of possible messages, i.e. $\msg{} = \bigcup_{p_i, p_j \in \proc} \texttt{Msg}^{p_i}_{p_j}$ . Our computational model requires the followings:
%\begin{enumerate}[label=(\roman*)]
%  \item Every in--transit message age is increased by 1 in every subround \sched{}. 
%  \[
%  \displayindent0pt
%  \displaywidth\textwidth
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp \,  m \in \confsched{t} \left( \buf{p_i}{p_j} \right) \Rightarrow \confsched{t} \left( \age{m} \right) = \gconf{t - 1} \left( \age{m} \right) + 1 
%  \]
%  \item Message ages do not change in other subrounds.
%  \begin{align*}
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp \,  m \in \confsnd{t} \left( \buf{p_i}{p_j} \right) & \Rightarrow \confsched{t} \left( \age{m} \right) = \confsnd{t} \left( \age{m} \right) \\
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp \,  m \in \confrcv{t} \left( \buf{p_i}{p_j} \right) & \Rightarrow \confrcv{t} \left( \age{m} \right) = \confsnd{t} \left( \age{m} \right) \\
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp \,  m \in \gconf{t} \left( \buf{p_i}{p_j} \right) & \Rightarrow \gconf{t} \left( \age{m} \right) = \confrcv{t} \left( \age{m} \right) 
%  \end{align*}
%  \item When a message is introduced in a subround~\snd{}, it is 0 time--unit old.
%  \begin{align*}
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp \,  & \left( m \in \confsnd{t} \left( \buf{p_i}{p_j} \right) \land m \notin \gconf{t-1} \left( \buf{p_i}{p_j} \right) \right) \\ 
%  & \qquad \Rightarrow \confsnd{t} \left( \age{m} \right) =  0 
%  \end{align*}
%  \item Every message buffer is unchanged in every subround $\sched{}$ and in every subround $\cop{}$.
%  \begin{align*}
%  \forall t  \, \forall p_i, p_j \ldotp \,  \confsched{t} \left( \buf{p_i}{p_j} \right) & = \gconf{t-1} \left( \buf{p_i}{p_j} \right) \\
%  \forall t  \, \forall p_i, p_j \ldotp \,  \confrcv{t} \left( \buf{p_i}{p_j} \right) & = \gconf{t} \left( \buf{p_i}{p_j} \right) 
%  \end{align*}
%\end{enumerate}
%In~\cite{CT96}, many models of partial synchrony were provided. Here we show only how to formalize the execution of instuctions $\sop{p}{m}{q}$ and $\rop{p}$, and partially synchronous constraints on process relative speed and message delay in case where $\Delta$ and $\Phi$ hold eventually for some fixed values.
%%
%\begin{itemize}
%  \item $\sop{p}{m}{q}$: The execution of this instruction in a~\snd{} configuration $\confsnd{t}$ can be interpreted with a following formula
%  \begin{align*}
%  & \,   m \notin \confsched{t} \left( \buf{p_i}{p_j}\right)   \\
%  \land &  \,  \confsnd{t} \left( \buf{p_i}{p_j}\right) = \left\{ m \right\} \cup \confsched{t} \left( \buf{p_i}{p_j}\right) 
%%  \land & \,  \forall p^{\prime} \ldotp p^{\prime} \neq p_j \Rightarrow \confsnd{t} \left( \buf{p_i}{p^{\prime}}\right) = \confsched{t} \left( \buf{p_i}{p^{\prime}}\right) )
%  \end{align*}
%  In other subrounds, no process sends any message.
%  \[
%  \confsched{t}.\sop{p}{m}{q} = \confrcv{t}.\sop{p}{m}{q} = \sigma_{t}.\sop{p}{m}{q} =  \False 
%  \]
%  
%  \item $\rop{p}$: The execution of this instruction in a~\rcv{} configuration $\confrcv{t}$ can be interpreted with a formula
%  \begin{alignat*}{3}
%  \exists S_1 \ldots S_N   \ldotp  & \bigwedge_{ 1 \leq k \leq N} && S_k \subseteq  \confsnd{t} \left( \buf{p_k}{p_i}\right) \land S_k \subseteq  \confrcv{t} \left( p_i \right).\mailbox \left[ p_k \right] \\
%  & \quad \; \land   && S_k \cup  \confsnd{t}  \left( p_i \right) \mailbox \left[ p_j \right] = \confrcv{t} \left( p_i \right) \mailbox \left[ p_j \right] \\  
%  & \quad \; \land \, &&  S_k \cup  \confsnd{t} \left( \buf{p_k}{p_i}\right) = \confrcv{t} \left( \buf{p_k}{p_i}\right) \\
%  & \quad \; \land \, && S_k = \confrcv{t}.\rop{p}[p_k] \\
%  & \quad \; \land \, && \confrcv{t}.\rop{p} =  \bigcup S_k 
%  \end{alignat*}
%  In other subrounds, no messages are delivered.
%  \[
%  \forall t \, \forall p, q \ldotp \, \confsched{t}.\rop{p}[q] = \confsnd{t}.\rop{p}[q]= \sigma_{t}.\rop{p}[q] =  \emptyset 
%  \]

\subsubsection{Logical formulas for partially synchronous constraints}
In~\cite{DLS88}, many models of message delay and relative process speed under partial synchrony were introduced.
In the following, we present logical formula for such constraints in case where parameters $\Delta$ and $\Phi$ hold eventually for some fixed values and faults are \emph{clean crashes}, and where a sequence of global configurations is \emph{admissible}.

\begin{definition}
  Let $\sys{N}$ be an instance of $\mathcal{A}$ whose indexes are $\nid$.
  Let $\pi = \gconf{0}\gconf{1}\ldots$ be an infinite path of glocal configurations.
  A sequence $\pi$ is \emph{admissible} if for every $k > 0$, we have $\conf_{4k - 4} \transsched \conf_{4k - 3} \transsnd \conf_{4k - 2} \transrcv \conf_{4k - 1} \transcomp \conf_{4k}$.
\end{definition}

\begin{itemize}
  \item \emph{Constraint $\Phi$}: Let $\sys{N}$ be an instance of $\mathcal{A}$ whose indexes are $\nid$.
  Let $\pi = \gconf{0}\gconf{1}\ldots$ be an admissible path of glocal configurations such that the global stabilization time on $\pi$ is $t_0$.
  For every time $t \geq t_0$, every correct process must take at least one step in  every global time interval $\left[ t, t + \Phi \right]$. Formally, we have
  \begin{align*}
  & \forall \pi = \gconf{0} \gconf{1} \ldots \forall t_0 \geq 0 \,  \forall t \geq t_0  \, \forall i \in \nid \colon \\
  & \quad \conf_{4(t + \Phi) - 3}(\pc[p]) \neq L_F  \Rightarrow \exists t \leq t_1 \leq t + \Phi  \colon \conf_{t_1}(\act[p]) 
  \end{align*}
  Recall that a configuration $ \conf_{4(t + \Phi) - 3}$ is constructed in the subround \sched{}.
  
  \item \emph{Constraint $\Delta$}: Let $\sys{N}$ be an instance of $\mathcal{A}$ whose indexes are $\nid$.
  Let $\pi = \gconf{0}\gconf{1}\ldots$ be an admissible path of glocal configurations such that the global stabilization time on $\pi$ is $t_0$.
  For every time $t \geq t_0$, if process $p_i$ executes an $\rcv(p_i)$ instruction at a time $t$, all messages which were sent to $p_i$ by time $t - \Delta$  must be delivered to $p_i$ by time $t$. 
  Formally, we have
  \begin{align*}
  & \forall \pi = \gconf{0} \gconf{1} \ldots \forall t_0 \geq 0 \,  \forall t \geq t_0  \, \forall i, j  \in \nid  \forall m_{ts} \in \msg_{ts} \colon \\
  & \quad \left( \conf_{4t-2}(\act[p_i]) \land \conf_{4t-2}(\pc[i]) = L_R  \land m_{ts} \in \conf_{4t-1}(\buf[j, i]) \right)   \\
  & \qquad \Rightarrow \conf_{4t-1}(\gc) - \conf_{4t-1}(m_{ts}[2]) < \Delta  
  \end{align*}
  Recall that a configuration $ \conf_{4(t + \Phi) - 1}$ is constructed in the subround  \rcv{}.

\end{itemize}

%From now on, we use the notation $\mathcal{A}$ to denote an arbitrary partially synchronous algorithm, and the notation $S_{\Pi}\left(\mathcal{A},\Delta, \Phi\right)$ to denote an instance of $\mathcal{A}$ with $\card{\Pi}$ distinguished processes.
%When the context is clear, we write  $\conf{N}{k} \leadsto \conf{N}{\ell}$ to refer a finite sequence of configurations starting from a configuration $\conf{N}{k}$ and ending in a configuration $\conf{N}{\ell}$ where $\ell \leq k$.

==> netys20/experiment.tex <==
To demonstrate the feasibility of our approach, we specified the failure detector~\cite{CT96} in~\tlap{}~\cite{lamport2002specifying}
\footnote{Our specification is available at \url{github.com/banhday/netys20.git}.}.
Our specification follows the model of computation in Section~\ref{sec:netys20-comp-model}.
It is close to the pseudo-code in Section~\ref{algo:detector1}, except that these tasks are organized in a  loop: task 1, task 2, and task 3.
%Moreover, our encoding contains the upper bounds on transmission time of messages and on the relative speeds of different processes, called $\Delta$ and $\Phi$ respectively.
%Like in~\cite{DLS88}, these parameters are named $Delta$ and $Phi$, respectively.
The user can verify our specification with different values of $\Delta$ and $\Phi$ by running model checkers TLC~\cite{yu1999model} and \apalache{}~\cite{KT19}.
Our experiments were set up in the synchronous case where $\Delta = 0$ and $\Phi = 1$.
%Our~\tlap{} specifications can be found in~\cite{netys20Spec}.
%To reduce the state space, we apply abstractions to a global clock, local clocks, and received messages.
%Our abstractions are explained in detail in our~\tlap{} specification.


\begin{table}[!htbp]
  \centering
  \caption{Checking the failure detector~\cite{CT96} in the synchronous case} \label{tab:exp}
  \begin{tabular}{>{\centering\arraybackslash}p{0.5cm} | >{\centering\arraybackslash}p{3.7cm} | >{\centering\arraybackslash}p{0.5cm}  c  >{\raggedleft\arraybackslash}p{1.5cm}  >{\raggedleft\arraybackslash}p{1.5cm} >{\raggedleft\arraybackslash}p{1.2cm}} 
    \# & Property & $N$ & Tool & Runtime & Memory & Depth \\  
    \hline
      1 & \multirow{6}{*}{Strong accuracy}             & 2   &  TLC & 2s  & 112M & 36 \\    
      2 &              & 2   & \apalache{}  & 1m  & 1.12G & 37\\                
      3 &              & 4   &  TLC & 17m & 774M  & 40 \\    
      4 &              & 4   & \apalache{}  & 72m & 2.27G & 41 \\          
      5 &              & 6   & TLC       & TO  & 943M & 2 \\    
      6 &              & 6   & \apalache{}  & TO  & 3M  & 31  \\          
      \hline            
      7 & \multirow{3}{*}{\shortstack{Eventually strong\\ accuracy}}  & 2   & TLC       & 2s  & 140M  & 36 \\
      8 &   & 4   & TLC       & 20m & 683M & 40 \\      
      9 &   & 6   & TLC       & TO  & 839M &  2 \\      
      \hline      
      10 & \multirow{3}{*}{Strong completeness}         & 2   & TLC       & 2s  & 134M & 36 \\      
      11 &         & 4   & TLC       & 23m & 678M & 40 \\
      12 &         & 6   & TLC       & TO  & 789M & 3 \\
      \hline
      13 & \multirow{5}{*}{Inductive invariant}        & 2   &   TLC       & 20s & 192M  &  \\
      14 &         & 2   & \apalache{}   & 1m  & 674M  &  \\    
      15 &         & 3   &    TLC       & TO & 1.1G &  \\   
      16 &         & 3   &  \apalache{}  & 3m  & 798M  &  \\       
      17 &         & 4   &  \apalache{}   & 31m & 1.14G &  \\    

      


  \end{tabular}
\end{table}

%\tht{The versions of \apalache{} and TLC is added.}

We ran the following experiments on a laptop with a core i7-6600U CPU and 16GB DDR4. 
We checked benchmarks with TLC in the \tlap{} Toolbox version 1.6.0~\cite{toolbox} and \apalache{} version~0.5.2 described in Chapter~\ref{chap:oopsla19}.
Table~\ref{tab:exp} presents the results in model checking the failure detectors~\cite{CT96} in the synchronous model.
From the theoretical viewpoint, an instance with $N = 1$ is necessary, but we show only interesting cases with $N \geq 2$ in Table~\ref{tab:exp}.
(We did check an instance with $N = 1$, and there are no errors in this instance.)
The strong accuracy property is the following safety property: 
$
 \G (\A p, q \in \nid \colon (\mathit{Correct}(p) \land \mathit{Correct}(q)) \Rightarrow \lnot \mathit{Suspected}(p, q))
$.
The column ``depth'' shows the maximum execution length used by our tool as
well as the maximum depth reached by TLC while running breadth-first search. 
For the second and forth benchmarks, we used
the diameter bound that was reported by TLC, which does exhaustive state exploration.
Hence, the verification results with \apalache{} are complete.
The abbreviation ``TO'' means timeout of 10 hours.
The inductive invariant  is on the transition $\leadsto$, and contains type invariants, constraints on the age of in-transit messages, and constraints on when a process executes a task.
This inductive invariant does not imply the safety properties of the Chandra and Toueg failure detector.

==> netys20/general_algo.tex <==

%Lemmas \ref{lem:UnboundedMsgBufOne}--\ref{lem:UnboundedMsgBuf} show that there exists an execution prefix such that message buffers in this time interval are unbound. 
%Moreover, Lemmas \ref{lem:BoundRcvdMsgDelay}--\ref{lem:BoundCorrMsgBuf} show that there exists an postfix such that every message buffer of a correct process in the
%postfix is bounded. 
%Under Assumption \ref{asmp:CrashProc}, we obtain two Lemmas \ref{lem:BoundMsgBuf}--\ref{lem:SilentCrashedProc} for crashed processes.

%\subsection{Underlying assumptions and interesting algorithm classes}

%Since every correct process follows the same deterministic protocol (Assumption 4), we can have Lemmas \ref{lem:PhiS} and \ref{lem:PhiR} for correct processes. 
%Intuitively, the guards $\Phi_S$ and $\Phi_R$ in these assumptions describe how often a correct process sends and receives messages. 
%The values of $\Phi_S$ and $\Phi_R$ depend on the algorithm implementation.
%In Section \ref{sec:fd}, we will discuss a specific algorithm -- Chandra and Toug's failure detector \cite{CT96}, and give specific values of $\Phi_R$ and $\Phi_S$ in this algorithm.
%
%Assumption \ref{asmp:CrashProc} is for crashed processes. 
%Intuitively, this assumption is used to keep the system configuration simple by immediately and repeatedly cleaning message buffers crashed processes.
%We will give more details in Section \ref{sec:Prop}, paragraph \emph{Crash models}.

This section describes interesting properties of the environment, and correct processes  which will be used in the verification task.

\subsection{Implicit bounds on the behavior of correct processes} 

While Constraints \ref{const:OmegaS} and \ref{const:OmegaR} are on the local time, 
Lemmas \ref{lem:PhiS} and \ref{lem:PhiR} show that our computational model implies constraints for $\mathit{Send}$ and $\mathit{Receive}$ in terms of global time.

\newcommand{\lemPhiS}{
  Let $\Phi_S \geq \Omega \times \Phi$. 
  For all the $t \geq t_0$, every correct process $p$ must execute the operator $\sendall{p}$ 
    at least once in every global time interval $\rho = \left[ t, t + \Phi_S \right]$
}

\begin{lemma} \label{lem:PhiS}
  \lemPhiS
\end{lemma}

\begin{proof}  
  Because of the constraint $\Delta$ on process relative speeds, 
    process $p$ takes at least $\Omega$ steps 
    in the time interval $\rho$.
  Hence, process $p$ must execute the operator $\mathit{Send}$ at least once
    in the time interval $\rho$
    due to Constraint \ref{const:OmegaS}.    \qed
\end{proof}

\begin{lemma} \label{lem:PhiR}
    Let $\Phi_S \geq \Omega \times \Phi$. 
  For all the $t \geq t_0$, every correct process $p$ must execute the operator $\receive{p}$ 
    at least once in every global time interval $\rho = \left[ t, t + \Phi_R \right]$.
\end{lemma}

\begin{proof}  
  By similar arguments for Lemma \ref{lem:PhiS}, it follows that 
    process $p$ must execute the operator $\receive{p}$ 
    at least once in the time interval $\rho = \left[ t, t + \Phi_R \right]$. \qed
\end{proof}

%\begin{assumption} \label{asmp:CrashProc}
%  When process $p$ crashes, its message buffer $\msgbuf{p}$ is clean empty immediately, and from now on no messages are stored in its buffer.
%\end{assumption}

%\begin{assumption} \label{asmp:talkative}
%  A correct process can execute only the action ``send--to--all'' to send messages to every process.
%\end{assumption}
%
%\begin{assumption} \label{asmp:laconic}
%  A correct process can execute the action ``send--to--some'' to send a message to a subset of processes. 
%\end{assumption}

%
%We call the class of algorithms satisfying Assumptions \ref{lem:PhiS} --\ref{lem:PhiR} as ``receptive''. 
%The ``receptive'' class contains three following subclasses: 
%\begin{enumerate}
%  \item Class ``talkative'': Correct processes can execute only the action ``send--to--all'' to send messages to every process. 
%  
%  \item Class ``laconic'': Correct processes can execute the action ``send--to--some'' to send a message to a subset of processes. 
%  
%  \item Class ``clean'': The system behavior must satisfy Assumption \ref{asmp:CrashProc}.
%\end{enumerate}





%\subsection{Properties} \label{sec:Prop}

%In this section, we discuss two classes of algorithms called ``talkative'' and ``

%In the following, we discuss the following:
%\begin{enumerate}
%  \item The number of in-transit messages before GST: Lemmas \ref{lem:UnboundedMsgBufOne}--\ref{lem:UnboundMsgBuf}, 
%  \item The lower bound on transmission time for messages sent to correct processes: Lemmas \ref{lem:BoundRcvdMsgDelay}--\ref{lem:GSTClean}, 
%  \item Crash models: under Assumption \ref{asmp:CrashProc},
%  \item The message buffers after GST: Lemmas \ref{lem:BoundCorrMsgBuf}--\ref{lem:BoundMsgBuf}, and
%  \item The silent period of crashed processes: Lemma \ref{lem:SilentCrashedProc}.
%\end{enumerate}
%
% shows that there exists an execution prefix such that message buffers in this time interval are unbound.
% shows that there exists an execution prefix such that message buffers in this prefix are unbound.
%Moreover, Lemmas -\ref{lem:BoundCorrMsgBuf} shows that there exists an postfix such that every message buffer of a correct process in the postfix is bound.
%Assumption  is to restrict the behavior related to crashed processes.
%Under this assumption, we obtain two Lemmas for crashed processes.



\subsection{Unbounded message buffers before GST} 

%Lemma \ref{lem:UnboundedMsgBufOne} shows that the message buffers in the class ``talkative'' are unbounded before the global stabilization time ($\gst{}$) $t_0$, even in case of two processes in the system. 
%Lemma \ref{lem:UnboundedMsgBufTwo} is for the class ``laconic''.
%It follows immediately that in both classes ``talkative'' and ``laconic'', the total number of messages in transit before $t_0$ is unbounded (Lemma \ref{lem:UnboundedMsgBuf}).


\newcommand{\lemUnboundedMsgBufOne}{
  Let $\mathit{MAX}$ be a natural number. 
  There exist an execution path $\pi$ in $S_{1..N}$ such that 
    the number of messages in the message buffer $\msgbuf{1, 2}$ at some time point is greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{1, 2}$.
}

\begin{lemma} \label{lem:UnboundedMsgBufOne}
  \lemUnboundedMsgBufOne
\end{lemma}

\begin{proof}
  Assume by contradiction that in every execution path, the number of messages in every message buffer is bounded by $\mathit{MAX}$.
  We will construct an execution path that violates this assumption.
  Recall that the system behavior is unrestricted before $t_0$. 
  Therefore, the following case exists:
  (i) no faults happen before $t_0$, and 
  (ii) no messages sent before $t_0$ were received before $t_0$, and 
  (iii) every correct process takes a step in every global tick.
  We choose an execution path $\pi$ such that
  its global stabilization time is $t_0 = 1 + \Phi_S \times (\mathit{MAX} + 1)$, and 
  all constraints (i)--(iii) are satisfied in $\pi$.
  By Lemma \ref{lem:PhiS}, we know that process 1 must execute the action $\sendall{1}$ at least $(\mathit{MAX} + 1)$ times in the interval $\left[1, t_0 - 1\right]$. 
  By condition (ii), the message buffer $\buf{1, 2}$ at the time point $t_0 - 1$ must have all messages which were sent by proocess 2 before the time point $ t_0 -1$. 
  Therefore, $\buf{1, 2}$ at the time point $t_0 - 1$ must have at least $\mathit{MAX} + 1$ messages.
  \qed
\end{proof}

%\begin{figure}[!hbt]
%  \begin{tikzpicture}
%  % draw horizontal line   
%  \draw[thick, -Triangle] (0,0) -- (0.75 * \ImageWidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%  
%  % draw vertical lines
%  \foreach \x in {0,1,...,5}
%  \draw (\x cm,3pt) -- (\x cm,-3pt);
%  
%  \foreach \x/\descr in {3/ t_0 }
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};
%  
%  \draw [thick,decorate,decoration={brace,amplitude=5pt}] (2,-.7) -- +(-2,0)
%  node [black,midway,font=\scriptsize, below=4pt] {Unbounded message buffers};
%  \end{tikzpicture}
%  \caption{Message buffers are unbounded before the global stabilization time $t_0$.} \label{fig:unboundedmsgbuffers}
%\end{figure}

%\newcommand{\lemUnboundedMsgBufTwo}{
%  Let $S$ be a partially synchronous system in the class ``laconic'' with 2 processes.
%  Let $\mathit{MAX}$ be a natural number. 
%  There exist an execution trace $\pi$ and a process $p_j$ such that the number of messages in the message buffer $\msgbuf{p_j}$ at some time point is greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{p_j}$.
%}

%\begin{lemma} \label{lem:UnboundedMsgBufTwo}
%  \lemUnboundedMsgBufTwo
%\end{lemma}
%
%\begin{proof}  
%  Consider an execution trace $\pi$ such that
%  its global stabilization time is $ t_0 = 2 + \Phi_S \times (2 \times \mathit{MAX} + 1)$,
%  and all following conditions are satisfied in the trace $\pi$: 
%  (i) no faults happen before $t_0$, and 
%  (ii) no messages sent before $t_0$ were received before $t_0$, and 
%  (iii) every correct process takes a step in every global tick.
%  We prove the following by contradiction: there exist processes $i, j \in \left\{1, 2\right\}$ such that process $i$ executes the action $\mathit{Send} \left( \_ , p_j \right)$ at least $\mathit{MAX} + 1$ times in the interval $\left[ 1, t_0 - 1 \right]$.
%  Assume by contradiction that for every pair of processes $p_i, p_j$, process $p_i$ has executed the action $\mathit{Send} \left( \_ , p_j \right)$ less than or equal to $\mathit{MAX}$ times in the interval $\left[1, t_0 - 2\right]$ (*).
%  Now let us investigate the behavior of process 1.
%  By Assumption \ref{lem:PhiS}, condition (iii) and the default value of $t_0$, we know that process 1 must execute the action $\mathit{Send} \left( \_, \_\right)$ at least $2 \times \mathit{MAX} + 1$ times in the interval $\left[ 1, t_0 - 2\right]$.
%  Because the given system has only two processes, the assumption (*) implies that the total number of time points when process 1 executes the action $\mathit{Send} \left(\_, \_\right)$ is less than or equal to $2 \times \mathit{MAX}$ times (contradiction).
%  It follows that there exists a process $p_j$ such that process 1 must execute the action $\mathit{Send} \left( \_ , p_j \right)$ at least $(\mathit{MAX} + 1)$ times in the time interval $\left[1, t_0 - 2\right]$.
%  This result implies that the message buffer $\msgbuf{p_j}$ at the time point $t_0 - 1$ must contain at least $(\mathit{MAX} + 1)$ messages by the condition (ii).
%\end{proof}


%\newcommand{\lemUnboundedMsgBuf}{
%In both classes ``talkative'' and ``laconic'', for every integer $\mathit{MAX}$ there exists an execution trace $\pi$ and a process $p_j$ such that the number of messages in $\msgbuf{p_j}$ at some time point must be greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{p_j}$.
%}
%
%\begin{lemma} \label{lem:UnboundedMsgBuf}
%\lemUnboundedMsgBuf  
%\end{lemma}

%\begin{proof} \label{lem:msgbuf_unbound_general}
%  Lemma \ref{lem:UnboundedMsgBuf} follows immediately from Lemmas \ref{lem:UnboundedMsgBufOne} and \ref{lem:UnboundedMsgBufTwo}. 
%\end{proof}

\subsection{The postfix}

In this section, we show that we can bound the time of
  messages sent to correct processes before GST in
  Lemma \ref{lem:MsgBeforeGST}, and
  the transmission time of messages sent to correct processes after GST in Lemma 
  Lemma \ref{lem:MsgAge}.

%Now we prove that there is eventually a lower bound on transmission time for messages sent to correct processes in the class ``receptive''. 
%Lemma \ref{lem:BoundRcvdMsgDelay} shows that this lower bound called $\Gamma$ is eventually reached since the time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R$, and $\Gamma = \Delta + (\Phi + 1) \times \Phi_R + 1$.
%%Because there eventually exists a connection between $\Phi_R$ and $\Phi$, the value of $\Gamma$ actually depends on $\Phi$. 
%The proof of Lemma \ref{lem:BoundRcvdMsgDelay} requires Lemmas \ref{lem:RepeatRcvAfterGST} and \ref{lem:GSTClean}.
%Lemma \ref{lem:RepeatRcvAfterGST} shows that every correct process $p$ must execute the action $\receive{p}$ at least once in an interval $\left[t, t + (\Phi + 1) \times \Phi_R \right]$ where time $t$ is later than time $t_0$, i.e. $t_0 \leq t$.
%Lemma \ref{lem:GSTClean} says that since the time point $T_0$, whose value is already assigned as $t_0 + \Delta + (\Phi + 1) \times \Phi_R$, every correct process does not receive any messages sent by $t_0$.
%
%\begin{figure}[!hbt]
%\centering
%\begin{tikzpicture}
%% draw horizontal line   
%\draw[thick, -Triangle] (0,0) -- (0.85\textwidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%
%% draw vertical lines
%\foreach \x in {0,0.5,...,9}
%\draw (\x cm,3pt) -- (\x cm,-3pt);
%
%\foreach \x/\descr in {1.5/t_0}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%\foreach \x/\descr in {7.5/\text{\textit{p} receives \textit{m}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%
%
%\foreach \x/\descr in {2.5/\text{\textit{q} sent \textit{m}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%\foreach \x/\descr in {5/\text{\textit{m} in \textit{msgBuf[p]}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%
%\draw[-, dashed, black] (6.5,-.3) --  +(-0.4,0);
%
%\draw[-Triangle, dashed, black] (3.8,-.3) --  +(-0.6,0);
%
%
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (2,0.4)  -- +(5.5,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Gamma = \Delta + (\Phi + 1) \times \Phi_R + 1$};
%\end{tikzpicture}
%\caption{The lower bound of message delay $\Gamma$ in the class ``receptive'' is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.}
%\end{figure}

\newcommand{\lemMsgBeforeGST}{
  Every message sent to correct process $p$  before $t_0$ 
  is received by time $t_0 + \Delta + \Phi_R$.
}

\begin{lemma} \label{lem:MsgBeforeGST}
  \lemMsgBeforeGST
\end{lemma}

\begin{proof}
Let $p$ be a correct process, 
  and $m$ be an arbitrary message which was sent to process $p$ before GST.
We know that message $m$ is at least $\Delta$ time-units old from the time point $t_0$ 
  because it was sent before $t_0$.
By Lemma \ref{lem:PhiR}, process $p$ must execute the operator $\mathit{Receive}(p)$ at some point $t$ where $t_0 + \Delta \leq t \leq t_0 + \Delta + \Phi_R$.
By the constraint $\Delta$, process $p$ must receive message $m$ at time $t$.
\qed
\end{proof}

\newcommand{\lemMsgAge}{
  Every message sent to correct process $p$ at some time $t \geq t_0$ 
  is received by time $t + \Delta + \Phi_R$.
}

\begin{lemma} \label{lem:MsgAge}
  \lemMsgAge
\end{lemma}

\begin{proof}
  By similar arguments in Lemma \ref{lem:MsgBeforeGST}. \qed{}
\end{proof}

By Lemmas \ref{lem:MsgBeforeGST}--\ref{lem:MsgAge}, we obtain Lemma \ref{lem:BoundedMsgBuf} which says that  
  every message buffer to a correct process is eventually and permanently bounded.

\newcommand{\lemBoundedMsgBuf}{
  Let $K = \Delta + \Phi_R$, and $p, q$ be arbitrary processes such that $q$ is correct.
  The number of messages in the buffer $\buf{p, q}$ is eventually and permanently bounded by $K$.
}

\begin{lemma} \label{lem:BoundedMsgBuf}
\lemBoundedMsgBuf
\end{lemma}

\begin{proof}
We prove Lemma \ref{lem:BoundedMsgBuf} by cases. There are two cases: 
\begin{enumerate}
\item \emph{Both processes $p$ and $q$ are correct.} By Lemmas \ref{lem:MsgBeforeGST} and \ref{lem:MsgAge}, it follows that the message buffer $\buf{p, q}$ contains only messages which are less than $\Delta + \Phi_R$ time-units old.
By Constraint \ref{const:SendToAll}, we know that there are no two different messages with the same age. 
Therefore, the message buffer $\buf{p, q}$ has at most $\Delta + \Phi_R$ messages.
In other words, the number of messages in $\buf{p, q}$ is bounded by $K$.


\item \emph{Process $q$ is correct and process $p$ crashes at some time $t_1$.} 
By Constraint \ref{const:NoRecover}, we know that 
  every message $m$ from process $p$ to process $q$ was sent before time $t_1$.
If process $p$ crashes before $t_0$, then by Lemma \ref{lem:MsgBeforeGST} we know that all of its messages will be received by $t_0 + \Delta + \Phi_R$.
If process $p$ crashes after $t_0$, then by Lemma \ref{lem:MsgAge}, it follows that every message from process $p$ will be received by the time point $t_1 + \Delta + \Phi_R$.
Therefore, after the time point $t_2 = \mathit{max}(t_0, t_1) + \Delta + \Phi_R$, it follows that $\buf{p, q}$ is permanently empty.

%\item \emph{Process $q$ crashes at some time $t_1$.} By Constraint \ref{const:CrashModel}, every message buffer to process $q$ is empty immediately.
\end{enumerate}
Hence, the message buffer is eventually and permanently bounded by $K$.
\qed
\end{proof}
%
%Lemma \ref{lem:HearingBound} says that 
%  a correct process must hear something from another correct process 
%  in every time interval with $\Phi_S + \Delta + \Phi_R$ ticks.
%Lemma \ref{lem:SilentPeriod} says that
%  every correct process eventually hears nothing from a crashed processes.
%  
%\newcommand{\lemHearingBound}{
%Let $\sigma = \left[ t, t + \Delta + \Phi_S + \Phi_R \right]$ be an arbitrary time interval after $\gst{} t_0$, i.e. $t_0 \leq t$. 
%Let $p, q$ be an arbitrary pair of correct processes.
%Then, process $p$ receives some message from process $q$ in the time interval $\sigma$.
%}
%
%\begin{lemma} \label{lem:HearingBound}
%\lemHearingBound
%\end{lemma}
%
%\begin{proof}
%By Lemma \ref{lem:PhiS}, process $q$ must send at least one message $m$ to process $p$ in the interval $\left[ t, t + Phi_S \right]$. 
%We have that message $m$ is at least $\Delta$ time-units  from the time $t + \Phi_S + \Delta$.
%By Lemma \ref{lem:PhiS}, process $p$ must execute the operator $\mathit{Receive}(p)$ at least once in the interval $\rho = \left[ t + \Phi_S + \Delta, t + \Phi_S + \Delta + \Phi_R \right]$.
%Therefore, process $p$ must receive message $m$ in the interval $\rho$.
%\qed
%\end{proof}
%
%
%%Finally, Lemma \ref{lem:SilentCrashedProc} says that correct processes eventually and forever hear nothing from crashed processes.
%%
%\newcommand{\lemSilentPeriod}{
%  If process $p$ crashes at time $t_{\mathit{crash}}$, every correct process $q$ does not receive any message from process $p$ after time $t = \mathit{max}\{ t_{\mathit{crash}}, \gst{} \} + \Delta + \Phi_R  + 1$.
%}
%
%\begin{lemma} \label{lem:SilentPeriod}
%  \lemSilentPeriod
%\end{lemma}
%
%\begin{proof}
%By similar arguments in the proof of Lemma \ref{lem:BoundedMsgBuf}, the second case.
%\qed
%\end{proof}

%\begin{figure}[!hbt]
%  \begin{tikzpicture}
%  % draw horizontal line   
%  \draw[thick, -Triangle] (0,0) -- (0.99\textwidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%  
%  % draw vertical lines
%  \foreach \x in {0,1,...,12}
%  \draw (\x cm,3pt) -- (\x cm,-3pt);
%  
%  \foreach \x/\descr in {3/\textit{GST}}
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};
%  
%  %% colored bar up
%  %\foreach \x/\perccol in
%  %{0/100,1/75,2/0,3/75}
%  %\draw[lightgray!\perccol!red, line width=4pt] 
%  %(\x,.5) -- +(1,0);
%  %\draw[-Triangle, dashed, red] (4,.5) --  +(4,0);
%  
%  % colored bar down
%  %\foreach \x/\perccol in
%  %{3/100,4/75,5/0}
%  %\draw[lightgray!\perccol!green, line width=4pt] 
%  %(\x,-.7) -- +(1,0);
%  %\draw[-Triangle, dashed, green] (6,-.7) --  +(1,0);
%  
%  % braces
%  \draw [thick ,decorate,decoration={brace,amplitude=5pt}] (4,0.4)  -- +(3,0) 
%  node [black,midway,above=4pt, font=\scriptsize] {$\Delta$};
%  
%  \draw [thick ,decorate,decoration={brace,amplitude=5pt}] (7,0.4)  -- +(2,0) 
%  node [black,midway,above=4pt, font=\scriptsize] {$\Phi_R$};
%  
%  \draw [thick,decorate,decoration={brace,amplitude=5pt}] (10,0.4) -- +(3,0)
%  node [black,midway,above=4pt,font=\scriptsize] {No messages from proc \textit{i}};
%  
%  \foreach \x/\descr in {4/\textit{Proc i crashes}}
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};  
%  \end{tikzpicture}
%  
%  \caption{Every crashed process is eventually and forever silent}
%  \label{fig:silentCrash}
%\end{figure}


%\begin{lemma} \label{lem:RepeatRcvAfterGST}
%  \lemRepeatRcvAfterGST
%\end{lemma}

%\newcommand{\lemRepeatRcvAfterGST}{
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Every correct process $p_i$ in $P$ must execute the action $\receive{p_i}$ at least once in a global time interval $\rho = \left[t, t + (\Phi + 1 )\times \Phi_R \right]$ since the GST $t_0$, i.e. $t_0 \leq t$.
%}
%
%\begin{lemma} \label{lem:RepeatRcvAfterGST}
%  \lemRepeatRcvAfterGST
%\end{lemma}
%
%\begin{proof}
%  It is easy to see that we can split every interval $\left[t, t + (\Phi + 1 )\times \Phi_R \right]$ into $\Phi_R$ disjoint intervals whose length is $\Phi$, where $t$ is an integer.
%  By the constraint $\Phi$ on process speed, every correct process $p$ must take at least $\Phi_R$ steps in the interval $\rho$.
%  Therefore, its local clock must tick at least $\Phi_R$ times in the interval $\rho$.
%  By Assumption \ref{lem:PhiR}, it follows that process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%\end{proof}
%
%\newcommand{\lemGSTClean}{
%%  Let $t$ be a time point after $t_0 + \Delta + \Phi_R$, that is $t_0 + \Delta + \Phi + 1 \geq t$.
%%  Let $m$ be a message sent to a process which is still correct until $t$.
%%  If message $m$ is in transit at time $t$, 
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Assume that a correct process $p$ in $P$ executes the action $\receive{p}$ after the global time point $t_0 + \Delta + (\Phi + 1) \times \Phi_R$, and receives message $m$.
%  Then message $m$ was sent at time $t_0$ or later.
%}
%
%\begin{lemma} \label{lem:GSTClean}
%  \lemGSTClean
%\end{lemma}
%
%\begin{proof}
%  By applying Lemma \ref{lem:RepeatRcvAfterGST} to the interval $\rho = \left[ t_0 + \Delta, t_0 + \Delta + (\Phi + 1) \times \Phi_R \right]$, we know that every correct process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%  Assume that process $p$ executes the action $\receive{p}$ at some time point $t^{\rho}_p$ in the interval $\rho$.
%  It immediately follows that $t^{\rho}_p$ is after $t_0 + \Delta$, i.e. $t_0 + \Delta \leq t^{\rho}_p$.
%  By the constraint $\Delta$ on message delay, we know that messages sent to process $p$ by time $t_0$ must be delivered by time $t^{\rho}_p$.
%  It follows that from the time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R + 1$ message buffers of correct processes only contain messages sent after $t_0$.
%  It implies that if process $p$ receives me message $m$ since the time point $T_0$, message $m$ must be sent at time $t_0$ or later.
%%  By the constraint $\Delta$ on message delay, we know that all messages sent to process $p$ before the time point $t^{\rho} - \Delta$ must be delivered to process $p$ by the time point $t^{\rho}$.
%%  First, we prove that every correct process $p \in P$ in the global time interval $\rho = \left[t_0 + \Delta, t_0 + \Delta + (\Phi + 1 )\times \Phi_R \right]$ must execute the action $\receive{p}$ at least once.
%%  ve into $\Phi_R$ 
%\end{proof}
%
%\newcommand{\lemBoundRcvdMsgDelay}{
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Let $p$ be a correct process in $P$, and $t$ $t$ be a time point later the global time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R$, i.e. $T_0 \leq t$, such that process $p$ executes the action $\receive{p}$ at time $t$ in the execution trace $\pi$.
%  Process $P$ receives only messages which were sent since the time point $t - \Delta -  (\Phi + 1) \times \Phi_R - 1$.
%  In other words, the lower bound of message delay called $\Gamma$ in algorithm $\mathcal{A}$ is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.
%}
%
%\begin{lemma} \label{lem:BoundRcvdMsgDelay}
%\lemBoundRcvdMsgDelay
%\end{lemma}
%
%\begin{proof}
%  By Lemma \ref{lem:RepeatRcvAfterGST}, process $p$ executed $\receive{p}$ at least once in the interval $\rho = \left[t - (\Phi + 1) \times \Phi_R - 1, t - 1 \right]$.
%  Assume that process $p$ executed the action $\receive{p}$ at some time point $t^{\rho}_p$ in the interval $\rho$.
%  It immediately follows that $t  - (\Phi + 1) \times \Phi_R - 1 \leq t^{\rho}_p$.
%  By an assumption $T_0 \leq t$, we know that the time point $t  - (\Phi + 1) \times \Phi_R - 1$ is after time $t_0$.
%  By Lemma \ref{lem:GSTClean}, it follows that after time $t^{\rho}_p$, the message buffer $\msgbuf{p}$ contains only messages sent from time $t^{\rho}_p - \Delta$.
%  Therefore, after executing the action $\receive{p}$ at time $t$, process $p$ cannot receive messages sent before the time point $t - \Delta -  (\Phi + 1) \times \Phi_R - 1$.
%  In other words, the lower bound of message delay called $\Gamma$ in algorithm $\mathcal{A}$ is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.
%%  
%%  First, we can split every interval $\rho = \left[t, t + (\Phi + 1 )\times \Phi_R \right]$ into $\Phi_R$ disjoint intervals whose length is $\Phi$, where $t$ is an integer.
%%  Now assume that $t_0 + \Delta \leq t$.
%%  By the constraint $\Phi$ on process speed, process $p_i$ must take at least $\Phi_R$ steps in the interval $\sigma$.
%%  Therefore, its local clock must tick at least $\Phi_R$ times in the interval $\rho$.
%%  By Assumption \ref{lem:PhiR}, it follows that process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%%  Assume that process $p$ executes the action $\receive{p}$ at some time point $t^{\rho}$ in the interval $\rho$.
%%  It immediately follows that $t^{\rho}$ is after $t_0$, i.e. $t_0 \leq t^{\rho}$.
%%  By the constraint $\Delta$ on message delay, we know that all messages sent to process $p$ before the time point $t^{\rho} - \Delta$ must be delivered to process $p$ by the time point $t^{\rho}$.
%%  Now consider the time interval $\sigma = \left[ t + \Delta + (\Phi + 1) \times \Phi_R + 1, t + \Delta + 2 \times (\Phi + 1) \times \Phi_R \right]$.
%%  Again by our assumptions, we know that process $p$ must execute the action $\receive{p}$ at least once in the time interval $\sigma$.
%%  Let $t^{\sigma}$ be a time point in the time interval $\sigma$ when process $p$ executed the action $\receive{p}$.
%%  By the fact (*), we know that only messages sent since the time point $t^{\rho} - \Delta$ can be delivered by process $p$ at this time point $t^{\sigma}$.
%%  Moreover, we have that 
%%  \[ t^{\sigma} - (t^{\rho} - \Delta) \leq t - (t^{\rho} - \Delta) \leq t - t^{\rho} + \Delta) \leq 2 * \Phi_R + \Delta \]
%%  Therefore, the gap between when the latest messages are sent and when they are received is bound by $2 * \Phi_R + \Delta$ since the time point $t_0 + \Delta + \Phi_R + 1$.
%\end{proof}
%
%
%
%
%
%\subsubsection{Crash models} \label{sec:CrashModel} \hfill
%
%Notice that Lemmas \ref{lem:BoundRcvdMsgDelay} and \ref{lem:GSTClean} describe nothing about the status of messages sent to faulty processes
%% nor the status of message buffers in the time interval $\left[ t_0, t_0 + \Delta + \Phi_R \right]$. 
%To keep the system configuration simple but reasonable, we require the following assumption:
%\begin{assumption} \label{asmp:CrashProc}
%When process $p$ crashes, its message buffer $\msgbuf{p}$ is clean empty immediately, and from now on no messages are stored in its buffer.
%\end{assumption}
%We can formalize the behavior of a crashed process in another way: it can be receive messages but neither do internal computation steps nor send messages. 
%However, the latter encoding requires another requirement about how often crashed process receives messages to ensure that every massage buffer in the system is bound.
%Hence, I think that Assumption \ref{asmp:CrashProc} is more reasonable, and it is more comfortable to specify the system with this assumption.
%Moreover, by applying Assumption \ref{asmp:CrashProc}, we next prove that every message buffer is eventually and forever bound.



%\subsubsection{Bounded message buffers in the postfix} \hfill
%
%%Assume that a correct process can send one message to all in one transition. By Lemma \ref{lem:BoundRcvdMsgDelay} and this assumption, we obtain Lemma \ref{lem:BoundMsgBuf} which says that message buffers of correct processes are eventually bound.
%
%\newcommand{\lemBoundCorrMsgBuf}{
%After the time $\gst{} + \Delta + \Phi_R + 1$, every message buffer has at most $\Omage_S + \Delta + \Phi_R$ messages.
%}
%
%\begin{lemma}
%After the time $\gst + \Delta + \Phi_R + 1$, every message buffer has at $\Phi_S + \Delta + \Phi_S$ messages.
%\end{lemma}

%\begin{proof}
%  Will be adopted.
%\end{proof}
%
%\begin{proof}
%  Let $t$ be a time point after $t_0 + \Delta + \Phi_R$, i.e. $t_0 + \Delta + \Phi_R + 1 \geq t$, and $p$ be a correct process until time $t$. 
%  We prove that the message buffer $\msgbuf{p}$ is bound at time $t$.
%  By Lemma \ref{lem:BoundRcvdMsgDelay}, we have that the message delay at time $t$ is bound by $2 * \Phi_R + \Delta$.
%  By our computational model, we know that every correct process can execute the action $\send{\_}{p}$ at most $2 * \Phi_R + \Delta$ times in the time interval $\sigma = \left[ t - (2 * \Phi_R + \Delta), t \right]$.
%  Moreover, by our assumption every execution $\send{\_}{p}$ can put only one message to the buffer $\msgbuf{p}$.
%  Therefore, the number of messages in $\msgbuf{p}$ at time $t$ is bound by $N * (2 * \Phi_R + \Delta)$.
%\end{proof}
%
%Perhaps the time point $t_0 + \Delta + \Phi_R + 1$ is not the first time every message buffer of a correct process is bound. 
%However, in our work the property that every message buffer is eventually and forever bound is good enough.
%With the crash model described in the previous, we obtain Lemma \ref{lem:BoundMsgBuf} which says that every message buffer is eventually and forever bound.
%
%\begin{figure}[!htb]
%\begin{tikzpicture}
%
%\draw[thick, -Triangle] (0,0) -- (0.9\textwidth,0) node[font=\scriptsize,below left=1pt and -8pt]{\textit{t}};
%
%% draw vertical lines
%\foreach \x in {0,1,...,10}
%\draw (\x cm,3pt) -- (\x cm,-3pt);
%
%\foreach \x/\descr in {3/\textit{GST}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%% colored bar up
%%\foreach \x/\perccol in
%%{0/100,1/75,2/0,3/75}
%%\draw[lightgray!\perccol!red, line width=4pt] 
%%(\x,.5) -- +(1,0);
%%\draw[-Triangle, dashed, red] (4,.5) --  +(4,0);
%
%\foreach \x/\perccol in
%{9/0,10/0}
%\draw[lightgray!\perccol!blue, line width=4pt]
%(\x,-0.4) -- +(1,0);
%
%
%% colored bar down
%%\foreach \x/\perccol in
%%{3/100,4/75,5/0}
%%\draw[lightgray!\perccol!green, line width=4pt] 
%%(\x,-.7) -- +(1,0);
%%\draw[-Triangle, dashed, green] (6,-.7) --  +(1,0);
%
%% braces
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (3,0.4)  -- +(3,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Delta$};
%
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (6,0.4)  -- +(2,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Phi_R$};
%
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (11,-.7) -- +(-2,0)
%node [black,midway,font=\scriptsize, below=4pt] {Bounded message buffers};
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (2,-.7) -- +(-2,0)
%node [black,midway,font=\scriptsize, below=4pt] {Unbounded message buffers};
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (8,-.7) -- +(-5,0)
%node [black,midway,font=\scriptsize, below=4pt] {Perhaps still unbounded message buffers?};
%\end{tikzpicture}
%\caption{Message buffers are unbounded before $\gst{}$. However, they are eventually and forever bounded.}
%\label{fig:MsgBuf}
%\end{figure}
%
%\begin{lemma} \label{lem:BoundMsgBuf}
%  Under Assumption \ref{asmp:CrashProc}, every message buffer is eventually and forever bound.
%\end{lemma}
%
%\begin{proof}
%It follows immediately by Lemma \ref{lem:BoundCorrMsgBuf} and Assumption \ref{asmp:CrashProc}.
%\end{proof}




==> netys20/id-sep.tex <==
%From now on, we use the notations:
%\begin{itemize}
%
%  \item  $S_{\mathit{IDs}}\left(\Delta, \Phi\right)$: describes a partially synchronous system 
%  which satisfies Constraints \ref{const:DP}--\ref{const:NoRecover}, and
%  has $\vert \mathit{IDs} \vert$ processes with unique IDs.
%  Whenever the context is clear, we simply write $S_{\mathit{IDs}}$.
%  For example, $S_{\left\{i, j\right\}}$ is a system with two processes $p_i$ and $p_j$, 
%  and $S_{1..N}$ is another system with $N$ processes $p_1, \ldots, p_N$.
%  
%  \item  $\mathit{Receive}(p_i) \left[ p_j\right]$: mentions messages from process $p_j$ 
%  which process $p_i$ has received after executing the operator $\mathit{Receive}(p_i)$.
%  
%  \item $s\left(p_i, X\right)$: is the value of local variable $X$ of process $p_i$ in global state $s$.
%  For example, the notation $s_{10}(p_1, \mathit{suspected}[p_2])$ describes whether process $p_1$ suspects process $p_2$ in global state $s_{10}$ where $\mathit{suspected}$ is a one--dimensional array.
%  Moreover, we override the notation $s\left(p_i, \mathit{Receive}(p_i) \left[ p_j\right] \right)$ to mention messages from process $p_j$ which process $p_i$ has received in global state $s$.
%  
%  \item $s\left(\mathit{msgBuf}[i, j]\right)$: messages in transit in $\mathit{msgBuf}[i, j]$ in state $s$.
%
%\end{itemize}

The ``ID--separated'' subclass contains partially synchronous distributed algorithms which satisfy following constraints:
\begin{enumerate}
  \item\label{const:DP} These parameters $\Delta$ and $\Phi$ hold eventually for some fixed values.

  
  \item\label{const:OmegaS} Every correct process executes the operator $\tsnd$ at least once 
  in every local time interval $\left[ t, t + \Omega \right]$ where $0 \leq t, 0 < \Omega$.

  
  \item\label{const:OmegaR} Every correct process executes the operator $\rop{}$ at least once 
  in every local time interval $\left[ t, t + \Omega \right]$ where $0 \leq t, 0 < \Omega$.
  
  \item Every local variable $X_i$ is a one-dimensional one in the form of $X_i[\mathit{id}_1, \ldots, \mathit{id}_n]$ 
  where $\left\{ \mathit{id}_1, \ldots, \mathit{id}_n \right\}$ is the set of process IDs, and $1 \leq i \leq m$.
  
  \item Instead of ``send--to--one'', when a process $p$ sends a message $m$, this message is sent to every process.  
  Therefore, we introduce a predicate $\texttt{Send}(p, m)$ and its evaluation at a~\tsnd{} configuration $\confsnd{t}$ can be interpreted as
  \begin{alignat*}{3}
  \forall p, q \ldotp & \, && \,  m \notin \confsched{t} \left( \buf{p}{q}\right)   \\
   &  \, \land && \, \confsnd{t} \left( \buf{p}{q}\right) = \left\{ m \right\} \cup \confsched{t} \left( \buf{p}{q}\right) 
   \end{alignat*}
    Notice that this assumption applies to the behavior of both correct processes and faulty ones.
    
  \item For each local variable $X_\ell$, there exists an $(M + 4)$--ary function $f_\ell$  such that for every transition $s \xrightarrow{\texttt{Rnd}} s^{\prime}$ where $s, s^{\prime}$ are global or intermediate states, and for every pair of processes $p_i$ and $p_j$, it follows 
  \begin{align*}
    s^{\prime}( p_i ).X_\ell [p_j] = f_\ell \big( \texttt{Rnd}, s(p_i).\lpc, &  s(\gpc \left[ p_i \right]), s^{\prime}.\rop{p_i}[p_j], \\
    & s ( p_i ).X_1, \ldots, s( p_i).X_M \big)   
  \end{align*}
  Intuitively, the update of $s^{\prime}(p_i).X_\ell[p_j]$ on only the current subround, what subround a process $p_i$ joins, its received messages from a process $p_j$, and the values of its local variables at an index $p_j$ in the current configuration.
%
%  \item\label{const:SendToAll} The primitive operator $\mathit{Send} (p)$ is \emph{send--to--others}, and it sends only one message to another whenever being executed.
%  Formally, if process $p_i$ executes $\mathit{Send}(p_i)$ to send message $m$ to others, we have that 
%  \[
%    \forall p_j \ldotp p_i \neq p_j \Rightarrow \mathit{msgBuf}^{\prime}[i,j] = \mathit{msgBuf}[i,j] \cup \left\{ m \right\}
%  \]
%   
%  \item\label{const:RmvdMsg} After being delivered, a set $S$ of messages are removed from the corresponding message buffer.  
%  Formally, we have that 
%  \[
%    \forall p_j \ldotp \mathit{mailbox}^{\prime}[p_i, p_j] \cap \mathit{msgBuf}^{\prime}[p_j, p_i] = \emptyset
%  \]
%  
%  \item\label{const:NoRecover} Only fail-stop-without-restart faults are considered in this computational model.
%  
%  \item\label{const:Separation} An algorithm must satisfy the \emph{``ID--separated''} constraints whose definition is given later. 
%  Intuitively, every local variable is a one-dimensional variable such that
%  it can be divided and grouped by processes' ID, and
%  each group is updated independently. 
  
  
%  \item\label{const:CrashModel} When process $p$ crashes, 
%  all of its message buffer $\msgbuf{\_, p}$ is clean empty immediately, 
%  and from now on no messages are stored in its buffer.
\end{enumerate}

%
%\emph{Useful notations.} In order to present partially syncronous constraints precisely with logical formulas, we introduce folllowing notations:
%
%\begin{itemize}
%  \item $\sigma_k$: a global state at a time $k$. 
%  
%  \item The notation $\gconf{t}(p_i)$ refers to the local state of process $p_i \in \proc$ at a time $t$.
%  Moreover, the notation $\gconf{t}(p_i).X$ refers to the value of the local variable $X$ of process $p_i$ at a time $t$.
%  If $X$ is an one-dimensional array, we would write $\gconf{t}(p_i).X[\mathit{id}]$ to refer to the value of $X$ at the index $\mathit{id}$.
%  
%  \item The notation $\gconf{t}(X)$ refers to $X$'s value at a time $t$ for each global variable $X$.
%  
%  \item Since processes can do different actions in a global step, we introduce an additional system variable~\pc{} to describe processes' status. Formally, we have $\pc{} : \proc \rightarrow \status$ where $\status = \left\{\inactive, \cop, \sop, \rop  \right\}$.
%  If $\gconf{t}\left(\pc\left(p_i\right)\right) =  \inactive$, then process $p_i$ does not take a step at a time $t$.
%  Moreover, if $\gconf{t}\left(\pc\left(p_i\right)\right) =  \cop$, then process $p_i$ does only internal computation, and neither~\sop{} no~\rop{} is executed by process $p_i$ at a time $t$.
%  In other cases where $\gconf{t}\left(\pc\left(p_i\right)\right) \in \left\{ \sop, \rop \right\}$, after process $p_i$ executes a corresponding operator, it can do additional internal computation.
%  Notice that the definition of~\pc{} is consistent with the constraint where a process cannot execute both~\sop{} and~\rop{} in a global tick.
%  
%  \item We assume that there exists an one-dimensional local variable called~\mailbox{} to store all received messages. 
%  Variable~\mailbox{} is indexed by processes' ID, and delivered messages are classified based on senders.
%  For example, $\gconf{t}(p_i).\mailbox[p_j]$ is a set of delivered messages from process $p_j$ to process $p_i$ at a time $t$. 
%  The above constraint on~\mailbox{} can be formalized as
%  \[
%  \forall t  \, \forall p_i, p_j, p_k \ldotp p_j \neq p_k \Rightarrow \gconf{t}(p_i).\mailbox[p_j] \cap \gconf{t}(p_i).\mailbox[p_k] = \emptyset
%  \]
%  
%  \item A function $\age : \msg \rightarrow \mathbb{N}$ to describe a time-unit old of a message where~\msg{} is a set of possible messages and $\mathbb{N}$ is a set of natural number (with 0). In our model, when new messages appears, their ages are 0 time--unit old, and the age of every in--transit message is increased by 1 in every global tick. Formally, we have
%  \begin{align*}
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp & \left( m \notin \gconf{t}\left( \buf{p_i}{p_j} \right) \land m \in \gconf{t + 1}\left( \buf{p_i}{p_j} \right) \right)\\
%  & \qquad \Rightarrow \gconf{t + 1}(\age (m) ) = 0  \\
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp & \left( m \in \gconf{t}\left( \buf{p_i}{p_j} \right) \land m \in \gconf{t + 1}\left( \buf{p_i}{p_j} \right) \right)\\
%  & \qquad \Rightarrow \gconf{t + 1}(\age (m) ) = \gconf{t + 1}(\age (m) ) + 1
%  \end{align*}  
%\end{itemize}
%

%\begin{definition}
%Let $\mathcal{A}$ be an arbitrary partially synchronous distributed algorithm. 
%Assume that every process has $m$ local variables $X_1, \ldots, X_M$.
%Algorithm $\mathcal{A}$ is called \emph{``ID--separated''} if
%\begin{enumerate}
%  \item Every local variable $X_i$ is a one-dimensional one in the form of $X_i[\mathit{id}_1, \ldots, \mathit{id}_n]$ 
%  where $\left\{ \mathit{id}_1, \ldots, \mathit{id}_n \right\}$ is the set of process IDs, and $1 \leq i \leq m$.
%  \item There exists a function $(m + 1)$--ary $f$ for each local variable $X_\ell$ such that the following condition is hold in every path $\pi = s_0 s_1 \ldots$ where $s_i$ is an global state:
%  For every $k > 0$, for every pair of processes $p_i$ and $p_j$, 
%  it follows that 
%  \begin{align*}
%  s_k \left( p_i, X_\ell[p_j] \right) = f \big(s_k \left( p_i, \mathit{Receive(p_i)}[p_j] \right), \, & s_{k-1} \left( p_i, X_1[p_j] \right), \ldots, \\
%  & s_{k-1} \left( p_i, X_M[p_j] \right)  \big)   \end{align*}
%  
%  
%\end{enumerate}

%\end{definition}  

While ``ID--separated'' constraints look restricted, this subclass contains many well-known algorithms, e.g. failure detectors \cite{CT96,AguileraDFT08}.
We will provide detailed arguments for this point later \footnote{Don't have a proof for \cite{AguileraDFT08} now. }.

==> netys20/id_sep.tex <==
%From now on, we use the notations:
%\begin{itemize}
%
%  \item  $S_{\mathit{IDs}}\left(\Delta, \Phi\right)$: describes a partially synchronous system 
%  which satisfies Constraints \ref{const:DP}--\ref{const:NoRecover}, and
%  has $\vert \mathit{IDs} \vert$ processes with unique IDs.
%  Whenever the context is clear, we simply write $S_{\mathit{IDs}}$.
%  For example, $S_{\left\{i, j\right\}}$ is a system with two processes $p_i$ and $p_j$, 
%  and $S_{1..N}$ is another system with $N$ processes $p_1, \ldots, p_N$.
%  
%  \item  $\mathit{Receive}(p_i) \left[ p_j\right]$: mentions messages from process $p_j$ 
%  which process $p_i$ has received after executing the operator $\mathit{Receive}(p_i)$.
%  
%  \item $s\left(p_i, X\right)$: is the value of local variable $X$ of process $p_i$ in global state $s$.
%  For example, the notation $s_{10}(p_1, \mathit{suspected}[p_2])$ describes whether process $p_1$ suspects process $p_2$ in global state $s_{10}$ where $\mathit{suspected}$ is a one--dimensional array.
%  Moreover, we override the notation $s\left(p_i, \mathit{Receive}(p_i) \left[ p_j\right] \right)$ to mention messages from process $p_j$ which process $p_i$ has received in global state $s$.
%  
%  \item $s\left(\mathit{msgBuf}[i, j]\right)$: messages in transit in $\mathit{msgBuf}[i, j]$ in state $s$.
%
%\end{itemize}

\subsection{\idsep{} constraints}

An algorithm under partial synchrony is called ``ID--separated'' if and only if it satisfies following constraints:
\begin{enumerate}
  \item\label{const:DP} These parameters $\Delta$ and $\Phi$ hold eventually for some fixed values.

  
%  \item\label{const:OmegaS} Every correct process executes the \snd{} operator $\tsnd$ at least once 
%  in every local time interval $\left[ t, t + \Omega \right]$ where $0 \leq t, 0 < \Omega$.

  
%  \item\label{const:OmegaR} Every correct process executes the operator $\rop{}$ at least once 
%  in every local time interval $\left[ t, t + \Omega \right]$ where $0 \leq t, 0 < \Omega$.
  
%  \item For every $k \geq 3$, for every $i \in \nid$, the local variable $x_k[i]$ of a process $p_i$  has type $\mathcal{T}_k \triangleq \nid \rightarrow D_k$ 
%  where $D_k$ is a set of possible values.
%  Recall that $x_1[i], x_2[i]$ are respectively $\pi[i], \mailbox[i]$.
  
%  \item Instead of ``send--to--one'', when a process $p$ sends a message $m$, this message is sent to every process.  
%  Therefore, we introduce a predicate $\texttt{Send}(p, m)$ and its evaluation at a~\snd{} configuration $\confsnd{t}$ can be interpreted as
%  \begin{alignat*}{3}
%  \forall p \forall m \ldotp & \, && (\exists q \ldotp \,  m \notin \confsched{t} \left( \buf{p}{q}\right) \land m \in \confsnd{t} \left( \buf{p}{q}\right) ) \\
%   &  \, \Rightarrow && \big( \, \quad \confsched{t}(\gpc[p]) \land  \confsched{t}(p).\lpc = \tsnd{} \\
%   &  \,  &&  \;\; \land  \forall q_1 \ldotp  \, m \notin \confsched{t} \left( \buf{p}{q_1}\right) \land m \in \confsnd{t} \left( \buf{p}{q_1}\right) \\
%   &  \,  &&  \;\; \land  \forall q_1 \ldotp  \card{ \confsched{t} \left( \buf{p}{q_1}\right) } + 1 = \card{ \confsnd{t} \left( \buf{p}{q_1}\right) }\\
%   &  \,  &&  \;\; \land  \forall p^{\prime} \ldotp \, p^{\prime} \neq p \Rightarrow \forall q_1 \ldotp  \confsnd{t} \left( \buf{p_i}{p^{\prime}}\right) = \confsched{t} \left( \buf{p_i}{p^{\prime}}\right)\big)
%   \end{alignat*}
%  \begin{align*}
%    \, & \forall p_j \ldotp \,   m \notin \confsched{t} \left( \buf{p_i}{p_j}\right)   \\
%    \land \, &   \forall p_j \ldotp \, \confsnd{t} \left( \buf{p_i}{p_j}\right) = \left\{ m \right\} \cup \confsched{t} \left( \buf{p_i}{p_j}\right) 
%  \end{align*}
%  Notice that this assumption applies to the behavior of both correct processes and faulty ones.
    
  \item For every $k \geq 3$, a variable $x^U_k$ in the process template $U$ is a one--dimensional array with types $\mathcal{T}_k \triangleq \nid \rightarrow D_k$ where $D_k$ is a set of values. \footnote{Recall that the first varible of a process template is instanced to the current instruction block $\pc[i]$ of a process $p_i$, the second one is instanced to message storages $\mailbox[i]$.}
%  Recall that $x_1[i], x_2[i]$ are respectively $\pc[i], \mailbox[i]$, and 
%  $m$ is the number of local variables.
    
%  \item For every local variable $x_k$ where $k \geq 3$, there exists  an $(m + 2)$--ary function $f_k$  such that for every internal transition $\conf_1 \xrightarrow{\texttt{Name}} \conf_2$, for every $i, j \in \nid $, it follows 
%  \begin{align*}
%    \conf_2( x_k[i, j] ) = f_k \big( \texttt{Name}, & \conf_1(\act[i]), \conf_1(\pc[i]),   \\
%    & \conf_2(\mailbox[i, j]), \conf_1(x_3[i, j]), \ldots, \conf_1(x_m[i, j]) \big)   
%  \end{align*}
  \item A process template has only one initial configuration $\rho_0$ such that 
  \begin{align*}
  & \rho_0(x^U_1) = L_S \\
  \land \, & \forall j \in \nid \colon \rho_0(x^U_2[j]) = \emptyset \\
  \land \, & \forall k \in 3..m \, \exists c_k \in D_k  \colon c = \rho_0(x^U_k[1]) = \ldots = \rho_0(x^U_k[N]) 
  \end{align*}
  where $c_k$ is a constant.
  
  \item There exists a function $g_1 \colon \mathit{BL} \rightarrow \mathit{BL}$, there exists a function $g_2 \colon \mathit{BL} \rightarrow \msg$, and for every $k \geq 3$ there exists an $m$--ary function $f_k \colon \mathit{BL} \times \texttt{Set}(\msg) \times D_3 \times D_m \rightarrow D_k $   such that for every pair of process configurations $\rho, \rho^{\prime} \in \Sigma^U$, for every $S_1, \ldots, S_N \subseteq \msg$, for every $m \in \msg$, it follows
  \begin{alignat*}{3}
    & && (\rho^{\prime}, \{m\})  = \localnext(\rho, S_1, \ldots, S_N) \\
    \Leftrightarrow \Big( &  && \rho^{\prime}(x^U_1) = g(\rho(x^U_1)) \\
    & \, \land \, && m = g_2(\rho(\pc)) \\
    & \, \land \, && \forall j \in \nid \colon \rho^{\prime}(x^U_2[j]) = \rho(x^U_2[j]) \cup S_j \\ 
    & \, \land \, && \forall j \in \nid \colon \rho^{\prime}(x^U_3)[j] = f_3 \big( \rho(x^U_1),  \rho^{\prime}(x^U_2[j]), \rho(x^U_3[j]), \ldots, \rho(x^U_m[j]) \big)  \\ 
    &  && \ldots \\    
    & \, \land \, && \forall j \in \nid \colon \rho^{\prime}(x^U_m)[j] = f_m \big( \rho(x^U_1),  \rho^{\prime}(x^U_2[j]), \rho(x^U_3[j]), \ldots, \rho(x^U_m[j]) \big) \Big) 
  \end{alignat*}

  Intuitively, the existence of a function $g_1, g_2$ implies that the update of a variable $x^U_1$ and the construction of a message $m$ depend on only $\rho(\pc.)$.
  In other words, they are independent from other variables.
%  \footnote{We can define a function $g$ as $rho^{\prime}(x^U_1) = g(\rho(x^U_1), \bigcup_{j \in \nid }S_i) $. } 
  The existence of a function $f_k$ implies that the value of $\rho(x^U_k[j])$  depends on only the current instruction block, a set of messages which has been delivered and stored in $\rho^{\prime}(x^U_2[j])$, and values of local variables at an index $j$, which are $x^U_3[j], \ldots, x^U_m[j]$  in the configuration $\rho$.
  Finally, the function $\localnext$ can be defined by the combination of functions $f_3, \ldots, f_m$.
  

  
  \item A global transition system has only one initial configuration $\conf_0$ such that  
  \begin{align*}
  & \conf_0(\gc) = 0 \\
  \land \, & \forall i \in \nid \colon \lnot \conf_0(\act[i) \land I_i \\
  \land \, & \forall i, j \in \nid \colon \conf_0(\buf[i, j]) = \emptyset 
  \end{align*}
  where $I_i$ is a predicate for the initial configuration of a process $p_i$.
  
  \item The faults are clean--crash.
%
%  \item\label{const:SendToAll} The primitive operator $\mathit{Send} (p)$ is \emph{send--to--others}, and it sends only one message to another whenever being executed.
%  Formally, if process $p_i$ executes $\mathit{Send}(p_i)$ to send message $m$ to others, we have that 
%  \[
%    \forall p_j \ldotp p_i \neq p_j \Rightarrow \mathit{msgBuf}^{\prime}[i,j] = \mathit{msgBuf}[i,j] \cup \left\{ m \right\}
%  \]
%   
%  \item\label{const:RmvdMsg} After being delivered, a set $S$ of messages are removed from the corresponding message buffer.  
%  Formally, we have that 
%  \[
%    \forall p_j \ldotp \mathit{mailbox}^{\prime}[p_i, p_j] \cap \mathit{msgBuf}^{\prime}[p_j, p_i] = \emptyset
%  \]
%  
%  \item\label{const:NoRecover} Only fail-stop-without-restart faults are considered in this computational model.
%  
%  \item\label{const:Separation} An algorithm must satisfy the \emph{``ID--separated''} constraints whose definition is given later. 
%  Intuitively, every local variable is a one-dimensional variable such that
%  it can be divided and grouped by processes' ID, and
%  each group is updated independently. 
  
  
%  \item\label{const:CrashModel} When process $p$ crashes, 
%  all of its message buffer $\msgbuf{\_, p}$ is clean empty immediately, 
%  and from now on no messages are stored in its buffer.
\end{enumerate}

%
%\emph{Useful notations.} In order to present partially syncronous constraints precisely with logical formulas, we introduce folllowing notations:
%
%\begin{itemize}
%  \item $\sigma_k$: a global state at a time $k$. 
%  
%  \item The notation $\gconf{t}(p_i)$ refers to the local state of process $p_i \in \proc$ at a time $t$.
%  Moreover, the notation $\gconf{t}(p_i).X$ refers to the value of the local variable $X$ of process $p_i$ at a time $t$.
%  If $X$ is an one-dimensional array, we would write $\gconf{t}(p_i).X[\mathit{id}]$ to refer to the value of $X$ at the index $\mathit{id}$.
%  
%  \item The notation $\gconf{t}(X)$ refers to $X$'s value at a time $t$ for each global variable $X$.
%  
%  \item Since processes can do different actions in a global step, we introduce an additional system variable~\pc{} to describe processes' status. Formally, we have $\pc{} : \proc \rightarrow \status$ where $\status = \left\{\inactive, \cop, \sop, \rop  \right\}$.
%  If $\gconf{t}\left(\pc\left(p_i\right)\right) =  \inactive$, then process $p_i$ does not take a step at a time $t$.
%  Moreover, if $\gconf{t}\left(\pc\left(p_i\right)\right) =  \cop$, then process $p_i$ does only internal computation, and neither~\sop{} no~\rop{} is executed by process $p_i$ at a time $t$.
%  In other cases where $\gconf{t}\left(\pc\left(p_i\right)\right) \in \left\{ \sop, \rop \right\}$, after process $p_i$ executes a corresponding operator, it can do additional internal computation.
%  Notice that the definition of~\pc{} is consistent with the constraint where a process cannot execute both~\sop{} and~\rop{} in a global tick.
%  
%  \item We assume that there exists an one-dimensional local variable called~\mailbox{} to store all received messages. 
%  Variable~\mailbox{} is indexed by processes' ID, and delivered messages are classified based on senders.
%  For example, $\gconf{t}(p_i).\mailbox[p_j]$ is a set of delivered messages from process $p_j$ to process $p_i$ at a time $t$. 
%  The above constraint on~\mailbox{} can be formalized as
%  \[
%  \forall t  \, \forall p_i, p_j, p_k \ldotp p_j \neq p_k \Rightarrow \gconf{t}(p_i).\mailbox[p_j] \cap \gconf{t}(p_i).\mailbox[p_k] = \emptyset
%  \]
%  
%  \item A function $\age : \msg \rightarrow \mathbb{N}$ to describe a time-unit old of a message where~\msg{} is a set of possible messages and $\mathbb{N}$ is a set of natural number (with 0). In our model, when new messages appears, their ages are 0 time--unit old, and the age of every in--transit message is increased by 1 in every global tick. Formally, we have
%  \begin{align*}
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp & \left( m \notin \gconf{t}\left( \buf{p_i}{p_j} \right) \land m \in \gconf{t + 1}\left( \buf{p_i}{p_j} \right) \right)\\
%  & \qquad \Rightarrow \gconf{t + 1}(\age (m) ) = 0  \\
%  \forall t  \, \forall p_i, p_j \forall m  \ldotp & \left( m \in \gconf{t}\left( \buf{p_i}{p_j} \right) \land m \in \gconf{t + 1}\left( \buf{p_i}{p_j} \right) \right)\\
%  & \qquad \Rightarrow \gconf{t + 1}(\age (m) ) = \gconf{t + 1}(\age (m) ) + 1
%  \end{align*}  
%\end{itemize}
%

%\begin{definition}
%Let $\mathcal{A}$ be an arbitrary partially synchronous distributed algorithm. 
%Assume that every process has $m$ local variables $X_1, \ldots, X_M$.
%Algorithm $\mathcal{A}$ is called \emph{``ID--separated''} if
%\begin{enumerate}
%  \item Every local variable $X_i$ is a one-dimensional one in the form of $X_i[\mathit{id}_1, \ldots, \mathit{id}_n]$ 
%  where $\left\{ \mathit{id}_1, \ldots, \mathit{id}_n \right\}$ is the set of process IDs, and $1 \leq i \leq m$.
%  \item There exists a function $(m + 1)$--ary $f$ for each local variable $X_\ell$ such that the following condition is hold in every path $\pi = s_0 s_1 \ldots$ where $s_i$ is an global state:
%  For every $k > 0$, for every pair of processes $p_i$ and $p_j$, 
%  it follows that 
%  \begin{align*}
%  s_k \left( p_i, X_\ell[p_j] \right) = f \big(s_k \left( p_i, \mathit{Receive(p_i)}[p_j] \right), \, & s_{k-1} \left( p_i, X_1[p_j] \right), \ldots, \\
%  & s_{k-1} \left( p_i, X_M[p_j] \right)  \big)   \end{align*}
%  
%  
%\end{enumerate}

%\end{definition}  

While ``ID--separated'' constraints look restricted, this subclass contains many well-known algorithms, e.g. failure detectors \cite{CT96,AguileraDFT08}.

\subsection{Example: Failure detectors}

==> netys20/id_separated.tex <==


In this section, we first show that two instances $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1, 2}(\mathcal{A},  \Delta, \Phi)$ of an arbitrary ``ID--separated'' algorithm $\mathcal{A}$ are trace equivalent.
It implies there exists a cutoff from $N$ to 2 for the number of processes.




To prove the trace equivalence of $S_{1..N}(\Delta, \Phi)$ and $S_{1, 2}(\Delta, \Phi)$, we first define two techniques for path constructions called ``IDs--projection'' and ``IDs--refillment''.
Lemmas \ref{lem:IDsProj} and \ref{lem:IDsRefill} shows that finite execution paths constructed with these techniques are legal ones in corresponding system instances.
Such results are extended for infinite paths in Lemmas  \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}

\subsection{Path constructions}

\begin{definition}
Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ and $\pi^2 = \gconf{0}^2 \gconf{1}^2 \ldots$ be arbitrary infinite execution paths of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$, respectively.
Path $\pi^2$  is called a \emph{\proj{k}} of path $\pi^N$ if the following property hold:

\begin{enumerate}
  \item The global stabilization time of two paths are the same.
    
  \item For every $i \in \{p_1, p_2\}$, it follows $\gconf{k}^N(\gpc[p_i]) = \gconf{k}^2(\gpc[p_i])$.
  
  \item For every $i, j \in \{1, 2\}$, it follows $\gconf{k}^N(\buf{p_i}{p_j}) = \gconf{k}^2(\buf{p_i}{p_j})$.
  
%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if process $p_i^N$ receives a set of messages $\mathit{Msgs}$ in state $s^N_k$, then process $p_i^2$ receives a set of messages $\{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ in state $s^2_k$. \footnote{TODO: Override notations here since $m$ is used for different messages in different system instances.}
%  
%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ and $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ are the same.
%  
%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
%  
%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^N$ crashes at time point $k$, then process $p_i^2$ also crashes at time point $k$.
\end{enumerate}

\end{definition}


\newcommand{\lemIDsProj}{
Let $\pi^N = s_0^N \ldots  s_\ell^N$ be an arbitrary finite execution path of $S_{1..N}(\Delta, \Phi)$ for some number $\ell \geq 0$.
There exists a finite path $\pi^2 = s^2_0 \ldots s^2_\ell$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an $\ell$--finite ``IDs--projection'' path of $\pi^N$.
}

\begin{lemma} \label{lem:IDsProj}
\lemIDsProj
\end{lemma}

\begin{proof}
  It is easy to see that the first constraint about the stabilization time is satisfied by the definition of those system instances. 
  In the following, we present how to construct an $\ell$--finite ``IDs--projection'' path of $\pi^N$, and explain how other constraints are satisfied.
  The construction is based on the induction on the length $\ell$ of an execution path. 
  
  \begin{itemize}
  \item \emph{Base case $\ell = 0$}. In the base case, path $\pi^N$ has only the initial state. 
  Lemma \ref{lem:IDsProj} is correct because it is safe to set the initial state of processes and message buffers in $S_{1..2}(\Delta, \Phi)$ such that for every $i, j \in \{1, 2\}$, for every local variable $X$, we have $s_0^N(p_i, X[p_j]) = s_0^2(p_i, X[p_j])$ and $s_0^N(\mathit{msgBuf}^N[i, j]) = s_0^2(\mathit{msgBuf}^N[i, j])$.
  
  \item Assume that Lemma \ref{lem:IDsProj} is correct for the case $\ell_0 \geq 0$. We prove the case $\ell_0 + 1$. By the induction hypothesis, there exists a finite path $\rho$ in $S_{1..2}(\Delta, \Phi)$ such that $\rho$ is an $\ell_0$--finite ``IDs--projection'' path for the prefix $s_0^N \ldots s_{\ell_0}^N$ of $\pi^N$. We will show that we can obtain $\pi^2$ by extending $\rho$ with a reachable state $s^2_{\ell}$. Here (and now) we present only the most complicated case where both $p_1$ and $p_2$ are still correct at time point $\ell$. For other cases where crashes happen, the proof is much simpler. \footnote{TODO: Provide some arguments for cases with crashes.} The construction of $s^2_\ell$ where processes $p^2_1$ and $p^2_2$ are still correct is given below.
  
  \begin{enumerate}
      \item Both processes $\pi^N_i$  and $\pi^2_i$ executes the same action on time point $\ell$ for every $i \in \{1, 2\}$. Notice that the action of $\pi^2_i$ is enable because of the induction hypothesis. As a result, the constraint $\Phi$ still holds in $\pi^2$ until $\ell$. (If not, the constraint $\Phi$ does not hold in the interval $[\ell - \Delta, \ell]$ in the execution path $\pi^N$. Contradiction) Therefore, the extension of $\rho$ in this way constructs a legal finite path which satisfies the second constraint.
      
      \item In the Send round in global tick $\ell$, it is easy that if message $m$ has been added to message bufer $\mathit{msgBuf}^N[i, j]$ for every $1 \leq i, j \leq 2$, then a corresponding message $m$ has been also added to message bufer $\mathit{msgBuf}^2[i, j]$. 
      By the induction hypothesis, it follows that until now message buffers $\mathit{msgBuf}^2[i, j]$ and $\mathit{msgBuf}^N[i, j]$ are the same for every $1 \leq i, j \leq 2$.
      Because our computational model does not allow ``send'' processes to receive any messages and not to join later rounds, we have that 
T      \begin{align*}
       s^N_\ell(p_i, X[p_j]) & = f(\{\}, s^N_{\ell_0}X_1[p_j], \ldots, , s^N_{\ell_0}X_m[p_j]) \text{, and } \\ 
       s^2_\ell(p_i, X[p_j]) & = f(\{\}, s^2_{\ell_0}X_1[p_j], \ldots, , s^2_{\ell_0}X_m[p_j])
      \end{align*}
      for every local variable $X$. Due to the induction hypothesis, we have that $s^N_{\ell_0}X_k[p_j] = s^2_{\ell_0}X_k[p_j]$ for every $k$. It follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$.
      
      \item In the Receive round, if message $m$ from process $p^N_j$ has been delivered to process $p^N_i$ for every $1 \leq i, j \leq 2$, then either message $m$ was already in $\mathit{msgBuf}^N[j, i]$ in $\ell_0$ or message $m$ has been added to $\mathit{msgBuf}^N[j, i]$ in the last Send round.
      In the first case, by induction hypothesis, it follows that $m$ was already in $\mathit{msgBuf}^2[j, i]$  in $\ell_0$. In the later case, by arguments in the second point, it follows that $m$ has been added in $\mathit{msgBuf}^2[j, i]$  in the last Send round.
      Therefore, it is possible for process $p^2_i$ to receive message $m$ in this Receive round.
      In other words, if process $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_\ell$, then it is safe to deliver a set of messages $\mathit{Msgs}^2 = \{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ to process $p_i^2$ in state $s^2_\ell$. 
      Therefore, we can construct $\pi^2$ such that the third constraint holds in $\pi^2$.
      Because processes $p^N_i$ and $p^2_i$ have received the same set of messages in this round, and message buffers $\mathit{msgBuf}^N[i, j]$ and $\mathit{msgBuf}^2[i, j]$ are the same for every $1 \leq i, j \leq 2$ before entering this round, such message buffers are still the same after this round.
      Moreover, by similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is a ``Receive'' process, and $X$ is a local variable.
      
      \item In the Internal Computation round, since (i) no messages are added to any message buffer and (ii) no messages are delivered, the second and third constraints obviously hold.
      By similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is an ``Internal Computation'' process, $1 \leq i, j \leq 2$, and $X$ is a local variable.
     
      \item By the merge of three round, it follows that constraints 2--6 holds by the construction of $\pi^2$.
  \end{enumerate}
  Therefore, Lemma \ref{lem:IDsProj} is correct in case of $\ell$. \footnote{The organization of the definition and proof of Lemma \ref{lem:IDsProj} seems a bit difficult to follow. Perhaps we should split it into smaller trunks.} \qed
  \end{itemize}
\end{proof}

\begin{definition}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
  Let $\pi^2 = s_0^2 \ldots s_\ell^2$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
  A finite execution path $\pi^N = s_0^N \ldots s_\ell^N$ is called a \emph{$\ell$--finite ``IDs--refillment'' path} of $\pi^2$ if the followings hold:
  
  \begin{itemize}
    \item The stabilization  time of two paths are the same.
    
    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ executes an operator $\mathit{Op}$ in state $s^2_k$, then process $p_i^N$ executes the same operator $\mathit{Op}$ in state $s^N_k$.
    
    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if processes $p_i^2$ receives messages $\mathit{Msgs}^2$ in state $s^2_k$, then processes $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_k$ such that
    \[
    \mathit{Msgs}^N = \mathit{Msgs}^2 \cup \{ m \mid m \in \mathit{msgBuf}[j][i] \land j \in 3..N \}
    \]
    
    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ and $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ are the same.
    
    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
    
    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ crashes at time point $k$, then process $p_i^N$ also crashes at time point $k$.
    
    \item For every $j \in 3..N$, process $p_j^N$ never crashes.
    
    \item For every $j \in 3..N$, process $p_j^N$ executes the operator $\mathit{Send}$ in state $s^N_0$.
    
    \item For every $j \in 3..N$,  process $p_j^N$ takes a transition in every global tick.
    
    
    \item For every $0 \leq k \leq \ell$, for every $j \in 3..N$, if process $p_j^N$ executes the operator $\mathit{Receive(j)}$ in state $s^N_k$, then every message which was sent to process $j^N$ and but not received will be delivered to process $p_j^N$ in state $s^N_k$.
    
  \end{itemize}
  
\end{definition}


\newcommand{\lemIDsRefill}{
Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
There exists a finite path $\pi^N = s^N_0 \ldots s^N_\ell$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an $\ell$--finite ``IDs--refillment'' path of $\pi^2$.
}

\begin{lemma} \label{lem:IDsRefill}
\lemIDsRefill
\end{lemma}

\begin{proof}
  The proof of Lemma \ref{lem:IDsRefill} is by the induction on the length $\ell$ of the execution path, and by similar arguments in the proof of Lemma \ref{lem:IDsProj} \qed
\end{proof}

\begin{definition}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary infinite execution path of $S_{1..N}(\Delta, \Phi)$.
  An infinite execution path $\pi^2 = s_0^2 s_1^2 \ldots$ is called an \emph{infinite ``IDs--projection'' path} of $\pi^N$ if for every number $\ell \geq 0$, its prefix $\pi^2 = s_0^2 \ldots s_\ell^2$ is an $\ell$--finite ``IDs--projection'' path of $\pi^N$.
\end{definition}


\newcommand{\lemIDsProjInf}{
  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary legal execution path of $S_{1..N}(\Delta, \Phi)$.
  There exists an infinite path $\pi^2 = s^2_0 s^2_1 \ldots$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an infinite ``IDs--projection'' path of $\pi^N$.
}

\begin{lemma} \label{lem:IDsProjInf}
  \lemIDsProjInf
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:IDsProjInf} by contradiction.
  Assume that no infinite path in $S_{1..2}(\Delta, \Phi)$ is an infinite ``IDs--projection'' path of $\pi^N$.
  Hence, there exists a number $\ell \geq 0$ such that the prefix $s_0^N \ldots s_\ell^N$ has no $\ell$--finite ``IDs--projection'' path. in $S_{1..2}(\Delta, \Phi)$. 
  Contradiction. \qed
\end{proof}


\begin{definition}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..2}(\Delta, \Phi)$  and $S_{1..N}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary infinite execution path of $S_{1..2}(\Delta, \Phi)$.
  An infinite execution path $\pi^N = s_0^N s_1^N \ldots$ is called an \emph{infinite ``IDs--refillment'' path} of $\pi^2$ if for every number $\ell \geq 0$, its prefix $\pi^N = s_0^N \ldots s_\ell^N$ is an $\ell$--finite ``IDs--refillment'' path of $\pi^2$.
\end{definition}


\newcommand{\lemIDsRefillInf}{
  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary legal execution path of $S_{1..2}(\Delta, \Phi)$.
  There exists an infinite path $\pi^N = s^N_0 s^N_1 \ldots$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an infinite ``IDs--refillment'' path of $\pi^2$.
}

\begin{lemma} \label{lem:IDsRefillInf}
  \lemIDsRefillInf
\end{lemma}

\begin{proof}
  By applying similar arguments in the proof of Lemma \ref{lem:IDsProjInf}.
  \qed
\end{proof}

\subsection{A cutoff of the number of processes}

From now on, the notation $\mathit{comp}(p_i, X, p_j, \mathit{val})$ denotes an atomic predicate  which means the local variable $X[p_j]$ of process $p_i$ has the value $\mathit{val}$. 

Moreover the notation $\mathit{comp}(\mathit{msgBuf}[i, j], \mathit{val})$ denotes an atomic predicate  which means the message buff $\mathit{msgBuf}[i, j]$  has the value $\mathit{val}$. 
Such predicates are called ``var--comp'' and ``buffer--comp'', respectively.

\begin{lemma}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``var--comp'' predicate whose indexes are 1 and 2.
  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
\end{lemma}

\begin{proof}
  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
\end{proof}

\begin{lemma}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``buffer--comp'' predicate whose indexes are 1 and 2.
  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
\end{lemma}

\begin{proof}
  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
\end{proof}


\begin{theorem} \label{thm:cutoff}
  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathcal{P}$ be a predicate built on ``var--comp'' and ``buffer--comp'' predicates whose indexes are 1 and 2.
  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathcal{P}$.
\end{theorem}

\begin{proof}
  We prove Theorem \ref{thm:cutoff} by induction on the structure of predicate $\mathcal{P}$. \qed
\end{proof}

%If $\textit{var}$ is one dimensional array, we override the notation by writing $\assgn{\textit{var}}{\{id_1\}}{\textit{val}}$.
%Such predicates are called ``assignment'' ones.



==> netys20/newcutoff.tex <==

In this section, we prove two cutoff results for the number of processes in checking properties $M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i}$  and $M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j}$ 
where $M_N$ is a global transition system defined in Section \ref{sec:GlobalTransSys}, $F_{i}, G_{i, j}$ are arbitrary LTL (linear temporal logic) formulas such that 
predicates in $F_{i}$  inspect only variables with an indexes $i$, and 
predicates in $G_{i, j}$  inspect only variables with two different indexes $i, j$.
These results are obtained with Theorems \ref{thm:NCutoffOneIndex}--\ref{thm:NCutoffTwoIndexes}.


The proof strategies are based on the symmetry properties and automorphisms of the process template and the global transition system. 
The reader can find the definitions of automorphism for states and transition systems in~\cite{emerson1993symmetry,emerson1995reasoning}.
More detailed, the proofs of Theorems \ref{thm:NCutoffOneIndex}--\ref{thm:NCutoffTwoIndexes} are based on following results: 
\begin{itemize}
\item Corollary \ref{cor:SymProcTemp} says that every index permutation on a set $\nid$ is an automorphism of the process template $U$;
  
\item Corollary \ref{cor:SymGlobalSys} says that every index permutation on a set $\nid$ is an automorphism of the transition system $M_N$ for every $N \geq 1$;

\item Corollary \ref{cor:TraceEquiv} says that $M_N, M_2$ are trace equivalent under a set $AP_{1, 2}$ of predicates which inspect only variables whose indexes is $\{1\}$, $\{2\}$, or both $\{1, 2\}$
for every $N \geq 2$.
\end{itemize}




\subsection{Index permutations and~\classname{} systems}

Before presenting theorems and lemmas in details, we would like to remind that the application of a permutation  $\perm$ to an indexed object $b$ is obtained from $b$ by simultaneously replacing every occurrence of index $i \in \nid$ by $\perm(i)$.
We overload the permutation by writing $\perm b$ to refer a new object constructed from a object $b$ by applying a permutation $\perm$ to $b$.

If $b$ is an unindexed object, then we have $\perm(b) = b$ for every permutation $\perm$. 
Recall that every message is unindexed.
Moreover, by definition of the process template, every cell in a global two--dimensional variable $x_k$ contains only unindexed values for every $3 \leq k \leq m$.



Lemma \ref{lem:PermArr} shows how a new array $\perm y$ is constructed from an array $y$ with type $\nid \rightarrow \mathcal{T}$ and a permutation $\perm$ where $\mathcal{T}$ is a set of unindexed values.
For example, assume $\conf(\pc) = [L_S, L_C, \loccrash]$ and $\perm = \{ 1 \mapsto 2, 2 \mapsto 1, 3 \mapsto 3\}$.
For a better reading, we rewrite $\conf(\pc)$ as $[1 \mapsto L_S, 2 \mapsto L_C, 3 \mapsto \loccrash]$.
Hence, we have 
\begin{align*}
\perm(\conf(\pc)) = \perm\conf(\pc) & = [\perm(1) \mapsto L_S, \perm(2) \mapsto L_C, \perm(3) \mapsto \loccrash] \\
& = [2 \mapsto L_S, 1 \mapsto L_C, 3 \mapsto \loccrash] \\
& = [L_C, L_S, \loccrash]
\end{align*}

\begin{lemma} \label{lem:PermArr}
Let $y$ be an array of type $\tau \colon \nid \rightarrow \mathcal{T}$ where values of type $\mathcal{T}$ are unindexed.
%Assume that $y[i] = c_i$ where $i \in \nid, c_i \in \mathcal{T}$.
Let $\perm, \perm^{-1}$ be permutations such that $\perm^{-1}$ is a inverse function of $\perm$.
It follows $\perm y = [y[\perm^{-1}(1)],  \ldots, y[\perm^{-1}(N)] ]$.
\end{lemma}

\begin{proof}
For a better reading, we rewrite $y$ as $[1 \mapsto y[1], \ldots, N \mapsto y[N]]$.
It follows $\perm y = [\perm(1) \mapsto y[1], \ldots, \perm(N) \mapsto y[N]]$.
By relocating cells in $\perm y $, we have that
$\perm y = [1  \mapsto y[\perm^{-1}(1)],  \ldots, N \mapsto y[\perm^{-1}(N)] ]$.
\end{proof}

\subsubsection{Index permutations as automorphisms of the process template.}

Let $U_N$ be a process template $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ defined as in Section \ref{sec:ProcTemp}.
Corollary \ref{cor:SymProcTemp} says that every permutation on a set $\nid$ of process indexes is an automorphism of $U$. 
The proof of Corollory \ref{cor:SymProcTemp} requires following lemmas:
\begin{itemize}
\item Lemma \ref{lem:PermProcType} says that the application of a permutation on process indexes to a process configuration generates a process configuration.
\item Lemma \ref{lem:SymTempInitConf} is for the initial process configuration.
\item Lemmas \ref{lem:PermProcSend}--\ref{lem:PermProcStutter} are for process transitions.
\end{itemize}

\newcommand{\corSymProcTemp}{
  Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of $U$.
}

\begin{corollary} \label{cor:SymProcTemp}
  \corSymProcTemp 
\end{corollary}

\begin{proof}
  It immediately follows from Lemmas \ref{lem:SymTempInitConf}--\ref{lem:PermProcStutter}.
\end{proof}

\newcommand{\lemPermProcType}{
  Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$,
  and $\rho \in \pstates{U}{N}$ be a process configuration.
  It follows that $\perm \rho \in \pstates{U}{N}$.
}

\begin{lemma} \label{lem:PermProcType}  
  \lemPermProcType
\end{lemma}

\begin{proof}
It immediately follows by Lemma \ref{lem:PermArr} and that fact that every index permutation preserves type information.
\end{proof}

\newcommand{\lemSymTempInitConf}{
  Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of the initial configuration $\ginitstate{N}$.
}

\begin{lemma} \label{lem:SymTempInitConf}
  \lemSymTempInitConf
\end{lemma}

\begin{proof}
It immediately follows by definition of $\pinitstate{U}{N}$. \qed
\end{proof}

\newcommand{\lemPermProcSend}{
Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}.
Let $m \in \msg$ be a message, and $\rho_0, \rho_1$ be process configurations in $\pstates{U}{N}$ such that $\rho_0 \procsnd{m} \rho_1$.
Let $\perm$ be a permutation on $\nid$.
It follows that $\perm \rho_0 \procsnd{m} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcSend}
\lemPermProcSend
\end{lemma}

\begin{proof}
We prove Lemma \ref{lem:PermProcSend} by utilizing the  properties of~\classname{} functions.
First, we have 
\begin{alignat*}{3}
\perm\rho_1(\pc^U) & = \rho_1(\pc) && \quad \text{(by } \rho_1(\pc^U) \text{ is an unindexed value)} \\
& = g_1(\rho_0(\pc^U)) && \quad \text{(by definition of function $g_1$)}              \\
& = g_1(\perm\rho_0(\pc^U)) && \quad \text{(by } \rho(\pc^U) \text{ is an unindexed value)}              
\end{alignat*}

We now check the $\mailbox$. 
Let $i$ be an arbitrary index in $\nid$.
It follows
\begin{alignat*}{3}
\perm\rho_1(\mailbox^U[i]) & = \rho_1(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = \rho_0(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by definition of $\procsnd{m}$)}              \\
& = \perm\rho_0(\mailbox^U[i])  && \quad \text{(by Lemma \ref{lem:PermArr})}  
\end{alignat*}
Hence, we have $\forall i \in \nid \colon \perm\rho_1(\mailbox^U[i]) = \perm\rho_0(\mailbox^U[i])$.

We now focus on a two--dimensional variable $x^U_3$.
Again, let $i$ be an arbitrary index in $\nid$. It follows
\begin{alignat*}{3}
\perm\rho_1(x^U_3[i]) & = \rho_1(x^U_3[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
& = f_3 \big( \rho_0(x^U_1),  \rho_1(x^U_2[\perm^{-1}(i)]), && \quad \text{(by definition of   $f_3$)}              \\
&  \qquad \rho_0(x^U_3[\perm^{-1}(i)]), \ldots, \rho(x^U_\ell[\perm^{-1}(i)]) \big) &&              \\
& = f_3 \big( \rho_0(\pc^U),  \rho_1(\mailbox^U[\perm^{-1}(i)]), && \quad \text{(by renaming)}              \\
& \qquad \rho_0(x^U_3[\perm^{-1}(i)]), \ldots, \rho_0(x^U_\ell[\perm^{-1}(i)]) \big) &&      \\
& = f_3 \big( \perm\rho_0(\pc^U),  \perm \rho_1(\mailbox^U[i]), && \quad \text{(by Lemma \ref{lem:PermArr})}              \\
& \qquad \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big) &&           
\end{alignat*}
Hence, we have 
\begin{align*}
\forall i \in \nid \colon \perm\rho_1(x^U_3[i]) =  f_3 \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
& \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
\end{align*}
By similar arguments for other variables, we have  
\begin{align*}
\forall k \in 3..\ell \, \forall i \in \nid \colon \perm\rho_1(x^U_k[i]) =  f_k \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
& \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
\end{align*}
%  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
It follows $\perm \rho_0 \procsnd{m} \perm\rho_1$ by the semantics of the transtion $\procsnd{m}$. \qed
\end{proof}


\newcommand{\lemPermProcReceive}{
  Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let $S_1, \ldots, S_N \subseteq \msg$ be $N$ sets of messages, and $\rho_0, \rho_1$ be process configurations such that $\rho_0 \procrcv{S_1}{S_N} \rho_1$. 
  Let $\perm$ be a permutation on $\nid$, and $\perm^{-1}$ be its inverse function.
  It follows that $\perm \rho_0 \procrcv{S_{\perm^{-1}(1)}}{S_{\perm^{-1}(N)}} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcReceive}
  \lemPermProcReceive
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:PermProcReceive} by utilizing the  properties of~\classname{} functions.
  First, we have 
  \begin{alignat*}{3}
  \perm\rho_1(\pc^U) & = \rho_1(\pc) && \quad \text{(by } \rho_1(\pc^U) \text{ is an unindexed value)} \\
  & = g_1(\rho_0(\pc^U)) && \quad \text{(by definition of function $g_1$)}              \\
  & = g_1(\perm\rho_0(\pc^U)) && \quad \text{(by } \rho(\pc^U) \text{ is an unindexed value)}              
  \end{alignat*}
  
  We now check the $\mailbox$. 
  Let $i$ be an arbitrary index in $\nid$.
  It follows
  \begin{alignat*}{3}
  \perm\rho_1(\mailbox^U[i]) & = \rho_1(\mailbox^U[\perm^{-1}(i)]) && \quad \text{(by Lemma \ref{lem:PermArr})}  \\
  & = \rho_0(\mailbox^U[\perm^{-1}(i)]) \cup S_{\perm^{-1}(i)} && \quad \text{(by definition of $\procrcv{S_1}{S_N}$)}              \\
  & = \perm\rho_0(\mailbox^U[i]) \cup S_{\perm^{-1}(i)}  && \quad \text{(by Lemma \ref{lem:PermArr})}  
  \end{alignat*}
  Hence, we have $\forall i \in \nid \colon \perm\rho_1(\mailbox^U[i]) = \perm\rho_0(\mailbox^U[i]) \cup S_{\perm^{-1}(i)}$.
  
  By similar arguments in the proof of Lemma \ref{lem:PermProcReceive}, we have  
  \begin{align*}
  \forall k \in 3..\ell \, \forall i \in \nid \colon \perm\rho_1(x^U_k[i]) =  f_k \big( & \perm\rho_0(\pc^U), \perm \rho_1(\mailbox^U[i]),               \\
  & \perm \rho_0(x^U_3[i]), \ldots, \perm \rho_0(x^U_\ell[i]) \big)
  \end{align*}
  %  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
  It follows $\perm \rho_0 \procrcv{S_{\perm^{-1}(1)}}{S_{\perm^{-1}(N)}} \perm\rho_1$. \qed
\end{proof}

The proofs of Lemmas \ref{lem:PermProcComp}--\ref{lem:PermProcStutter} are similar (and simpler) the above proofs of Lemmas \ref{lem:PermProcSend} and \ref{lem:PermProcReceive}.

\newcommand{\lemPermProcComp}{
  Let $U_N = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be process configurations such that $\rho_0 \proccomp \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \proccomp \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcComp}
  \lemPermProcComp
\end{lemma}

\newcommand{\lemPermProcCrash}{
  Let $U_N = = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be process configurations such that $\rho_0 \proccrash{U} \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \proccrash{U} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcCrash}
  \lemPermProcCrash
\end{lemma}

\newcommand{\lemPermProcStutter}{
  Let $U_N = = (\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N})$ be a process template defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be process configurations such that $\rho_0 \procstutter \rho_1$. 
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \procstutter \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermProcStutter}
  \lemPermProcStutter
\end{lemma}

\subsubsection{Index permutations as automorphisms of the global system.}

We now study automorphisms of a global transition system $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ defined as in Section \ref{sec:GlobalTransSys}.
Corollary \ref{cor:SymGlobalSys} says that every permutation on a set $\nid$ of process indexes is an automorphism of $M_N$.
The proof strategy of Corollary \ref{cor:SymGlobalSys} is similar to one of Corollary \ref{cor:SymProcTemp}, and its proof requires following lemmas:
\begin{itemize}
  \item Lemma \ref{lem:PermGlobalType} says that the application of a permutation on process indexes to a global configuration generates a global configuration.
  \item Lemma \ref{lem:SymGlobalInitConf} is for the initial process configuration.
  \item Lemmas \ref{lem:PermGlobalSchedule}--\ref{lem:PermGlobalStutter} are for global internal transitions and stuttering transition.
  \item Lemma \ref{lem:PermGlobalTrans} is for the global observable transition.
\end{itemize}

\newcommand{\corSymGlobalSys}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ defined as in Section \ref{sec:GlobalTransSys}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of $M_N$.
}

\begin{corollary} \label{cor:SymGlobalSys}
  \corSymGlobalSys 
\end{corollary}

\begin{proof}
  It immediately follows from Lemmas \ref{lem:PermGlobalType}--\ref{lem:PermGlobalStutter}.
\end{proof}

\newcommand{\lemPermGlobalType}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$,
  and $\rho \in \gstates{U}$ be a process configuration.
  It follows that $\perm \rho \in \gstates{U}$.
}

\begin{lemma} \label{lem:PermGlobalType}  
  \lemPermGlobalType
\end{lemma}

\begin{proof}
  It immediately follows by Lemma \ref{lem:PermArr} and that fact that every index permutation preserves type information.
\end{proof}

\newcommand{\lemSymGlobalInitConf}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}, 
  and $\perm$ be a permutation on $\nid$.
  A permutation $\perm$ is an automorphism of the initial configuration $\ginitstate{N}$.
}

\begin{lemma} \label{lem:SymGlobalInitConf}
  \lemSymGlobalInitConf
\end{lemma}



\begin{proof}
  By definition, we have
  \begin{align*}
  \perm (\ginitstate{N})  & = (\perm (\ginitstate{N}(\act)), \perm (\ginitstate{N}(\buf)), \perm (\ginitstate{1}(x_1)) \ldots , \perm( \ginitstate{N}(x_\ell)))
  \end{align*}
  Since $\forall i \in \nid \colon \ginitstate{N}(\act[i]) = \False$, it follows that 
  \[
  \forall i \in \nid \colon (\perm\ginitstate{N})(\act[\perm(i)]) = \False
  \]
  Hence, we have $\perm(\ginitstate{N}(\act)) = \ginitstate{N}(\act)$ .
   
  We have $\perm(\ginitstate{N}(\buf)) = \ginitstate{N}(\buf)$, and $\perm(\ginitstate{N}(x_k)) = \ginitstate{N}(x_k)$ for every $1 \leq k \leq m$  by similar arguments.
  Hence, it follows $\perm(\ginitstate{N}) = \ginitstate{N}$.
  \qed
\end{proof}

\newcommand{\lemPermGlobalSchedule}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \transsched \rho_1$.
  Let $\perm$ be a permutation on $\nid$.
  It follows that (a) $\perm \rho_0 \transsched \perm \rho_1$, and (b) if a process $p_i$ is crashed in $\conf_1$, then a process $p_{\perm(i)}$ is  crashed in $\perm \conf_1$.
}

\begin{proof}
  content...
\end{proof}

\begin{lemma} \label{lem:PermGlobalSchedule}
  \lemPermGlobalSchedule
\end{lemma}

\begin{proof}
  For every $i \in \nid$, we have 
  \[  \perm\conf_0(\act[\perm(i)]) = \conf_0(\act[i]) = \False \]
  Hence, a subround Schedule can start with a configuration $\perm \conf_0$.
  Now we focus on process transitions. By Lemmas \ref{lem:PermArr} and \ref{lem:PermProcCrash} and \ref{lem:PermProcStutter}, we have
  \begin{alignat*}{3}
  & \perm\conf_1(\pc[\perm(i)])  = \conf_1(\pc[i]) 
  && \\
   \land \, &  \perm\conf_0(\pc[\perm(i)])  = \conf_0(\pc[i])  && \\
  \land \, & \pcreate(\conf_0, i) \translocalfault{i} \pcreate(\conf_1, i) && \Rightarrow  \pcreate(\perm \conf_0, \perm(i)) \translocalfault{\perm(i)} \pcreate(\perm \conf_1, \perm(i)) \\
  \land \, & \pcreate(\conf_0, i) \translocalstutter{i} \pcreate(\conf_1, i) && \Rightarrow  \pcreate(\perm \conf_0, \perm(i)) \translocalstutter{\perm(i)} \pcreate(\perm \conf_1, \perm(i)) 
  \end{alignat*}
  It implies \ref{lem:PermGlobalSchedule}(b). Now we focus on message buffers.
  For every $i, j \in \nid$, we have
  \begin{alignat*}
  \perm \conf_1(\buf[\perm(i), \perm(j)]) & = \conf_1(\buf[i, j]) && \quad \text{(by Lemma \ref{lem:PermArr})} \\
  & = \conf_0(\buf[i, j]) && \quad \text{(by Schedule constraints)} \\
  & = \perm \conf_0(\buf[\perm(i), \perm(j)]) && \quad \text{(by Lemma \ref{lem:PermArr})} 
  \end{alignat*}
  It implies that every message buffer is unchanged.
  Since every constrain in the subround Schedule hole in $\perm \conf_0$ and $\perm \conf_1$, it follows that Lemma \ref{lem:PermGlobalSchedule}(a) is correct.
  Therefore, Lemma \ref{lem:PermGlobalSchedule} is correct. \qed
\end{proof}

\newcommand{\lemPermGlobalSend}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \transsnd \rho_1$.
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \transsnd \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermGlobalSend}
  \lemPermGlobalSend
\end{lemma}

\begin{proof}
  In order to prove that $\perm \conf_0 \transsnd \perm \conf_1$, we show that all  constraints in the subround Send hold in $\perm \conf_0$ and $\perm \conf_1$.
  The most complicated constraint is for when a correct process $\pcreate(\conf_1, i)$  sends a message $m$ to all in this subround.
  We prove that a process $\pcreate(\perm \conf_1, \perm(i))$ also sends a message $m$ to all, and a message $m$ is also added in corresponding message buffers in $\perm \conf_1$.
  
  By Lemma \ref{lem:PermArr}, we have
  \begin{align*}
  & \perm\conf_1(\pc[\perm(i)])  = \conf_1(\pc[i]) \\
  \, \land \, &  \perm\conf_0(\pc[\perm(i)])  = \conf_0(\pc[i])  \\
  \, \land \, & \perm\conf_1(\act[\perm(i)]) = \conf_1(\act[i])   \\
  \, \land \, &  \perm\conf_0(\act[\perm(i)]) = \conf_0(\act[i]) 
  \end{align*}
  Therefore, a process $\pcreate(\perm\conf_0, \perm(i))$ is enable to send a message to all, and it becomes inactive in $\perm \conf_1$.
  It follows that $ \pcreate(\perm \conf_0, \perm (i)) \procsnd{m} (\perm \conf_1, \perm (i))$ by Lemma \ref{lem:PermProcSend}.
  Now we show that a message $m$ is fresh in every message buffer from $\pcreate(\perm \conf_1, \perm(i))$ in $\perm \conf_1$. By Lemma \ref{lem:PermArr}, it follows that
  \begin{align*}
  \forall i, j \in \nid \colon & \conf_0(\buf[i, j]) = \perm \conf_0(\buf[\perm(i), \perm(j)]) \\
  \forall i, j \in \nid \colon & \conf_1(\buf[i, j]) = \perm \conf_1(\buf[\perm(i), \perm(j)])
  \end{align*}
  It implies
  \begin{align*}
  \forall i, j \in \nid \colon & m \notin \conf_0(\buf[i, j]) \Leftrightarrow m \notin  \perm  \conf_0(\buf[\perm(i), \perm(j)]) \\
  \forall i, j \in \nid \colon & m \in  \conf_1(\buf[i, j]) \Leftrightarrow m \in \perm  \conf_1(\buf[\perm(i), \perm(j)])
  \end{align*}
  Hence, a message $m$ has just added into message buffers $\perm \conf_1(\buf[\perm(i), \perm(j)])$ in this subround. 
  Moreover, by Lemma \ref{lem:PermProcStutter}, if a process $p_j$ takes a stuttering step in this subround, then a process $p_{\perm(j)}$ also takes a stuttering step.
  Moreover, message buffers from both $p_j$ and $p_{\perm(j)}$ are unchanged.
  It follows  $\perm \conf_0 \transsnd \perm \conf_1$. \qed 
\end{proof}

\newcommand{\lemPermGlobalReceive}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \transrcv \rho_1$.
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \transrcv \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermGlobalReceive}
  \lemPermGlobalReceive
\end{lemma}

\begin{proof}
  In order to prove that $\perm \conf_0 \transrcv \perm \conf_1$, we show that all  constraints in the subround Receive hold in $\perm \conf_0$ and $\perm \conf_1$.
  The most complicated constraint is for when $N$ sets of messages $S_1, \ldots, S_N \subseteq \msg$ are delivered to a  process $\pcreate(\conf_1, i)$ in this subround.
  We prove that $N$ sets of messages $S_{\perm^{-1}{1}}, \ldots, S_{\perm^{-1}{N}} \subseteq \msg$  are delivered to a  process $\pcreate(\perm \conf_1, \perm(i))$ where $\perm^{-1}$ is an inverse function of $\perm$.
  
  By Lemma \ref{lem:PermArr}, we have
  \begin{align*}
  & \perm\conf_1(\pc[\perm(i)])  = \conf_1(\pc[i]) \\
  \, \land \, &  \perm\conf_0(\pc[\perm(i)])  = \conf_0(\pc[i])  \\
  \, \land \, & \perm\conf_1(\act[\perm(i)]) = \conf_1(\act[i])   \\
  \, \land \, &  \perm\conf_0(\act[\perm(i)]) = \conf_0(\act[i]) 
  \end{align*}
  Therefore, a process $\pcreate(\perm\conf_0, \perm(i))$ is enable to receive messages, and it becomes inactive in $\perm \conf_1$.
  By Lemma \ref{lem:PermProcReceive}, it follows that 
  \[ \pcreate(\perm \conf_0, \perm (i)) \translocalrcv{\perm(i)}{S_{\perm^{-1}(1)}}{S_{\perm^{-1}(N)}} (\perm \conf_1, \perm (i))
  \] 
  Now we show that such sets of messages are removed from corresponding message buffers. By Lemma \ref{lem:PermArr}, it follows that
  \begin{align*}
  \forall i, j \in \nid \colon & \conf_0(\buf[i, j]) = \perm \conf_0(\buf[\perm(i), \perm(j)]) \\
  \forall i, j \in \nid \colon & \conf_1(\buf[i, j]) = \perm \conf_1(\buf[\perm(i), \perm(j)])
  \end{align*}
  It implies that for every $j \in \nid$, we have
  \begin{align*}
  & S_{\perm^{-1}(j)} \notin \perm  \conf_0(\buf[\perm(i), \perm^{-1}(j)]) \\
  \land \, &  S_{\perm^{-1}(j)} \cup \perm  \conf_1(\buf[\perm(i), \perm^{-1}(j)]) = \perm  \conf_0(\buf[\perm(i), \perm^{-1}(j)])
  \end{align*}
  Hence, sets of messages $S_{\perm^{-1}(1)}, \ldots, S_{\perm^{-1}(N)}$ are removed from message buffers $\perm \conf(\buf[\perm(1)]), \ldots, \perm \conf(\buf[\perm(i), N])$, respectively.
  Moreover, by Lemma \ref{lem:PermProcStutter}, it follows that if a process $p_j$ takes a stuttering step in this subround, then a process $p_{\perm(j)}$ also takes a stuttering step.
%  Moreover, message buffers from both $p_j$ and $p_{\perm(j)}$ are unchanged.
  It follows  $\perm \conf_0 \transrcv \perm \conf_1$. \qed 
\end{proof}

\newcommand{\lemPermGlobalComp}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \transcomp \rho_1$.
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \transcomp \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermGlobalComp}
  \lemPermGlobalComp
\end{lemma}

\begin{proof}
By similar arguments in the proofs of Lemmas \ref{lem:PermGlobalSend}--\ref{lem:PermGlobalReceive}.
\end{proof}

\newcommand{\lemPermGlobalStutter}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \xrightarrow{\tau} \rho_1$ where $\xrightarrow{\tau}$ is a stuttering transition.
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \xrightarrow{\tau} \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermGlobalStutter}
  \lemPermGlobalStutter
\end{lemma}

\begin{proof}
  By similar arguments in the proofs of Lemmas \ref{lem:PermGlobalSend}--\ref{lem:PermGlobalReceive}.
\end{proof}

\newcommand{\lemPermGlobalTrans}{
  Let $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$ be a global transition system defined as in Section \ref{sec:ProcTemp}.
  Let $\rho_0, \rho_1$ be global configurations in $\gstates{N}$ such that $\rho_0 \leadsto \rho_1$.
  Let $\perm$ be a permutation on $\nid$.
  It follows that $\perm \rho_0 \leadsto \perm \rho_1$.  
}

\begin{lemma} \label{lem:PermGlobalTrans}
  \lemPermGlobalTrans
\end{lemma}

\begin{proof}
  Since $\conf_0 \leadsto \conf_1$, there exists three global configuration $\rho_1, \rho_2, \rho_3$ such that
  \[
  \conf_0 \transsched \rho_1 \transsnd \rho_2 \transrcv \rho_3 \transcomp \conf_2
  \]
  By Lemma \ref{lem:PermGlobalType}, it follows that all of $\perm \rho_1 , \perm \rho_2, \perm \rho_3$ are global configurations in $\gstates{N}$. 
  By Lemma \ref{lem:PermGlobalSchedule}, it follows $\perm\conf_1 \transsched \perm \rho_1$. 
  By Lemma \ref{lem:PermGlobalSend}, it follows . 
  By Lemma \ref{lem:PermGlobalReceive}, it follows $\perm\rho_2 \transrcv \perm \rho_3$. 
  By Lemma \ref{lem:PermGlobalComp}, it follows $\perm\rho_3 \transcomp \perm \conf_2$.
  Therefore, we have $\perm \conf_1 \leadsto \perm \conf_2$. \qed
\end{proof}


\subsection{Cutoff results of~\classname{} algorithms}

\begin{theorem} \label{thm:NCutoffOneIndex}
  Let $\mathcal{A}$ be an~\classname{} algorithm, and $M_1, M_N$ be its instances for some $N \geq 1$.
  Let $F_{i}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with  one index $i$.
  It follows that
  $
  M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i} \Leftrightarrow M_1, \ginitstate{1} \models  F_{1}
  $.
\end{theorem}

\begin{proof}
  Let $i$ be an index in $\nid$.
  There exists a permutation $\perm$ on a set $\nid$ such that $\perm(i) = 1$ .
  By definition of index permutations, it follows
  \[
  M_N, \ginitstate{N} \models  F_{i} \Leftrightarrow \perm(M_N), \perm(\ginitstate{N}) \models  F_{\perm(i)}
  \]
  By the assumption, we have $F_{\perm(i)} = F_{1}$.
  By Lemma \ref{cor:SymGlobalSys}, it follows  $\perm(\ginitstate{N}) = \ginitstate{N}$ and $\perm(M_N) = M_N$.
  Therefore, it follows
  \[
  M_N, \ginitstate{N} \models  F_{i} \Leftrightarrow M_N, \ginitstate{N} \models  F_{1}
  \]
  Since $i$ are arbitray, we have
  $
  M_N, \ginitstate{N} \models  F_{1} 
  \Leftrightarrow M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i}
  $.
  By Corollary \ref{cor:TraceEquiv}, we have
  $
  M_N, \ginitstate{N} \models  F_{1} \Leftrightarrow M_2, \ginitstate{2} \models  F_{1}
  $.
  It follows that
  \[
  M_N, \ginitstate{N} \models \bigwedge_{i \in \nid} F_{i} \Leftrightarrow M_2, \ginitstate{2} \models  F_{1}
  \]
  Therefore, Theorem \ref{thm:NCutoffOneIndex} is correct. \qed
\end{proof}



\begin{theorem} \label{thm:NCutoffTwoIndexes}
  Let $\mathcal{A}$ be an~\classname{} algorithm, and $M_2, M_N$ be its instances for some $N \geq 2$.
  Let $G_{i, j}$ is an arbitrary LTL (linear temporal logic) formula whose predicates inspect only variables with two different indexes $i, j \in \nid$.
  It follows 
  $
  M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  $.
\end{theorem}

\begin{proof}
  Let $i, j$ be different indexes in $\nid$.
  There exists a permutation $\perm$ on a set $\nid$ such that $\perm(i) = 1$ and $\perm(j) = 2$.
  By definition of index permutations, it follows
  $
  M_N, \ginitstate{N} \models  G_{i, j} \Leftrightarrow \perm(M_N), \perm(\ginitstate{N}) \models  G_{\perm(i), \perm(j)}
  $.
  By the assumption, we have $G_{\perm(i), ,\perm(j)} = G_{1,2}$.
  By Lemma \ref{cor:SymGlobalSys}, it follows $\perm(\ginitstate{N}) = \ginitstate{N}$ and $\perm(M_N) = M_N$.
  Therefore, it follows
  \[
  M_N, \ginitstate{N} \models  G_{i, j} \Leftrightarrow M_N, \ginitstate{N} \models  G_{1, 2}
  \]
  Since $i,j$ are arbitray, we have
  $
  M_N, \ginitstate{N} \models  G_{1, 2} 
  \Leftrightarrow M_N, \ginitstate{N} \models \bigwedge^{i \neq j}_{i, j \in \nid} G_{i, j}
  $.
  By Corollary \ref{cor:TraceEquiv}, we have
  $
  M_N, \ginitstate{N} \models  G_{1, 2} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  $.
  It follows that
  \[
  M_N, \ginitstate{N} \models \bigwedge^{i \in \nid}_{j \in \nid \setminus \{i\}} G_{i, j} \Leftrightarrow M_2, \ginitstate{2} \models  G_{1, 2}
  \]
  Therefore, Theorem \ref{thm:NCutoffTwoIndexes} is correct. \qed
\end{proof}




\subsection{Trace equivanlence of $M_2$ and $M_N$ under $AP_{1,2}$}

The main result in this section is Corollary \ref{cor:TraceEquiv} which says that two instances $M_N, M_2$ of an arbitrary~\classname{} algorithm are trace equivalent under a set $AP_{1, 2}$ of predicates which inspect only variables whose indexes are $\{1\}, \{2\}$, or both $\{1, 2\}$.
The proof of Corollary \ref{cor:TraceEquiv} is based on a construction technique for global configurations which is presented in Constructions \ref{const:ProcConfProj}--\ref{const:GlobalConfProj}, and two Lemmas \ref{lem:IDProjPath} and \ref{lem:IDRefilledPath}.

To keep the presentation simple, when the context is clear, we write $U_N$, instead of fully $U_N = \left(\pstates{U}{N}, \trans{U}{N}, \sigma^U_N, \pinitstate{U}{N}\right)$, which are defined in Section \ref{sec:GlobalTransSys}.
We also write $M_N$, instead of fully $M_N = \left( \gstates{N}, \trans{G}{N}, \sigma^G_N, \ginitstate{N} \right)$.
%
%\emph{ID--projection}.
%The ID--project technique is presented in Definition \ref{def:IDProj}.
%
%  Lemma \ref{lem:IDProjConf} shows that a configuration constructed with the~\idsep{} technique from another configuration in $\sys{N}$ is a legal configuration in~$\sys{2}$.


\newcommand{\corTraceEquiv}{
  Let $\mathcal{A}$ be an~\classname{} algorithm, and $M_2, M_N$ be its instances for some $N \geq 2$.
  Let $AP_{1, 2}$ be a set of predicates which inspect only variables whose indexes are $\{1\}, \{2\}$, or both $\{1, 2\}$
  It follows that $M_N, M_2$ are trace equivalent under $AP_{1,2}$.
}

\begin{corollary} \label{cor:TraceEquiv}
\corTraceEquiv
\end{corollary}



\begin{construction} \label{const:ProcConfProj}
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be two process templates of $\mathcal{A}$ for some $N \geq 2$, and
  $\conf^N \in \pstates{U}{N}$ be a process configuration of $U_N$.
  We construct an interpretation $\conf^2$ from $\conf^N$ in the following way:
  \begin{enumerate}
    \item For every process $i \in \{1, 2\}$, it follows  $\conf^2(\pc[i]) = \conf^N(\pc[i])$.
    
    \item For every $3 \leq k \leq \ell$, for every $i \in \{1, 2\}$, it follows that  $\conf^2(x^U_k[i]) = \conf^N(x^U_k[i])$.    
  \end{enumerate}  
\end{construction}



\begin{construction} \label{const:GlobalConfProj}
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be two global transitions of two instances of $\mathcal{A}$ for some $N \geq 2$, and
  $\conf^N \in \gstates{N}$ be a global configuration in $M_N$.
  We construct an interpretation $\conf^2$ of $M_2$ from $\conf^N$ in the following way:
  \begin{enumerate}
  \item For every process $i \in \{1, 2\}$, it follows $\conf^2(\act[i]) = \conf^N(\act[i]) $ and  $\conf^2(\pc[i]) = \conf^N(\pc[i])$.
    
  \item For every $i, j \in \{1, 2\}$, it follows $\conf^2(\buf[i, j]) = \conf^N(\buf[i, j])$.
    
  \item For every $2 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, it follows that  $\conf^2(x_k[i, j]) = \conf^N(x_k[i, j])$.    
  \end{enumerate}  
\end{construction}

Lemma \ref{lem:ProjProcConfType} says that an interpretation constructed  with Construction \ref{const:ProcConfProj} is a process configuration of $U_2$.
Lemma \ref{lem:ProjGlobalConfType} says that an interpretation constructed  with Construction \ref{const:GlobalConfProj} is a global configuration of $M_2$.
Interpretations constructed with Constructions \ref{const:ProcConfProj} and \ref{const:GlobalConfProj} are called \emph{\projconf}.

\newcommand{\lemProjProcConfType}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$ for some $N \geq 2$.
  Let $\conf^N \in \pstates{U}{N}$ be a global configuration.
  Let $\conf^2$ be an interpretation constructed from $\conf^N$ of $U_N$ with Construction \ref{const:ProcConfProj}.
  It follows that $\conf^2$ is a process configuration of $M_2$.
}

\begin{lemma} \label{lem:ProjProcConfType}
  \lemProjProcConfType
\end{lemma}

\begin{proof}
  By definition of Construction \ref{const:ProcConfProj}, it is to see that for every variable with type $x \colon \mathcal{T}$ in $U_2$, an interpretation $\conf^2$ assigns a value in $\mathcal{T}$ to $x$.
  Therefore, a configuration $\conf^2$ is a process configuration of $U_2$. \qed
\end{proof}


\newcommand{\lemProjGlobalConfType}{
 Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
 Let $M_N, M_2$ be global transitions of two instances of $\mathcal{A}$ for some $N \geq 2$.
 Let $\conf^N \in \gstates{N}$ be a global configuration.
 Let $\conf^2$ be an interpretation constructed from $\conf^N$ of $M_N$ with Construction \ref{const:GlobalConfProj}.
 It follows that $\conf^2$ is a global configuration of $M_2$.
}

\begin{lemma} \label{lem:ProjGlobalConfType}
\lemProjGlobalConfType
\end{lemma}

\begin{proof}
By definition of Construction \ref{const:GlobalConfProj}, it is to see that for every variable with type $x \colon \mathcal{T}$ in $M_2$, an interpretation $\conf^2$ assigns a value in $\mathcal{T}$ to $x$.
Therefore, a configuration $\psi^2$ is a globa configuration in $M_2$. \qed
\end{proof}

Now we prove Lemma \ref{lem:IDProjPath} that the application of Construction \ref{const:GlobalConfProj} to an admissible sequence in $M_N$ constructs an admissible sequence in $M_2$.
The proof strategy for Lemma \ref{lem:IDProjPath} is similar to one for Lemma \ref{lem:SymGlobalInitConf}, and requires following lemmas:
\begin{enumerate}
\item Lemma \ref{lem:ProjInitProcConf} says that the application of Construction \ref{const:ProcConfProj} to an initial process configuration of $M_N$ constructs an initial process configuration of $M_2$. 

\item Lemmas \ref{lem:ProjProcSend}, \ref{lem:ProjProcReceive}, \ref{lem:ProjProcComp}, \ref{lem:ProjProcCrash} and \ref{lem:ProjProcStutter} says that Construction \ref{const:ProcConfProj} preserves the process transition relations.

\item Lemma \ref{lem:ProjInitGlobalConf} says that the application of Construction \ref{const:GlobalConfProj} to an initial global configuration of $M_N$ constructs an initial global configuration of $M_2$. 

\item Lemmas \ref{lem:ProjGlobalSchedule}, \ref{lem:ProjGlobalSend}, \ref{lem:ProjGlobalReceive}, \ref{lem:ProjGlobalComp}, \ref{lem:ProjGlobalStutter}, and \ref{lem:ProjGlobalTrans} says  the application of Construction \ref{const:GlobalConfProj} to a tuple $\conf_0 \xrightarrow{\mathit{action}} \conf_1 \in \sigma^G_N$ constructs a tuple $\conf^{\prime}_0 \xrightarrow{\mathit{action}^{\prime}} \conf^{\prime}_1 \in \sigma^G_2$ where $\mathit{action}^{\prime}$ is similar with $\mathit{action}$ or a stuttering step.
\end{enumerate}


\newcommand{\lemIDProjPath}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be two transition systems of two instances of $\mathcal{A}$ for some $N \geq 2$.
  Let $pi^N = \conf^N_0 \conf^N_1 \ldots$ be an admissible sequence of configurations in $M_2$.
  Let $pi^2 = \conf^2_0 \conf^2_1 \ldots$ be a sequence of configurations of $M_2$  such that $\conf^2_k$ is an~\projconf{} of $\conf^N_k$ for every $k \geq 0$.
  It follows that $\pi^2$ is admissible in $M_2$.
}


\begin{lemma} \label{lem:IDProjPath}
\lemIDProjPath
\end{lemma}

\begin{proof}
It immediately follows by Lemmas \ref{lem:ProjInitGlobalConf}, \ref{lem:ProjGlobalStutter}, \ref{lem:ProjGlobalSched}, \ref{lem:ProjGlobalSend}, \ref{lem:ProjGlobalReceive}, and \ref{lem:ProjGlobalComp}.
\end{proof}

\newcommand{\lemProjInitProcConf}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be two process templates  of $\mathcal{A}$ for some $N \geq 2$.
  Let $\pinitstate{U}{N}$ be an initial configuration in $U_N$, and $\conf^2$ be an~\projconf{} of $\pinitstate{U}{N}$.  
  It follows that $\conf^2 = \pinitstate{U}{2}$.
}

\begin{lemma} \label{lem:ProjInitProcConf}
  \lemProjInitProcConf
\end{lemma}

\begin{proof}
  It immediately follows by Construction \ref{const:ProcConfProj} and the definition of $\pinitstate{U}{2}$. \qed
\end{proof}

\newcommand{\lemProjProcSend}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$.
  Let $m \in \msg$ be a message, and $\rho_0, \rho_1 \in \pstates{U}{N}$ be process configurations such that $\rho_0 \procsnd{m} \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{prime}_1$ be process configurations with Construction \ref{const:ProcConfProj}.
  It follows that $\rho^{\prime}_0 \procsnd{m} \rho^{\prime}_1 \in \sigma^U_2$.  
}

\begin{lemma} \label{lem:ProjProcSend}
  \lemProjProcSend
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:ProjProcSend} by utilizing the  properties of~\classname{} functions.
  First, we have 
  \begin{alignat*}{3}
  \rho^{\prime}_1(\pc) & = \rho_1(\pc) && \quad \text{(by Construction \ref{const:ProcConfProj})} \\
  & = g_1(\rho_0(\pc)) && \quad \text{(by definition of function $g_1$)}              \\
  & = g_1(\rho^{\prime}_0(\pc)) && \quad \text{(by Construction \ref{const:ProcConfProj})}              
  \end{alignat*}
  
  We now check the $\mailbox$. 
  Let $i$ be an arbitrary index in $\tid$.
  It follows
  \begin{alignat*}{3}
  \rho^{\prime}_1(\mailbox[i]) & = \rho_1(\mailbox[i]) && \quad \text{(by Construction \ref{const:ProcConfProj})}  \\
  & = \rho_0(\mailbox[i]) && \quad \text{(by definition of $\procsnd{m}$)}              \\
  & = \rho^{\prime}_0(\mailbox[i])  && \quad \text{(by Construction \ref{const:ProcConfProj})}  
  \end{alignat*}
  Hence, we have $\forall i \in \tid \colon \rho^{\prime}_1(\mailbox[i]) = \rho^{\prime}_0(\mailbox[i])$.
  
  We now focus on a two--dimensional variable $x^U_3$.
  Again, let $i$ be an arbitrary index in $\tid$. It follows
  \begin{alignat*}{3}
  \rho^{\prime}_1(x_3[i]) & = \rho_1(x_3[i]) && \quad \text{(by Construction \ref{const:ProcConfProj})}  \\
  & = f_3 \big( \rho_0(x_1),  \rho_1(x_2[i]), \rho_0(x_3[i]), \ldots, \rho(x_\ell[i]) \big) && \quad \text{(by definition of   $f_3$)}              \\
  & = f_3 \big( \rho_0(\pc),  \rho_1(\mailbox[i]), \rho_0(x_3[i]), \ldots, \rho_0(x_\ell[i]) \big) && \quad \text{(by renaming)}              \\
  & = f_3 \big( \rho^{\prime}_0(\pc),  \rho^{\prime}_1(\mailbox[i]), \rho^{\prime}_0(x_3[i]), \ldots, \rho^{\prime}_0(x_\ell[i]) \big) && \quad \text{(by Construction \ref{const:ProcConfProj})}              
  \end{alignat*}
  Hence, we have 
  $
  \forall i \in \tid \colon \perm\rho^{\prime}_1(x_3[i]) =  f_3 \big( \rho^{\prime}_0(\pc), \rho^{\prime}_1(\mailbox[i]),\rho^{\prime}_0(x_3[i]), \ldots, \rho^{\prime}_0(x_\ell[i]) \big)
  $.
  By similar arguments for other variables, we have  
  \begin{align*}
  \forall k \in 3..\ell \, \forall i \in \tid \colon \rho^{\prime}_1(x_k[i]) =  f_k \big( & \rho^{\prime}_0(\pc),  \rho^{\prime}_1(\mailbox[i]),               \\
  & \rho^{\prime}_0(x_3[i]), \ldots, \rho^{\prime}_0(x_\ell[i]) \big)
  \end{align*}
  %  Let $\perm^{-1}$ be an inverse permutation of $\perm$.
  By Lemma \ref{lem:ProjProcConfType}, we have $\rho^{\prime}_0, \rho^{\prime}_1 \in \pstates{U}{2}$.
  It follows $ \rho^{\prime}_0 \procsnd{m} \rho^{\prime}_1 \in \sigma^U_2$ by the semantics of the transtion $\procsnd{m}$. \qed
\end{proof}

\newcommand{\lemProjProcReceive}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$.
  Let $S_1, \ldots, S_N \subseteq \msg$ be sets of messages, and $\rho_0, \rho_1 \in \pstates{U}{N}$ be process configurations such that $\rho_0 \procrcv{S_1}{S_N} \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{prime}_1$ be process configurations with Construction \ref{const:ProcConfProj}.
  It follows that $\rho^{\prime}_0 \procrcv{S_1}{S_2} \rho^{\prime}_1 \in \sigma^U_2$.  
}

\begin{lemma} \label{lem:ProjProcReceive}
  \lemProjProcReceive
\end{lemma}

\begin{proof}
  We prove Lemma \ref{lem:ProjProcReceive} by utilizing the  properties of~\classname{} functions.
  First, we have 
  \begin{alignat*}{3}
  \rho^{\prime}_1(\pc) & = \rho_1(\pc) && \quad \text{(by Construction \ref{const:ProcConfProj})} \\
  & = g_1(\rho_0(\pc)) && \quad \text{(by definition of function $g_1$)}              \\
  & = g_1(\rho^{\prime}_0(\pc)) && \quad \text{(by Construction \ref{const:ProcConfProj})}              
  \end{alignat*}
  
  We now check the $\mailbox$. 
  Let $i$ be an arbitrary index in $\tid$.
  It follows
  \begin{alignat*}{3}
  \rho^{\prime}_1(\mailbox[i]) & = \rho_1(\mailbox[i]) && \quad \text{(by Construction \ref{const:ProcConfProj})}  \\
  & = \rho_0(\mailbox[i]) \cup S_{i} && \quad \text{(by definition of $\procrcv{S_1}{S_N}$)}              \\
  & = \rho^{\prime}_0(\mailbox[i]) \cup S_{i}  && \quad \text{(by Construction \ref{const:ProcConfProj})}  
  \end{alignat*}
  Hence, we have $\forall i \in \tid \colon \rho^{\prime}_1(\mailbox[i]) = \rho^{\prime}_0(\mailbox[i]) \cup S_{i}$.
  
  By similar arguments in the proof of Lemma \ref{lem:ProjProcReceive}, we have  
  \begin{align*}
  \forall k \in 3..\ell \, \forall i \in \tid \colon \rho^{\prime}_1(x_k[i]) =  f_k \big( & \rho^{\prime}_0(\pc), \perm \rho^{\prime}_1(\mailbox[i]),               \\
  & \perm \rho^{\prime}_0(x_3[i]), \ldots, \perm \rho^{\prime}_0(x_\ell[i]) \big)
  \end{align*}  
  By Lemma \ref{lem:ProjProcConfType}, we have $\rho^{\prime}_0, \rho^{\prime}_1 \in \pstates{U}{2}$.
  It follows $\rho^{\prime}_0 \procrcv{S_{1}}{S_{2}} \rho^{\prime}_1$. \qed
\end{proof}

The proofs of Lemmas \ref{lem:ProjProcComp}, \ref{lem:ProjProcCrash} and \ref{lem:ProjProcStutter} are obtained by applying similar arguments in the proofs of Lemmas \ref{lem:ProjProcSend} and \ref{lem:ProjProcReceive}.


\newcommand{\lemProjProcComp}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$.
  Let $\rho_0, \rho_1 \in \pstates{U}{N}$ be process configurations such that $\rho_0 \proccomp \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{prime}_1$ be process configurations with Construction \ref{const:ProcConfProj}.
  It follows that $\rho^{\prime}_0 \proccomp \rho^{\prime}_1 \in \sigma^U_2$.  
}

\begin{lemma} \label{lem:ProjProcComp}
  \lemProjProcComp
\end{lemma}

\newcommand{\lemProjProcCrash}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$.
  Let $\rho_0, \rho_1 \in \pstates{U}{N}$ be process configurations such that $\rho_0 \proccrash \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{prime}_1$ be process configurations with Construction \ref{const:ProcConfProj}.
  It follows that $\rho^{\prime}_0 \proccrash \rho^{\prime}_1 \in \sigma^U_2$.  
}

\begin{lemma} \label{lem:ProjProcCrash}
  \lemProjProcCrash
\end{lemma}

\newcommand{\lemProjProcStutter}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $U_N, U_2$ be process templates of $\mathcal{A}$.
  Let $\rho_0, \rho_1 \in \pstates{U}{N}$ be process configurations such that $\rho_0 \procstutter \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{prime}_1$ be process configurations with Construction \ref{const:ProcConfProj}.
  It follows that $\rho^{\prime}_0 \procstutter \rho^{\prime}_1 \in \sigma^U_2$.  
}

\begin{lemma} \label{lem:ProjProcStutter}
  \lemProjProcStutter
\end{lemma}

Now we turn to properties of global configurations under~Constructions \ref{const:GlobalConfProj}.

\newcommand{\lemProjInitGlobalConf}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be two transition systems of two instances of $\mathcal{A}$ for some $N \geq 2$.
  Let $\ginitstate{N}$ be an initial configuration in $M_N$, and $\conf^2$ be an~\projconf{} of $\conf^N$.  
  It follows that $\conf^2 \Leftrightarrow \ginitstate{2}$.
}

\begin{lemma} \label{lem:ProjInitGlobalConf}
\lemProjInitGlobalConf
\end{lemma}

\begin{proof}
It immediately follows by Construction \ref{const:GlobalConfProj} and the definition of $\ginitstate{N}$. \qed
\end{proof}

\newcommand{\lemProjGlobalStutter}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transstutter \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{\prime}_1$ be process configurations with Construction \ref{const:GlobalConfProj}.
  It follows that $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$.  
}

\begin{lemma} \label{lem:ProjGlobalStutter}
  \lemProjGlobalStutter
\end{lemma}

\begin{proof}
By Lemma \ref{lem:ProjGlobalConfType}, we have $\rho^{\prime}_0, \rho^{prime}_1 \in \gstates{2}$.
By the assumption and Construction \ref{const:GlobalConfProj}, we have $\rho^{\prime}_0 = \rho^{prime}_1$.
It follows $\rho^{\prime}_0 \transstutter \rho^{prime}_1 \in \sigma^G_2$. \qed
\end{proof}

\newcommand{\lemProjGlobalSchedule}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transsched \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{\prime}_1$ be process configurations with Construction \ref{const:GlobalConfProj}.
  It follows that either $\rho^{\prime}_0 \transsched \rho^{\prime}_1 \in \sigma^G_2$ or $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$.  
}

\begin{lemma} \label{lem:ProjGlobalSchedule}
  \lemProjGlobalSchedule
\end{lemma}

\begin{proof}
We have $\conf_0(\act[i]) = \conf^{\prime}_0(\act[i])$ for every $i \in \tid$ by Construction \ref{const:GlobalConfProj}.
Therefore, the subround Schedule can start with a global configuration $\conf^{\prime}_0$. 
If  $\pcreate(\conf_0, i) \proccrash \pcreate(\conf_1, i)$, then $\pcreate(\conf^{\prime}_0, i) \proccrash \pcreate(\conf^{\prime}_1, i)$ by Lemma \ref{lem:ProjProcCrash}. 
If  $\pcreate(\conf_0, i) \procstutter \pcreate(\conf_1, i)$, then $\pcreate(\conf^{\prime}_0, i) \procstutter \pcreate(\conf^{\prime}_1, i)$ by Lemma \ref{lem:ProjProcStutter}.
Moreover, by Construction \ref{const:GlobalConfProj}, the message buffers in $\conf^{\prime}_0$ and $\conf^{\prime}_1$ are the same.
Therefore, if $\conf^{\prime}_1(\act[i]) = False$ and $\pcreate(\conf^{\prime}_0, i) \procstutter \pcreate(\conf^{\prime}_1, i)$ for every $i \in \tid$, it follows that  $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$. 
Otherwise, we have $\rho^{\prime}_0 \transsched \rho^{\prime}_1 \in \sigma^G_2$.
\end{proof}

\newcommand{\lemProjGlobalSend}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transsnd \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{\prime}_1$ be process configurations with Construction \ref{const:GlobalConfProj}.
  It follows that either $\rho^{\prime}_0 \transsnd \rho^{\prime}_1 \in \sigma^G_2$ or $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$.  
}

\begin{lemma} \label{lem:ProjGlobalSend}
  \lemProjGlobalSend
\end{lemma}

\begin{proof}
We have $\conf_0(\act[i]) = \conf^{\prime}_0(\act[i])$ and $\conf_0(\pc[i]) = \conf^{\prime}_0(\pc[i])$ for every $i \in \tid$ by Construction \ref{const:GlobalConfProj}.
Therefore, it follows $\CanRun(\conf_0, i, \locsnd) \Leftrightarrow \CanRun(\conf^{\prime}_0, i, \locsnd)$ for every $i \in \tid$. 

If both processes $\pcreate(\conf_0, 1), \pcreate(\conf_0, 2)$ cannot take a step from $\conf_0$, then processes $\pcreate(\conf^{\prime}_0, 1), \pcreate(\conf^{\prime}_0, 2)$ cannot take a step from $\conf^{\prime}_0$. Therefore, we have that $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$. 

By Lemma \ref{lem:ProjProcSend}, if there exists a message $m \in \msg$ such that $\pcreate(\conf_0, i) \procsnd{m} \pcreate(\conf_1, i)$, it follows that $\pcreate(\conf^{\prime}_0, i) \procsnd{m} \pcreate(\conf^{\prime}_1, i)$ for every $i \in \tid$.
Now we show that a message $m$ is fresh in every message buffer from $\pcreate(\conf^{\prime}_1, i)$ in $\conf^{\prime}_1$. 
By Construction \ref{const:GlobalConfProj}, it follows that
\begin{align*}
\forall j \in \tid \colon & \conf_0(\buf[i, j]) = \conf^{\prime}_0(\buf[i, j]) \\
\forall j \in \tid \colon & \conf_1(\buf[i, j]) = \conf^{\prime}_1(\buf[i, j])
\end{align*}
It implies
\begin{align*}
\forall j \in \tid \colon & m \notin \conf_0(\buf[i, j]) \Leftrightarrow m \notin   \conf^{\prime}_0(\buf[i, j]) \\
\forall j \in \tid \colon & m \in  \conf_1(\buf[i, j]) \Leftrightarrow m \in  \conf^{\prime}_1(\buf[i, j])
\end{align*}
Hence, a message $m$ has just added into message buffers $\conf^{\prime}_1(\buf[i, j])$ in this subround. 
It follows  $\conf^{\prime}_0 \transsnd \conf^{\prime}_1$. \qed 
\end{proof}


\newcommand{\lemProjGlobalReceive}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transrcv \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{\prime}_1$ be process configurations with Construction \ref{const:GlobalConfProj}.
  It follows that either $\rho^{\prime}_0 \transrcv \rho^{\prime}_1 \in \sigma^G_2$ or $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$.  
}

\begin{lemma} \label{lem:ProjGlobalReceive}
  \lemProjGlobalReceive
\end{lemma}

\begin{proof}
By applying similar arguments in the proofs of Lemmas \ref{lem:ProjProcSend}.
\end{proof}

\newcommand{\lemProjGlobalComp}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transcomp \rho_1 \in \sigma^U_N$. 
  Let $\rho^{\prime}_0, \rho^{\prime}_1$ be process configurations with Construction \ref{const:GlobalConfProj}.
  It follows that either $\rho^{\prime}_0 \transcomp \rho^{\prime}_1 \in \sigma^G_2$ or $\rho^{\prime}_0 \transstutter \rho^{\prime}_1 \in \sigma^G_2$.  
}

\begin{lemma} \label{lem:ProjGlobalComp}
  \lemProjGlobalComp
\end{lemma}

\begin{proof}
  By applying similar arguments in the proofs of Lemmas \ref{lem:ProjProcSend}.
\end{proof}

\newcommand{\lemIDRefilledPath}{
  Let $\mathcal{A}$ be an arbitrary~\classname{} algorithm.
  Let $M_N, M_2$ be global transition systems of $\mathcal{A}$ for some $N \geq 2$.
  Let $\rho_0, \rho_1 \in \gstates{N}$ be global configurations such that $\rho_0 \transcomp \rho_1 \in \sigma^U_N$. 
  Let $\pi^2 = \conf_0 \conf_1 \ldots $ be an admissible sequence in $M_2$.
  Let $\pi^N$ be a sequence constructed from $\pi^2$ such that
  \begin{enumerate}
    \item A configuration $\conf^N_0$ is initial, i.e. $\conf^N_0 = \ginitstate{N}$.
    
    \item Assume that $\conf^2_k \transsched \conf^2_{k + 1}$ is the first subround Schedule in $\pi$, we have 
    \begin{itemize}
    \item Configurations $\conf^N_0, \ldots, \conf^N_{k}$  are the same.
    \item The subround $\conf^N_{k + 1}$ schedules all process $p_3, \ldots, p_N$ become crashes.
    \end{itemize}    
    \item For every process $i \in \{1, 2\}$, it follows $\conf^2(\act[i]) = \conf^N(\act[i]) $ and  $\conf^2(\pc[i]) = \conf^N(\pc[i])$.
    
    \item For every $i, j \in \{1, 2\}$, it follows $\conf^2(\buf[i, j]) = \conf^N(\buf[i, j])$.
    
    \item For every $2 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, it follows that  $\conf^2(x_k[i, j]) = \conf^N(x_k[i, j])$.   
    
    \item Every variable which has at least one index different from $\{1, 2\}$ is unchanged from the $(k+2)^{th}$ configuration.
  \end{enumerate} 
  It follows that $\pi^N$ is admissible in $M_N$.
}

\begin{lemma} \label{lem:IDRefilledPath}
  \lemIDRefilledPath
\end{lemma}

\begin{proof}
  Notice that only two processes $p_1, p_2$ can take a step in $\pi^N$.
  By applying similar arguments in the proofs of Lemmas \ref{lem:ProjGlobalSchedule}, \ref{lem:ProjGlobalSend}, \ref{lem:ProjGlobalReceive}, and \ref{lem:ProjGlobalComp}, it follows that $\pi^N$ is admissible in $M_N$.
\end{proof}

%
%\begin{proof}
%  First, we prove that $\conf{2}{0}$ is consistent with an initial state $\sys{2}$ by the construction. By Lemma \ref{lem:IDProjConf}, it follows that $\conf{2}{0}$ is a configuration in  $\sys{2}$. Since $\conf{N}{0}$ is consistent with an initial state in $\sys{N}$, so is $\conf{2}{0}$ in $\sys{2}$.
%
%  
%%  Therefore, $\conf{2}{0}$ is consistent with a global state  in $\sys{2}$.
%%  Moreover, since $\conf{N}{0}$ is consistent with an initial state in $\sys{N}$ and the construction of $\conf{2}{0}$, it immediately follows that  $\conf{2}{0}$ is consistent with an initial state $\sys{2}$.
%
%  
%  Second, we prove that every sequence $\conf{2}{4k - 4} \rightarrow \ldots \rightarrow \conf{2}{4k}$ is a refinement of a global transition at a time $k$ by induction on $k$.
%  \begin{enumerate}
%    \item \emph{Base case.} By the lemma hypothesis, we have that
%    \[
%    \conf{N}{1} \xrightarrow{\sched{}} \conf{N}{1} \xrightarrow{\tsnd{}} \conf{N}{2} \xrightarrow{\trcv{}}  \conf{N}{3} \xrightarrow{\cop{}} \conf{N}{4} 
%    \]
%    We need to prove that a sequence of configurations $\conf{2}{0} \rightarrow \conf{2}{1} \rightarrow \conf{2}{2} \rightarrow \conf{2}{3} \rightarrow \conf{2}{4}$ 
%%    $ \tconfsched{1}  \rightarrow \tconfsnd{1}  \rightarrow \tconfrcv{1}  \rightarrow \sigma^2_1$
%%    such that 
%%    \[
%%    \conf{2}{1} = \tconfsched{1} \land \conf{2}{2} = \tconfsnd{1} \land \conf{2}{3} = \tconfrcv{1} \land \conf{2}{4} = \sigma^2_1
%%    \]
%    presents respectively subrounds Schedule, Send, Receive, and Computation.
%    By Lemma \ref{lem:IDProjConf}, $\conf{2}{k}$ is a configuration in $\sys{2}$ for every $1 \leq k \leq 4$.
%    Therefore, we need to prove that every constraint in a subround \texttt{Rnd} hold in the corresponding transition.
%    The proof is by cases. \\
%    \emph{$\bullet$ Transition $\conf{2}{0} \rightarrow \conf{2}{1}$}. We will show that this transition satisfies every constraint in the subround \sched{}.
%    By the construction of $\conf{2}{1}$, we have 
%    \begin{itemize}
%     \item $\forall p, q \in \{p_1, p_2\} \, \forall 1 \leq \ell \leq M \colon   \conf{2}{1}(p).X_\ell[q] = \conf{N}{1}(p).X_\ell[q]$
%    
%    \item $\forall p, q \in \{p_1, p_2\} \colon    \conf{2}{1}(p).\mailbox[q] = \conf{N}{1}(p).\mailbox[q]$ 
%    
%    \item $\forall p, q \in \{p_1, p_2\} \colon   \conf{2}{1}(\buf{p}{q}) = \conf{N}{1}(\buf{p}{q}) $
%    
%    \item $\forall p \in \{p_1, p_2\} \colon   \conf{2}{1}(\gpc[p]) = \conf{N}{1}(\gpc[p]) \land  \conf{2}{1}(p).\lpc = \conf{N}{1}(p).\lpc$ 
%    
%    \item $\forall p, q \in \{p_1, p_2\} \, \forall m \in \psi^2(\buf{p}{q}) \colon   \psi^2(\age{m}) = \psi^N(\age{m})$ 
%  \end{itemize}
%  Since $\conf{N}{0} \rightarrow \conf{N}{1}$ is a send transition, we have that
% \begin{itemize}
%    \item $\forall p, q \in \{p_1, p_2\} \, \forall 1 \leq \ell \leq M \colon   \conf{N}{1}(p).X_\ell[q] = \conf{N}{0}(p).X_\ell[q]$
%    
%    \item $\forall p, q \in \{p_1, p_2\} \colon    \conf{N}{1}(p).\mailbox[q] = \conf{N}{0}(p).\mailbox[q]$ 
%    
%    \item $\forall p, q \in \{p_1, p_2\} \colon   \conf{N}{1}(\buf{p}{q}) = \conf{N}{0}(\buf{p}{q}) $
%    
%    \item $\forall p \in \{p_1, p_2\} \colon   \conf{2}{1}(\gpc[p]) \in \Boolean \land  \conf{N}{1}(p).\lpc = \conf{N}{0}(p).\lpc$ 
%    
%    \item $\forall p, q \in \{p_1, p_2\} \, \forall m \in \psi^N(\buf{p}{q}) \colon  \psi^N_1(\age{m}) = \psi^N_0(\age{m}) + 1$ 
%  \end{itemize}
%  It follows that every in--transit message age is increased by 1 in $\conf{2}{1}$, and only variable $\gpc$ can be updated in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$.
%  Therefore, every constraint in the subround Send holds in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$.
%
%  \emph{$\bullet$ Transition $\conf{2}{1} \rightarrow \conf{2}{2}$}. We will show that this transition satisfies every constraint in the subround Send.
%   By the ID--projection construction, a process $p^N_i$ takes a step in this subround Send if and only a process $p^2_i$ takes a step in this subround  for every $i \in \left\{ 1, 2 \right\}$.
%  Assume that a process $p^N_i$ performs an instruction $\tsnd(p^N_i, m)$ in a transition $\conf{N}{1} \rightarrow \conf{N}{2}$. We prove that a process $p^2_i$ performs an instruction $\tsnd(p^2_i, m)$ in a transition $\conf{2}{1} \rightarrow \conf{2}{2}$.
%  Since $m$ has been sent by a process $p^N_i$, we have
%  \begin{align*}
%  \, & \forall p^N_j \colon     m \notin \conf{N}{1} \left( \buf{p^N_i}{p^N_j}\right)   \\
%  \land \, &   \forall p_j \colon   \conf{N}{2} \left( \buf{p^N_i}{p^N_j}\right) = \left\{ m \right\} \cup \conf{N}{1} \left( \buf{p^N_i}{p^N_j}\right) 
%  \end{align*}
%
%  We have $\conf{2}{\ell}(\buf{p^2_i}{q^2_j})  = \conf{N}{\ell}(\buf{p^N_i}{q^N_j})$ for every $1 \leq i, j \leq 2$ and $1 \leq \ell \leq 2$ by the construction of $\conf{2}{2}$ and $\conf{2}{2}$.
%  It follows that 
%  \begin{align*}
%  \, & \forall p^2_j \colon     m \notin \conf{2}{1} \left( \buf{p^2_i}{p^2_j}\right)   \\
%  \land \, &   \forall p_j \colon   \conf{2}{2} \left( \buf{p^2_i}{p^2_j}\right) = \left\{ m \right\} \cup \conf{2}{1} \left( \buf{p^2_i}{p^2_j}\right) 
%  \end{align*}
%  
%  Moreover, we have $\conf{2}{2}(\age{m}) = 0$.
%  Hence, it follows $\conf{2}{2}.\tsnd(p^2_i, m) = \top$.
%  Now we consider which messages  a process $p^2_i$ has received from a process $p_j$ in this round where $i, j \in \left\{ 1, 2 \right\}$. 
%  By the construction of $\conf{2}{2}$, we have 
%  \begin{align*}
%  \conf{2}{2}(p^2_i).\mailbox[p^2_j] & = \conf{N}{2}(p^N_i).\mailbox[p^N_j]
%  = \conf{N}{1}(p^N_i).\mailbox[p^N_j] \\
%  & = \conf{2}{1}(p^2_i).\mailbox[p^2_j]
%  \end{align*}
%  
%  
%%  Since we are considering the subround $\tsnd^N$, it follows  $\conf{N}{1}(\buf{p^2_j}{p^2_i}) \subseteq \conf{N}{2}(\buf{p^2_j}{p^2_i})$.
%  Therefore, we need to prove that $\conf{2}{2}.\rop{p^2_i}[p^2_j]  = \emptyset$.
%  By the construction of $\conf{2}{2}$, it follows $\conf{2}{1}(\buf{p^2_j}{p^2_i}) \subseteq \conf{2}{2}(\buf{p^2_j}{p^2_i})$.
%  It immediately follows that $\conf{2}{2}.\rop{p^2_i}[p^2_j]  = \emptyset$.
%  In other worlds, a process $p^2_i$ has not received any message in this round, and it is consistent with the evaluation of $\conf{2}{2}(p^2_i).\mailbox[p^2_j]$ for every $i, j \in \left\{ 1, 2 \right\}$.
%  Now we prove that every variable's value  $\conf{2}{2}(p^2_i).X_\ell[p^2_j]$ satisfies the corresponding \idsep{} constraint for every $i, j \in \left\{ 1, 2 \right\}$, and $1 \leq \ell \leq M$.
%  Since $\sys{N}$ is ``ID--separation'' and we are considering the subround $\tsnd$, it follows
%  \begin{alignat*}{3}
%  \conf{N}{2}( p^N_i ).X_\ell [p^N_j] & = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
%  & && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M 
%  \big)   
%  \end{alignat*}
%  Since $\conf{N}{2}( p^N_i ).X_\ell [p^N_j] = \conf{2}{2}( p^2_i ).X_\ell [p^2_j]$, we have 
%  \begin{alignat*}{3}
%  \conf{2}{2}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
%  & && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M 
%  \big)   
%  \end{alignat*}
%  It immediately follows that
%  \begin{alignat*}{3}
%  \conf{2}{2}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
%  & && \conf{2}{2}.\trcv(p^2_i)[p^2_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}( p^2_i).X_M 
%  \big)   
%  \end{alignat*}
%  since the later function application is with the same arguments of the first.
%  Finally, by the construction of $\conf{2}{2}$, it is easy to check that every ``not--running'' process does not change its local state and not receive any message in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$. Therefore, this transition simulates a subround Send.
%
%
%  \emph{$\bullet$ Transition $\conf{2}{2} \rightarrow \conf{2}{3}$}. We will show that this transition satisfies every constraint in the subround Receive. 
%  By the ID--projection construction, a process $p^N_i$ takes a step in this subround Receive if and only a process $p^2_i$ takes a step in this subround  for every $i \in \left\{ 1, 2 \right\}$.
%  Hence, we first consider only ``running'' processes. 
%  Assume that a process $p^N_i$ has received a set $S$ of messages from a process $p^N_j$ in a transition $\conf{N}{2} \rightarrow \conf{N}{3}$. 
%  We prove that a process $p^2_i$ has received the same set $S$ of messages from a process $p^2_j$ in a transition $\conf{2}{2} \rightarrow \conf{2}{3}$.
%  By the construction of $\pi^2$, we have 
%  \begin{align*}
%    \conf{N}{2}(\buf{p^N_j}{p^N_i}) & = \conf{2}{2}(\buf{p^N_j}{p^N_i}) \\ \conf{N}{3}(\buf{p^N_j}{p^N_i}) & = \conf{2}{3}(\buf{p^N_j}{p^N_i}) \\
%    \conf{N}{3}.\trcv(p^N_i)[p^N_j] & = S = \conf{N}{2}(\buf{p^N_j}{p^N_i}) \setminus \conf{N}{3}(\buf{p^N_j}{p^N_i}) 
%  \end{align*}
%  It follows that $S = \conf{2}{2}(\buf{p^2_i}{p^2_j}) \setminus \conf{2}{3}(\buf{p^2_i}{p^2_j})$.
%  Moreover, due to 
%  \begin{align*}
%  \conf{N}{3}(p^N_i).\lpc[p^N_j] & = \conf{N}{2}(p^N_i).\lpc[p^N_j] \cup S \\
%  \conf{N}{3}(p^N_i).\mailbox[p^N_j] & = \conf{2}{3}(p^2_i).\mailbox[p^2_j] \\
%  \conf{N}{2}(p^N_i).\mailbox[p^N_j] & = \conf{2}{2}(p^2_i).\mailbox[p^2_j]
%  \end{align*}
%  we have that 
%  $
%  \conf{2}{3}(p^2_i).\mailbox[p^2_j] = \conf{2}{2}(p^2_i).\mailbox[p^N_j] \cup S
%  $.
%  It implies that a process $p^2_i$ has received a set $S$ of messages from a process $p^2_j$.
%  By similar arguments in the above proof for the subround Send, it follows that every variable's value $\conf{2}{3}(p^N_i).X_\ell[p^2_j]$  satisfies the corresponding \idsep{} constraint, i.e.
%  \begin{alignat*}{3}
%  \conf{2}{3}( p^2_i ).X_\ell [p^2_j] & = f_\ell \big( && \tsnd{}, \conf{2}{2}(p^2_i).\lpc,   \conf{2}{3}(\gpc \left[ p^2_i \right]),  \\
%  & && \conf{2}{3}.\trcv(p^2_i)[p^2_j], \conf{2}{2}( p^2_i ).X_1, \ldots, \conf{2}{2}( p^2_i).X_M 
%  \big)   
%  \end{alignat*}
%  Finally, for every ``not--running'' process $p^2 \in \left\{ p^2_1, p^2_2 \right\}$, i.e. $\conf{2}{2}(p^2).\lpc \neq \trcv{}$ or $\conf{2}{3}(\gpc[p^2]) = \bot$, it is easy to check that (i) a process $p^2$ does not update its local state and (ii) message buffers related to  $p^i$ are unchanged. 
%  Therefore, every constraint in the subround $\trcv{}$ is satisfied in the transition $\conf{2}{2} \rightarrow \conf{2}{3}$.
%  
%  \emph{$\bullet$ Transition $\conf{2}{3} \rightarrow \conf{2}{4}$}. We will show that this transition satisfies every constraint in the subround \cop{}.  
%  By the construction of $\conf{2}{4}$ and $\conf{N}{4}$, we have
%  \begin{alignat*}{3}
%    \conf{2}{4}(\buf{p^2_i}{p^2_j}) & = \conf{N}{4}(\buf{p^N_i}{p^N_j}) && = \conf{N}{3}(\buf{p^N_i}{p^N_j}) \\
%    & && = \conf{2}{3}(\buf{p^N_i}{p^N_j}) \\    
%    \conf{2}{4}(p^2_i).\mailbox[p^2_j] & = \conf{N}{4}(p^2_i).\mailbox[p^2_j] && = \conf{N}{3}(p^2_i).\mailbox[p^2_j] \\
%    & && = \conf{2}{3}(p^2_i).\mailbox[p^2_j]    
%  \end{alignat*}
%  It follows no process has sent or received any message in the transition $\conf{2}{3} \rightarrow \conf{2}{4}$.
%  Now we prove that every variable's value  $\conf{2}{2}(p^2_i).X_\ell[p^2_j]$ satisfies the corresponding \idsep{} constraint for every $i, j \in \left\{ 1, 2 \right\}$, and $1 \leq \ell \leq M$.
%  It follows  
%  \begin{alignat*}{3}
%  \conf{2}{4}(p^2_i).X_\ell[p^2_j] & = \conf{N}{3} && (p^N_i).X_\ell[p^N_j]  \\
%  & = f_\ell \big( && \cop{}, \conf{N}{3}(p^N_i).\lpc,   \conf{N}{4}(\gpc \left[ p^N_i \right]),  \\
%  & && \conf{N}{4}.\trcv(p^N_i)[p^N_j], \conf{N}{3}( p^N_i ).X_1, \ldots, \conf{N}{3}(p^N_i).X_M  \big)  \\
%  & = f_\ell \big( && \cop, \conf{2}{3}(p^2_i).\lpc,   \conf{2}{4}(\gpc \left[ p^2_i \right]),  \\
%  & && \conf{2}{4}.\trcv(p^2_i)[p^2_j], \conf{2}{3}( p^2_i ).X_1, \ldots, \conf{2}{3}(p^2_i).X_M  \big)    
%  \end{alignat*}
%  Therefore, every constraint in the subround \cop{} is hold in the transition $\conf{2}{3} \rightarrow \conf{2}{4}$.
%  \item \emph{Induction step for a sequence $\conf{2}{4k - 4} \rightarrow \conf{2}{4k - 3} \rightarrow \conf{2}{4k - 2} \rightarrow \conf{2}{4k - 1} \rightarrow \conf{2}{4k}$.} The proof is similar for the base case.
%  \item Therefore, every sequence $\conf{2}{4k - 4} \rightarrow \conf{2}{4k - 3} \rightarrow \conf{2}{4k - 2} \rightarrow \conf{2}{4k - 1} \rightarrow \conf{2}{4k}$ is a refinement of a global transition at a time $k$.
%  \end{enumerate}
%  Thirdly, we prove that both constraints $\Delta$ and $\Phi$ are hold in the path $\pi^2$ by contradiction. 
%  \begin{itemize}
%  \item \emph{Constraint $\Delta$}: Assume that there exist a transition $\conf{2}{t-1} \xrightarrow{\trcv{}} \conf{2}{t}$ in $\pi^2$ for some $t \geq t_0$, two processes $p^2_i, p^2_j \in \left\{p^2_1, p^2_2 \right\}$, and a message $m$ such that 
%  \begin{alignat*}{4}
%  \noindent
%  \, & m \in \conf{2}{t - 1}(\buf{p^2_j}{p^2_i}) &&  \land  \conf{2}{t - 1}(\gpc[p^2_i])  &&& \,  \land \,  \conf{2}{t - 1}([p^2_i]).\lpc = \trcv{}  \\
%  \land \, &   m \in \conf{2}{t}(\buf{p^2_j}{p^2_i})  && \land \conf{2}{t}(\age{m}) \geq \Delta &&& 
%%  \land \, &  m \in \conf{2}{t}(\buf{p^2_j}{p^2_i}) && \\
%  \end{alignat*}  
%  By the construction of configurations $\conf{2}{t}$ and $\conf{2}{t - 1}$, we have 
%  \begin{align*}
%  \conf{2}{t - 1}(\buf{p^2_j}{p^2_i}) & =  \conf{N}{t - 1}(\buf{p^N_j}{p^N_i}) \\
%  \conf{2}{t}(\buf{p^2_j}{p^2_i}) & =  \conf{N}{t}(\buf{p^N_j}{p^N_i}) \\
%  \forall m \colon   m \in \conf{2}{t - 1}([p^2_i]).\lpc = \trcv{} & \Rightarrow \conf{2}{t}(\age{m}) = \conf{N}{t}(\age{m})
%  \end{align*}
%  Therefore, a message $m$ is not delivered to a process $p^N_i$ in the transition $\conf{N}{t-1} \xrightarrow{\trcv{}} \conf{N}{t}$, and it is at least $\Delta$ time--units old in a configuration $\conf{N}{t}$.
%  It implies the constraint $\Delta$ is violated in $\pi^N$.
%  Contradiction. 
%  
%  \item \emph{Constraint $\Phi$}: By the proof related to the subround \sched{}, it follows that the transition $\conf{2}{4k} \rightarrow \conf{2}{4k + 1}$ is for the subround \sched{} for every $k \geq 0$. 
%  Assume that there exist a number $t \geq t_0$, a correct process $p^2 \in \left\{ p^2_1, p^2_2  \right\}$ such that 
%  $
%  \conf{2}{4t - 3}(\gpc[p^2])  =  \ldots = \conf{2}{4(t + \Delta) - 3}(\gpc[p^2]) = \bot
%  $.
%  In other words, a process $p^2$ does not take any step in the time interval $\left[ t, t + \Phi \right]$. 
%  By the construction of $\pi^2$, we have that $\conf{2}{k}(\gpc[p^2]) = \conf{N}{k}(\gpc[p^2])$ for every $k \geq 0$.
%  Therefore, we have
%  \[
%  \conf{N}{4t - 3}(\gpc[p^N])  =  \ldots = \conf{N}{4(t + \Delta) - 3}(\gpc[p^N]) = \bot
%  \]
%  It implies that a process $p^N$ does not take any step in the time interval $\left[ t, t + \Phi \right]$ after the global stabilization time $t_0$. 
%  Contradiction.
%  
%
%\end{itemize}
%  Therefore, a sequence of configurations $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ is an admissible path in $\sys{2}$. \qed                                                                                                                                                                              
%\end{proof}
%
%%\begin{construction}
%%  Let $t > 0$ be an arbitrary natural number. Let $\lambda^2_k = \conf{2}{4t-4} \leadsto \conf{2}{4t}$ and $\lambda^N_k = \conf{N}{4t-4} \leadsto \conf{N}{4t}$ be finite sequences of configurations in $\sys{2}$ and $\sys{N}$, respectively, such that such sequences are a refinement of some global transition at a time $t$.
%%  The sequence $\lambda^N_t$ is called an \idrefill{} of $\lambda^2_t$ if the following properties hold:
%%  \begin{enumerate}
%%  \item A configuration $\conf{2}{k}$ is an ID--projection of $\conf{N}{k}$ for every $4t - 4 \leq k \leq 4k$.
%%  
%%  \item Every process $p \in \left\{ p_1, \ldots, p_N \right\}$ takes a step at a time $t$. Formally, we have $\forall p \colon   \conf{N}{4t-3}(\gpc[p])$.
%%  
%%  \item If a process $p \in \left\{ p_3, \ldots, p_N \right\}$ performs the instruction $\trcv{}$ in this transition, then all in--transit messages which were sent to $p_i$ are delivered in this transition. Formally, we have
%%  \begin{align*} \forall p \colon   & \left( \conf{N}{4t-4}(p).\lpc = \trcv{} \land \, \conf{N}{4t-3}.\gpc[p] \right) \\
%%  & \qquad \Rightarrow \forall q \colon   \conf{N}{4t-1}(\buf{q}{p} = \emptyset) 
%%  \end{align*}
%%  \end{enumerate}
%%\end{construction}
%
%\begin{lemma} \label{lem:IDRefillConf}
%Let $\conf{2}{0} \leadsto \conf{2}{4}$ be a refinement of a global transition in $\sys{2}$.
%%Let $k$ be a number and $\conf{2}{k - 1}$ be configuration in $\sys{2}$ such that $k > 0$ and a configuration $\conf{2}{k - 1}$ is consistent with some global state. 
%Let $\conf{N}{0}$ be a configuration in $\sys{N}$ such that
%
%\begin{enumerate}  
%\item A configuration $\conf{2}{0}$ is an ID--projection of $\conf{N}{0}$.
%\item All processes $p^N_3, \ldots, p^N_N$ are already crashed in $\conf{N}{0}$, and their related message buffers are empty.
%\item A configuration $\conf{N}{0}$ is consistent with a global state in $\sys{N}$.
%\end{enumerate} 
%
%There exist configurations $\conf{N}{1}, \ldots, \conf{N}{4}$ such that a sequence $\conf{N}{0} \leadsto \conf{N}{4}$ is a refinement of a global transition in $\sys{N}$ and $\conf{N}{4}$ is consistent with a global state in $\sys{N}$.
%\end{lemma}
%
%\begin{proof}
%The proof is by on the construction of configurations $\conf{N}{1}, \ldots, \conf{N}{4}$.
%Since processes $p^N_3, \ldots, p^N_N$ are already crashed in $\conf{N}{0}$ and their related buffers are empty, we need to consider only two processes $p^N_1, p^N_2$ and the messages buffers between two processes. 
%A configuration $\conf{N}{k}$ for every $1 \leq k \leq 4$ is constructed as following:
%
%  \begin{enumerate}
%  \item $\forall i \in 3..N \colon   \conf{N}{k}(p^N_i).\lpc = \texttt{``Crash''}$
%  
%  \item $\forall i \in 3..N, j \in 1..N \colon   \conf{N}{k}(\buf{p^N_i}{p^N_j}) = \conf{N}{k}(\buf{p^N_j}{p^N_i}) = \emptyset $
%  
%  \item $\forall i \in 1..2 \colon   \conf{N}{k}(\gpc[p^N_i]) = \conf{2}{k}(\gpc[p^2_i]) \land \conf{N}{k}(p^N_i).\lpc = \conf{2}{k}(p^2_i).\lpc$
%  
%  \item $\forall i, j \in 1..2 \forall k \in 1..M \colon   \conf{N}{k}(p^N_i).X_k[p^N_j] = \conf{2}{k}(p^2_i).X_k[p^2_j]$
%  
%  \item $\forall i \in 1..2, j \in 3..N \, \forall \ell \in 1..M \colon   \conf{N}{k}(p^N_i).X_\ell[p^N_j] = \\
%  \text{} \quad f_\ell \big(  \texttt{Rnd}, \conf{N}{k-1}(p^N_i).\lpc,  \conf{N}{k-1}(\gpc \left[ p^N_i \right]), \conf{N}{k-1}.\trcv(p^N_i)[p^N_j],  \\    
%  \text{        } \qquad \conf{N}{k-1}( p^N_i ).X_1, \ldots,  \conf{N}{k-1}(p^N_i).X_M 
%  \big)   $
%  
%  \item $\forall i, j \in \left\{1, 2 \right\}  \colon   \conf{N}{k}(p^N_i).\mailbox[p^N_j] = \conf{2}{k}(p^2_i).\mailbox[p^2_j]$
%  
%  \item $\forall i \in 1..2, j \in 3..N  \colon   \conf{N}{k}(p^N_i).\mailbox[p^N_j] = \emptyset$
%\end{enumerate}  
%It immediately follows from the construction that every configuration $\conf{N}{k}$ is one in $\sys{N}$. Now we consider each transition. 
%
%\emph{$\bullet$ Transition $\conf{N}{0} \rightarrow \conf{N}{1}$}. Since neither process states nor message buffers are changed in the transition $\conf{2}{0} \rightarrow \conf{2}{1}$, it immediately follows that neither process states nor message buffers are changed in the transition $\conf{N}{0} \rightarrow \conf{N}{1}$. Therefore, every constraint for the subround \sched{} holds in the transition $\conf{N}{0} \rightarrow \conf{N}{1}$. 
%
%\emph{$\bullet$ Transition $\conf{N}{1} \rightarrow \conf{N}{2}$}. 
%Let $p^N_i \in \left\{ p^N_1, p^N_2 \right\}$ be a ``running'' process in this transition.
%By similar arguments in the proof of Lemma \ref{lem:IDsProjInf} for the subround Send, it follows that (i) a message $m$ has been sent by a process $p^N_i$ in this transition if and only if a message $m$ has been sent by a process $p^2_i$ in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$, and (ii) no in--transit message is removed in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$.
%Moreover, for every $1 \leq \ell \leq M$, for every $p^N_j \in \left\{ p^N_1, p^N_2 \right\}$, we have 
%\begin{alignat*}{3}
%\conf{N}{2}(p^N_i).X_\ell[p^N_j] & = \conf{2}{2} && (p^2_i).X_\ell[p^2_j]  \\
%& = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
%& && \conf{2}{2}.\trcv(p^N_i)[p^N_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}(p^2_i).X_M  \big)  \\
%& = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
%& && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M  \big)    
%\end{alignat*}
%Hence, every constraint for the subround Send holds in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$. 
%
%\emph{$\bullet$ Transition $\conf{N}{1} \rightarrow \conf{N}{2}$}. 
%Let $p^N_i \in \left\{ p^N_1, p^N_2 \right\}$ be a ``running'' process in this transition.
%By similar arguments in the proof of Lemma \ref{lem:IDsProjInf} for the subround Send, it follows that (i) a message $m$ has been sent by a process $p^N_i$ in this transition if and only if a message $m$ has been sent by a process $p^2_i$ in the transition $\conf{2}{1} \rightarrow \conf{2}{2}$, and (ii) no in--transit message is removed in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$.
%Moreover, for every $1 \leq \ell \leq M$, for every $p^N_j \in \left\{ p^N_1, p^N_2 \right\}$, we have 
%\begin{alignat*}{3}
%\conf{N}{2}(p^N_i).X_\ell[p^N_j] & = \conf{2}{2} && (p^2_i).X_\ell[p^2_j]  \\
%& = f_\ell \big( && \tsnd{}, \conf{2}{1}(p^2_i).\lpc,   \conf{2}{2}(\gpc \left[ p^2_i \right]),  \\
%& && \conf{2}{2}.\trcv(p^N_i)[p^N_j], \conf{2}{1}( p^2_i ).X_1, \ldots, \conf{2}{1}(p^2_i).X_M  \big)  \\
%& = f_\ell \big( && \tsnd{}, \conf{N}{1}(p^N_i).\lpc,   \conf{N}{2}(\gpc \left[ p^N_i \right]),  \\
%& && \conf{N}{2}.\trcv(p^N_i)[p^N_j], \conf{N}{1}( p^N_i ).X_1, \ldots, \conf{N}{1}(p^N_i).X_M  \big)    
%\end{alignat*}
%The variable value at indexes $p^N_3, \ldots, p^N_N$ is satisfied the ``ID--separated'' constraint by the construction.
%Hence, every constraint for the subround Send holds in the transition $\conf{N}{1} \rightarrow \conf{N}{2}$. 
%
%\emph{$\bullet$ Transitions $\conf{N}{2} \rightarrow \conf{N}{3} \rightarrow \conf{N}{4}$}. By applying similar arguments in the proof of Lemma \ref{lem:IDProjPath} and in the above proof for the case Send.
%
%As a result, Lemma \ref{lem:IDRefillConf} is correct.
%\qed
%\end{proof}
%
%\begin{lemma} \label{lem:IDRefillment}
%Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$.
%There exists an admissible sequences of configurations $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ in $\sys{N}$ such that a configuration $\conf{2}{k}$ is an ID--projection of $\conf{N}{k}$ for every $k \geq 0$.
%\end{lemma}
%
%
%
%
%\begin{proof}
%  We prove Lemma \ref{lem:IDRefillment} by a constructive proof.
%  First, we describe the initial state of $\pi^N$, and iteratively construct a subsequence $\conf{N}{4t-4} \leadsto \conf{N}{4t}$ for every $t > 0$.
%  Let $\conf{N}{0}$ be a state of $\sys{N}$ such that 
%  \begin{enumerate}
%  \item $\forall i \in 3..N \colon   \conf{N}{0}(p^N_i).\lpc = \texttt{``Crash''}$
%
%  \item $\forall i \in 3..N, j \in 1..N \colon   \conf{N}{0}(\buf{p^N_i}{p^N_j}) = \conf{N}{0}(\buf{p^N_j}{p^N_i}) = \emptyset $
%  
%  \item $\forall i \in 1..2 \colon   \conf{N}{0}(\gpc[p^N_i]) = \conf{2}{0}(\gpc[p^2_i]) \land \conf{N}{0}(p^N_i).\lpc = \conf{2}{0}(p^2_i).\lpc$
%  
%  \item $\forall i, j \in 1..2 \forall k \in 1..M \colon   \conf{N}{0}(p^N_i).X_k[p^N_j] = \conf{2}{0}(p^2_i).X_k[p^2_j]$
%
%  \item $\forall i \in 1..2, j \in 3..N \, \forall k \in 1..M \colon   \conf{N}{0}(p^N_i).X_k[p^N_j] = \conf{2}{0}(p^2_i).X_k[p^2_1]$
%    
%  \item $\forall i, j \in \left\{1, 2 \right\}  \colon   \conf{N}{0}(p^N_i).\mailbox[p^N_j] = \conf{2}{0}(p^2_i).\mailbox[p^2_j]$
%  
%  \item $\forall i \in 1..2, j \in 3..N  \colon   \conf{N}{0}(p^N_i).\mailbox[p^N_j] = \emptyset$
%  \end{enumerate}
%  It is easy to check that (i) $\conf{N}{0}$ is an initial state in $\sys{N}$ and (ii) a configuration $\conf{2}{0}$ is an ID--projection of $\conf{N}{0}$.
%
%  For the construction of the postfix, we iteratively apply the construction and arguments in Lemma \ref{lem:IDRefillConf} for every $k$.
%  \qed
%\end{proof}
%
%
%\newcommand{\corEquivAtomicFixedLocalRead}{
%Let $\mathit{AP}$ be a set of atomic predicates whose is in the form of either $p_i.\lpc = \mathit{val}$ or $p_i.X_\ell[p_j] = \mathit{val}$ where $p_i, p_j$ are processes in $\left\{p_1, p_2 \right\}$, and $X_\ell$ is a local variable.
%Then, two systems $\sys{2}$  and $\sys{N}$ are trace equivalent under $\mathit{AP}$.
%}
%
%\begin{corollary} \label{cor:EquivAtomicFixedLocalRead}
%\corEquivAtomicFixedLocalRead
%\end{corollary}
%
%\begin{proof}
%It immediately follows by Lemmas \ref{lem:IDProjPath} and \ref{lem:IDRefillConf}.
%\end{proof}
%
%
%
%\newcommand{\lemEquivFixedLocalRead}{
%  Let $\idsepalgo{}$ be an \idsep{} algorithm with fixed values for $\Delta$ and $\Phi$.
%  Let $\sys{2}$ and $\sys{N}$ be two instances of $\idsepalgo$
%  Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ and $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ be admissable infinite sequences of configurations respectively in $\sys{2}$ and $\sys{N}$ such that a configuration $\conf{2}{k}$ is an ID--projection of a configuration $\conf{N}{k}$ for every $k \geq 0$.
%  Let $F(p_1, p_2)$ be an arbitrary formula based on local read prediates with indexes $p_1, p_2$.
%  It follows that $\conf{2}{k} \models F(p_1, p_2)$ if and only if $\conf{N}{k} \models F(p_1, p_2)$ for every $k \geq 0$.
%}
%
%\begin{lemma} \label{lem:EquivFixedLocalRead}
%\lemEquivFixedLocalRead
%\end{lemma}
%
%\begin{proof}
%  Let $k$ be a number such that $k \geq 0$. We prove the direction $(\Rightarrow)$ by induction on the structure of $F(p_1, p_2)$. 
%  The base case immediately follows by Corollary \ref{cor:EquivAtomicFixedLocalRead}. 
%  The proof of the induction step is by cases for the negation $\lnot$ and the conjunction $\land$ since the rest of connectives can be replaced with such connectives. 
%  Notice that every quantified variable in $F(p_1, p_2)$ is bounded in a finite domain $\left\{p_1, p_2\right\}$, we could eliminate the quantifer $\forall$ with the conjuction $\land$.
%  
%  \begin{itemize}   
%  \item  \emph{Case $ F(p_1, p_2) = \lnot F_1(p_1, p_2)$.} 
%  By the induction hypothesis, it follows that $\conf{2}{k} \models F_1(p_1, p_2) \Rightarrow \conf{N}{k} \models F_1(p_1, p_2)$. 
%  Hence, we have that if $\conf{2}{k} \models \lnot F_1(p_1, p_2)$, then $\conf{N}{k} \models \lnot F_1(p_1, p_2)$. 
%  
%  \item \emph{Case $ F(p_1, p_2) =  F_1(p_1, p_2) \land F_2(p_1, p_2)$.}
%  By the induction hypothesis, it follows that $\conf{2}{k} \models F_i(p_1, p_2) \Rightarrow \conf{N}{k} \models F_i(p_1, p_2)$ for every $1 \leq i \leq 2$.
%  Hence, we have that if $\conf{2}{k} \models \lnot F(p_1, p_2)$, then $\conf{N}{k} \models \lnot F(p_1, p_2)$. 
%  
%  
%  \end{itemize}
%  
%  
%  
%  Hence, the direction $(\Rightarrow)$ holds. The proof for another direction is similar.
%\qed
%\end{proof}
%
%\subsection{Quantified formulas with local read predicates}
%
%%The following results are with 
%To extend the previous result, we first prove Lemmas \ref{lem:RenameOne}--\ref{lem:RenameTwo} which says that two instances $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ of an \idsep algorithm are equivalent under a renaming function where $u, v$ are distinguished processes' id. 
%Then, Theorem \ref{thm:EquivLocalRead} says that two instances  $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ of an~\idsep algorithm $\mathcal{A}$ are equivalent under a renaming function and a local read formula $F(p_u, p_v)$ where $u, v$ are distinguished processes' id. 
%Finally, we provide a discussion about the application in checking a class of LTL formulas in the form of $\lozenge \square \forall p_i, p_j \colon   F(p_i, p_j)$.
%
%
%\newcommand{\lemRenameOne}{
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm.
%  Let $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ be instances of $\mathcal{A}$  where $p_u, p_v$ are distinguished processes. 
%  Let $h \colon \left\{p_1, p_2\right\} \rightarrow \left\{ p_u, p_v \right\}$ be a bijective function such that $h(p_1) = p_v$ and $h(p_2) = p_v$.
%%  \begin{enumerate}
%%  \item 
%  Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$. Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%%  \begin{subequations}
%  \begin{align*}
%  \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h(p_i)}{h(p_j)}) \\
%  \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h(p_i)]) \\
%  \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h(p_i)).X[h(p_j)] \\
%  \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h(p_i)).\lpc 
%  \end{align*} 
%  
%%\end{subequations}
%%  for every $p_i, p_j \in \left\{p_1, p_2\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$.
%%  Then, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
%%  
%%   \item Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be an admissible sequence of configuration in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$. Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%%  \begin{subequations}
%%  \begin{align}
%%  \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h^{-1}(p_i)}{h^{-1}(p_j)}) \\
%%  \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h^{-1}(p_i)]) \\
%%  \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h^{-1}(p_i)).X[h^{-1}(p_j)] \\
%%  \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h^{-1}(p_i)).\lpc 
%%  \end{align} 
%%  \end{subequations}
%%  for every $p_i, p_j \in \left\{p_u, p_v\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$ and $h^{-1}$ is a inverse function of a renaming function $h$.
%%  Then, a sequence $\pi^{\prime}$ is admissible in $\sys{2}$.
%%  \end{enumerate}
%  }
%
%\begin{lemma} \label{lem:RenameOne}
%\lemRenameOne
%\end{lemma}
%
%\begin{proof}
%The existence of $\pi^{\prime}$ is demonstrated by a constructive proof.
%  By similar arguments in the proof of Lemma \ref{lem:IDProjConf}, it follows that $\conf{\prime}{0}$ is an initial state in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
%  By similar arguments in the proof of Lemma \ref{lem:IDProjPath}, it follow that $\conf{\prime}{4t - 4} \leadsto \conf{\prime}{4t}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ for every $t \geq t_0$, and both constraints $\Delta$ and $\Phi$ hold in $\pi^{\prime}$.
%  Hence, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
%  
%%  \item By similar arguments in the above proof, it follows that the sequence $\pi$ is admissible in $\sys{2}$. \qed
%%\end{enumerate}
%\end{proof}
%
%\newcommand{\lemRenameTwo}{
%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm.
%  Let $\sys{2}$ and $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$ be instances of $\mathcal{A}$  where $p_u, p_v$ are distinguished processes. 
%  Let $h \colon \left\{p_1, p_2\right\} \rightarrow \left\{ p_u, p_v \right\}$ be a bijective function such that $h(p_1) = p_v$ and $h(p_2) = p_v$.
%%  \begin{enumerate}
%%    \item Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be an admissible sequence of configurations in $\sys{2}$. Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%%    %  \begin{subequations}
%%    \begin{align}
%%    \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h(p_i)}{h(p_j)}) \\
%%    \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h(p_i)]) \\
%%    \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h(p_i)).X[h(p_j)] \\
%%    \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h(p_i)).\lpc 
%%    \end{align} 
%%    
%    %\end{subequations}
%    %  for every $p_i, p_j \in \left\{p_1, p_2\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$.
%    %  Then, a sequence $\pi^{\prime}$ is admissible in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$.
%    %  
%    %   \item 
%    Let $\pi^{\prime} = \conf{\prime}{0} \conf{\prime}{1} \ldots$ be an admissible sequence of configuration in $S_{\left\{u, v\right\}}( \mathcal{A}, \Delta, \Phi)$. Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be a sequence of configurations  such that these sequences have the same global stabilization time, and the following properties hold
%    %  \begin{subequations}
%      \begin{align*}
%      \conf{}{t}(\buf{p_i}{p_j}) & = \conf{\prime}{t}(\buf{h^{-1}(p_i)}{h^{-1}(p_j)}) \\
%      \conf{}{t}(\gpc[p_i]) & = \conf{\prime}{t}(\gpc[h^{-1}(p_i)]) \\
%      \conf{}{t}(p_i).X[p_j] & = \conf{\prime}{t}(h^{-1}(p_i)).X[h^{-1}(p_j)] \\
%      \conf{}{t}(p_i).\lpc & = \conf{\prime}{t}(h^{-1}(p_i)).\lpc 
%      \end{align*} 
%    %  \end{subequations}
%      for every $p_i, p_j \in \left\{p_u, p_v\right\}$, for every $X \in \left\{ X_1, \ldots, X_M, \mailbox \right\}$ and $h^{-1}$ is a inverse function of a renaming function $h$.
%      Then, a sequence $\pi^{\prime}$ is admissible in $\sys{2}$.
%%  \end{enumerate}
%}
%
%\begin{lemma} \label{lem:RenameTwo}
%  \lemRenameTwo
%\end{lemma}
%
%\begin{proof}
%  By similar arguments in the proof of \ref{lem:RenameOne}, it follows that the sequence $\pi$ is admissible in $\sys{2}$. \qed  
%\end{proof}
%
%\newcommand{\thmEquivLocalRead}{
%  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
%  Let $F(p_u, p_v)$ be a local read formula where $p_u, p_v \in \left\{ p_1, \ldots, p_N \right\}$.
%  Let $h$ be a bijective renaming function such that $h(p_1) = p_u$ and $h(p_v) = p_2$.
%  \begin{enumerate}
%  \item Let $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$ be an admissible infinite sequence of configurations in $\sys{N}$. There exists an admissible infinite sequence of configurations $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$   in $\sys{2}$ such that if $\conf{N}{k} \models F(p_u, p_v)$ then $\conf{2}{k} \models F(h^{-1}(p_u), ^{-1}(p_v))$ for every $k \geq 0$  where $h^{-1}$ is a inverse function.
%        
%  \item Let $\pi^2 = \conf{2}{0} \conf{2}{1} \ldots$ be an admissible infinite sequence of configurations in $\sys{2}$. There exists an admissible infinite sequence of configurations $\pi^N = \conf{N}{0} \conf{N}{1} \ldots$   in $\sys{N}$ such that if $\conf{2}{k} \models F(h^{-1}(p_u), h^{-1}(p_v))$ then $\conf{N}{k} \models F(p_u, p_v)$ for every $k \geq 0$
%  where $h^{-1}$ is a inverse function.
%  \end{enumerate}
%}
%
%
%\begin{theorem} \label{thm:EquivLocalRead}
%  \thmEquivLocalRead
%\end{theorem}
%
%\begin{proof}
%  We first present a proof for part 1. 
%  By Lemma \ref{lem:IDProjPath}, there exist an admissible sequence  of configurations $\pi = \conf{}{0} \conf{}{1} \ldots$ in $S_{u, v}(\mathcal{A})$ such that a configuration $\conf{}{k}$ is an~\idsep{} of $\conf{N}{k}$ for every $k \geq 0$.
%  By Lemma \ref{lem:EquivFixedLocalRead}, it follows that if $\conf{N}{k} \models F(p_u, p_v)$
%  then $\conf{}{k} \models F(p_u, p_v)$ for every $k \geq 0$.
%  By Lemma \ref{lem:EquivFixedLocalRead}, it follows that if $\conf{N}{k} \models F(p_u, p_v)$
%  then $\conf{2}{k} \models F(h^{-1}(p_u), h^{-1}(p_v))$ for every $k \geq 0$.
%    
%  The proof for part 2 is similar.  \qed
%\end{proof}
%
%\newcommand{\lemStrongLivenessWithFiniteDomains}{
%  Let $S$ be a labelled transition system, and $\varphi_1, \ldots \varphi_n$ be first-order predicates.
%  Assume that $S \models \square \lozenge \left( \varphi_1 \lor \ldots \lor \varphi_n \right) $.
%  There exists a number $i$ such that $1 \leq i \leq n$ and $S \models \square \lozenge  \varphi_i $.
%}
%
%
%\begin{lemma} \label{lem:StrongLivenessWithFiniteDomains}
%\lemStrongLivenessWithFiniteDomains
%\end{lemma}
%
%\begin{proof}
%  We prove Lemma \ref{lem:StrongLivenessWithFiniteDomains} by contradiction.
%  Assume that $S \not\models \square \lozenge \varphi_i$ for every $i$. 
%  It follows that $S \models \lozenge \square \lnot \varphi_i$ for every $i$.
%  Let $\pi = \sigma_0 \sigma_1 \ldots$ be an arbitrary path of $S$.
%  It follow that $\exists t_i \colon t_i \geq 0 \land \big( \forall t \colon t \geq t_i \Rightarrow \sigma_t \models \lnot \varphi_i \big)$ for every $1 \leq i \leq n$.
%  Let $T = \mathop{\mathit{MAX}} \left\{t_1, \ldots , t_n \right\}$.
%  It follows that $\forall t \colon t \geq T \Rightarrow \sigma_t \models \lnot \varphi_i $ for every $1 \leq i \leq n$.
%  It implies that $\exists T \colon T \geq 0 \land \big( \forall t \colon t \geq T \Rightarrow \sigma_t \models \bigwedge_{1 \leq i \leq n} \lnot \varphi_i \big)$. 
%  In other words, we have $S \not\models \square \lozenge \left( \varphi_1 \lor \ldots \lor \varphi_n \right)$.
%  Contradiction. \qed
%\end{proof}
%
%\newcommand{\corNCutoffInStrongLiveness}{
%  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
%  Let $F(p, q)$ be a local read formula with free variables $p, q$. 
%  It follows $\sys{N} \models \lozenge \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q) $ if and only if $\sys{2} \models \lozenge \square \forall p, q \in \{p^2_1, p^2_2 \} \colon  F(p, q) $.
%}
%
%\begin{corollary} \label{cor:NCutoffInStrongLiveness}
%\corNCutoffInStrongLiveness
%\end{corollary}
%
%\begin{proof} We prove both directions by contradiction. 
%  To keep the presentation simple, we use two notations  $G_N \triangleq \sys{N} \models \lozenge \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q)$ and $G_2 \triangleq \sys{2} \models \lozenge \square \forall p, q \in \{p^2_1,  p^2_2 \} \colon  F(p, q)$ in the following proofs.
%  \begin{enumerate}
%  \item Assume that $\sys{N} \models G_N $ but $\sys{2} \not\models G_2 $.
%  We have
%  \begin{align*}
%    \sys{2} \not\models G_2
%  \, \Leftrightarrow \,  & \sys{2} \not\models \lozenge \square \bigwedge_{p, q \in \{p^2_1, p^2_2 \}}   F(p, q)  \\
%  \, \Leftrightarrow \,    & \sys{2} \models  \square \lozenge \bigvee_{p, q \in \{p_1, p_2 \}} \lnot F(p, q)
%  \end{align*}
%  
% 
%  Hence, there exists $p^2_0, q^2_0 \in \left\{p^2_1, p^2_2\right\}$ such that $
%  \sys{2} \models \square \lozenge \lnot F(p^2_0, q^2_0)$ by Lemma \ref{lem:StrongLivenessWithFiniteDomains}.
%  By Theorem \ref{thm:EquivLocalRead}, it follows $\sys{N} \models \square \lozenge \lnot F(p^N_0, q^N_0)$.
%  Contradiction.
%  
%  \item  Assume that  $\sys{2} \models G_2 $ but $\sys{N} \lnot\models G_N$. 
%  We have
%  \begin{align*}
%  \sys{N} \not\models G_N
%  \, \Leftrightarrow \,  & \sys{N} \not\models \lozenge \square \bigwedge_{p, q \in \{p^N_1, \ldots, p^N_N \}}   F(p, q)  \\
%  \, \Leftrightarrow \,    & \sys{N} \models  \square \lozenge \bigvee_{p, q \in \{p^N_1, \ldots, p^N_N \}} \lnot F(p, q)
%  \end{align*}
%  By Lemma \ref{lem:StrongLivenessWithFiniteDomains}, there exists $p^N_0, q^N_0 \in \left\{p^N_1, \ldots, p^N_N\right\}$ such that $
%  \sys{N} \models \square \lozenge \lnot F(p^N_0, q^N_0)$ .
%  By Theorem \ref{thm:EquivLocalRead}, there exists $p^2_0, q^2_0 \in \left\{p^2_1,  p^2_2\right\}$  such that $
%  \sys{2} \models \square \lozenge \lnot F(p^2_0, q^2_0)$. 
%  Contradiction.
%  \end{enumerate}
%  Therefore, Corollary \ref{cor:NCutoffInStrongLiveness} is correct. \qed
%\end{proof}
%
%\newcommand{\corNCutoffInSafety}{
%  Let~$\idsepalgo$ be an~\idsep{} algorithm with two instances $\tinst$ and $\ninst$ where $N \geq 0$.
%  Let $F(p, q)$ be a local read formula with free variables $p, q$. 
%  It follows $\sys{N} \models  \square \forall p, q \in \{p^N_1, \ldots, p^N_N \} \colon  F(p, q) $ if and only if $\sys{2} \models  \square \forall p, q \in \{p^2_1, p^2_2 \} \colon  F(p, q) $.
%}
%
%\begin{corollary} \label{cor:NCutoffInSafety}
%  \corNCutoffInSafety
%\end{corollary}
%
%\begin{proof}
%It immediately follows by Corollary \ref{cor:NCutoffInStrongLiveness}. \qed
%\end{proof}
%
%\begin{remark}
%By Corollaries \ref{cor:NCutoffInStrongLiveness} and \ref{cor:NCutoffInSafety}, the problem of checking many useful properties in the form of $\lozenge \square \forall p, q \colon F(p, q)$ or $ \square \forall p, q \colon F(p, q)$ for~\idsep{} algorithms of all sizes  can be reduced to checking them on instances with two processes where $F(p,q)$ is a formula based on local read atomic predicate.
%In other words, such properties of~\idsep{} algorithms have a cutoff of 2.
%\end{remark}
%
%%To prove the trace equivalence of $S_{1..N}(\Delta, \Phi)$ and $S_{1, 2}(\Delta, \Phi)$, we first define two techniques for path constructions called ID--projection and ``ID--refillment''.
%%Lemmas \ref{lem:IDsProj} and \ref{lem:IDsRefill} shows that finite execution paths constructed with these techniques are legal ones in corresponding system instances.
%%Such results are extended for infinite paths in Lemmas  \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}
%%
%%\subsection{Path constructions}
%%
%%\begin{definition}
%%Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%%Let $\pi^N = \gconf{0}^N \gconf{1}^N \ldots$ and $\pi^2 = \gconf{0}^2 \gconf{1}^2 \ldots$ be arbitrary infinite execution paths of $S_{1..N}(\mathcal{A}, \Delta, \Phi)$ and $S_{1..2}(\mathcal{A}, \Delta, \Phi)$, respectively.
%%Path $\pi^2$  is called a \emph{\proj{k}} of path $\pi^N$ if the following property hold:
%%
%%\begin{enumerate}
%%  \item The global stabilization time of two paths are the same.
%%    
%%  \item For every $i \in \{p_1, p_2\}$, it follows $\gconf{k}^N(\gpc[p_i]) = \gconf{k}^2(\gpc[p_i])$.
%%  
%%  \item For every $i, j \in \{1, 2\}$, it follows $\gconf{k}^N(\buf{p_i}{p_j}) = \gconf{k}^2(\buf{p_i}{p_j})$.
%%  
%%%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if process $p_i^N$ receives a set of messages $\mathit{Msgs}$ in state $s^N_k$, then process $p_i^2$ receives a set of messages $\{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ in state $s^2_k$. \footnote{TODO: Override notations here since $m$ is used for different messages in different system instances.}
%%%  
%%%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ and $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ are the same.
%%%  
%%%  \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
%%%  
%%%  \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^N$ crashes at time point $k$, then process $p_i^2$ also crashes at time point $k$.
%%\end{enumerate}
%%
%%\end{definition}
%%
%%
%%\newcommand{\lemIDsProj}{
%%Let $\pi^N = s_0^N \ldots  s_\ell^N$ be an arbitrary finite execution path of $S_{1..N}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%%There exists a finite path $\pi^2 = s^2_0 \ldots s^2_\ell$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an $\ell$--finite ID--projection path of $\pi^N$.
%%}
%%
%%\begin{lemma} \label{lem:IDsProj}
%%\lemIDsProj
%%\end{lemma}
%%
%%\begin{proof}
%%  It is easy to see that the first constraint about the stabilization time is satisfied by the definition of those system instances. 
%%  In the following, we present how to construct an $\ell$--finite ID--projection path of $\pi^N$, and explain how other constraints are satisfied.
%%  The construction is based on the induction on the length $\ell$ of an execution path. 
%%  
%%  \begin{itemize}
%%  \item \emph{Base case $\ell = 0$}. In the base case, path $\pi^N$ has only the initial state. 
%%  Lemma \ref{lem:IDsProj} is correct because it is safe to set the initial state of processes and message buffers in $S_{1..2}(\Delta, \Phi)$ such that for every $i, j \in \{1, 2\}$, for every local variable $X$, we have $s_0^N(p_i, X[p_j]) = s_0^2(p_i, X[p_j])$ and $s_0^N(\mathit{msgBuf}^N[i, j]) = s_0^2(\mathit{msgBuf}^N[i, j])$.
%%  
%%  \item Assume that Lemma \ref{lem:IDsProj} is correct for the case $\ell_0 \geq 0$. We prove the case $\ell_0 + 1$. By the induction hypothesis, there exists a finite path $\rho$ in $S_{1..2}(\Delta, \Phi)$ such that $\rho$ is an $\ell_0$--finite ID--projection path for the prefix $s_0^N \ldots s_{\ell_0}^N$ of $\pi^N$. We will show that we can obtain $\pi^2$ by extending $\rho$ with a reachable state $s^2_{\ell}$. Here (and now) we present only the most complicated case where both $p_1$ and $p_2$ are still correct at time point $\ell$. For other cases where crashes happen, the proof is much simpler. \footnote{TODO: Provide some arguments for cases with crashes.} The construction of $s^2_\ell$ where processes $p^2_1$ and $p^2_2$ are still correct is given below.
%%  
%%  \begin{enumerate}
%%      \item Both processes $\pi^N_i$  and $\pi^2_i$ executes the same action on time point $\ell$ for every $i \in \{1, 2\}$. Notice that the action of $\pi^2_i$ is enable because of the induction hypothesis. As a result, the constraint $\Phi$ still holds in $\pi^2$ until $\ell$. (If not, the constraint $\Phi$ does not hold in the interval $[\ell - \Delta, \ell]$ in the execution path $\pi^N$. Contradiction) Therefore, the extension of $\rho$ in this way constructs a legal finite path which satisfies the second constraint.
%%      
%%      \item In the Send round in global tick $\ell$, it is easy that if message $m$ has been added to message bufer $\mathit{msgBuf}^N[i, j]$ for every $1 \leq i, j \leq 2$, then a corresponding message $m$ has been also added to message bufer $\mathit{msgBuf}^2[i, j]$. 
%%      By the induction hypothesis, it follows that until now message buffers $\mathit{msgBuf}^2[i, j]$ and $\mathit{msgBuf}^N[i, j]$ are the same for every $1 \leq i, j \leq 2$.
%%      Because our computational model does not allow ``send'' processes to receive any messages and not to join later rounds, we have that 
%%T      \begin{align*}
%%       s^N_\ell(p_i, X[p_j]) & = f(\{\}, s^N_{\ell_0}X_1[p_j], \ldots, , s^N_{\ell_0}X_m[p_j]) \text{, and } \\ 
%%       s^2_\ell(p_i, X[p_j]) & = f(\{\}, s^2_{\ell_0}X_1[p_j], \ldots, , s^2_{\ell_0}X_m[p_j])
%%      \end{align*}
%%      for every local variable $X$. Due to the induction hypothesis, we have that $s^N_{\ell_0}X_k[p_j] = s^2_{\ell_0}X_k[p_j]$ for every $k$. It follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$.
%%      
%%      \item In the Receive round, if message $m$ from process $p^N_j$ has been delivered to process $p^N_i$ for every $1 \leq i, j \leq 2$, then either message $m$ was already in $\mathit{msgBuf}^N[j, i]$ in $\ell_0$ or message $m$ has been added to $\mathit{msgBuf}^N[j, i]$ in the last Send round.
%%      In the first case, by induction hypothesis, it follows that $m$ was already in $\mathit{msgBuf}^2[j, i]$  in $\ell_0$. In the later case, by arguments in the second point, it follows that $m$ has been added in $\mathit{msgBuf}^2[j, i]$  in the last Send round.
%%      Therefore, it is possible for process $p^2_i$ to receive message $m$ in this Receive round.
%%      In other words, if process $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_\ell$, then it is safe to deliver a set of messages $\mathit{Msgs}^2 = \{ m \in \mathit{Msgs} \mid m_{id} \in \{1, 2 \} \}$ to process $p_i^2$ in state $s^2_\ell$. 
%%      Therefore, we can construct $\pi^2$ such that the third constraint holds in $\pi^2$.
%%      Because processes $p^N_i$ and $p^2_i$ have received the same set of messages in this round, and message buffers $\mathit{msgBuf}^N[i, j]$ and $\mathit{msgBuf}^2[i, j]$ are the same for every $1 \leq i, j \leq 2$ before entering this round, such message buffers are still the same after this round.
%%      Moreover, by similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is a ``Receive'' process, and $X$ is a local variable.
%%      
%%      \item In the Internal Computation round, since (i) no messages are added to any message buffer and (ii) no messages are delivered, the second and third constraints obviously hold.
%%      By similar arguments in for the Send round, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$ where $p_i$ is an ``Internal Computation'' process, $1 \leq i, j \leq 2$, and $X$ is a local variable.
%%     
%%      \item By the merge of three round, it follows that constraints 2--6 holds by the construction of $\pi^2$.
%%  \end{enumerate}
%%  Therefore, Lemma \ref{lem:IDsProj} is correct in case of $\ell$. \footnote{The organization of the definition and proof of Lemma \ref{lem:IDsProj} seems a bit difficult to follow. Perhaps we should split it into smaller trunks.} \qed
%%  \end{itemize}
%%\end{proof}
%%
%%\begin{definition}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%%  Let $\pi^2 = s_0^2 \ldots s_\ell^2$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%%  A finite execution path $\pi^N = s_0^N \ldots s_\ell^N$ is called a \emph{$\ell$--finite ``ID--refillment'' path} of $\pi^2$ if the followings hold:
%%  
%%  \begin{itemize}
%%    \item The stabilization  time of two paths are the same.
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ executes an operator $\mathit{Op}$ in state $s^2_k$, then process $p_i^N$ executes the same operator $\mathit{Op}$ in state $s^N_k$.
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, for an arbitrary set of messages $\mathit{Msgs}$, if processes $p_i^2$ receives messages $\mathit{Msgs}^2$ in state $s^2_k$, then processes $p_i^N$ receives a set of messages $\mathit{Msgs}^N$ in state $s^N_k$ such that
%%    \[
%%    \mathit{Msgs}^N = \mathit{Msgs}^2 \cup \{ m \mid m \in \mathit{msgBuf}[j][i] \land j \in 3..N \}
%%    \]
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, message buffers $\mathit{msgBuf}^2[i, j]$ in state $s^2_k$ and $\mathit{msgBuf}^N[i, j]$ in state $s^N_k$ are the same.
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $i, j \in \{1, 2\}$, for every local variable $X \in \left\{ X_1, \ldots, X_M \right\}$, it follows that $s^N_\ell(p_i, X[p_j]) = s^2_\ell(p_i, X[p_j])$. 
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $i \in \{1, 2\}$, if process $p_i^2$ crashes at time point $k$, then process $p_i^N$ also crashes at time point $k$.
%%    
%%    \item For every $j \in 3..N$, process $p_j^N$ never crashes.
%%    
%%    \item For every $j \in 3..N$, process $p_j^N$ executes the operator $\mathit{Send}$ in state $s^N_0$.
%%    
%%    \item For every $j \in 3..N$,  process $p_j^N$ takes a transition in every global tick.
%%    
%%    
%%    \item For every $0 \leq k \leq \ell$, for every $j \in 3..N$, if process $p_j^N$ executes the operator $\mathit{Receive(j)}$ in state $s^N_k$, then every message which was sent to process $j^N$ and but not received will be delivered to process $p_j^N$ in state $s^N_k$.
%%    
%%  \end{itemize}
%%  
%%\end{definition}
%%
%%
%%\newcommand{\lemIDsRefill}{
%%Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary finite execution path of $S_{1..2}(\Delta, \Phi)$ for some number $\ell \geq 0$.
%%There exists a finite path $\pi^N = s^N_0 \ldots s^N_\ell$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an $\ell$--finite ``ID--refillment'' path of $\pi^2$.
%%}
%%
%%\begin{lemma} \label{lem:IDsRefill}
%%\lemIDsRefill
%%\end{lemma}
%%
%%\begin{proof}
%%  The proof of Lemma \ref{lem:IDsRefill} is by the induction on the length $\ell$ of the execution path, and by similar arguments in the proof of Lemma \ref{lem:IDsProj} \qed
%%\end{proof}
%%
%%\begin{definition}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%%  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary infinite execution path of $S_{1..N}(\Delta, \Phi)$.
%%  An infinite execution path $\pi^2 = s_0^2 s_1^2 \ldots$ is called an \emph{infinite ID--projection path} of $\pi^N$ if for every number $\ell \geq 0$, its prefix $\pi^2 = s_0^2 \ldots s_\ell^2$ is an $\ell$--finite ID--projection path of $\pi^N$.
%%\end{definition}
%%
%%
%%\newcommand{\lemIDsProjInf}{
%%  Let $\pi^N = s_0^N s_1^N \ldots$ be an arbitrary legal execution path of $S_{1..N}(\Delta, \Phi)$.
%%  There exists an infinite path $\pi^2 = s^2_0 s^2_1 \ldots$ in $S_{1..2}(\Delta, \Phi)$ such that $\pi^2$ is an infinite ID--projection path of $\pi^N$.
%%}
%%
%%\begin{lemma} \label{lem:IDsProjInf}
%%  \lemIDsProjInf
%%\end{lemma}
%%
%%\begin{proof}
%%  We prove Lemma \ref{lem:IDsProjInf} by contradiction.
%%  Assume that no infinite path in $S_{1..2}(\Delta, \Phi)$ is an infinite ID--projection path of $\pi^N$.
%%  Hence, there exists a number $\ell \geq 0$ such that the prefix $s_0^N \ldots s_\ell^N$ has no $\ell$--finite ID--projection path. in $S_{1..2}(\Delta, \Phi)$. 
%%  Contradiction. \qed
%%\end{proof}
%%
%%
%%\begin{definition}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..2}(\Delta, \Phi)$  and $S_{1..N}(\Delta, \Phi)$ be two instances of $\mathcal{A}$.
%%  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary infinite execution path of $S_{1..2}(\Delta, \Phi)$.
%%  An infinite execution path $\pi^N = s_0^N s_1^N \ldots$ is called an \emph{infinite ``ID--refillment'' path} of $\pi^2$ if for every number $\ell \geq 0$, its prefix $\pi^N = s_0^N \ldots s_\ell^N$ is an $\ell$--finite ``ID--refillment'' path of $\pi^2$.
%%\end{definition}
%%
%%
%%\newcommand{\lemIDsRefillInf}{
%%  Let $\pi^2 = s_0^2 s_1^2 \ldots$ be an arbitrary legal execution path of $S_{1..2}(\Delta, \Phi)$.
%%  There exists an infinite path $\pi^N = s^N_0 s^N_1 \ldots$ in $S_{1..N}(\Delta, \Phi)$ such that $\pi^N$ is an infinite ``ID--refillment'' path of $\pi^2$.
%%}
%%
%%\begin{lemma} \label{lem:IDsRefillInf}
%%  \lemIDsRefillInf
%%\end{lemma}
%%
%%\begin{proof}
%%  By applying similar arguments in the proof of Lemma \ref{lem:IDsProjInf}.
%%  \qed
%%\end{proof}
%%
%%\subsection{A cutoff of the number of processes}
%%
%%From now on, the notation $\mathit{comp}(p_i, X, p_j, \mathit{val})$ denotes an atomic predicate  which means the local variable $X[p_j]$ of process $p_i$ has the value $\mathit{val}$. 
%%
%%Moreover the notation $\mathit{comp}(\mathit{msgBuf}[i, j], \mathit{val})$ denotes an atomic predicate  which means the message buff $\mathit{msgBuf}[i, j]$  has the value $\mathit{val}$. 
%%Such predicates are called ``var--comp'' and ``buffer--comp'', respectively.
%%
%%\begin{lemma}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``var--comp'' predicate whose indexes are 1 and 2.
%%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
%%\end{lemma}
%%
%%\begin{proof}
%%  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
%%\end{proof}
%%
%%\begin{lemma}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathit{pred}$ be an atomic ``buffer--comp'' predicate whose indexes are 1 and 2.
%%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathit{pred}$.
%%\end{lemma}
%%
%%\begin{proof}
%%  It immediately follows by Lemmas \ref{lem:IDsProjInf} and \ref{lem:IDsRefillInf}. \qed
%%\end{proof}
%%
%%
%%\begin{theorem} \label{thm:cutoff}
%%  Let $\mathcal{A}$ be an arbitrary~\idsep{} algorithm with $M$ local variables $X_1, \ldots, X_M$.
%%  Let $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ be two instances of $\mathcal{A}$, and $\mathcal{P}$ be a predicate built on ``var--comp'' and ``buffer--comp'' predicates whose indexes are 1 and 2.
%%  Two instances $S_{1..N}(\Delta, \Phi)$  and $S_{1..2}(\Delta, \Phi)$ are trace equivalent under the predicate  $\mathcal{P}$.
%%\end{theorem}
%%
%%\begin{proof}
%%  We prove Theorem \ref{thm:cutoff} by induction on the structure of predicate $\mathcal{P}$. \qed
%%\end{proof}
%%
%%%If $\textit{var}$ is one dimensional array, we override the notation by writing $\assgn{\textit{var}}{\{id_1\}}{\textit{val}}$.
%%%Such predicates are called ``assignment'' ones.



==> netys20/prop_in_dls.tex <==

%Lemmas \ref{lem:UnboundedMsgBufOne}--\ref{lem:UnboundedMsgBuf} show that there exists an execution prefix such that message buffers in this time interval are unbound. 
%Moreover, Lemmas \ref{lem:BoundRcvdMsgDelay}--\ref{lem:BoundCorrMsgBuf} show that there exists an postfix such that every message buffer of a correct process in the
%postfix is bounded. 
%Under Assumption \ref{asmp:CrashProc}, we obtain two Lemmas \ref{lem:BoundMsgBuf}--\ref{lem:SilentCrashedProc} for crashed processes.

%\subsection{Underlying assumptions and interesting algorithm classes}

%Since every correct process follows the same deterministic protocol (Assumption 4), we can have Lemmas \ref{lem:PhiS} and \ref{lem:PhiR} for correct processes. 
%Intuitively, the guards $\Phi_S$ and $\Phi_R$ in these assumptions describe how often a correct process sends and receives messages. 
%The values of $\Phi_S$ and $\Phi_R$ depend on the algorithm implementation.
%In Section \ref{sec:fd}, we will discuss a specific algorithm -- Chandra and Toug's failure detector \cite{CT96}, and give specific values of $\Phi_R$ and $\Phi_S$ in this algorithm.
%
%Assumption \ref{asmp:CrashProc} is for crashed processes. 
%Intuitively, this assumption is used to keep the system configuration simple by immediately and repeatedly cleaning message buffers crashed processes.
%We will give more details in Section \ref{sec:Prop}, paragraph \emph{Crash models}.

This section describes interesting properties of the environment, and correct processes  which will be used in the verification task.

\subsubsection{Implicit bounds on the behavior of correct processes} 

While Constraints \ref{const:OmegaS} and \ref{const:OmegaR} are on the local time, 
Lemmas \ref{lem:PhiS} and \ref{lem:PhiR} show that our computational model implies constraints for $\mathit{Send}$ and $\mathit{Receive}$ in terms of global time.

\newcommand{\lemPhiS}{
  Let $\Phi_S \geq \Omega \times \Phi$. 
  For all the $t \geq t_0$, every correct process $p$ must execute the operator $\sendall{p}$ 
    at least once in every global time interval $\rho = \left[ t, t + \Phi_S \right]$
}

\begin{lemma} \label{lem:PhiS}
  \lemPhiS
\end{lemma}

\begin{proof}  
  Because of the constraint $\Delta$ on process relative speeds, 
    process $p$ takes at least $\Omega$ steps 
    in the time interval $\rho$.
  Hence, process $p$ must execute the operator $\mathit{Send}$ at least once
    in the time interval $\rho$
    due to Constraint \ref{const:OmegaS}.    \qed
\end{proof}

\begin{lemma} \label{lem:PhiR}
    Let $\Phi_S \geq \Omega \times \Phi$. 
  For all the $t \geq t_0$, every correct process $p$ must execute the operator $\receive{p}$ 
    at least once in every global time interval $\rho = \left[ t, t + \Phi_R \right]$.
\end{lemma}

\begin{proof}  
  By similar arguments for Lemma \ref{lem:PhiS}, it follows that 
    process $p$ must execute the operator $\receive{p}$ 
    at least once in the time interval $\rho = \left[ t, t + \Phi_R \right]$. \qed
\end{proof}

%\begin{assumption} \label{asmp:CrashProc}
%  When process $p$ crashes, its message buffer $\msgbuf{p}$ is clean empty immediately, and from now on no messages are stored in its buffer.
%\end{assumption}

%\begin{assumption} \label{asmp:talkative}
%  A correct process can execute only the action ``send--to--all'' to send messages to every process.
%\end{assumption}
%
%\begin{assumption} \label{asmp:laconic}
%  A correct process can execute the action ``send--to--some'' to send a message to a subset of processes. 
%\end{assumption}

%
%We call the class of algorithms satisfying Assumptions \ref{lem:PhiS} --\ref{lem:PhiR} as ``receptive''. 
%The ``receptive'' class contains three following subclasses: 
%\begin{enumerate}
%  \item Class ``talkative'': Correct processes can execute only the action ``send--to--all'' to send messages to every process. 
%  
%  \item Class ``laconic'': Correct processes can execute the action ``send--to--some'' to send a message to a subset of processes. 
%  
%  \item Class ``clean'': The system behavior must satisfy Assumption \ref{asmp:CrashProc}.
%\end{enumerate}





%\subsection{Properties} \label{sec:Prop}

%In this section, we discuss two classes of algorithms called ``talkative'' and ``

%In the following, we discuss the following:
%\begin{enumerate}
%  \item The number of in-transit messages before GST: Lemmas \ref{lem:UnboundedMsgBufOne}--\ref{lem:UnboundMsgBuf}, 
%  \item The lower bound on transmission time for messages sent to correct processes: Lemmas \ref{lem:BoundRcvdMsgDelay}--\ref{lem:GSTClean}, 
%  \item Crash models: under Assumption \ref{asmp:CrashProc},
%  \item The message buffers after GST: Lemmas \ref{lem:BoundCorrMsgBuf}--\ref{lem:BoundMsgBuf}, and
%  \item The silent period of crashed processes: Lemma \ref{lem:SilentCrashedProc}.
%\end{enumerate}
%
% shows that there exists an execution prefix such that message buffers in this time interval are unbound.
% shows that there exists an execution prefix such that message buffers in this prefix are unbound.
%Moreover, Lemmas -\ref{lem:BoundCorrMsgBuf} shows that there exists an postfix such that every message buffer of a correct process in the postfix is bound.
%Assumption  is to restrict the behavior related to crashed processes.
%Under this assumption, we obtain two Lemmas for crashed processes.



\subsubsection{Unbounded message buffers before GST} 

%Lemma \ref{lem:UnboundedMsgBufOne} shows that the message buffers in the class ``talkative'' are unbounded before the global stabilization time ($\gst{}$) $t_0$, even in case of two processes in the system. 
%Lemma \ref{lem:UnboundedMsgBufTwo} is for the class ``laconic''.
%It follows immediately that in both classes ``talkative'' and ``laconic'', the total number of messages in transit before $t_0$ is unbounded (Lemma \ref{lem:UnboundedMsgBuf}).


\newcommand{\lemUnboundedMsgBufOne}{
  Let $\mathit{MAX}$ be a natural number. 
  There exist an execution path $\pi$ in $S_{1..N}$ such that 
    the number of messages in the message buffer $\msgbuf{1, 2}$ at some time point is greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{1, 2}$.
}

\begin{lemma} \label{lem:UnboundedMsgBufOne}
  \lemUnboundedMsgBufOne
\end{lemma}

\begin{proof}
  Assume by contradiction that in every execution path, the number of messages in every message buffer is bounded by $\mathit{MAX}$.
  We will construct an execution path that violates this assumption.
  Recall that the system behavior is unrestricted before $t_0$. 
  Therefore, the following case exists:
  (i) no faults happen before $t_0$, and 
  (ii) no messages sent before $t_0$ were received before $t_0$, and 
  (iii) every correct process takes a step in every global tick.
  We choose an execution path $\pi$ such that
  its global stabilization time is $t_0 = 1 + \Phi_S \times (\mathit{MAX} + 1)$, and 
  all constraints (i)--(iii) are satisfied in $\pi$.
  By Lemma \ref{lem:PhiS}, we know that process 1 must execute the action $\sendall{1}$ at least $(\mathit{MAX} + 1)$ times in the interval $\left[1, t_0 - 1\right]$. 
  By condition (ii), the message buffer $\buf{1, 2}$ at the time point $t_0 - 1$ must have all messages which were sent by proocess 2 before the time point $ t_0 -1$. 
  Therefore, $\buf{1, 2}$ at the time point $t_0 - 1$ must have at least $\mathit{MAX} + 1$ messages.
  \qed
\end{proof}

%\begin{figure}[!hbt]
%  \begin{tikzpicture}
%  % draw horizontal line   
%  \draw[thick, -Triangle] (0,0) -- (0.75 * \ImageWidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%  
%  % draw vertical lines
%  \foreach \x in {0,1,...,5}
%  \draw (\x cm,3pt) -- (\x cm,-3pt);
%  
%  \foreach \x/\descr in {3/ t_0 }
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};
%  
%  \draw [thick,decorate,decoration={brace,amplitude=5pt}] (2,-.7) -- +(-2,0)
%  node [black,midway,font=\scriptsize, below=4pt] {Unbounded message buffers};
%  \end{tikzpicture}
%  \caption{Message buffers are unbounded before the global stabilization time $t_0$.} \label{fig:unboundedmsgbuffers}
%\end{figure}

%\newcommand{\lemUnboundedMsgBufTwo}{
%  Let $S$ be a partially synchronous system in the class ``laconic'' with 2 processes.
%  Let $\mathit{MAX}$ be a natural number. 
%  There exist an execution trace $\pi$ and a process $p_j$ such that the number of messages in the message buffer $\msgbuf{p_j}$ at some time point is greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{p_j}$.
%}

%\begin{lemma} \label{lem:UnboundedMsgBufTwo}
%  \lemUnboundedMsgBufTwo
%\end{lemma}
%
%\begin{proof}  
%  Consider an execution trace $\pi$ such that
%  its global stabilization time is $ t_0 = 2 + \Phi_S \times (2 \times \mathit{MAX} + 1)$,
%  and all following conditions are satisfied in the trace $\pi$: 
%  (i) no faults happen before $t_0$, and 
%  (ii) no messages sent before $t_0$ were received before $t_0$, and 
%  (iii) every correct process takes a step in every global tick.
%  We prove the following by contradiction: there exist processes $i, j \in \left\{1, 2\right\}$ such that process $i$ executes the action $\mathit{Send} \left( \_ , p_j \right)$ at least $\mathit{MAX} + 1$ times in the interval $\left[ 1, t_0 - 1 \right]$.
%  Assume by contradiction that for every pair of processes $p_i, p_j$, process $p_i$ has executed the action $\mathit{Send} \left( \_ , p_j \right)$ less than or equal to $\mathit{MAX}$ times in the interval $\left[1, t_0 - 2\right]$ (*).
%  Now let us investigate the behavior of process 1.
%  By Assumption \ref{lem:PhiS}, condition (iii) and the default value of $t_0$, we know that process 1 must execute the action $\mathit{Send} \left( \_, \_\right)$ at least $2 \times \mathit{MAX} + 1$ times in the interval $\left[ 1, t_0 - 2\right]$.
%  Because the given system has only two processes, the assumption (*) implies that the total number of time points when process 1 executes the action $\mathit{Send} \left(\_, \_\right)$ is less than or equal to $2 \times \mathit{MAX}$ times (contradiction).
%  It follows that there exists a process $p_j$ such that process 1 must execute the action $\mathit{Send} \left( \_ , p_j \right)$ at least $(\mathit{MAX} + 1)$ times in the time interval $\left[1, t_0 - 2\right]$.
%  This result implies that the message buffer $\msgbuf{p_j}$ at the time point $t_0 - 1$ must contain at least $(\mathit{MAX} + 1)$ messages by the condition (ii).
%\end{proof}


%\newcommand{\lemUnboundedMsgBuf}{
%In both classes ``talkative'' and ``laconic'', for every integer $\mathit{MAX}$ there exists an execution trace $\pi$ and a process $p_j$ such that the number of messages in $\msgbuf{p_j}$ at some time point must be greater than $\mathit{MAX}$, i.e. $\mathit{MAX} < \# \msgbuf{p_j}$.
%}
%
%\begin{lemma} \label{lem:UnboundedMsgBuf}
%\lemUnboundedMsgBuf  
%\end{lemma}

%\begin{proof} \label{lem:msgbuf_unbound_general}
%  Lemma \ref{lem:UnboundedMsgBuf} follows immediately from Lemmas \ref{lem:UnboundedMsgBufOne} and \ref{lem:UnboundedMsgBufTwo}. 
%\end{proof}

\subsubsection{The postfix}

In this section, we show that we can bound the time of
  messages sent to correct processes before GST in
  Lemma \ref{lem:MsgBeforeGST}, and
  the transmission time of messages sent to correct processes after GST in Lemma 
  Lemma \ref{lem:MsgAge}.

%Now we prove that there is eventually a lower bound on transmission time for messages sent to correct processes in the class ``receptive''. 
%Lemma \ref{lem:BoundRcvdMsgDelay} shows that this lower bound called $\Gamma$ is eventually reached since the time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R$, and $\Gamma = \Delta + (\Phi + 1) \times \Phi_R + 1$.
%%Because there eventually exists a connection between $\Phi_R$ and $\Phi$, the value of $\Gamma$ actually depends on $\Phi$. 
%The proof of Lemma \ref{lem:BoundRcvdMsgDelay} requires Lemmas \ref{lem:RepeatRcvAfterGST} and \ref{lem:GSTClean}.
%Lemma \ref{lem:RepeatRcvAfterGST} shows that every correct process $p$ must execute the action $\receive{p}$ at least once in an interval $\left[t, t + (\Phi + 1) \times \Phi_R \right]$ where time $t$ is later than time $t_0$, i.e. $t_0 \leq t$.
%Lemma \ref{lem:GSTClean} says that since the time point $T_0$, whose value is already assigned as $t_0 + \Delta + (\Phi + 1) \times \Phi_R$, every correct process does not receive any messages sent by $t_0$.
%
%\begin{figure}[!hbt]
%\centering
%\begin{tikzpicture}
%% draw horizontal line   
%\draw[thick, -Triangle] (0,0) -- (0.85\textwidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%
%% draw vertical lines
%\foreach \x in {0,0.5,...,9}
%\draw (\x cm,3pt) -- (\x cm,-3pt);
%
%\foreach \x/\descr in {1.5/t_0}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%\foreach \x/\descr in {7.5/\text{\textit{p} receives \textit{m}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%
%
%\foreach \x/\descr in {2.5/\text{\textit{q} sent \textit{m}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%\foreach \x/\descr in {5/\text{\textit{m} in \textit{msgBuf[p]}}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%
%\draw[-, dashed, black] (6.5,-.3) --  +(-0.4,0);
%
%\draw[-Triangle, dashed, black] (3.8,-.3) --  +(-0.6,0);
%
%
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (2,0.4)  -- +(5.5,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Gamma = \Delta + (\Phi + 1) \times \Phi_R + 1$};
%\end{tikzpicture}
%\caption{The lower bound of message delay $\Gamma$ in the class ``receptive'' is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.}
%\end{figure}

\newcommand{\lemMsgBeforeGST}{
  Every message sent to correct process $p$  before $t_0$ 
  is received by time $t_0 + \Delta + \Phi_R$.
}

\begin{lemma} \label{lem:MsgBeforeGST}
  \lemMsgBeforeGST
\end{lemma}

\begin{proof}
Let $p$ be a correct process, 
  and $m$ be an arbitrary message which was sent to process $p$ before GST.
We know that message $m$ is at least $\Delta$ time-units old from the time point $t_0$ 
  because it was sent before $t_0$.
By Lemma \ref{lem:PhiR}, process $p$ must execute the operator $\mathit{Receive}(p)$ at some point $t$ where $t_0 + \Delta \leq t \leq t_0 + \Delta + \Phi_R$.
By the constraint $\Delta$, process $p$ must receive message $m$ at time $t$.
\qed
\end{proof}

\newcommand{\lemMsgAge}{
  Every message sent to correct process $p$ at some time $t \geq t_0$ 
  is received by time $t + \Delta + \Phi_R$.
}

\begin{lemma} \label{lem:MsgAge}
  \lemMsgAge
\end{lemma}

\begin{proof}
  By similar arguments in Lemma \ref{lem:MsgBeforeGST}. \qed{}
\end{proof}

By Lemmas \ref{lem:MsgBeforeGST}--\ref{lem:MsgAge}, we obtain Lemma \ref{lem:BoundedMsgBuf} which says that  
  every message buffer to a correct process is eventually and permanently bounded.

\newcommand{\lemBoundedMsgBuf}{
  Let $K = \Delta + \Phi_R$, and $p, q$ be arbitrary processes such that $q$ is correct.
  The number of messages in the buffer $\buf{p, q}$ is eventually and permanently bounded by $K$.
}

\begin{lemma} \label{lem:BoundedMsgBuf}
\lemBoundedMsgBuf
\end{lemma}

\begin{proof}
We prove Lemma \ref{lem:BoundedMsgBuf} by cases. There are two cases: 
\begin{enumerate}
\item \emph{Both processes $p$ and $q$ are correct.} By Lemmas \ref{lem:MsgBeforeGST} and \ref{lem:MsgAge}, it follows that the message buffer $\buf{p, q}$ contains only messages which are less than $\Delta + \Phi_R$ time-units old.
By Constraint \ref{const:SendToAll}, we know that there are no two different messages with the same age. 
Therefore, the message buffer $\buf{p, q}$ has at most $\Delta + \Phi_R$ messages.
In other words, the number of messages in $\buf{p, q}$ is bounded by $K$.


\item \emph{Process $q$ is correct and process $p$ crashes at some time $t_1$.} 
By Constraint \ref{const:NoRecover}, we know that 
  every message $m$ from process $p$ to process $q$ was sent before time $t_1$.
If process $p$ crashes before $t_0$, then by Lemma \ref{lem:MsgBeforeGST} we know that all of its messages will be received by $t_0 + \Delta + \Phi_R$.
If process $p$ crashes after $t_0$, then by Lemma \ref{lem:MsgAge}, it follows that every message from process $p$ will be received by the time point $t_1 + \Delta + \Phi_R$.
Therefore, after the time point $t_2 = \mathit{max}(t_0, t_1) + \Delta + \Phi_R$, it follows that $\buf{p, q}$ is permanently empty.

%\item \emph{Process $q$ crashes at some time $t_1$.} By Constraint \ref{const:CrashModel}, every message buffer to process $q$ is empty immediately.
\end{enumerate}
Hence, the message buffer is eventually and permanently bounded by $K$.
\qed
\end{proof}
%
%Lemma \ref{lem:HearingBound} says that 
%  a correct process must hear something from another correct process 
%  in every time interval with $\Phi_S + \Delta + \Phi_R$ ticks.
%Lemma \ref{lem:SilentPeriod} says that
%  every correct process eventually hears nothing from a crashed processes.
%  
%\newcommand{\lemHearingBound}{
%Let $\sigma = \left[ t, t + \Delta + \Phi_S + \Phi_R \right]$ be an arbitrary time interval after $\gst{} t_0$, i.e. $t_0 \leq t$. 
%Let $p, q$ be an arbitrary pair of correct processes.
%Then, process $p$ receives some message from process $q$ in the time interval $\sigma$.
%}
%
%\begin{lemma} \label{lem:HearingBound}
%\lemHearingBound
%\end{lemma}
%
%\begin{proof}
%By Lemma \ref{lem:PhiS}, process $q$ must send at least one message $m$ to process $p$ in the interval $\left[ t, t + Phi_S \right]$. 
%We have that message $m$ is at least $\Delta$ time-units  from the time $t + \Phi_S + \Delta$.
%By Lemma \ref{lem:PhiS}, process $p$ must execute the operator $\mathit{Receive}(p)$ at least once in the interval $\rho = \left[ t + \Phi_S + \Delta, t + \Phi_S + \Delta + \Phi_R \right]$.
%Therefore, process $p$ must receive message $m$ in the interval $\rho$.
%\qed
%\end{proof}
%
%
%%Finally, Lemma \ref{lem:SilentCrashedProc} says that correct processes eventually and forever hear nothing from crashed processes.
%%
%\newcommand{\lemSilentPeriod}{
%  If process $p$ crashes at time $t_{\mathit{crash}}$, every correct process $q$ does not receive any message from process $p$ after time $t = \mathit{max}\{ t_{\mathit{crash}}, \gst{} \} + \Delta + \Phi_R  + 1$.
%}
%
%\begin{lemma} \label{lem:SilentPeriod}
%  \lemSilentPeriod
%\end{lemma}
%
%\begin{proof}
%By similar arguments in the proof of Lemma \ref{lem:BoundedMsgBuf}, the second case.
%\qed
%\end{proof}

%\begin{figure}[!hbt]
%  \begin{tikzpicture}
%  % draw horizontal line   
%  \draw[thick, -Triangle] (0,0) -- (0.99\textwidth,0) node[font=\scriptsize,below left=3pt and -8pt]{\textit{t}};
%  
%  % draw vertical lines
%  \foreach \x in {0,1,...,12}
%  \draw (\x cm,3pt) -- (\x cm,-3pt);
%  
%  \foreach \x/\descr in {3/\textit{GST}}
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};
%  
%  %% colored bar up
%  %\foreach \x/\perccol in
%  %{0/100,1/75,2/0,3/75}
%  %\draw[lightgray!\perccol!red, line width=4pt] 
%  %(\x,.5) -- +(1,0);
%  %\draw[-Triangle, dashed, red] (4,.5) --  +(4,0);
%  
%  % colored bar down
%  %\foreach \x/\perccol in
%  %{3/100,4/75,5/0}
%  %\draw[lightgray!\perccol!green, line width=4pt] 
%  %(\x,-.7) -- +(1,0);
%  %\draw[-Triangle, dashed, green] (6,-.7) --  +(1,0);
%  
%  % braces
%  \draw [thick ,decorate,decoration={brace,amplitude=5pt}] (4,0.4)  -- +(3,0) 
%  node [black,midway,above=4pt, font=\scriptsize] {$\Delta$};
%  
%  \draw [thick ,decorate,decoration={brace,amplitude=5pt}] (7,0.4)  -- +(2,0) 
%  node [black,midway,above=4pt, font=\scriptsize] {$\Phi_R$};
%  
%  \draw [thick,decorate,decoration={brace,amplitude=5pt}] (10,0.4) -- +(3,0)
%  node [black,midway,above=4pt,font=\scriptsize] {No messages from proc \textit{i}};
%  
%  \foreach \x/\descr in {4/\textit{Proc i crashes}}
%  \node[font=\scriptsize, text height=1.75ex,
%  text depth=.5ex] at (\x,-.3) {$\descr$};  
%  \end{tikzpicture}
%  
%  \caption{Every crashed process is eventually and forever silent}
%  \label{fig:silentCrash}
%\end{figure}


%\begin{lemma} \label{lem:RepeatRcvAfterGST}
%  \lemRepeatRcvAfterGST
%\end{lemma}

%\newcommand{\lemRepeatRcvAfterGST}{
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Every correct process $p_i$ in $P$ must execute the action $\receive{p_i}$ at least once in a global time interval $\rho = \left[t, t + (\Phi + 1 )\times \Phi_R \right]$ since the GST $t_0$, i.e. $t_0 \leq t$.
%}
%
%\begin{lemma} \label{lem:RepeatRcvAfterGST}
%  \lemRepeatRcvAfterGST
%\end{lemma}
%
%\begin{proof}
%  It is easy to see that we can split every interval $\left[t, t + (\Phi + 1 )\times \Phi_R \right]$ into $\Phi_R$ disjoint intervals whose length is $\Phi$, where $t$ is an integer.
%  By the constraint $\Phi$ on process speed, every correct process $p$ must take at least $\Phi_R$ steps in the interval $\rho$.
%  Therefore, its local clock must tick at least $\Phi_R$ times in the interval $\rho$.
%  By Assumption \ref{lem:PhiR}, it follows that process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%\end{proof}
%
%\newcommand{\lemGSTClean}{
%%  Let $t$ be a time point after $t_0 + \Delta + \Phi_R$, that is $t_0 + \Delta + \Phi + 1 \geq t$.
%%  Let $m$ be a message sent to a process which is still correct until $t$.
%%  If message $m$ is in transit at time $t$, 
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Assume that a correct process $p$ in $P$ executes the action $\receive{p}$ after the global time point $t_0 + \Delta + (\Phi + 1) \times \Phi_R$, and receives message $m$.
%  Then message $m$ was sent at time $t_0$ or later.
%}
%
%\begin{lemma} \label{lem:GSTClean}
%  \lemGSTClean
%\end{lemma}
%
%\begin{proof}
%  By applying Lemma \ref{lem:RepeatRcvAfterGST} to the interval $\rho = \left[ t_0 + \Delta, t_0 + \Delta + (\Phi + 1) \times \Phi_R \right]$, we know that every correct process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%  Assume that process $p$ executes the action $\receive{p}$ at some time point $t^{\rho}_p$ in the interval $\rho$.
%  It immediately follows that $t^{\rho}_p$ is after $t_0 + \Delta$, i.e. $t_0 + \Delta \leq t^{\rho}_p$.
%  By the constraint $\Delta$ on message delay, we know that messages sent to process $p$ by time $t_0$ must be delivered by time $t^{\rho}_p$.
%  It follows that from the time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R + 1$ message buffers of correct processes only contain messages sent after $t_0$.
%  It implies that if process $p$ receives me message $m$ since the time point $T_0$, message $m$ must be sent at time $t_0$ or later.
%%  By the constraint $\Delta$ on message delay, we know that all messages sent to process $p$ before the time point $t^{\rho} - \Delta$ must be delivered to process $p$ by the time point $t^{\rho}$.
%%  First, we prove that every correct process $p \in P$ in the global time interval $\rho = \left[t_0 + \Delta, t_0 + \Delta + (\Phi + 1 )\times \Phi_R \right]$ must execute the action $\receive{p}$ at least once.
%%  ve into $\Phi_R$ 
%\end{proof}
%
%\newcommand{\lemBoundRcvdMsgDelay}{
%  Let $\mathcal{A}$ be a ``receptive'' algorithm with processes $P = \left\{p_1, \ldots, p_n \right\}$.
%  Let $\pi$ be an execution trace in $\mathcal{A}$ and its global stabilization time is $t_0$.
%  Let $p$ be a correct process in $P$, and $t$ $t$ be a time point later the global time point $T_0 = t_0 + \Delta + (\Phi + 1) \times \Phi_R$, i.e. $T_0 \leq t$, such that process $p$ executes the action $\receive{p}$ at time $t$ in the execution trace $\pi$.
%  Process $P$ receives only messages which were sent since the time point $t - \Delta -  (\Phi + 1) \times \Phi_R - 1$.
%  In other words, the lower bound of message delay called $\Gamma$ in algorithm $\mathcal{A}$ is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.
%}
%
%\begin{lemma} \label{lem:BoundRcvdMsgDelay}
%\lemBoundRcvdMsgDelay
%\end{lemma}
%
%\begin{proof}
%  By Lemma \ref{lem:RepeatRcvAfterGST}, process $p$ executed $\receive{p}$ at least once in the interval $\rho = \left[t - (\Phi + 1) \times \Phi_R - 1, t - 1 \right]$.
%  Assume that process $p$ executed the action $\receive{p}$ at some time point $t^{\rho}_p$ in the interval $\rho$.
%  It immediately follows that $t  - (\Phi + 1) \times \Phi_R - 1 \leq t^{\rho}_p$.
%  By an assumption $T_0 \leq t$, we know that the time point $t  - (\Phi + 1) \times \Phi_R - 1$ is after time $t_0$.
%  By Lemma \ref{lem:GSTClean}, it follows that after time $t^{\rho}_p$, the message buffer $\msgbuf{p}$ contains only messages sent from time $t^{\rho}_p - \Delta$.
%  Therefore, after executing the action $\receive{p}$ at time $t$, process $p$ cannot receive messages sent before the time point $t - \Delta -  (\Phi + 1) \times \Phi_R - 1$.
%  In other words, the lower bound of message delay called $\Gamma$ in algorithm $\mathcal{A}$ is eventually bounded by $\Delta + (\Phi + 1) \times \Phi_R + 1$.
%%  
%%  First, we can split every interval $\rho = \left[t, t + (\Phi + 1 )\times \Phi_R \right]$ into $\Phi_R$ disjoint intervals whose length is $\Phi$, where $t$ is an integer.
%%  Now assume that $t_0 + \Delta \leq t$.
%%  By the constraint $\Phi$ on process speed, process $p_i$ must take at least $\Phi_R$ steps in the interval $\sigma$.
%%  Therefore, its local clock must tick at least $\Phi_R$ times in the interval $\rho$.
%%  By Assumption \ref{lem:PhiR}, it follows that process $p$ must execute the action $\receive{p}$ at least once in the interval $\rho$.
%%  Assume that process $p$ executes the action $\receive{p}$ at some time point $t^{\rho}$ in the interval $\rho$.
%%  It immediately follows that $t^{\rho}$ is after $t_0$, i.e. $t_0 \leq t^{\rho}$.
%%  By the constraint $\Delta$ on message delay, we know that all messages sent to process $p$ before the time point $t^{\rho} - \Delta$ must be delivered to process $p$ by the time point $t^{\rho}$.
%%  Now consider the time interval $\sigma = \left[ t + \Delta + (\Phi + 1) \times \Phi_R + 1, t + \Delta + 2 \times (\Phi + 1) \times \Phi_R \right]$.
%%  Again by our assumptions, we know that process $p$ must execute the action $\receive{p}$ at least once in the time interval $\sigma$.
%%  Let $t^{\sigma}$ be a time point in the time interval $\sigma$ when process $p$ executed the action $\receive{p}$.
%%  By the fact (*), we know that only messages sent since the time point $t^{\rho} - \Delta$ can be delivered by process $p$ at this time point $t^{\sigma}$.
%%  Moreover, we have that 
%%  \[ t^{\sigma} - (t^{\rho} - \Delta) \leq t - (t^{\rho} - \Delta) \leq t - t^{\rho} + \Delta) \leq 2 * \Phi_R + \Delta \]
%%  Therefore, the gap between when the latest messages are sent and when they are received is bound by $2 * \Phi_R + \Delta$ since the time point $t_0 + \Delta + \Phi_R + 1$.
%\end{proof}
%
%
%
%
%
%\subsubsection{Crash models} \label{sec:CrashModel} \hfill
%
%Notice that Lemmas \ref{lem:BoundRcvdMsgDelay} and \ref{lem:GSTClean} describe nothing about the status of messages sent to faulty processes
%% nor the status of message buffers in the time interval $\left[ t_0, t_0 + \Delta + \Phi_R \right]$. 
%To keep the system configuration simple but reasonable, we require the following assumption:
%\begin{assumption} \label{asmp:CrashProc}
%When process $p$ crashes, its message buffer $\msgbuf{p}$ is clean empty immediately, and from now on no messages are stored in its buffer.
%\end{assumption}
%We can formalize the behavior of a crashed process in another way: it can be receive messages but neither do internal computation steps nor send messages. 
%However, the latter encoding requires another requirement about how often crashed process receives messages to ensure that every massage buffer in the system is bound.
%Hence, I think that Assumption \ref{asmp:CrashProc} is more reasonable, and it is more comfortable to specify the system with this assumption.
%Moreover, by applying Assumption \ref{asmp:CrashProc}, we next prove that every message buffer is eventually and forever bound.



%\subsubsection{Bounded message buffers in the postfix} \hfill
%
%%Assume that a correct process can send one message to all in one transition. By Lemma \ref{lem:BoundRcvdMsgDelay} and this assumption, we obtain Lemma \ref{lem:BoundMsgBuf} which says that message buffers of correct processes are eventually bound.
%
%\newcommand{\lemBoundCorrMsgBuf}{
%After the time $\gst{} + \Delta + \Phi_R + 1$, every message buffer has at most $\Omage_S + \Delta + \Phi_R$ messages.
%}
%
%\begin{lemma}
%After the time $\gst + \Delta + \Phi_R + 1$, every message buffer has at $\Phi_S + \Delta + \Phi_S$ messages.
%\end{lemma}

%\begin{proof}
%  Will be adopted.
%\end{proof}
%
%\begin{proof}
%  Let $t$ be a time point after $t_0 + \Delta + \Phi_R$, i.e. $t_0 + \Delta + \Phi_R + 1 \geq t$, and $p$ be a correct process until time $t$. 
%  We prove that the message buffer $\msgbuf{p}$ is bound at time $t$.
%  By Lemma \ref{lem:BoundRcvdMsgDelay}, we have that the message delay at time $t$ is bound by $2 * \Phi_R + \Delta$.
%  By our computational model, we know that every correct process can execute the action $\send{\_}{p}$ at most $2 * \Phi_R + \Delta$ times in the time interval $\sigma = \left[ t - (2 * \Phi_R + \Delta), t \right]$.
%  Moreover, by our assumption every execution $\send{\_}{p}$ can put only one message to the buffer $\msgbuf{p}$.
%  Therefore, the number of messages in $\msgbuf{p}$ at time $t$ is bound by $N * (2 * \Phi_R + \Delta)$.
%\end{proof}
%
%Perhaps the time point $t_0 + \Delta + \Phi_R + 1$ is not the first time every message buffer of a correct process is bound. 
%However, in our work the property that every message buffer is eventually and forever bound is good enough.
%With the crash model described in the previous, we obtain Lemma \ref{lem:BoundMsgBuf} which says that every message buffer is eventually and forever bound.
%
%\begin{figure}[!htb]
%\begin{tikzpicture}
%
%\draw[thick, -Triangle] (0,0) -- (0.9\textwidth,0) node[font=\scriptsize,below left=1pt and -8pt]{\textit{t}};
%
%% draw vertical lines
%\foreach \x in {0,1,...,10}
%\draw (\x cm,3pt) -- (\x cm,-3pt);
%
%\foreach \x/\descr in {3/\textit{GST}}
%\node[font=\scriptsize, text height=1.75ex,
%text depth=.5ex] at (\x,-.3) {$\descr$};
%
%% colored bar up
%%\foreach \x/\perccol in
%%{0/100,1/75,2/0,3/75}
%%\draw[lightgray!\perccol!red, line width=4pt] 
%%(\x,.5) -- +(1,0);
%%\draw[-Triangle, dashed, red] (4,.5) --  +(4,0);
%
%\foreach \x/\perccol in
%{9/0,10/0}
%\draw[lightgray!\perccol!blue, line width=4pt]
%(\x,-0.4) -- +(1,0);
%
%
%% colored bar down
%%\foreach \x/\perccol in
%%{3/100,4/75,5/0}
%%\draw[lightgray!\perccol!green, line width=4pt] 
%%(\x,-.7) -- +(1,0);
%%\draw[-Triangle, dashed, green] (6,-.7) --  +(1,0);
%
%% braces
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (3,0.4)  -- +(3,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Delta$};
%
%\draw [thick ,decorate,decoration={brace,amplitude=5pt}] (6,0.4)  -- +(2,0) 
%node [black,midway,above=4pt, font=\scriptsize] {$\Phi_R$};
%
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (11,-.7) -- +(-2,0)
%node [black,midway,font=\scriptsize, below=4pt] {Bounded message buffers};
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (2,-.7) -- +(-2,0)
%node [black,midway,font=\scriptsize, below=4pt] {Unbounded message buffers};
%
%\draw [thick,decorate,decoration={brace,amplitude=5pt}] (8,-.7) -- +(-5,0)
%node [black,midway,font=\scriptsize, below=4pt] {Perhaps still unbounded message buffers?};
%\end{tikzpicture}
%\caption{Message buffers are unbounded before $\gst{}$. However, they are eventually and forever bounded.}
%\label{fig:MsgBuf}
%\end{figure}
%
%\begin{lemma} \label{lem:BoundMsgBuf}
%  Under Assumption \ref{asmp:CrashProc}, every message buffer is eventually and forever bound.
%\end{lemma}
%
%\begin{proof}
%It follows immediately by Lemma \ref{lem:BoundCorrMsgBuf} and Assumption \ref{asmp:CrashProc}.
%\end{proof}




==> netys20/tcutoff.tex <==
In this section, we focus on another parameter of~\idsep{} algorithms: the global stabilization time $t_0$.
Our target is to find specific constraints which allow us to reduce the problem of checking properties on a path with an arbitrary global stabilization time $t_0$ of such algorithms to checking them on another path whose global stabilization time is 0.

In the following, we introduce a subclass class of~\idsep{} algorithms which is called $\talgo$ (?), and a subclass of local read properties which is called $\tprop$ (?)

\begin{itemize}  
\item $\mathbf{Algo}$: All messages sent by a correct process have the same content.

\item $\mathbf{Prop}$: A checking property is in the form of $\lozenge F$ such that 
\begin{enumerate}
\item Every atomic predicate in $F$ is local read.


%\item For every variable $p.\lpc$ in $F$ where $p$ is a process, there exists a finite set $S$ such that for every admissible sequence of configurations, the value of $p.\lpc$ is eventually bounded in $S$

\item For every variable in the form of $p.X[q]$, every admissible sequence of configurations, there exists a number $K_0 > 0$, such that for every $K \geq K_0$, the value of $p.X[q]$ is eventually determined by received messages from a process $q$ in $K$ last deliveries. This constraint is formalized in Definition \ref{def:EDVar}.

\item A checking property may have local read atomic predicates for $\lpc$.
\end{enumerate} 
\end{itemize}


%Such conditions work only with two classes of local variables which are presented in Definitions \ref{def:EBVar} and \ref{def:EDVar}. 
%Intuitively, given a execution path, a value of a variable in the first class contains eventually fixed to constants in this path, and a value of a variable in the later class eventually depends on only $K$ last sets of received messages.
%Then, we prove Lemma \ref{lem:GSTElim} which says that if checking properties is in the form of $\lozenge F $ where local read atomic predicates of a formula $F$ contain only variables as in Definitions \ref{def:EBVar} and \ref{def:EDVar}, a reduction for the global stabilization time is enable.
%The proofs of Lemma \ref{lem:GSTElim} is based on Lemmas \ref{lem:GSTElimFixedConst} and \ref{lem:GSTElimEDVar} and \ref{lem:GSTElimPath}



%\begin{definition} \label{def:EBVar}
%Let $\sys{N}$ be an instance of an arbitrary~\idsep{} algorithm $\idsepalgo$ for some numbers $\Delta, \Phi$ and $N$. 
%Let $\pi = \conf{}{0} \conf{}{1} \ldots$ be an admissible sequence of configurations in $\sys{N}$, and $p$ be a process. 
%A local variable $X$ of a process $p$ is \emph{eventually fixed to a constant $\mathbf{c} $ on a sequence $\pi$} if there exists  there exists a time $T$ such that $\conf{}{t}(p).X = \mathbf{c}$ for every time $t\geq T$.
%Formally, we have that
%  $
%  \exists T \forall t \colon t \geq T \Rightarrow \conf{}{t}(p).X = \mathbf{c}
%  $.
%\end{definition}
%  
\begin{definition} \label{def:EDVar}
  Let $\sys{N}$ be an instance of an arbitrary~\idsep{} algorithm $\idsepalgo$ for some numbers $\Delta, \Phi$ and $N$. 
%  Let $\pi = \conf{}{0} \conf{}{1}$ be an admissible sequence of configurations in $\sys{N}$.  
  Let $p, q$ be a process, and $X$ be a variable with type $\proc \rightarrow \mathcal{V} $ where $\mathcal{V}$ is a finite set of values. A variable $p.X[q]$ is \emph{eventually determined by a bounded delivery history with a process $q$ }  if 
%  there exists a number $K_0 \geq 1$, there exists a time $T \geq 0$  such that for every number $K \geq K_0$, there exists a $K$--ary function, for every time $t \geq T$, the value of $\conf{}{t}(p).X[q]$ depends on only received messages from a process $q$ in $K$ last deliveries of a process $p$.
%  Formally, we have
  the following property holds
%  \begin{align*}
%  \forall K \geq 1 & \exists g \in Message^K \rightarrow \mathit{Val} \forall \pi = \conf{}{0} \conf{}{1}\ldots \in \mathit{Admissible(\sys{N})} \\
%  \exists T &   \geq 0 \, \exists K_0 \geq 1 \forall t \geq T \colon \\
%  &   \qquad \quad K \geq K_0 \Rightarrow \\
%%  \exists T & \geq 0 \, \exists K_0 \geq 1 \, \forall K \geq K \exists g \in Message^K \rightarrow \mathit{Val} \forall t \geq T \, \exists t_1, \ldots, t_K \colon \\
%  & \;\;\, \bigwedge \quad t_1 < \ldots < t_K \leq t \\
%  &  \bigwedge_{1 \geq i \geq K} \left( \conf{}{t_i}.\gpc[p] \land \conf{}{t_i}(p).\lpc = \trcv{} \right) \\
%  &  \bigwedge_{1 \geq i < K} \left( \forall t^{\prime} \colon t_i < t^{\prime} < t_{i + 1} \Rightarrow \left( \lnot \conf{}{t_i}.\gpc[p] \lor \conf{}{t_i}(p).\lpc \neq \trcv{} \right)\right) \\
%  & \;\;\, \bigwedge \quad  \conf{}{t}(p).X[q] = g \left( \conf{}{t_1 + 1}.\rop{p}[q], \ldots, \conf{}{t_K + 1}.\rop{p}[q] \right)
%  \end{align*}
  \begin{align*}
  \exists T & \geq 0 \, \exists K_0 \geq 1 \, \forall K \geq K \E g \in Message^K \rightarrow \mathit{Val} \forall t \geq T \, \exists t_1, \ldots, t_K \colon \\
  & \;\;\, \bigwedge \quad t_1 < \ldots < t_K \leq t \\
  &  \bigwedge_{1 \geq i \geq K} \left( \conf{}{t_i}.\gpc[p] \land \conf{}{t_i}(p).\lpc = \trcv{} \right) \\
  &  \bigwedge_{1 \geq i < K} \left( \forall t^{\prime} \colon t_i < t^{\prime} < t_{i + 1} \Rightarrow \left( \lnot \conf{}{t_i}.\gpc[p] \lor \conf{}{t_i}(p).\lpc \neq \trcv{} \right)\right) \\
  & \;\;\, \bigwedge \quad  \conf{}{t}(p).X[q] = g \left( \conf{}{t_1 + 1}.\rop{p}[q], \ldots, \conf{}{t_K + 1}.\rop{p}[q] \right)
  \end{align*}
  where $g$ is some $K$--ary function, and $\mathit{Val}$ is a set of possible values of $p.X[q]$, and $\mathit{Admissible(\idsepalgo)}$ is a set of admissible sequences in $\sys{N}$
\end{definition}



\newcommand{\lemGSTElim}{
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let $\lozenge F$ be a $\tprop$ property.
  It follows if every admissible sequene of configurations  with the global stabilization time $t_0 = 0$ is a model of $\lozenge F$ in $\sys{N}$, then $\sys{N}$ is a model of $\lozenge F$, i.e. $\sys{N} \models \lozenge F$.
}



\begin{lemma} \label{lem:GSTElim}
  \lemGSTElim
\end{lemma}

\begin{proof}
  Let $\pi$ be an arbitrary admissible sequence of configurations in $\sys{N}$.
  By Lemma \ref{lem:EventuallySameDelHist}, there exists an admissible sequence of configurations $\pi_0$ with the globalization time 0 in $\sys{N}$ such that both paths $\pi_0$ and $\pi$ eventually agree on the delivery history.
  By Lemma \ref{lem:GSTElimPath}, it follows that $\pi \models \lozenge F$ if and only if $\pi_0 \models \lozenge F$.
  Therefore, if every execution path $\pi_0$ with the global stabilization time $t_0 = 0$ is a model of $\lozenge F$, then $\lozenge F$, then $\sys{N} \models \lozenge F$.
\qed
\end{proof}


Definitions \ref{def:EventSameDelHist} and \ref{def:EventSameActHist} are used in the statement of following lemmas.

\begin{definition} \label{def:EventSameDelHist}
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ and $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be two admissible sequences of configurations in $\sys{N}$ such that their global stabilization time are respectively 0 and $t_0$.
  Two paths $\pi^0$ and $\pi^{t_0}$ \emph{eventually agree on the delivery history} if the following property holds:  
  $
  \exists T  \geq 0 \exists \delta \geq 0 \forall t \geq T \forall p, q \colon \conf{0}{t }.\buf{p}{q} = \conf{t_0}{t + \delta}.\buf{p}{q}
  %\exists S \colon &  (\conf{0}{t}.\gpc[p] && \land \conf{0}{t}(p).\lpc = \trcv{} &&& \land \conf{0}{t+1}.\trcv(p)[q] = S) \\
  %\Leftrightarrow &  (\conf{t_0}{t}.\gpc[p]  && \land \conf{t_0}{t}(p).\lpc = \trcv{}  &&& \land \conf{t_0}{t+1}.\trcv(p)[q] = S )
  $.
\end{definition}

\begin{definition} \label{def:EventSameActHist}
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ and $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be two admissible sequences of configurations in $\sys{N}$ such that their global stabilization time are respectively 0 and $t_0$.
  Two paths $\pi^0$ and $\pi^{t_0}$ \emph{eventually agree on the action history} if the following property holds:  
  \begin{alignat*}{3}
    \exists T  \geq 0 \exists \delta \geq 0 \forall t \geq T \forall p \colon & &&  \conf{0}{t }(p).\lpc = \conf{t_0}{t + \delta}(p).\lpc \\
    & \, \land && \conf{0}{t }.\gpc[p] = \conf{t_0}{t + \delta}.\gpc[p]
  \end{alignat*}

  %\exists S \colon &  (\conf{0}{t}.\gpc[p] && \land \conf{0}{t}(p).\lpc = \trcv{} &&& \land \conf{0}{t+1}.\trcv(p)[q] = S) \\
  %\Leftrightarrow &  (\conf{t_0}{t}.\gpc[p]  && \land \conf{t_0}{t}(p).\lpc = \trcv{}  &&& \land \conf{t_0}{t+1}.\trcv(p)[q] = S )
%  \]
\end{definition}


\newcommand{\lemEventuallySameDelHist}{
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let  $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be an admissible sequence of configurations  with the global stabilizatim time $t_0$ in $\sys{N}$ .
  There exists an admissible sequence of configurations 
  $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ with the global stabilization time 0 in $\sys{N}$
  such that $\pi^0$ and $\pi^{t_0}$ are eventually agree on the delivery history.
}

\begin{lemma} \label{lem:EventuallySameDelHist}
\lemEventuallySameDelHist
\end{lemma}

\begin{proof}
\emph{(Sketch)}. A sequence $\pi^0$ is constructed by the projection of the postfix $\conf{t_0}{t_0} \conf{t_0}{t_0 + 1} \ldots$ of a sequence $\pi^{t_0}$, and filter received messages. 
We set $\delta = t_0$ and $T = t_0 + \Phi_R \times \Phi + 1$.
Notice that the initial state $\conf{0}{0}$ of $\pi^{0}$ might be different from the state $\conf{t_0}{t_0}$ of $\pi^{t_0}$ because other variables might have different values.
However, for the agreement of delivery history, we do not need to care about the rest of variables.
\end{proof}

\newcommand{\corEventuallyPC}{
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let  $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be an admissible sequence of configurations  with the global stabilizatim time $t_0$ in $\sys{N}$ .
  Let
  $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ with the global stabilization time 0 in $\sys{N}$
  such that $\pi^0$ and $\pi^{t_0}$ are eventually agree on the delivery history from a time $T$ and with a distance $\delta$.
  Let $p.X[q]$ be a $\tprop$ variable where $p, q$ are processes, and $X$ is a one--dimensional local variable.
  Let $\mathbf{p} \triangleq p.X[q] = \mathit{v}$ be a predicate where  $\mathit{v}$ is a value.
  It follows that 
  \[
  \forall t \geq T \colon \conf{0}{t} \models \mathbf{p}  \Leftrightarrow \conf{t_0}{t + \delta} \models \mathbf{p}
  \].
}

\begin{corollary} \label{cor:EventuallyPC}
  \corEventuallyPC
\end{corollary}

\begin{proof}
\emph{(Issue)} Add more constraints to make sure that the functions $g$ for $p.X[q]$ in two paths $\pi^0$ and $\pi^{t_0}$ is enable to merge.
\end{proof}

\newcommand{\lemEventuallySameActHist}{
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let  $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be an admissible sequence of configurations  with the global stabilizatim time $t_0$ in $\sys{N}$ .
  There exists an admissible sequence of configurations 
  $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ with the global stabilization time 0 in $\sys{N}$
  such that $\pi^0$ and $\pi^{t_0}$ are eventually agree on the action history.
}

\begin{lemma} \label{lem:EventuallySameActHist}
  \lemEventuallySameActHist
\end{lemma}


\begin{proof}
  \emph{(Sketch)}. A sequence $\pi^0$ is constructed by the projection of the postfix $\conf{t_0}{t_0} \conf{t_0}{t_0 + 1} \ldots$ of a sequence $\pi^{t_0}$. 
\end{proof}

\newcommand{\corEventuallyBoundedDelHist}{
  Let $\idsepalgo$  be an $\talgo$ algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let  $\pi^{t_0} = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be an admissible sequence of configurations  with the global stabilizatim time $t_0$ in $\sys{N}$ .
  Let
  $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ with the global stabilization time 0 in $\sys{N}$
  such that $\pi^0$ and $\pi^{t_0}$ are eventually agree on the action history from a time $T$ and with a distance $\delta$.
  Let $\mathbf{p} \triangleq p.\lpc = \mathit{v}$ be a predicate where $p$ is a process, and $\mathit{v}$ is a instruction block.
  It follows that $\forall t \geq T \colon \conf{0}{t} \models \mathbf{p}  \Leftrightarrow \conf{t_0}{t + \delta} \models \mathbf{p} $.
}

\begin{corollary} \label{cor:EventuallyBoundedDelHist}
  \corEventuallyBoundedDelHist
\end{corollary}

\newcommand{\lemGSTElimPath}{
Let $\idsepalgo$  be an~\idsep algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
Let $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ and $\pi_T = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be two execution path of $\sys{N}$ such that their global stabilizatim time are respectively 0 and $t_0$, and they eventually agree on the delivery history.
Let $\mathbf{p}$ be a local read atomic predicate on a variable which is eventually fixed to the same value $\mathbf{c}$ both paths $\pi^0$ and $\pi^{t_0}$.
There exists a time $K$ such that $\conf{0}{t} \models \mathbf{p} \Leftrightarrow \conf{t_0}{t} \models \mathbf{p}$ for every time $t \geq K$.
}




%
%\begin{lemma} \label{lem:GSTElimPath}
%  \lemGSTElimPath
%\end{lemma}


\newcommand{\lemGSTElimFixedConst}{
  Let $\idsepalgo$  be an~\idsep algorithm, and $\sys{N}$ be an instace of $\idsepalgo$.
  Let $\pi^0 = \conf{0}{0} \conf{0}{1} \ldots$ and $\pi_T = \conf{t_0}{0} \conf{t_0}{1} \ldots$ be two execution path of $\sys{N}$ such that their global stabilizatim time are respectively 0 and $t_0$, and they eventually agree on the delivery history.
  Let $\mathbf{p}$ be a local read atomic predicate on a variable which is eventually fixed to the same value $\mathbf{c}$ both paths $\pi^0$ and $\pi^{t_0}$.
  There exists a time $K$ such that $\conf{0}{t} \models \mathbf{p} \Leftrightarrow \conf{t_0}{t} \models \mathbf{p}$ for every time $t \geq K$.
}
%
%\begin{lemma} \label{lem:GSTElimFixedConst}
%  \lemGSTElimFixedConst
%\end{lemma}


\newcommand{\lemGSTElimDeterDelHist}{
}

==> related-work.tex <==

Research papers about
partially synchronous algorithms, including papers about failure
detectors~\cite{larrea1999efficient,aguilera2006consensus,aguilera2008implementing}
contain manual proofs and no formal specifications.
Without these details, proving those distributed algorithms with interactive theorem provers~\cite{cousineau2012tla,mcmillan2020ivy} is impossible.
To test a candidate $I$ for an inductive invariant with fixed parameters, system designers can apply probabilistic random 
%inductive invariant 
checking with~\tlap{} and TLC~\cite{lamport2018using}.
However, this approach randomly explores a subset of the execution space.
Hence, it can show a counterexample to induction, but cannot prove that $I$ is an inductive invariant.
We prove inductive invariants in small cases with the model checker~\apalache{}~\cite{konnov2019tla}.
%\tlap{} and its model checker TLC were used to specify and verify partially synchronous algorithms in case of fixed parameters~\cite{lamport2005real}.
%The explicit-time
%approach in~\cite{abadi1991old,lamport2005real} is closed to our encoding of ages of in-transit messages.
%To avoid the state explosion, we developed an abstraction of in-transit messages.
%in case of arbitrary time bounds, both the explicit-time
%approach and our encoding lead to infinite state spaces.
%The explicit-time approach works fine for specifying and proving prop
%erties of real-time algorithms~\cite{}
%focus on real-valued variables, while all variables and time
%constraints in the failure detector of Chandra and Toueg are in the
%domain of integers.
%\jw{can we have a stronger argument against real values. Is this the only limitation these approaches have?}
System designers can use timed automata~\cite{alur1994theory} and parametric verification
frameworks~\cite{larsen1997uppaal,andre2012imitator,lime2009romeo}
to specify and verify timed systems.
In the context of timed systems, we are aware of only one paper about verification of failure detectors~\cite{atif2012formal}.
In this paper, the authors used three tools, namely UPPAAL~\cite{larsen1997uppaal}, mCRL2~\cite{bunte2019mcrl2}, and FDR2~\cite{roscoe2010understanding} to verify small instances of a failure detector based on a logical ring arrangement of 
processes.
%Time parameters in these instances are bounded.
Their verification approach required that message buffers were bounded, and had restricted behaviors in the specifications.
Moreover, they did not consider the bound $\Phi$ on the relative speed of processes.
In contrast, there are no restrictions on message buffers, and no ring topology in the
Chandra and Toueg failure detector.
Moreover, our work is to verify the Chandra and
Toueg failure detector in case of arbitrary bounds.
%Moreover, our work is to verify in case of arbitrary bounds.
In recent years, automatic parameterized verification techniques~\cite{konnov2017parameterized,stoilkovska2019verifying,druagoi2020programming} have been introduced for distributed systems, but they are designed for synchronous and/or asynchronous models.
%Hence, these techniques cannot cope with time constraints under partial synchrony.
Interactive theorem provers have been used to prove correctness of distributed algorithms recently. 
For example, researchers proved safety of Tendermint consensus with Ivy~\cite{ivyTendermint}.


%The specifications in~\cite{ivyTendermint} are in decidable theories supported by Ivy.
%Our Ivy specifications for the failure detector are not in such decidable theories.
